Understanding the Security Risks of Decentralized Exchanges by Uncovering Unfair Trades in the Wild

DEX, or decentralized exchange, is a prominent class of decentralized finance (DeFi) applications on blockchains, attracting a total locked value worth tens of billions of USD today. This paper presents the first large-scale empirical study that uncovers unfair trades on popular DEX services on Ethereum and Binance Smart Chain (BSC). By joining and analyzing 60 million transactions, we find 671,400 unfair trades on all six measured DEXes, including Uniswap, Balancer, and Curve. Out of these unfair trades, we attribute 55,000 instances, with high confidence, to token thefts that cause a value loss of more than 3.88 million USD. Furthermore, the measurement study uncovers previously unknown causes of extractable value and real-world adaptive strategies to these causes. Finally, we propose countermeasures to redesign secure DEX protocols and to harden deployed services against the discovered security risks.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

==> ccs-body.tex <==
\section{Introduction}

This is a sample!  It does not have a lot of fancy stuff in it, but if
you want to see a more complex sample, look at the original ACM
templates.

To fill up enough text to fill up 3 pages, we've included the CCS Call
for Papers three times.  It is always a good idea to include some
gratuitious citations to recent CCS papers~\cite{medvinsky1993netcash,
  bellare1993random, anderson1993cryptosystems, blaze1993cryptographic}.

\input{cfp}
\input{cfp}
\input{cfp}

\section{Conclusions}

In conclusion, it is rarely a good idea to include the same section three times in a paper, or to have a conclusion that does not conclude.

\appendix

\section{Location}

Note that in the new ACM style, the Appendices come before the References.

\input{cfp}

\begin{acks}
% TODO: For the submission, don't include acknowledgments since they would most likely deanonymize you.
\end{acks}


==> cfp.tex <==
\section{Call for Papers}

The conference seeks submissions presenting novel research results in
all aspects of computer and communications security and privacy,
including both practical and theoretical contributions.

\subsection{Paper Submission Information}

Submissions must be received at \url{https://ccs17.hotcrp.com/} by the
strict deadline of {\bf 19 May 2017 at 8:59 PM PDT (UTC-7)}.
Submitted papers must not substantially overlap with papers that have
been published or that are simultaneously submitted to a journal,
conference, or workshop. Submissions must be anonymized and avoid
obvious self-references.

CCS has traditionally required that authors submitting papers
guarantee that an author will be able to present their paper at the
conference. We recognize, however, that the current travel
restrictions and screening processes may make it impossible or
uncomfortable for some authors to travel to the conference. The venue
for CCS 2017 was selected several years ago, and we do not wish to
exclude any potential authors who may have difficulty traveling due to
recent changes in US immigration practices.  CCS welcomes submissions
by authors of all nationalities, and will make allowances for
presenting papers electronically or with non-author presenters in
cases where paper authors are unable to travel to the United States.

Submissions will be evaluated based on their scientific merit,
novelty, importance, presentation quality, and relevance to computer
and communications security and privacy.  If a paper includes work
that raises ethical concerns it is up to the authors to convince the
reviewers that appropriate practices were followed to minimize
possible harm and that any harm caused by the work is greatly
outweighed by its benefits. The review process will be carried out in
two phases and authors will have an opportunity to provide a
length-limited response to the first-phase reviews.

\subsection{Paper Format}

Submissions must be single PDF files containing at most 12 pages in
the required new ACM format (see
\url{https://www.sigsac.org/ccs2017/format} for details and templates,
which you have presumably found if you are reading this!) of body
content, with any number of additional pages for the bibliography,
well-marked appendices, and any desired supplementary material.  When
relevant, submitters may include reviews from past submissions and
responses to them in the supplementary material.

Reviewers are not required to consider the appendices or supplementary
material, however, so submissions need to be intelligible and
convincing without them.  Submissions not meeting these guidelines, or
playing games to work around page limits, will be rejected by the PC
chairs without review.  In particular, papers should not use squeezing
tricks to adjust the (already very dense) ACM paper format, and moving
discussion of key related work or important definitions to appendices
may be grounds for rejection.

\subsection{Practice Talks}

Following the lead of USENIX Enigma, we want to improve the quality of
the conference and provide a better experience for both presenters and
attendees by holding practice sessions before the conference (see
\url{https://www.sigsac.org/ccs2017/practicefaq}). Presenting authors
of accepted papers are expected to participate in an on-line practice
session approximately three weeks before the conference.

\subsection{Conflicts of Interest}

The conference requires cooperation from both authors and program
committee members to ensure a process that is both fair in practice
and perceived to be fair by everyone. When submitting a paper, authors
are required to identify members of the program committee who may not
be able to provide an unbiased review.  This includes people with
strong personal or professional relationships such as advisor/advisee,
members of the same organization, and close collaborators (for
example, recent or repeated co-authors). In general, this means anyone
who a reasonable person with all the relevant information would
question as an impartial reviewer. The program co-chairs reserve the
right to request a more specific description of a conflict-of-interest
declaration from authors.

Program committee members who have a conflict of interest with a
paper, including program co-chairs, will be excluded from evaluation
and discussion of the paper, but because submissions are anonymous to
reviewers it is important for submitting authors to identify these
conflicts. In the case of a program co-chair, the other co-chairs who
do not have conflicts will be responsible for managing that paper.
Program co-chairs are not permitted to be involved as co-authors in
any submissions.




==> sty/usepackage_config_copy.tex <==
%using latex.XXX file to cusotmize style
%customized tools
%\usepackage{amssymb}
%\usepackage{times}


\usepackage{amsfonts}
\usepackage{subfig}
\usepackage{wrapfig}
\usepackage{float}
\usepackage{multirow, graphicx}
\usepackage{algorithm}
\usepackage{algpseudocode} %algorithm: use algorithmicx package, to refer to http://en.wikibooks.org/wiki/LaTeX/Algorithms_and_Pseudocode#Typesetting_using_the_algorithmicx_package
\usepackage{amsmath}
\usepackage{siunitx}
\usepackage{textcomp}


%squeeze space 
%\setlength{\belowcaptionskip}{2pt}
%\setlength{\abovecaptionskip}{2pt}
%\setlength{\floatsep}{0.25\floatsep}
%\setlength{\dblfloatsep}{0.25\dblfloatsep}
%\setlength{\textfloatsep}{0.25 \textfloatsep}
%\setlength{\dbltextfloatsep}{0.25\dbltextfloatsep}
%\setlength{\intextsep}{0.25\intextsep}

%reduce whitespace surrounding section titles.
%\newcommand{\subparagraph}{} %from stackexchange: The titlesec package assumes all of the section levels provided by the standard classes are present. This includes the subparagraph level. The IEEEtrans class doesn't define a level subparagraph
%\usepackage[compact]{titlesec}  
%\titleformat{\paragraph}[runin]{\normalfont\itshape}{\theparagraph}{3pt}{} %keep paragraph title in the same line.
%TODO: to add manually a ":" to each of paragraph headings!

%TODO: to manually add \vspace{-.5cm} into authors and paper title, which reduce the whitespace in the front page.

%\usepackage{sty/simplemargins}
%    \setleftmargin{0.6in}
%    \setrightmargin{0.70in}
%    \settopmargin{0.55in}
%    \setbottommargin{0.55in}

%use to set line spacing for whole document
%f:http://en.wikibooks.org/wiki/LaTeX/Paragraph_Formatting#Line_spacing
%\usepackage{setspace} %dont use this alone (with sig-alternate)! footnote with 9 will show.
%\singlespacing
%\onehalfspacing
%\doublespacing
%\setstretch{1.1}


\usepackage{xspace} 

%url
\usepackage{url}
\def\UrlBreaks{\do\/\do-}
%\usepackage[breaklinks]{hyperref}
%\usepackage{breakurl}

%\usepackage{sty/widetext} %show equation in two columns

\usepackage{stackrel}

\let\oldemptyset\emptyset
\let\emptyset\varnothing

%cut words in middle when running out of space in a line.

%\pagestyle{empty} %this removes the page number
%\pagenumbering{gobble} %this really remove page numbers
\thispagestyle{plain}
\pagestyle{plain} %this enforce page number

\ifdefined\TTSTYLETARGETreport
% bibliography
\usepackage[
    backend=bibtex,
    maxbibnames=100,
    firstinits=true,
    bibstyle=numeric,
    citestyle=numeric
%    bibstyle=alphabetic,
%    citestyle=alphabetic
]{biblatex}
\addbibresource{ads.bib}
\addbibresource{lsm.bib}
\addbibresource{bkc.bib}
\addbibresource{dos.bib}
\addbibresource{odb.bib}
\addbibresource{cacheattacks.bib}
\addbibresource{sc.bib}
\addbibresource{crypto.bib}
\addbibresource{sgx.bib}
\addbibresource{diffpriv.bib}
\addbibresource{txtbk.bib}
\addbibresource{distrkvs.bib}
\addbibresource{vc.bib}
\addbibresource{yuzhetang.bib}
\fi

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\usepackage{enumitem}

\usepackage{todonotes}
%\usepackage{pxfonts}
%\input{sty/wheels-usepackage.tex} %%
\sloppy



==> text/ZZZ.tex <==
\section{More Measurement Results: Fees of Violating Transactions}

\textcolor{blue}{Rational thieves tend to send violating transactions with a high gas price. We explore how high the gas price was set in the withdrawal transaction to compare to the typical transaction in the block. For each withdrawal transaction we found, we record the block number. Afterward, we traversal all the transactions in the specific block to evaluate the average gas price by taking the total gas divided total transaction fee. The ratio of the gas price in the violating transaction to the average gas price tells the difference. We choose 3413/1000 violating transactions from block $\#10252074$ to $\#12730520$ with the order by block number. To clearly show the ratio of the transaction fee, we aggregate every 10/100 blocks into one tick. Figure \ref{fig:tx_fee_ratio_100} shows that 13 out of 34 nodes with gas prices $1.3X$ greater than the average fee. The highest node is $6.7X$. Figure \ref{fig:tx_fee_ratio_10} has 33 nodes with gas price $1.3X$ greater than average. The highest gas price is $43X$. The result shows that part of the violations intendedly increase their gas price to ensure their transaction is included in the blockchain as soon as possible.
}

\begin{figure}[!ht]
  \begin{center}
    \subfloat[3413-block history with 100-block ticks]{%
      \includegraphics[width=0.25\textwidth]{figures/gasprice_ratio_100.eps}
      \label{fig:tx_fee_ratio_100}
    }%
    %\hspace{-0.2cm}%
    \subfloat[1000-block history with 10-block ticks]{%
      \includegraphics[width=0.25\textwidth]{figures/gasprice_ratio_10.eps}
      \label{fig:tx_fee_ratio_10}
    }%
  \end{center}
  \caption{Normalized Gas price of violating wtihdrawal transactions over the normal Gas price (of other transactions in the same block).}
\end{figure}


\textcolor{blue}{
\section{Attack verification on ropsten testnet}
}
\textcolor{blue}{
To verify the feasibility of the attacks, we replay Violation I and Violation III in the ropsten testnet. 
}


\textcolor{blue}{
{\bf Case study of Violation I}: The process of replaying Violation I depicted in Figure~\ref{fig:testnetcase1}. First, we deploy a rebase token and a normal token on the testnet called AMPL and TokenA. We create a pool with the Uniswap contract. We add liquidity $1*10^7$ of AMPL and $10000$ of TokenA to the pool. Then, the AMPL token issuer sends transaction $tx_1$ to rebase the token supply among all AMPL token holders, including a Uniswap V2 pool account (CA $0x954d$). Finally, Alice (EOA $0x1940$) calls the victim pool's \texttt{swap()} in $tx_2$ and withdraws $100$ TokenA from the victim. 
}

\textcolor{blue}{
{\bf Case study of Violation III}:The process of replaying Violation III depicted in Figure~\ref{fig:testnetcase2}. We deploy two tokens called TokenA and TokenB and the corresponding pool. We add liquidity $10000$ of TokenA and $2000$ of TokenB to the pool. Suppose the victim Alice(EOA $0x1940$) intends to swap 10 token B to 40 token A. She deposits 10 tokenB to uniswap:pair(CA 0x7164) by sending the tx1 through \texttt{transfer()}. Then Bob(EOA 0x0a56) recognizes this opportunity and sends tx2 to withdraw 40 tokenA immediately after Alice's transaction. He successfully benefits from the transaction. Afterward, when Alice wants to withdraw her token in tx3, she fails because Bob had already withdrawn her tokens.
}

\begin{figure*}[!bhtp]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/jiaqitest_rebase.eps} 
  \caption{Replay of Violation I on Ropsten testnet}
  \label{fig:testnetcase1}
 \end{figure*}
 \begin{figure*}[!bhtp]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/jiaqitest.eps} 
  \caption{Replay of Violation III on Ropsten testnet}
  \label{fig:testnetcase2}
 \end{figure*}





==> text/eval_uniswap.tex <==
\begin{table*}[!htbp] %force in current page, disable float.
\caption{Discovered atomicity anomalies}
\label{tab:anomalies}\centering{\small
\begin{tabularx}{0.65\textwidth}{ |X|c|c|c|c|c|c| }
  \hline
 Exchanges  & \# of txs & Value & \textsc{ATOMIC} & \multicolumn{3}{|l|}{Anomalous swaps}  \\ \cline{5-7}
            &   ($\times{}10^3$)  & & swaps (\textsc{A}) & \textsc{U} & \textsc{F} & I \\ \hline
 Uniswap-V2 (router) & 6374.3   &  $~70.4\cdot{}10^9$ USD & $6.37\cdot{}10^6$ & N/A & 0 & 32 \\ \hline
 BancorX             & 6.1      &  $9.5\cdot{}10^3$ ETH & $6139$             & 4 & 0 & 0 \\ \hline
\ignore{
 Uniswap-V2 (pool)   & 15.5     &  $~0.23\cdot{}10^9$ USD & $61$     & 3   & 15352 & 0 \\ \hline
}
\end{tabularx}
}
\end{table*}

We obtain the Uniswap's transactions from May 04, 2020 (i.e., Uniswap-V2's launch date) to July 08, 2021 by querying Google's BigQuery service~\cite{me:eth:bigquery}. The transactions and their internal calls are ported into our trace database.
In the database, there are 6627 pairs of tokens and thus the same number of liquidity pools. We run the method described above on this database, and obtain the results in Table~\ref{tab:anomalies}. For transactions calling \texttt{wrappedSwaps}, we find there are $6.37\cdot{}10^6$ \textsc{ATOMIC} single-transaction swaps. We find 32 cases in which two swaps' execution is interleaved. The cause is that tokens such as 
aSUSD keep changing their balance, leading to the difference between the account balance maintained in Uniswap-V2's contract and the balance in the token contract. This leads to a \textsc{FREERIDE} opportunity.
We also measure block delay between two transfers of the atomic swaps and report the rsults in Table~\ref{tab:delay:uniswap}.

\ignore{
Second, for transactions that bypass the router and directly call the pool, we find only $61$ out of $15.5\cdot{}10^3$ transactions are \textsc{ATOMIC} swaps. The rest are \textsc{FREERIDE}.
}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Block delay between two transfers of a swap on Uniswap-V2}
\label{tab:delay:uniswap}\centering{\small
\begin{tabularx}{0.30\textwidth}{ |X|c|c| }
  \hline
  Block delay & Percentage & \% of two-traders\\ \hline
  $0$ & 82.4\% & XXX \\ \hline
  $1$ & 13.5\% & XXX \\ \hline
  $2$ & 1.4\% & XXX \\ \hline
  $3$ & 1.4\% & XXX \\ \hline
  $10$ & 1.4\% & XXX \\ \hline
\end{tabularx}
}
\end{table}

\ignore{
\begin{figure}
\begin{center}
    \includegraphics[width=0.35\textwidth]{./expfigure/exp-uniswap1.eps}
    \caption{Uniswap TransferOut-TransferIn block difference distribution} \label{uniswap}
\end{center}
\end{figure}
}

\clearpage

\subsection{Attack Confirmation}

\begin{figure}
\begin{center}
  \includegraphics[width=0.45\textwidth]{figures/workflow_overall.eps}
  \caption{Overall workflow for trace analysis} 
\label{fig:workflow:overall}
\end{center}
\end{figure}

Given the discovered swap anomalies, we conduct further analysis to confirm they are actual attacks. Specifically, a swap anomaly constitutes an attack only when one can find an ``attacker'' account who gain profit (illicitly) from the swap at the expense of an ``victim'' account. For different anomalies, this requirement translates into different measurable conditions: 1) For a two-trader swap to be part of an attack, the necessary condition is that the two trader accounts must belong to different physical users. 2) For interleaved swaps to constitute an attack, whether the swaps are interleaved must affect the value transferred in at least one swap. By this means, the attacker can benefit from interleaved execution. 3) For an UNDERWATER anomaly to be an attack, the anomalous transaction cannot be the one to pay DEX fees. Overall, the ``attack confirmation'' conditions are summarized in Table~\ref{XXX}. We propose anomaly-specific analysis for attack confirmation.

\subsection{Confirm Attacks of Two-trader Swaps}

\subsubsection{Account Behavior Anlaysis}

In swaps involving two traders, the necessary condition to constitute an attack is the two trader accounts belong to different real-world entities (i.e., an attacker and a victim). To distinguish the attack case from the case that the two accounts belong to the same entity, our idea is to exploit the different behavior the two accounts exhibit when they belong to an attacker and victim entities (in the real world). Specifically, the victim experiencing financial loss in such an attack swap may switch to a safer way to use the DEX (e.g., from multi-transaciton swap to single-transaction swap by router contract). An attacker may be a frontrunning bot who send a large volume of request victimizing many accounts.

{\bf Related work: Address clustering}: In the existing literature, the address linkage problem has been studied, that is, determining if two addresses on the same blockchain belong to the same physical user. There are two existing methods: 1) Conducting transaction graph analysis using heuristics such as change addresses and atomic spending of Bitcoin outputs~\cite{XXX}. However, the existing heuristics are specific to Bitcoin's UTXO model (e.g., atomic output spending is specific to Bitcoin and inapplicable to Ethereum or other smart-contract blockchains). 2) Using external/background knowledge to deanonymize a physical user and to further link the user's multiple addresses. For instance, one deanonymization method~\cite{XXX} is to monitor the transaction-propagation traffic and identify the node IP that first propagates the transactions from the target account. YYY The problem in this method is heavyweight. 

Recent work clusters~\cite{XXX:Address clustering in Ethereum} addresses on Ethereum based on several heuristics, for instance, different addresses use the same deposit addresses generated on-demand by DEX belong to the same entity. In contrast, this work links two trader addresses using new heuristics specific to the swap scenarios.

\input{text/lst_checkAttackerVictim.tex}

\subsubsection{The Framework}

Given swaps with two traders, the framework first characterizes the traders' swap behavior. Specifically, given an anomalous swap of two traders, it extracts the two traders' accounts, say Alice who sends the $tfIn$ transaction and Bob who sends the $tfOut$ transaction. Then, it retrieves Alice's other transactions doing the swaps, and tags each such transaction $tx_A$ with two labels. The first label matches the case of $tx_A$ to one of the followings: A0, A1, A2, U, F, as explained in Table~\ref{tab:txlabel}. If the transaction $tx_A$ incurs an $tfOut$ operation in an atomic swap (i.e., the first label being A0 or A2), it assigns the second label $L_2$ indicating which account the $tfOut$ transfer coins to. Thus, Alice can be characterized by the two labels of all the swaps she has sent, namely $V_1=\{\{L_1\}, \{L_2\}\}$. We call $V_1$ Alice's raw feature vector, based on which more vector representations will be extracted as will be discussed. 

The framework then similarly constructs Bob's feature vectors, with the notable difference that the second label $L_2$ is assigned for Bob only when the first label is either $A0$ or $A1$.

\begin{table}[!htbp] %force in current page, disable float.
\caption{Transaction labels: The first label $L_1$}
\label{tab:txlabel}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |c|X| }
  \hline
$A0$ & An atomic swap in one transaction.  \\ \hline
$A1$ & A $tfIn$ operation in an atomic swap where the $tfOut$ is carried out in a separate transaction. \\ \hline
$A2$ & A $tfOut$ operation in an atomic swap where the $tfIn$ is carried out in a separate transaction.  \\ \hline
$U$ & A transaction running a standalone $tfIn$ operation in a UNDERWATER swap.  \\ \hline
$F$ & A transaction running a standalone $tfOut$ operation in a FREERIDE swap. \\ \hline
\end{tabularx}
}
\end{table}

In the second step, the framework establishes ``signatures'' that model different traders' behavior, including an attacker trader, victim trader and benign trader. In this step, a generic approach is manual labeling in which different traders' roles are modeled by feature-vector ``patterns'' based on heuristics. For instance, a Uniswap-V2 trader Alice is likely to be a victim if she sends a $tfIn$ transaction (A1) before switching to use routers (A0) as a safer resort. We express this behavior by a vector pattern (in regular expression) $L_1=.*A1[A0]+$. For another instance, a UniswapV2 trader Bob is likely to be an attacker, such as a frontrunning bot, who sends many $tfOut$ transactions (A2) that pay to many different trader accounts. We express this heuristic as another feature-vector pattern $L_1=.*A2*.* \and \|L_2\|>10$, where more than $10$ different traders is a configurable threshold. There are service-specific methods to construct the signatures as will be described.

The third step takes as input anomalous swaps of two traders and produces decisions whether each input swap constitutes an attack instance. Internally, this step matches each input swap's trader accounts with the signatures of different trader roles (including attacker, victim and benign trader). The matchmaking is solved as a substring match problem where the string is an input swap's raw feature vector and the pattern is a signature. If a swap's two traders match a pair of attacker and victim, this swap is tagged as an attack. If a swap's both traders match benign users, the swap is not an attack. For instance, Alice's feature vector $A0,A2,A0,A0,A0$ would be matched successfully against the attacker pattern/signature $.*A2[A0]+$, making any swaps Alice involved be an attack.
\begin{figure}
\begin{center}
  \includegraphics[width=0.45\textwidth]{figures/analysis_2traders.eps}
  \caption{Attack confirmation analysis on 2-trader swaps} 
  \label{fig:analysis:2traders}
\end{center}
\end{figure}

Overall, the framework detects the set of attack instances out of anomalous swaps with two traders. The detection workflow is illustrated in Figure ~\ref{fig:analysis:2traders}.

\clearpage


==> text/intro.tex <==
\section{Introduction}

Recent years have witnessed the rise of Decentralized Finance (DeFi) on blockchains. A prominent class of DeFi applications is Decentralized Exchange (DEX) which allows traders to swap their assets from one type of token to another. 
On Ethereum, the most popular DEX services that account for more than 95\% of the market (incl. Uniswap~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer}) {\color{purple} all run AMM protocols or Automated Market Maker~\cite{me:etherscan:topdex}.} In an AMM, a trader account deposits one token to a smart-contract instance, called a pool, and withdraws a certain amount of other tokens from the pool. Besides token swaps, an AMM
%\footnote{This paper uses terms ``AMM'' and ``DEX'' interchangeably.} 
pool supports the operation of adding/removing ``liquidity'' where liquidity-provider accounts deposit/withdraw tokens to/from the pool to increase/decrease token reserves in the pool and to support future trades\footnote{This paper uses terms ``token swap'' and ``trade'', interchangeably.}. 

AMM can be exploited to extract value illicitly. Well known AMM attacks include sandwich attacks and arbitrage~\cite{DBLP:conf/sp/DaianGKLZBBJ20,DBLP:journals/corr/abs-2101-05511,DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2105-02784,DBLP:conf/sp/ZhouQCLG21}. In both attacks, an adversarial trader sends crafted transactions and execute {\it multiple} trades against a victim pool. Illicit value can be extracted as the multiple trades can exploit the difference in token exchange rates at different times (i.e., in sandwich attacks~\cite{DBLP:journals/corr/abs-2101-05511}) or across different pools (i.e., in arbitrage~\cite{DBLP:journals/corr/abs-2105-02784}).

%Another AMM misuse is to list scam tokens~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21} that impersonate other tokens to trick their traders. 

\begin{figure}[b!ht]
\begin{center}
\includegraphics[width=0.425\textwidth]{figures/workflow7.eps}
\end{center}
\caption{Transaction-analysis workflow to discover operation-wise atomicity violations (described in \S~\ref{sec:detectviolatingswap}) and to detect and characterize the instances of theft attacks (\S~\ref{sec:attack}) and lost tokens (\S~\ref{sec:losttokens}).}
\label{fig:workflow7}
\end{figure}

{%\color{blue}
\vspace{2pt}\noindent\textbf{Discovering atomicity violations}. 
This work aims at studying a different class of AMM exploits: Instead of abusing price differences across multiple trades, the attacker exploits the broken atomicity of a single trade. Specifically, a safe AMM operation, such as a trade, requires executing a sequence of token deposits and withdrawals in an all-or-nothing manner (i.e., operation-wise atomic execution\footnote{Note that atomicity in this paper refers to the granularity of an individual AMM operation, which should be differentiated from transaction-wise atomicity used in the literature~\cite{DBLP:journals/corr/abs-2101-05511}.}).
Violation of this atomicity implies financial risks or even the occurrence of attacks. For instance, executing a token swap by a standalone withdrawal (i.e., without the matching deposit) could indicate an incident of theft in which the thief withdraws value from the victim AMM pool without making any deposit. For another instance, a token swap by a standalone deposit (without a matching withdrawal) could mean an adversarial AMM pool denying the legitimate withdrawal request from the trader who has made a deposit.
Note that the existing AMM exploits, such as sandwich attacks and arbitrage, do not violate operation-wise atomicity.

By connecting together and analyzing over $60$ million transactions on Ethereum and Binance Smart Chain (BSC), to our surprise, we find that atomicity violations widely exist among deployed AMM services: 
Committing these violations are the most popular services, including Uniswap V2~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer}.
In total, they have performed more than $671$ thousand AMM trades and liquidity operations violating atomicity, which exhibit various patterns including standalone token deposit, standalone withdrawal, account mismatch, and value mismatch.

%To understand the nature of the atomicity violations, that is, whether they occur by accident or are committed intentionally, we formulate the following hypothesis: 1) The atomicity violations in which the deposited value is below the value withdrawn could indicate token thefts in which a thief account attacks by extracting value from a victim AMM or trader account. 2) The atomicity violations in which the deposited value exceeds the value withdrawn could indicate AMM denial of service in which a victim trader depositing value is declined of withdrawal service. Specifically, we focus on the lost-token risks in which the victim trader deposits tokens by mistakes.

\vspace{2pt}\noindent\textbf{Understanding atomicity violations}. 
We aim to understand the nature of the atomicity violations, whether they are accidents or intentional crimes. While different atomicity violations can be attributed to different threats (e.g., denial of service mentioned above), we mainly focus on the prominent cases of token theft in our measurement result.

Detecting theft from the atomicity violations is challenging. This is because the ground truth often includes off-chain activities unaccounted for.
%which are unobservable. 
For instance, when attributing a standalone withdrawal to theft, one has to know that the party making the deposit to accounts and the party withdrawing from the accounts are controlled by two distinct physical entities, which is known to be an intractable problem with only on-chain data; known heuristics such as address clustering~\cite{DBLP:conf/fc/Victor20,DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:conf/sp/HuangALIBMLLSM18,DBLP:books/daglib/0040621} do not apply here (see \S~\ref{sec:discoveryproblem} for detail).

To address the challenge, we propose three detection methods and cross-check them on each violation instance. First, we propose heuristics to match accounts' on-chain behavior against rational attack strategies. 
For instance, a rational thief, in fear of value extracted by competing thieves, would send crafted transactions with aggressively high fees and with short deposit-to-withdrawal delay, which can be used as a signature for detecting thefts.
Second, to eliminate the possibilities of benign value extraction, we propose detecting the frontrunning among multiple withdrawer accounts of the same pool, which shows the conflict of interest among withdrawals. Unlike existing works scanning the entire blockchain history and mempools~\cite{DBLP:conf/uss/TorresCS21,DBLP:conf/sp/DaianGKLZBBJ20}, we optimize the frontrunning detection by focusing on atomicity-violating withdrawals and failed token withdrawals. Third, we also search the Internet for user complaints about our violation cases' accounts. The latter two methods jointly show ill-intention of the value extraction. 

Overall, our method is an end-to-end transaction-analysis pipeline, depicted in Figure~\ref{fig:workflow7}, which first discovers atomicity violations and then detects attack instances in thefts and lost tokens.

%We found in practice the exploitable deposits can be created in a variety of unexpected application scenarios, including free token giveaways (i.e., airdropping), tokens redistributing fees to privileged shareholder accounts, tokens bearing interest, tokens that can adjust or rebase total supply, buggy smart contracts, and unsafe user interface that executes a swap in two separate transactions, etc. 

\vspace{2pt}\noindent\textbf{Findings}. 
On the Ethereum mainnet and BSC fork, we discover $55$ thousand theft attacks mounted by $258$ distinct attacker accounts with high confidence, inflicting a loss of more than $3.88$ million USD stolen from $978$ victim accounts.
Each attack instance we found matches at least one indicator. 
As the measurement results show, real-world users exploit the undefined behavior in the AMM protocols, such as rebasing token supply, token interest and other non-standard token features, to successfully withdraw value. Interestingly, the attackers {\it adapt} their behavior to different exploits: When the attacker is to extract value from interest-bearing tokens, she waits long enough, typically hundreds of Ethereum blocks, for the interest to accumulate and to become profitable. Given other kinds of deposits, such as token rebase, the same attacker instead wastes no time extracting the illicit value, typically within one or two blocks, to prevent frontrunning.

%One cause of the atomicity violations is that certain non-standard token operations unspecified in the AMM protocols (e.g., rebasing token supply and interest-bearing tokens) are mistreated as token deposit that allows subsequent token withdrawal to succeed. This manifests in standalone withdrawals. Another cause is that certain token deposits are not intended for withdrawal (e.g., airdrop and token lost-and-found), which results in standalone deposits.

\ignore{
We further study attackers' and victims' behavior by tracking their money flow and their actions to create/destroy smart contracts. Our study uncovers the systematic criminal activities: the crime bosses use mixer services to hide their identities while sending commissions and instructions. After the attack, the money is sent to various DeFi services to maximize illicit profit. Exploit smart contracts are widely used to improve attack success rates.
}

From the violations that cannot be attributed to theft, we further detect the instances of denial of service. Particularly, we formulate the problem of detecting lost tokens where the deposits are made by mistake, and the AMM refuses to return the tokens. We propose threat indicators by assuming the victim accounts' rational behavior after lost tokens. Our measurement result on Ethereum confirms the existence of lost tokens on Uniswap V3, Curve and Balancer (inflicting a total value of $57,000$ USD lost unfairly by these AMMs). We note that the atomicity violations could imply other threats than theft and lost tokens, and a comprehensive study is left for future research. 
%is out of the scope of this work.

%why it is hard to design secure AMM in practice?
{\color{purple}
\tangSide{Resp. Q1}
By design, all six AMM services measured are vulnerable to either token theft or lost tokens. The root cause is two-fold: First, the ERC20 standard has design flaws. Specifically, the \texttt{transfer} function does not allow tracking the history of token senders, rendering it hard or costly to enforce access control. Second, token implementations may exhibit the behavior undefined in the ERC20 standard, such as token rebase. This undefined behavior causes token theft (see \S~\ref{sec:counter:space} in detail). 
\tangSide{Resp. Q8}
Besides, the discovered design flaws of ERC20 standard apply to any DeFi smart contracts built on ERC20 tokens, beyond just DEX/AMM (discussed in \S~\ref{sec:riskanalysis}). 
%The design flaws are orthogonal to the protocol-level provable security of various swap schemes surveyed in \S~\ref{sec:rw}. 
}

\vspace{2pt}\noindent\textbf{Mitigation}. 
We propose a secure design of AMM pool, in which the pool verifies the deposit transaction using ETHRelay protocols~\cite{me:ethrelay,DBLP:conf/blockchain2/FrauenthalerSSS20,me:btcrelay,DBLP:conf/aft/DaveasKKZ20} and can enforce access control on withdrawal against the original depositor account. While avoiding thefts and lost tokens, the ETHRelay procedure in smart contracts incurs a high cost, optimizing which is left for future works toward practicality. In addition to redesigning AMM pools, we propose building an off-chain infrastructure (a benign bot) to automatically discover withdrawal opportunities, claim the value ahead of actual attackers, and refund the victims. 

{\color{blue}\tangSide{Resp. Q7}
Our secure redesigns of AMM pool for Uniswap V2/V3 are open-sourced at GitHub~\cite{me:mitigate:v2}/~\cite{me:mitigate:v3}.
}

{\color{blue}\tangSide{Resp. Q1/Q8}
Note that existing ``atomic'' or fair exchange protocols~\cite{DBLP:conf/ccs/CampanelliGGN17,DBLP:journals/corr/abs-1911-09148,DBLP:conf/ndss/MalavoltaMSKM19,DBLP:conf/ccs/0001MM19,DBLP:journals/corr/MillerBKM17,DBLP:conf/podc/Herlihy18,DBLP:conf/ccs/CampanelliGGN17} do not help solve the security risks uncovered in this work. The latter stems from the ERC20 token standard and is applicable to any DeFi smart contracts built on ERC20 tokens. As validated in our study (see \S~\ref{sec:rw}), implementing protocol-level fair exchanges on real-world ERC20 tokens faces the same implementation-level risk discovered in this work. 
}


\vspace{2pt}\noindent\textbf{Contributions}. Our contributions are outlined below: 

\vspace{2pt}\noindent$\bullet$\textit{ New findings}. We discover a total of $3.88$ million USD worth of stolen value by measuring and analyzing atomicity violations on six popular AMM services on Ethereum and BSC. 
The discovered token theft attacks uncover the previously unknown patterns of extractable value (e.g., token rebase, interest, airdrop, buggy application smart contracts) and expose the adaptive attack strategies that occur offline and otherwise would have been hidden. 
{\color{purple} \tangSide{Resp. Q6} After disclosure to both AMM and token developers, the discovered bugs have been confirmed by the Uniswap team.}
%We further study the criminal infrastructures and campaigns mounted to systematically prepare, execute and finalize the theft attacks.

\vspace{2pt}\noindent$\bullet$\textit{ New techniques}. We develop an end-to-end analytical pipeline to detect atomicity violations and relevant attacks from Ethereum transaction traces, including an efficient join algorithm and various heuristics to automatically discover and cross-check token theft and lost tokens. 

\noindent
{\bf Roadmap}: We survey the related work in Section \S~\ref{sec:rw}. Section \S~\ref{sec:background} introduces the background of AMM and its specification. The discovery of atomicity violations is in \S~\ref{sec:detectviolatingswap}. Detection of theft attacks is presented in \S~\ref{sec:attack}. Detection of lost tokens is in \S~\ref{sec:losttokens}. 
Countermeasures are presented in \S~\ref{sec:mitigate}. Bug disclosure is in \S~\ref{sec:disclosure} with the conclusion in \S~\ref{sec:conclude}.

\section{Related Work}
\label{sec:rw}

We survey the most relevant works and compare them against this one. Due to the space limit, we defer the extended related work to Appendix~\ref{appdx:rw}.

\noindent
{\bf BEV}: In DeFi, a prominent class of attacks exploit transaction reordering to gain blockchain extractable value or BEV. At an abstract level, a BEV can be extracted by two essential steps: An adversarial account first looks for {\it profitable opportunity} and then, to claim the profit, sends {\it frontrunning/backrunning} transactions against competing accounts in a so-called Priority Gas Auction (PGA) game. There could be unlimited causes of profitability opportunities in smart contracts, and the notable ones are arbitrage, sandwich attacks, liquidation, etc. 

Existing research detects BEV attack instances from Ethereum transactions. As shown in Table~\ref{tab:bev}, the research works can be classified by the profitable opportunities exploited and the attack vectors (i.e., frontrunning, backrunning, or others). Specifically, Damian, et al.~\cite{DBLP:conf/sp/DaianGKLZBBJ20} are among the first to study extractable value on Ethereum and detect the arbitrage-by-frontrunning incidents on early-day DEX'es (e.g., TokenStores). The detection method is by collecting blockchain data for confirmed transactions and monitoring mempools for unconfirmed transactions. Torres, et al.~\cite{DBLP:conf/uss/TorresCS21} present a large-scale measurement study on Ethereum that detect generic frontrunning attacks by finding pairs of transactions (that win and lose the frontrunning game). Qin, et al.~\cite{DBLP:journals/corr/abs-2101-05511} measure BEV attacks on Ethereum of various causes including liquidation, sandwich attacks, arbitrage, and others captured by their transaction-replay techniques. Wang, et al.~\cite{DBLP:journals/corr/abs-2105-02784} detect the instances of arbitrage on Uniswap-V2, by finding profitable cycles on the token-transfer graph. Zhou, et al.~\cite{DBLP:conf/sp/ZhouQCLG21} discover arbitrage opportunities by finding profitable cycles among token-token exchange rates in real time. Xia, et al.~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21} detect scam tokens listed on Uniswap V2 that impersonate other tokens to trick their traders; the scam-token signature is the pool of a shorter-lived life span of transactions than normal pools.

{\it This work's distinction to known BEV}: Arbitrage and sandwich attacks are two known patterns to extract BEV from AMM. In arbitrage, the profitable opportunities come from the difference in token exchange rates between AMM pools. In sandwich attacks, the profitable opportunities come from the imminent price changes caused by pending trades. 1) Both BEV attacks exploit or manipulate token prices. In both attacks, the attacker monitors certain conditions on the token prices to determine the timing of value extraction.
In this work, the ``extractable value'' stolen from the theft comes from the AMM design flaw that allows permissionless withdrawal. To extract the value, the attacker does not monitor token prices; instead, she monitors the presence of exploitable deposit (non-standard token deposit such as rebase) to determine when to extract the value.
2) In addition, in existing arbitrage and sandwich attacks, the attack success does not require breaking the atomicity of individual AMM operations. That is, a successful sandwich attack (or arbitrage attack) can be composed of a sequence of token swaps that are atomic. By contrast, the theft attacks studied in this work require breaking the atomicity of AMM operations.
Therefore, the theft attacks studied in this work are fundamentally different from the BEV-based attacks~\cite{DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2101-05511,DBLP:journals/corr/abs-2105-02784,DBLP:conf/sp/ZhouQCLG21}, due to their difference in causes and execution conditions. 

\begin{table}[!htbp] %force in current page, disable float.
\caption{Related works on discovering and measuring BEV}
\label{tab:bev}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |l|X| }
  \hline
 Research works  & BEV causes \\ \hline
 Damian, et al.~\cite{DBLP:conf/sp/DaianGKLZBBJ20}
 & Arbitrage (multi-trade) \\ \hline
 Torres, et al.~\cite{DBLP:conf/uss/TorresCS21}
 & Generic (multi-trade) \\ \hline
 Qin, et al.~\cite{DBLP:journals/corr/abs-2101-05511} 
 & Arbitrage, sandwich, liquidation, replayable txs (multi-trade) \\ \hline
 Wang, et al.~\cite{DBLP:journals/corr/abs-2105-02784} 
 & Arbitrage (multi-trade) \\ \hline
 Zhou, et al.~\cite{DBLP:conf/sp/ZhouQCLG21} 
 & New arbitrage (multi-trade) \\ \hline
 This work
 & Permissionless pool withdrawal (single-trade) \\ \hline
\end{tabularx}
}
\end{table}

\ignore{
\begin{table}[!htbp] %force in current page, disable float.
\caption{Related works on discovering and measuring BEV}
\label{tab:bev}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |l|X|X| }
  \hline
 Research works  & BEV causes & Attack vectors \\ \hline
 Damian, et al.~\cite{DBLP:conf/sp/DaianGKLZBBJ20}
 & Arbitrage (multi-trade) & Frontrun \\ \hline
 Torres, et al.~\cite{DBLP:conf/uss/TorresCS21}
 & Generic (multi-trade) & Frontrun (external) \\ \hline
 Qin, et al.~\cite{DBLP:journals/corr/abs-2101-05511} 
 & Arbitrage, sandwich, liquidation, replayable txs (multi-trade) & Frontrun/backrun \\ \hline
 Wang, et al.~\cite{DBLP:journals/corr/abs-2105-02784} 
 & Arbitrage (multi-trade) & N/A \\ \hline
 Zhou, et al.~\cite{DBLP:conf/sp/ZhouQCLG21} 
 & New arbitrage (multi-trade) & N/A \\ \hline
 This work
 & Permissionless pool withdrawal (single-trade) & Frontrun/backrun \\ \hline
\end{tabularx}
}
\end{table}
}

{\color{blue}\tangSide{Resp. Q1/Q8}
\noindent{\bf 
Provable secure swap protocols}: Protocol designs for atomic swaps have been studied extensively in the literature. Different swap models have been considered including contingent payments~\cite{DBLP:conf/ccs/CampanelliGGN17} in which swaps occur between an off-chain digital good and an on-chain token, payment channels/networks~\cite{DBLP:journals/corr/abs-1911-09148,DBLP:conf/ndss/MalavoltaMSKM19,DBLP:conf/ccs/0001MM19,DBLP:journals/corr/MillerBKM17} in which multiple swaps occur off-chain and are batched into fewer transactions on-chain, atomic cross-chain swaps~\cite{DBLP:conf/podc/Herlihy18} in which pegged tokens on one blockchain are swapped with tokens on another blockchain, etc. Most existing protocols consider the model of swapping assets between two mutually untrusted blockchain accounts (e.g., EOA in Ethereum) mediated through smart contracts or scripts on blockchain. Internally, they are constructed using primitives such as zero-knowledge proofs (e.g., in ZKCP~\cite{DBLP:conf/ccs/CampanelliGGN17}), time-lock smart contracts (e.g., in payment channels and atomic cross-chain swaps). 

This work focuses on the case of deployed AMMes on Ethereum, and they should be differentiated from the provable secure swaps in the following senses: First, AMM swaps assets between an EOA and a smart-contract account (i.e., a pool), while the provable secure protocols consider swapping between two EOAs with counterparty risk. Second, AMM swaps two on-chain tokens, which are different from the swap models described above. 
}

\noindent
{\bf Smart contract vulnerabilities and attacks}: Existing research has covered the automatic discovery of new smart-contract vulnerability~\cite{DBLP:conf/ccs/LuuCOSH16,DBLP:conf/uss/KruppR18} and detection of attack instances of known vulnerabilities~\cite{DBLP:conf/uss/ZhangZZL20,DBLP:conf/uss/ZhouYXCY020,DBLP:conf/uss/SuSDL0XL21,DBLP:conf/uss/0001L21}. These two lines of researches tackle generic program-level attacks such as reentrancy attacks~\cite{DBLP:conf/ndss/RodlerLKD19,DBLP:conf/sp/CecchettiYNM21} and transaction ordering dependencies, which are not DeFi specific as in this work.

{\color{blue}\tangSide{Resp. Q5}
\noindent{\bf 
Blockchain denial of service}: The system service of a public blockchain can be denied by manipulating mining incentives~\cite{mirkin2019bdos}, flooding the network with spam transactions~\cite{DBLP:conf/fc/BaqerHMW16,DBLP:conf/ccs/LiWT21,DBLP:conf/imc/LiTCWL21}, creating Sybil nodes to partition the network and eclipse victim nodes~\cite{DBLP:conf/uss/HeilmanKZG15}, and exhausting nodes' computing resource by running computation-intensive smart contracts~\cite{DBLP:journals/corr/abs-1909-07220}. Recently proposed DETER attacks show that one can send invalid transactions at zero Ether cost to deny the mempool service~\cite{DBLP:conf/ccs/LiWT21,DBLP:conf/imc/LiTCWL21}. Gas based protection can be evaded by crafting smart contracts with under-priced instructions~\cite{DBLP:journals/corr/abs-1909-07220}.

The DoS in this work refers specifically to lost tokens, in which a user having deposited tokens is unable to withdraw value. Lost tokens need not run large computations or send a flood of many transactions. Gas and transaction fees do not protect Ethereum from lost tokens.
}

\section{Background}
\label{sec:background}

Ethereum blockchain supports two types of addresses: An externally owned account (EOA), which is an Ether owner's public key, and a contract account (CA), which is the memory address the smart contract runs on miners. An Ethereum transaction includes a sender address, a receiver address, the Ether value transferred, and the optional input data that specifies smart-contract calls.

ERC20 is a popular standard on token interfaces on Ethereum. The ERC20 functions include \texttt{transfer} which allows a token owner to transfer her tokens to another account, \texttt{approve} which allows an owner to delegate the spending of her tokens to another delegatee account, \texttt{transferFrom} that allows a delegatee account to spend tokens on behalf of the original owner under the approved token limit, \texttt{balanceOf} that allows anyone to get an account's token balance, etc.

In an AMM or automated market maker, there are four parties: an AMM pool (a deployed smart contract), two tokens, say $T_0$ and $T_1$ (deployed smart contracts), traders or liquidity providers (each of which owns an externally-owned account/EOA or a deployed smart contract account). 
An AMM minimally supports two operations: 1) token swap between a trader account and the pool smart contract, and 2) liquidity addition/removal between a provider account and the pool smart contract. 
A trader (liquidity provider) can be either a normal user or a malicious attacker. 

In a $swapToken$ operation, the trader deposits $dx$ units of token $T_0$ to the pool's account and receives from the pool $dy$ units of token $T_1$. The AMM internally determines the token exchange rate (or value of $dy$) by enforcing the invariant on some function. For instance, Uniswap is a constant-product market maker where the invariant function is the product of the two token balance.

In an $addLiquidity$ operation, the liquidity provider deposits $dx$ units of token $T_0$, deposits $dy$ units of token $T_1$, and withdraws a certain amount of ``base'' tokens $T_{\texttt{LP}}$. A remove-liquidity workflow is the reverse of add-liquidity, in that the liquidity provider deposits tokens $T_{\texttt{LP}}$ and withdraws tokens $T_0$ and $T_1$ at a certain ratio.

AMM protocols instantiate the above specification. Token deposit can be realized by either directly \texttt{transfer} the tokens to the pool or doing so indirectly via calling \texttt{approve} and \texttt{transferFrom} functions. Different protocols' functions are listed in Table~\ref{tab:uniswapv2:api}.

\begin{table}[!htbp] %force in current page, disable float.
\caption{AMM protocols' API in $swapToken$ and $addLiquidity$ operations. $T_0$/$p$/$*$ represent deposited token/pool/arbitrary smart contract.}
\centering{\footnotesize
\begin{tabularx}{0.5\textwidth}{ |l|X|l| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
Layer & $swapToken$ & $addLiquidity$ \\ \hline
Uniswap V2
& $T_0$.\texttt{transfer}() & $T_0$.\texttt{transfer}() \\ 
& $p$.\texttt{swap}() & $T_1$.\texttt{transfer}() \\ 
 & & $p$.\texttt{mint}() \\ 
\cline{2-3}
& $*$.\texttt{transferFrom}() & $*$.\texttt{transferFrom}() \\ 
& $p$.\texttt{swap}() & $*$.\texttt{transferFrom}() \\ 
 & & $p$.\texttt{mint}() \\ 
\hline
Uniswap V3
& $p$.\texttt{swap}() & $p$.\texttt{mint}() \\ 
\hline
Balancer
& $p$.\texttt{swapExactAmountIn}() & $p$.\texttt{joinpool}() \\ 
\hline
Curve
& $p$.\texttt{exchange}() & $p$.\texttt{add\_liquidity}() \\ 
\hline
\end{tabularx}
}
\label{tab:uniswapv2:api}
\end{table}

\noindent
{\bf Atomicity specification}: 
%The AMM protocol specifies what function calls are acceptable to be a token deposit (and withdrawal); for instance, in Uniswap V2, a token deposit is a call to a token's \texttt{transfer} function can be a token deposit. A call to a pool's \texttt{swap} function can be a token withdrawal. 
An AMM operation executes a sequence of token deposits and withdrawals; the correctness means the atomic operation execution. Without loss of generality, we use token swap as an example in the description, while the extension to liquidity operations is straightforward. Given a token swap, we call the account calling the deposit function by the depositor and the account receiving the token withdrawal by the withdrawer.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/anomalies.eps}
\end{center}
\vspace{-0.1in}
\caption{Atomic operations (token swaps) and violations.}
\label{fig:swaps}
\end{figure}

\begin{itemize}[leftmargin=0.5cm]
%\setlength{\itemindent}{-1em}
\item
An atomic token swap consists of a token deposit of one token worth value $v$ and a withdrawal of another token worth the same value. The depositor and withdrawer accounts are either the same or match a function call if both deposit and withdrawal are in the same transaction. 

\item
{\bf Atomicity violation I} is a standalone withdrawal that does not match any token deposit.

\item
{\bf Atomicity violation II} is a standalone deposit that does not match any token withdrawal. 

\item
{\bf Atomicity violation III} is an account mismatch in which the depositor and withdrawer accounts in a sequence of otherwise matched deposits and withdrawals do not match. For instance, as shown in Figure~\ref{fig:swaps}, the deposit is issued from Account Alice, and the withdrawal is from Bob.

\item
{\bf Atomicity violation IV} is a lower-value deposit in which the deposited value is lower than the value withdrawn.

\item
{\bf Atomicity violation V} is a higher-value deposit in which the deposited value is higher than the value withdrawn. Both Violations IV and V are cases of value mismatch.
\end{itemize}

Figure~\ref{fig:swaps} shows five atomicity violation patterns and the atomic case of a token swap.
{%\color{blue}
%\tangSide{In response to Q1}
In particular, we stress that Violations IV/V are different from the existing extractable-value (MEV) attacks. In our violation cases, each instance deals with a {\it single} AMM operation, say a swap, and a single exchange-rate value. That is, it is a pair of token deposit and withdrawal where the exchange rate takes effect upon the withdrawal. Suppose in a swap, Alice deposits $x$ units of token $T_0$ and then withdraws $y'$ units of token $T_1$. If it is a violation IV, $y'>y$ where $x/y$ is the exchange rate upon withdrawal. This is unlike the existing MEV attacks, where each attack instance deals with {\it multiple} AMM operations and exploits the change of exchange rates at different operation times, such as arbitrage and sandwich attacks.
}

%We believe atomicity violation implies anomalous activities. For instance, a standalone withdrawal could imply value theft where the withdrawer is able to extract value from the AMM pool without depositing any value. A violation-III token swap implies theft in which the withdrawer is able to extract value from a victim depositor. For another example, a standalone deposit could imply lost tokens where a trader makes a mistake depositing value but is unable to withdraw it.

At last, we formulate two AMM risks: token theft attacks and lost tokens as a risk of losing usability.

\noindent
{\bf Threat: Theft attack}: An attacker trader monitors a target AMM pool's state, both on and off the blockchain. The attacker estimates the profitability of the AMM pool and, upon the right timing, sends crafted transactions to call AMM operations. The attack/theft is successful if the attacker's account is able to withdraw a value higher than the value she deposited. Specifically, the attacker's capabilities include monitoring confirmed transactions in the blocks and unconfirmed transactions in the off-chain mempool. 

The victim can be the AMM pool itself or another account from which the attacker extracts deposited value. In the latter case, the victim account can be another trader (e.g., in Violation III) or another non-standard ``depositor'' (e.g., in Violation I). For instance, a non-standard depositor can be a token issuer rebasing the token supply (i.e., $P_1$ as described in \S~\ref{sec:profitabledeposits}).

In addition, we formulate the notion of ``lost tokens'', which indicates the lack of desirable features, or in other words, poor usability.

\noindent
{\bf Poor usability: Lost tokens}: Suppose a trader deposits a token to an AMM pool using an unsupported interface. The trader who wants a refund of the token can not succeed. This results in an unwanted situation where the token or Ether deposited by mistake is permanently lost.








%------------------old version---------------------------



==> text/lst_checkAttackerVictim.tex <==
\lstset{style=mystyle}

\begin{lstlisting}[caption=Subquery Q3,
                   linerange={1-21},
                   firstnumber=1,
                   deletekeywords={[2]INT},
                   morekeywords={clustered},
                   framesep=8pt,
                   xleftmargin=40pt,
                   framexleftmargin=40pt,
                   frame=tb,
                   framerule=0pt, 
                   label=code:sameentity,
                   float,floatplacement=H
                   ]
void confirmAttack2Traders(Swap[] swaps){
   Map<String, Swap> index = buildIndex(swaps); 
   for(Swap swap : swaps){
    Alice = swap.tfIn.msg_sender;
    Bob = swap.tfOut.msg_sender;
    int[] AliceFea=ExtractFeature(Alice);
    int[] BobFea= ExtractFeature(Bob);
    if(checkAttackerVictim(AliceFea, BobFea, index) > T) //T is a threshold of confidence.
        attacks.add(swap);
    }}

int[] extractFeature(Account X){
  txs = findRelevantTxsSentBy(X)
  for (int i=0; i<txs.length; i++)  labels[i]=labelT(txs[i])
  return labels;
}

int checkAttackerVictim(int[] AliceFeatures, int[] BobFeatures, Map<String, Swap} index){
    int score = 0;
    if(checkAliceChangeT1toT4(AliceFeatures)) score ++;
    if(checkBobAttackManyAlices(BobFeatures)) score ++;
    return score;
}
\end{lstlisting}



==> text/lst_codeanalysis.tex <==
\lstset{style=mystyle}

\begin{lstlisting}[caption=Subquery Q3,
                   linerange={1-21},
                   firstnumber=1,
                   deletekeywords={[2]INT},
                   morekeywords={clustered},
                   framesep=8pt,
                   xleftmargin=40pt,
                   framexleftmargin=40pt,
                   frame=tb,
                   framerule=0pt, 
                   label=code:sameentity,
                   float,floatplacement=H
                   ]
void findBackdoor(Token t){
  for(Node n : balanceOf.getCFG()){
    if(n.isReturn()) Vs.add(n);
  }
  for(Variable vv : readStateVar())
    for(Node v : Vs) {
      if(is_Kdependent(vv, v)){
         for(Function f : readFunctions()){ 
           is_tainted(vv, f) candidates.add(f);
         }
      } 
  }
  //remove false positives
  for(Function f : candidates)
    if(is_falsePositive(f)) candidates.remove(f);
  return candidates;
}
\end{lstlisting}



==> text/misc/2_intro.tex <==
Recent years witness the advent and mass adoption of blockchains and their applications, notably in the domain of Decentralized Finance (DeFi). A foundational and essential DeFi function is Decentralized Exchange or DEX. A DEX allows a trader account, say Alice, to send value in one token and receive the same value in another token.

On blockchains, a typical architecture is that a DEX smart contract interacts with token smart contracts to complete a swap. Specifically, swapping tokens $t0$ and $t1$ is carried out by running two \texttt{transfer} calls to $t0$'s and $t1$'s smart contracts, respectively. Ideally, a swap's two \texttt{transfer} calls should run in a single transaction to ensure atomicity (i.e., executed in an all-or-nothing manner). Deviation from this norm constitutes anomalies and illicit profitable opportunities. For instance, a standalone token transfer can suggest an account receives a token without sending one. For another instance, running the two transfers in two separate transactions could mean a backrunning opportunity for the adversaries to claim the profit created in the first transfer/transaction. 
While the existing literature has examined DEX attacks, such as arbitrage~\cite{DBLP:journals/corr/abs-2103-02228}, front-running and scam tokens~\cite{XXX}, these attacks do not violate swap atomicity and it is an open problem to understand the presence and impacts of swaps violating atomicity on DEX?

This work aims to find swap anomalies in today's large-scale deployed DEX'es and detect attacks that systematically harvest the illicit profit. We specifically focus on the case of Uniswap, which is the protocol underneath today's dominating DEX'es including Uniswap-V2~\cite{XXX}, Uniswap-V3~\cite{XXX} and Sushiswap~\cite{XXX} which account for a total of more than $90\%$ DEX market share on the Ethereum mainnet (as of Jan. 2022~\cite{me:etherscan:topdex}), as well as Pancakeswap~\cite{XXX}, which is the top-$1$ DEX on Binance Smart Chain. In total, the four Uniswap-based DEX'es have served a total of XXX USD worth of swaps.


\noindent
{\bf Method: Trace analytics}:
Our proposed approach is an end-to-end semi-automated data-analytical pipeline, starting from the raw Ethereum data (events and transactions). The pipeline consists of three essential components: anomaly detection, attack detection and characterization, and cause analysis. 

To detect swap anomalies, we construct DEX-relevant data records from the Ethereum raw data and join the records to find mismatches and anomalous swaps. 

An actual attack requires an anomalous swap to occur between two distinct  real-world entities (i.e. an attacker and victim). This is essentially to detect the real-world linkage between two Ethereum accounts which, however, is hidden in the blackbox off-chain states and is difficult to detect. To tackle the challenge, we propose to characterize involved accounts' behavior within and beyond the anomalous swaps. We propose several heuristic-based attack signatures and detect attacks by matching account behavior to at least two signatures. We additionally collect the attack ground truth through online user complaints and validate the detection method.

We collect the trace data of four major Uniswap-based DEX'es (aforementioned) and run our trace analysis pipeline. Our results are two-fold: 1) swap anomalies and causes, 2) attack instances, 3) attacker behavior and ecosystem. In addition, we present the four common causes of the swap anomalies.

\noindent
{\bf Findings: Swap anomalies and causes}
We find anomalous swaps worth more than 3XXX million USD on Uniswap-V2. These swap anomalies either run transfers in two separate transactions (Type-II swap) or are a standalone transfer in a dedicated transaction that does not match any other transaction (Type-III swap). Besides the normal causes such as high swap fees, our findings reveal some unexpected cases of atomicity violation: 

1) Many standalone swaps (Type-III) are caused by non-standard token behavior: That is, the DEX smart contract interacts with tokens via standard functions (e.g., in ERC20) but makes implicit assumptions on non-standard token behavior, which can be false. For instance, we found 1.26 million USD worth of Type-III swaps allow freeride and are caused by \texttt{rebase}, a non-standard but common token operation through which the token issuer updates the balance of all token holders to deal with real-world needs such as inflation. Rebase invalidates DEX's assumption that any balance updates of DEX's account is due to some in-progress swap. There are other non-standard token operations such as interest, airdrop, etc. that cause Type-III swap anomalies. 

2) Buggy DEX smart contracts that, in some code path (e.g., due to mishandling exceptions), violates swap atomicity or sets erroneous exchange value. We found there are 0.205 million USD swaps on Uniswap V2 and XXX USD worth of swaps on Uniswap V3 are due to this cause.

3) API misuse, where a Uniswap-V3 trader uses Uniswap-V2 API/workflow, which results in Type-IIXXX swap anomalies on Uniswap-V3.

\noindent
{\bf Attack detection and ecosystems}: 
Based on the swap anomalies, we detect XXX attack instances, accumulating a total of XXX USD worth of illicit money flow.

---

Contribution:

\noindent{\bf Findings}: We discover a total of three million USD worth of swaps that violate atomicity, by measuring four popular Uniswap services on Ethereum and BSC. 

We identify and characterize the attackers and victims involved in these anomalous swap activities to shed light on the underground ecosystem that strategically exploits atomicity violation to gain illicit profit.

We analyze the causes of swap anomalies, including non-standard token operations in rebase/interest and erroneous exception handling in router smart contracts. We design effective attacks by exploiting the different causes.

\noindent{\bf Discovery technology}: We propose an end-to-end analytical pipeline to detect attacks in Uniswap transaction traces. Specifically, we propose an efficient join algorithm to discover atomicity, and several heuristics/indicators to automatically detect attackers/victims from anomalous swaps.

\noindent{\bf Mitigation strategies}: For partly errors, we build a fuzzer with a test oracle to automate the testing of the router smart contracts to develop.

\section{Swap Specifications}
\label{sec:model}

\noindent
{\bf Transfer}: In a transfer operation $tf=\langle{}sender,receiver,token,value,txID\rangle{}$, account $sender$ transfers $value$ in $token$ to account $receiver$ in a transction of $txID$. The transfer call can be internal or external, where an internal transfer call is issued by a smart contract and an external call is issued by an EOA (external owner account).  

{\bf Swap}: 
A (normal) swap occurs between two accounts where account Alice transfers value to Bob in one token, and Bob transfers back the same value in another token to Alice. For the sake of simplicity, we consider the case of a swap of two transfers. 

A swap is atomic, if two transfers, say $tfIn$ and $tfOut$, match in sender/receiver and value. Specifically, 

\begin{eqnarray}
& \begin{cases}
tfIn.sender &\text{= } tfOut.receiver \\
tfIn.receiver &\text{= } tfOut.sender 
\label{eqn:atomic:tfmatch}
\end{cases} & \\
& tfIn.value * rate \text{= } tfOut.value &
\label{eqn:atomic:valmatch}
\end{eqnarray}

Note that $rate$ is the exchange rate between $tfIn.token$ and $tfOut.token$.

Deviating from atomicity, there are different anomalies conditions: 1) Transfer count mismatch where there is one standalone transfer. That is, Equations~\ref{eqn:atomic:tfmatch} do not hold. There are two cases in this anomaly: either Alice receiving value without sending value (i.e., freeride~\cite{DBLP:conf/podc/Herlihy18}) or Alice sending value without receiving value (i.e., underwater~\cite{DBLP:conf/podc/Herlihy18}). 

2) Value mismatch where the value Alice receives does not match the value Alice sends, with respect to the exchange rate. That is, Equation~\ref{eqn:atomic:valmatch} does not hold. There are two cases: either Alice receiving more value than the value sent (i.e., discount~\cite{DBLP:conf/podc/Herlihy18}) or Alice receiving less value than the value sent (i.e., overcharge~\cite{DBLP:conf/podc/Herlihy18}). 

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/anomalies.eps}
\end{center}
\caption{Swaps of three types: Type II and III are anomalies.}
\label{fig:swaps}
\end{figure}

We define three patterns of swaps:

\begin{itemize}
\item
A Type-I swap is an atomic swap whose transfers occur in one transaction.
\item
A Type-II swap is an atomic swap whose transfers occur in more than one transaction.
\item
A Type-III swap is a swap whose value does not match or whose transfer count does not match (i.e., a standalone transfer).
\end{itemize}

\section{Background: Uniswap}

\begin{figure}[!ht]
\centering
\subfloat[\texttt{swap} workflow]{%
\includegraphics[width=0.225\textwidth]{figures/uniswap-v2.eps}
\label{fig:uniswap2:swap}
}%
\hspace{0.05in}
\subfloat[\texttt{addLiquidity} workflow]{%
\includegraphics[width=0.225\textwidth]{figures/uniswap2-addliquidity.eps}
\label{fig:uniswap2:addliquidity}
}%
\caption{The Uniswap protocol}
\label{fig:uniswap2}
\end{figure}

{\bf Uniswap} is a decentralized exchange (DEX) protocol based on automated market maker (AMM). The Uniswap protocol is very successful in practice and powers several large-scale DEX instances including the top-3 DEXs on Ethereum, that is, Uniswap-V2, Uniswap-V3, Sushiswap (taking more than $90\%$ market (all time) as of Jan. 2022~\cite{me:etherscan:topdex}) and top-1 DEX on Binance Smart Chain, namely Pancakeswap. 

There are two common workflows in the Uniswap protocol: 1) \texttt{swap} which allows a trader to swap tokens, and 2) \texttt{addLiquidity} which allows a trader to deposit the two tokens to Uniswap's pool.

{\it \texttt{swap} workflow}: The Uniswap protocol facilitates the exchange of two tokens, say TokenIn and TokenOut, between two blockchain accounts, a trader and a so-called liquidity pool. 
As shown in Figure~\ref{fig:uniswap2}, in the first step, the trader account calls TokenIn's transfer function to transfer certain value to the pool account (i.e., tfIn). In the second step, the trader calls the swap function in the Uniswap's pool smart contract, which further calls TokenOut's transfer function (i.e., tfOut). 
In particular, the pool checks the balance difference between the pool smart contract and the token. If a difference is found, the pool assumes the balance update is from the trader who calls the swap function next.

The liquidity pool runs AMM and maintains the token reserves, based on which the exchange rate is calculated algorithmically. 

In practice, the trader can be an EOA account or a smart contract. In the former case, the two steps (i.e., $tfIn$ and $swap$) are two separate transactions. In the latter case, the actual trader delegates operation to a smart contract, called router. The trader EOA sends one transaction to invoke router smart contract, which conducts the two steps (tfIn and swap) in two internal calls. 

{\it \texttt{addLiquidity} workflow}: As shown in Figure~\ref{fig:uniswap2:addliquidity}, a trader, be it either an EOA or a smart contract account, transfers $TokenIn$ and $TokenOut$, at a certain ratio, to the liquidity pool, and then calls the pool's \texttt{addLiquidity} function, which returns a Uniswap-specific token (called LP token) to the trader.

\subsection{Threat Model}

An attacker is an EOA. Their goal is to steal tokens/value from a liquidity pool of a Uniswap-based DEX. The attacker does so by monitoring some conditions on the DEX state in real-time and sending crafted transactions to the DEX to illicitly claim the value stored there. A victim is an EOA whose tokens are stolen or illicitly extracted by the attacker EOA.

An attacker and a victim are involved in an anomalous swap. That is, a victim EOA transfers the value to the pool, which then transfers the value out to the attacker EOA. We distinguish two concepts: Swap anomaly and DEX attack. First, a DEX attack must occur with an anomalous swap that violates atomicity. An atomic swap, even with the deposit address being different from the sender address, is unlikely to be an attack instance, as the deposit address is specified by the sender. Second, while a DEX attack must be with an anomalous swap, the reverse is not true -- An anomalous swap does not have to be an attack. For instance, as we will see, an anomalous swap whose two transfers do not match in value can be caused by high fees (charged either by the pool or the token), which does not involve an attacker EOA.

\subsection{System Overview}
\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/workflow5.eps}
\end{center}
\caption{Workflow of data analytics to detect anomalies and attacks, as well as to analyze attackers'/victims' behavior.}
\label{fig:workflow:overall}
\end{figure*}

Figure~\ref{fig:workflow:overall} shows the overall data-analytical workflow. The input data is the XXX raw Ethereum transactions that we crawled from an Ethereum exploration web service, \url{https://bloxy.info/search}. {\bf 1) Anomaly detection}: We first run the proposed anomaly detection algorithm to discover anomalous swaps. {\bf 2) Attack detection}: From the anomalous swaps, we further detect actual attack instances, each with a pair of distinct attacker and victim accounts. {\bf 3) Behavior analysis}: The third-step conducts an in-depth analysis to uncover a variety of attackers' and victims' behavior including attacking strategies, attacking footprint, victim footprint, etc.
These three steps are described in \S~\ref{sec:anomaly}, \S~\ref{sec:attack}, and \S~\ref{sec:behavior} in the rest of this paper.

\section{Swap Anomaly Detection}
\label{sec:anomaly}

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.35\textwidth]{figures/workflow4.eps}
\end{center}
\caption{Overall data-analytical workflow}
\label{fig:workflow}
\end{figure}

\noindent
{\bf System overview}: 
Our goal is to detect DeFi attacks on Uniswap through measuring swap anomalies. The overall trace-analysis workflow, illustrated in Figure~\ref{fig:workflow}, consists of four steps: Preparing raw blockchain data (e.g., events and transactions) into DEX specific data records, match-making data records to find anomaluous swaps, detecting attacks and profiling attackers/victims' behavior in the swap anomalies, and finally analyzing the attack root causes in several case studies. This section covers the first two steps in fiding swap anomalies, while the next two sections present attack detection and characterization (\S~\ref{sec:detect}) and root cause analysis (\S~\ref{sec:cause}).

\subsection{Data Preparation}

The goal here is to prepare the raw blockchain data into the $tfIn$-and-$tfOut$ data schema used in Swap specification in \S~\ref{sec:model}. The raw blockchain data includes smart-contract events and function calls. We specifically select relevant information to Uniswap DEX.
Suppose the target is a liquidity pool and its two associated tokens (e.g., $tokenIn$ and $tokenOut$ as in Figure~\ref{fig:uniswap2}).
To reconstruct candidate the $tfIn$ records, we select all the calls that invoke one of the two tokens' transfer/transferFrom/mint functions and that transfer tokens to the pool's account. A reconstructed record is $tfIn(valIn, txID)$. 

To reconstruct candidate $tfOut$ records, we select the calls to the pool's function \texttt{swapCall}/\texttt{addLiquidity}. We also collect the events emitted by the pool. In particular, the Uniswap pool's events contain the mapping between $valIn$ and $ valOut$, so that it can reconstruct records $tfOut(valIn,valOut,txID)$. 

Here, we include $addLiquidity$ as a $tfOut$ candidate, because otherwise it could introduce false positives in our matchmaking step. 
Specifically, recall Figure~\ref{fig:uniswap2:addliquidity} where the \texttt{addLiquidity} workflow includes token transfers to the pool. 
Thus, a transfer call to TokenIn can be part of an \texttt{addLiquidity} workflow, and without distinguishing it to the case that it belongs to the \texttt{swap} workflow, the match-making step may mis-classify it as an underwater swap.

In summary, the data preparation produces two sets of data records. The first set contains the data records for $tfIn$ candidates including the selected function calls to transfer, transferFrom and mint, as described above. The second set stores the $tfOut$ candidates,  including the calls to functions swap and addLiquidities.

\subsection{Match-making Algorithm}
\label{sec:mmalgo}

\noindent{\bf Design goal and design space}: The goal is to join the two traces in order to find the anomalous swaps that violate atomicity. On the one hand, as one tfOut candidate (e.g., a swap) can match an arbitrary number of tfIn candidates, in theory, the join operation should be done on the powersets of tfIn/tfOut traces, which is clearly unscalable — for instance, the powerset of a $n$-record set has $2^n$ elements. On the other hand, if any approximation is applied to design more efficient join algorithm, one does not want to introduce false-positive swap anomalies, that is, the artifacts that mis-detected by the join algorithm and that can be avoided in a more precise join algorithm. 

Our algorithm design leverages a key invariant we observe in Uniswap's smart contract to save the search complexity without producing false positives. Specifically, Uniswap's liquidity pool smart contract runs in a single thread, and a swap/addLiquidity, say $C$, must only match any transfers that occur before $C$ and after $C$'s predecessor call to swap or addLiquidity. This invariant greatly saves the search space of match and allows to linearly merge the two traces with entries ordered by time.

\lstset{style=mystyle}
\begin{lstlisting}[caption=Psuedocode to find mismatch,
                   linerange={1-21},
                   firstnumber=1,
                   deletekeywords={[2]INT},
                   morekeywords={clustered},
                   framesep=8pt,
                   xleftmargin=40pt,
                   framexleftmargin=40pt,
                   frame=tb,
                   framerule=0pt, 
                   label=code:findmismatch,
                   float,floatplacement=H
                   ]
//tfIns and swapOrAddL are both ordered by time
def findMismatch(Record[] tfIns, Record[] tfOuts):
    for joinedpair in joinByTxId(tfIns, tfOuts):
        removeMatch(tfIns, tfOuts, joinedpair.i1, joinedpair.i2, joinedpair.j1, joinedpair.j2);
    for joinedpair in joinByTemporalSimilarity(tfIns, tfOuts):
        removeMatch(tfIns, tfOuts, joinedpair.i1, joinedpair.i2, joinedpair.j1, joinedpair.j2);
   
def removeMatch(Record[] tfIns, Record[] tfOuts, int i1, int i2, int j1, int j2){
    for s in powerset(tfIns[i1 ... i2]):
        for t in powerset(tfOuts[j1 ... j2]):   
        if sumValue(s) ==  sumValue(t):
            tfIns.markRemoval(s); 
            tfOuts.markRemoval(t); 
            return;
\end{lstlisting}

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.325\textwidth]{figures/automata3.eps}
\end{center}
\caption{Matchmaking algorithm in two steps that produces the Type-II and Type-III patterns that violate swap atomicity.}
\label{fig:automata}
\end{figure}

\noindent{\bf The algorithm}:
The proposed algorithm in Listing~\ref{code:findmismatch} takes as input the traces of tfIn and tfOut records and produces as output the swap anomalies it finds. The algorithm internally runs in two rounds. In the first round, it equi-joins the tfIn records with tfOut records based on their transaction IDs. In each joined tuple, which is a set of tfIn records and tfOut records in the same transaction, it match the tfIn and tfOut records. As shown by the removeMatch function in~\ref{XXX}, it finds a group of tfIn records that match a group of tfOut records in value. Specifically, if the tfIn record has the same value with a tfOut record in the same transaction (XXX), it constitutes a normal swap or addLiquidity operation, and the two records are removed from the two traces. If the value mismatches. it merges the two records into one, that is, the one with larger value. For instance, if a transfer of value 5 and a swap of value 8 are in the same transaction, it replaces the two records in the dataset with a merged swap record of value 8-5=3.

The second round runs a similar join-then-matchmaking process with the first round. The only difference is the join condition is temporal similarity, that is, a record tfOut[i] joins tfIn records that occur before tfOut[i] and after tfOut[i-1] (assuming tfIn and tfOut records are ordered in time). After the joined pair is produced, it runs the same match-making function and remove the matched cases.

After these rounds, what's left in the table are the mismatches.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.25\textwidth]{figures/join_problem2.eps}
\caption{Example on joining \texttt{swapEvent} and \texttt{tfIn} records}
\label{fig:joinproblem}
\end{figure}

{\it An example}: In Figure~\ref{fig:joinproblem} shows two example traces of tfIn and tfOut records. The two traces are aligned and sorted by time. Assume each record is handled by a distinct transaction. The figure shows that two matched cases (in green). The first transfer tf1 is a standalone tfIn (i.e., underwater) and the second swap is a standalone tfOut (i.e., freeride). In the red shade is a pair of tfIn and tfOut whose value does not match (a discount).

\subsection{Measurement Results}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Swap anomalies on Uniswap-based DEXs}
\label{tab:1}\centering{\footnotesize
\begin{tabularx}{0.5\textwidth}{ |X|c|c|c|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
  Swap types                & \# of \texttt{tfIn} & \# of  \texttt{tfOut} & Value/Diff (\$M) & Causes \\ \hline
  \multicolumn{5}{|l|}{Uniswap V2}   \\  \hline
 Type-I  & $52.7*10^6$  & $52.7*10^6$   & $6.18*10^5$  & Atomic swap \\ \hline
 Type-II  & $762$  & $761$   & {\bf $0.486$}  & Directly interact pool without router \\ \hline
 Type-II  & $35$  & $35$   & {\bf $0.205$}  & Router with partly error \\ \hline
 Type-III (Overcharge) & $2.01*10^5$ & $2.01*10^5$ & $23.3$ ($3.64$) & fees/penalty (1tx) \\ \hline
 Type-III (Discount) & $3879$ & $3879$ & {\bf $0.185$ ($0.094$)} & rebase (1tx) \\ \hline
 Type-III (Freeride) & $4767$ & $0$ & {\bf $1.26$} & Rebase/interest
\\ \hline
\end{tabularx}
}
\end{table}

We collect the traces of four Uniswap-based DEX'es and analyze the traces using the methods described in \S~\ref{sec:mmalgo}. The four DEX'es are Uniswap V2 on Ethereum, Uniswap V3 on Ethereum, Sushiswap on Ethereum, and Pancakeswap on Binance Smart Chain. We present the results of Uniswap V2 and Pancakeswap here in Table~\ref{tab:1}, while leaving the lesser interesting results of the other two DEX instances to Appendix~\ref{XXX}.

For each DEX, we report the measured cases of atomic swaps (i.e., value matched), discount/overcharge (i.e., value mismatched), and freeload/underwater (i.e., standalone transfer). In particular, when matching records in the same transaction in value, we only report the case with value difference larger than 10\%; we are aware that most DEX routers charge fees lower than 10\%, which are normal use cases and less interesting in the sense of finding anomalies. For each case, we report the number of transfers involved (including both tfIn and tfOut), as well as the total value. To estimate the value, we crawl the historical exchange rates reported by etherscan (\url{https://etherscan.io/tokens}) on the same day/hour of the reported swap. We also select high-value cases and report their causes.

In Table~\ref{tab:1}, on Uniswap V2, the majority of swaps, with total value of $618$ billion USD and in more than 0.5 billion Ethereum transactions (as in the third row of the table), are atomic ones, each of which is carried out by one transaction calling a router smart contract (recall Figure~\ref{fig:uniswap2}). Besides, as shown in the fourth row, there are $761$ atomic swaps, each of which is carried out by two or three transactions that directly call Uniswap's pool smart contract. The fifth row shows $35$ swaps that match in value but invoke a router smart contract with ``partly error.'' The case of ``partly error'' router smart contract is discussed in more details in \S~\ref{sec:partlyerror}.

On Uniswap V2, more than $20$ thousand swaps are overcharge, which are caused by the particularly high fees by the operating routers or tokens. For instance, some tokens enforce a fee scheme to penalize the token deposit and to encourage the withdrawal. 

3879 swaps are discount, where a trader account receives profit. A primary cause is a token's rebase operation that occurs before the swap, as will be described in details in \S~\ref{sec:rebase}.

In the eighth row, $4767$ swaps are standalone tfIn operations  (i.e., Freeride) that directly call the liquidity pool's swap function. In total, they are worth $1.26$ million USD. The profit come from the tokens' non-standard rebase operation or interest behavior.

\subsection{Case 1: Non-Standard Token Operations}
\label{sec:cases:rebase}

Token rebase is a non-standard token operation (e.g., not specified in ERC20) typically called by a privileged account. It supports increasing/decreasing a token's total supply by directly adjusting {\it all} token holders' balance. For instance, a token rebase can trigger to double all token owners' balance. The operation is useful in finance scenarios, such as stabilizing the token price.

Suppose a UniswapV2 pool receives a swapCall right after one of its tokens is rebased. The standalone swapCall after the rebase would succeed, constituting a Type-III anomaly.

Likewise, some tokens support interest, as a non-standard behavior. That is, the token balance increases at an interest rate over time. If one of a UniswapV2 pool's tokens supports interest, a standalone swapCall that occur a sufficiently long period after the previous swap would succeed and constitute a Type-III anomaly.  

The root cause of this type of anomaly is due to the way Uniswap-V2's pool manages its token reserves and misuses it to track the transfer-in in a swap. Specifically, UniswapV2 maintains a cached copy of its token balance (apart from the token smart contract).\footnote{The cached balance is supposed to calculate the two token's exchange rate and is necessary to accumulate the exchange rate over time in a defense against the pump-and-dump scheme that misuses the rate as a price oracle~\cite{Adams2020UniswapVC}.} However, Uniswap-V2 abuses this cached balance to track the amount of value transferred-in in a swap. While this (ab)use may be necessary to support flexible forms of transfer-ins (e.g., meta-transaction~\cite{XXX}), it would mistake a token rebase/interest as a legitmate transfer-in and falsely approves the transfer-out operation.

In essence, the pool smart contract makes a false assumption on the undefined behavior (not standardized in ERC20) of third-party tokens, including token rebase, interest, etc. In this misuse paradigm, a rebase operation creates a profitable/freeride opportunity which is seized by a subsequent swap call with crafted arguments to gain illicit profit. 

\section{Attack Detection}
\label{sec:attack}
\subsection{Detection Problem}
{\bf Attack specification}: In this work, we consider an adversarial trader who intentionally steals tokens from Uniswap pools without depositing other tokens. We specify three necessary conditions for an token-steal attack to hold: A1) the attacker account must gain profit; A2) the attacker cannot be the same with the victim account; A3) the attacker must intentionally mount the attack to gain the profit. 

To be more specific, consider as an example a Type-II swap where an account Alice deposits tokenIn in a pool in the first transaction, and the pool sends tokenOut to another account Bob. Clearly, Bob does receive profit from this swap, that is, Condition A1) holds. Condition A2) excludes the case that Alice and Bob are two public keys controlled by the same entity in the physical world. Condition A3) excludes the case that Bob's profit can be accident, that is, Bob is a normal/lucky trader who happens to swap tokens right after the Alice's profitable transaction.

In general, both Type-II and Type-III swap anomalies present profitable opportunities that could be exploited by an intentional attacker but could also be taken by a cautious or lucky trader. In Type-II swap, the profitable opportunity is presented in the first transaction (recall Figure~\ref{XXX}). In Type-III swap, the profitable opportunity is presented by an external event (e.g., the non-standard token \texttt{rebase} operation as will be described in the case study in \S~\ref{sec:cases:rebase}). 

{\bf Attack detection problem}: The goal in this section is to analyze the call traces to distinguish intentional attacks from accidental traders in the Type-II and Type-III swaps.

Detecting atomicity-violating attacks is non-trivial. Conditions A2 and A3 are not directly observable with the public blockchain data: For A2, the linkage between two blockchain accounts or the linkage between an account and a physical-world entity is off-chain information, which is hidden and opaque. Thus, knowing the account linkage is fundamentally difficult. Likewise, for A3, an account's intention is hidden and may not be directly observable.

Uncovering blockchain account linkage has been studied in the context of blockchain deanonymization. However, existing techniques, such as address clustering, are either ineffective or require off-chain background knowledge.

\subsection{Detection Method}

{\bf Detection method}: We characterize account behavior to detect atomicity-violating attacks on Uniswap. To distinguish attacks from accidental events, we use the following detection heuristics. Specifically, consider an account who receives tokens without paying tokens in an anomalous swap is an attacker candidate. An account who pays tokens without receiving another token in an anomalous swap is a victim candidate. 

\begin{itemize}
\item[D1] {\bf Systematic attacks}: 
If a candidate attacker account who receives profit from a large number of anomalous swaps and from a diverse set of pools or victim accounts, the account is an intentional attacker.
\item[D2] {\bf All-take-no-give}:
If a candidate account who receives profit by directly interacting with Uniswap's pool without going through a router smart contract, the account is an intentional attacker. The rationale is that an attacker directly calling a pool's swap function knowingly does so to receive benefit without doing a fair trade.
\item[D3] {\bf Switch-after-attack}:
If a candidate victim account switches to the safer router right after the anomalous swap, the account is an actual victim. 
\item[D4] {\bf Failed transactions}:
If a candidate attacker account sends a large number of failed transactions, the account is an attacker.
\item[D5] {\bf Cash-out}: 
If a candidate attacker account transfers what is received from an anomalous swap to a mixer service (i.e., cash-out immediately), the account is an actual attacker.
\end{itemize}

\subsection{Measurement Results}

\begin{table*}[h]
\begin{tabular}{|p{1.25cm}|p{1.25cm}|p{2cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{1.1cm}|p{1.3cm}|}
\hline
Attacker & \# attacks & Value stolen & \multicolumn{2}{|c|}{Attacker pattern} & \multicolumn{4}{|c|}{Victim pattern} & \# pools & \# victims\\
\cline{4-9}
accounts & {~} & ($10^3$ USD) & A1 & A2 & V1 & V2 & V3 & V4 & {~} & {~}\\
%#\multicolumn{2}{|l|}{Number of TransferOut}\\
\hline
1 & 38 & 556 & & 38 & 38 &  &  &  & 23 &  + 7\\
\hline
2 & 14 & 239 & & 14 & 14 &  &  &  & 1 &  + 3\\
\hline
3 & 7 & 113 & & 7 & 7 &  &  &  & 1 &  + 4\\
\hline
4 & 3 & 101 & & 3 & 3 &  &  &  & 7 &  1 + 1\\
\hline
5 & 49 & 101 & & 49 & 30 & 2 & 2 & 2 & 3 &  2 + 4\\
\hline
6 & 1231 & 20 & & 1231 & 97 & 39 &  &  & 210 & 12 + 5\\
\hline
7 & 28 & 16 & & 28 & 6 & 3 &  &  & 19 &  + 4\\
\hline
8 & 6 & 12 & & 6 & 6 &  &  &  & 4 &  + 3\\
\hline
9 & 5 & 7 & & 5 & 2 &  & 3 &  & 3 &  3 + 1\\
\hline
10 & 199 & 6 & & 199 &  & 199 &  &  & 1 &  + 0\\
\hline
\end{tabular}%
\caption{Attackers and their patterns}
\label{table:analysis}
\end{table*}


\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_attacker_timeline.eps}
\end{center}
\caption{Timeline of detected attacks.
Data from 07/09/2020 (block no. 10422671) - 06/29/2021 (block no. 12727620).}
\label{fig:attack}
\end{figure*}

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_victim_timeline.eps}
\end{center}
\caption{Timeline of detected victims. 
Data from 08/25/2020 (block no. 10731770) - 06/16/2021 (block no. 12645092).}
\label{fig:victim}
\end{figure*}

\section{Behavior Analysis and Eco-System Profiling}
\label{sec:behavior}

\section{Related Works}

This work is related to blockchain data analysis. We survey two bodies of related works, that is, blockchain-data analysis for attack detection and user de-anonymization.


{\bf Detecting Smart-Contract Program-level Attacks}: Attack detection on blockchain generally works as distilling the attack signatures from known vulnerabilities and attack patterns and matching certain representation of smart-contract execution (e.g., in transactions, function-call graph or instruction traces) against the attack signatures. There are known patterns of smart-contract program-level attacks, such as reentrancy attacks, transaction order dependency, etc. Existing works tackle the detection of program-level attacks on Ethereum-like blockchains. 
 
TxSpectror~\cite{DBLP:conf/uss/ZhangZZL20} records and replays Ethereum transactions into fine-grained EVM instruction traces, which are stored in datalog databases and queries to compare against the signatures of known attacks. Similarly, Zhou et al~\cite{DBLP:conf/uss/ZhouYXCY020} model the coarse-grained traces of smart contract function calls and match them against known attack signatures. At its core, two function calls are modeled, that is, smart contract creation/destroy and token transfers (money flow). Su et al~\cite{DBLP:conf/uss/SuSDL0XL21} uses reported attack instances to extract attack signatures, and it discovers new attacks as well as uncovers the attacker/victim behavior by systematically analyzing the Ethereum blockchain traces. Other similar work~\cite{DBLP:conf/uss/0001L21} detects the attack instances of known vulnerabilities.  

{\bf Detecting DeFi Protocol-level Attacks}: In addition to detecting program-level attacks, there are related works on detecting protocol-level attacks on deployed DeFi applications. Notable DeFi attack patterns include frontrunning, arbitrage, etc. 

Torres, et al.~\cite{DBLP:conf/uss/TorresCS21} detects front-running attacks by matching Ethereum transactions against a signature of success-failure transaction pair. Qin et al~\cite{DBLP:journals/corr/abs-2101-05511} systemizes different types of front-running attacks and measures the attacks and mitigations in the wild.

Front-running attacks are a class of attacks in which the attacker inserts a malicious transaction before the victim transaction to extract illicit profit (e.g., to win an auction bid unfairly). More generally, front-running is a class of MEV or miner extractable value, in which transaction order can be manipulated by a profit-driven miner to receive additional profit.

Arbitrage attacks work by an aggressive trader gain profit by exploiting difference of exchange rates across different DEXes/price oracles. Wang, et al~\cite{DBLP:journals/corr/abs-2105-02784} detects cyclic arbitrage on Uniswap-V2, by finding profitable cycles on token-transfer graph (nodes are tokens and edges are transfers). Similarly, Zhou, et al~\cite{DBLP:conf/sp/ZhouQCLG21} discovers profit-generating transitions in real time by finding cycles  and leveraging solvers.





{\bf User de-anonymization}: While blockchain accounts and their activities are visible, the linkage of accounts (which are public keys) with real-world identities is not directly observable. There are existing works to infer blockchain account linkage in efforts to deanonymize users. Specifically, there are three types of linkage information: 1) Whether a specific account is linked to a specific real-world user identity. Existing works~\cite{DBLP:conf/fc/KoshyKM14} monitor a blockchain network' traffic of transactions propagated from an IP and link the transaction sender's account with the IP. Other works~\cite{XXX} aggregate transaction volume of a given account and use background knowledge to link the account to real-world ID.

2) Whether two blockchain accounts are linked, as the sender and receiver, in a privacy-enhanced transaction. Mixing services are intended to break the sender-receiver linkage. There are existing works aimed at reconstructing the sender-receiver relation on transactions relayed through mixing services. In particular, address reuse is a heuristic to link transaction senders/receivers on Bitcoin like blockchains~\cite{DBLP:conf/uss/YousafKM19,DBLP:conf/uss/KalodnerMLGPCN20}.

3) Whether two blockchain accounts are shared by the same real-world user. On Bitcoin, transaction graph analysis~\cite{DBLP:books/daglib/0040621} are proposed to recover the account linkage. Particularly, address clustering heuristics are proposed. For instance, two accounts that are co-spent by a Bitcoin transaction or that involve a change are likely to be controlled by the same off-chain user. These address clustering heuristics are useful only in the context of  Bitcoin's UTXO model. Address clustering is useful to uncover the money flow in online criminal activities such as ransomware payments on Bitcoin~\cite{DBLP:conf/sp/HuangALIBMLLSM18}. 

Of most relevance to this work is the address clustering techniques proposed to link Ethereum accounts~\cite{DBLP:conf/fc/Victor20}. Specifically, the observation is that some DEX'es support the deposit address, that is, trader Alice swapping token T0 for token T1 can specify a ``deposit'' address to receive T1. Multiple accounts using the same deposit address are likely to be the same off-chain user. 

This work is different from Ethereum account linkage. In this work, the attack detection problem is to verify whether two Ethereum accounts are from two off-chain users, which is different from detecting if two accounts are linked by the same off-chain user. Moreover, the Ethereum address clustering work~\cite{DBLP:conf/fc/Victor20} has to assume that the swap is atomic, normal one, so that they can attribute address sharing to the cause of the same off-chain user. By contrast, in this work, we do observe two sender accounts share the same deposit address, but they are caused by two victim accounts whose swaps are grabbed by the same attack account, as verified by our analysis of attacker/victim behavior.



==> text/misc/ZZZ.tex <==
{\bf Insecurity of Uniswap V3}: 


 {\bf Enforcing Atomicity in Pools}: As analyzed previously, the root cause of Uniswap V2's vulnerability is that the liquidity pool does not enforce swap atomicity, but instead expose overly flexible API for the application-specific routers to enforce it. The benefit is that the pool supports flexible forms of deposits and withdrawals, such as a trader can externally transfer tokens to make deposit. 

One can ensure swap atomicity at the expense of less pool-API flexibility. Specifically, the pool smart contract can ensure {\it every} swap must be executed in one transaction and that transaction sends deposit and withdrawal of the same value in all code paths. For instance, Uniswap V3 enforces the one-transaction rule by having the pool to call back the router to transfer the deposit. However, this design does not support the legitimate use cases where the deposit and withdrawal need to be in two separate transactions.
, such as cross-chain swaps and stable coin swaps.

Alternatively, the pool can maintain states to support atomic deposit and withdrawal across transactions. The pool ensures that the value deposited can only be withdrawn by designated traders.


==> text/misc/case_bancorx.tex <==
\section{Case study: BancorX}

\subsection{Approach}
\begin{figure}\centering
\includegraphics[width=0.3\textwidth]{figures/protocol_pegged_bancorx.eps}
\caption{BancorX protocol for cross-chain swaps}
\label{fig:protocol:bancorx}\end{figure}

\noindent
{\bf Preliminary of BancorX protocol}:
BancorX works between a pair of blockchains both of which are required to support smart contracts. As shown in Figure~\ref{fig:protocol:bancorx}, in Step \ballnumber{1}, the trader makes the deposit on the ``source'' smart contract by calling function \texttt{xTransfer}. In Step \ballnumber{2}, the custodian monitors the ``source'' blockchain's transaction history and is notified of the invocation of \texttt{xTransfer} in the previous step. In Step \ballnumber{3}, the custodian invokes the ``destination'' smart contract's function \texttt{reportTx} that mints the pegged token under the trader's account. In deployment, there are $3$ custodians, and only when all of them call \texttt{reportTx} the token mint can occur.
Also, BancorX is a  ``symmetrically'' protocol and can be deployed in both directions between a pair of blockchains, for instance, transferring assets from Ethereum to EOS and from EOS to Ethereum.

\noindent
{\bf Method}:
We follow the general approach described in \S~\ref{sec:generalmethod} by constructing a trace database and conducting data analytics on it. Specifically, the BancorX trace database contains the transactions and function calls on both source and destination blockchains. Consider transferring assets from Ethereum to EOS as an example. The database contains all Ethereum transactions and EOS transactions.
We run the SQL query as defined in List~\ref{sql:bancorx} on the database. As a cross-chain swap cannot be done in a single transaction, we only consider the case of multi-transaction swaps. The third SQL query joins two intermediary results, $T1$ and $T2$, on the following conditions: equality of receiver account (i.e., \texttt{pay\_to} argument in Table~\ref{tab:api}), value (i.e., argument \texttt{\_amount}) and transaction ID (i.e., argument \texttt{txID}).
This method can capture atomic swaps (\textsc{A}) and anomalies (including \textsc{U}, \textsc{F}, \textsc{O}, and \textsc{D}).

\input{text/lst_sql_bancorx.tex}

\subsection{Result}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Time difference of Ethereum's \texttt{xTransfer} and EOS's \texttt{reportTx} in BancorX swaps}
\label{tab:bancorx:timediff}\centering{\small
\begin{tabularx}{0.275\textwidth}{ |X|c| }
  \hline
  Time delay (minutes) & Percentage \\ \hline
  [0,2] & 1.06\% \\ \hline
  [2,3] & 19.34\% \\ \hline
  [3,4] & 35.13\% \\ \hline
  [4,5] & 24.84\% \\ \hline
 [5,6] & 11.59\% \\ \hline
 [6,10] & 6.1\% \\ \hline
 [10,60] & 0.74\% \\ \hline
 [60,600] & 0.82\% \\ \hline
 [600,1200] & 0.47\% \\ \hline
\end{tabularx}
}
\end{table}

We get the BancorX's EOS trace from xblock dataset~\cite{zheng2020xblockeos} and Ethereum trace from Google’s BigQuery service~\cite{me:eth:bigquery}.
We match the cross-chain transactions from these two blockchains by using \texttt{txHash} of Ethereum and \texttt{txID} of EOS.
We measure if it mints tokens on the EOS blockchain after the \texttt{xTransfer} is sent on Ethereum and how many reporters report to the \texttt{xTransfer} transaction.


We find that Ethereum to EOS has $3$ cases that no tokens are minted on EOS. Two of these cases occurred on February 25, 2019 and one case happened on April 12, 2019. Each of these $3$ cases only have $2$ \texttt{reportTx} transaction. The first two \texttt{reportTx} are all sent within $5$ minuts after the the \texttt{xTransfer} included in the Ethereum blockchain. The missing of the third \texttt{reportTx} transaction causes the atomicity anomalies. 
We then measure the reporting time delay, which is the time difference between an initiate \texttt{xTransfer} transaction and a \texttt{reportTx} transaction.
Table~\ref{tab:bancorx:timediff} illustrates the distribution of time difference transferring tokens from Ethereum to EOS. 
$98.06\%$ of the \texttt{reportTx} transactions are sent within $10$ minutes after their corresponding \texttt{xTransfer} transactions. 

Interestingly, we found $52$ \texttt{reportTx} (accounting for $0.47\%$ of all cases) calls are sent more than $10$ hours after the \texttt{xTransfer} included in the Ethereum blockchain. Among them, $15$ \texttt{reportTx} are the only one that larger than $10$ hours from $3$ \texttt{reportTx} of the corresponding \texttt{xTransfer}. $4$ of them are the case that two of the \texttt{reportTx} corresponding to a \texttt{xTransfer} are longer than $10$ hours. The rest $33$ case are that all $3$ \texttt{reportTx} are longer than $10$ hours. The largest delay we find is a \texttt{xTransfer} sent on April 20, 2019, the first corresponding \texttt{reportTx} is sent in $3$ minutes, but the third \texttt{reportTx} is sent in around $20$ hours.

\ignore{
We get the BancorX's EOS trace from xblock dataset~\cite{zheng2020xblockeos} and Ethereum trace from Google’s BigQuery service~\cite{me:eth:bigquery}.
We match the cross-chain transactions from these two blockchains by using \texttt{txHash} of Ethereum and \texttt{txID} of EOS.
We measure how many reporters report to an initial \texttt{xTransfer} transaction and if it mints tokens on the other blockchain.
We find that Ethereum to EOS has $4$ cases that only have $2$ \texttt{reportTx} transaction and no tokens are minted on EOS. There is no the third \texttt{reportTx} transaction even it happened more than $1$ year ago.

We then measure the reporting time delay, which is the time difference between an initiate \texttt{xTransfer} transaction and a \texttt{reportTx} transaction.
Table~\ref{tab:bancorx:timediff} illustrates the distribution of time difference transferring tokens from Ethereum to EOS. 
$98.06\%$ of the \texttt{reportTx} transactions are sent within $10$ minutes after their corresponding \texttt{xTransfer} transactions. Interestingly, we found $52$ cases (accounting for $0.47\%$ of all cases) whose \texttt{reportTx} calls are sent more than $10$ hours after the \texttt{xTransfer} calls.
}
\ignore{
The average reporting delay of transferring tokens from EOS to Ethereum is larger than transferring tokens from Ethereum to EOS.
As shown in Figure~\ref{fig:Time difference EOS to Ethereum}, the distribution of time difference transferring tokens from EOS to Ethereum illustrated in Figure~\ref{fig:Time difference EOS to Ethereum} shows only $49.90\%$ of reportTx transactions are sent within $10$ minutes. There are even $10.67\%$ of reportTx transactions are sent after $10$ hours.}


==> text/misc/lst1.tex <==
\definecolor{mygreen}{rgb}{0,0.6,0}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\ttfamily,        % the size of the fonts that are used for the code
  keywordstyle=\color{red}\bfseries,       % keyword style
  showstringspaces=false,
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={(*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  language=Java,                 % the language of the code
  morekeywords={*,pay_to,txid,_bitcoinHeaders,txID,_amount,_txIndexInBlock,...},            % if you want to add more keywords to the set
  numbers=none,                    % where to put the line-numbers; possible values are (none, left, right)
%  numbersep=5pt,                   % how far the line-numbers are from the code
%  numberstyle=\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
%title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{table*}[!htbp] %force in current page, disable float.
\caption{Smart-contract functions. The arguments in red are used to match transactions in multi-transaction swaps.}
\label{tab:api}\centering{\small
\noindent
\begin{tabular}{|p{2cm}|p{14cm}|}
\hline
Smart contracts & Functions \\ \hline
ERC20 & \begin{lstlisting}[aboveskip=-4pt,belowskip=-4pt]
transfer(address pay_from, address pay_to);
\end{lstlisting}\\ \hline
Uniswap-V2 & \begin{lstlisting}[aboveskip=-4pt,belowskip=-4pt]
swap(uint amount0Out, uint amount1Out, address pay_to, bytes calldata data)
\end{lstlisting}\\ \hline
BancorX &
\begin{lstlisting}[aboveskip=-4pt,belowskip=-4pt]
xTransfer(bytes32 _toBlockchain, bytes32 pay_to, uint256 _amount[, uint256 _id])
reportTx(bytes32 _fromBlockchain, uint256 txID, address pay_to, uint256 _amount, uint256 _xTransferId)
\end{lstlisting}
\\ \hline
wBTC &
\begin{lstlisting}[aboveskip=-4pt,belowskip=-4pt]
confirmMintRequest(bytes32 requestHash) external onlyCustodian
addMintRequest(uint amount, string txid, string depositAddress) external onlyMerchant 
\end{lstlisting}
  \\ \hline
tBTC &
\begin{lstlisting}[aboveskip=-4pt,belowskip=-4pt]
provideBTCFundingProof(bytes4 _txVersion, bytes memory _txInputVector, bytes memory _txOutputVector, bytes4 _txLocktime, uint8 _fundingOutputIndex, bytes memory _merkleProof, uint256 _txIndexInBlock, bytes memory _bitcoinHeaders) 
provideRedemptionProof(bytes4 _txVersion, bytes memory _txInputVector, bytes memory _txOutputVector, bytes4 _txLocktime, bytes memory _merkleProof, uint256 _txIndexInBlock, bytes memory _bitcoinHeaders) 
\end{lstlisting}
\\ \hline
\ignore{
}
\end{tabular} 
}
\end{table*}



==> text/misc/lst_q3.tex <==
\definecolor{mygreen}{rgb}{0,0.6,0}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={(*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{purple},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{HTML}{C42043}
\definecolor{backcolour}{HTML}{F2F2F2}
\definecolor{bookColor}{cmyk}{0,0,0,0.90}  
\color{bookColor}

\lstset{upquote=true}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{codepurple},
    numberstyle=\numberstyle,
    stringstyle=\color{blue},
    basicstyle=\footnotesize\ttfamily,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=10pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
}
\lstset{style=mystyle}

\begin{lstlisting}[caption=Subquery Q3,
                   linerange={1-21},
                   firstnumber=1,
                   deletekeywords={[2]INT},
                   morekeywords={clustered},
                   framesep=8pt,
                   xleftmargin=40pt,
                   framexleftmargin=40pt,
                   frame=tb,
                   framerule=0pt, 
                   label=sql:uniswap,
                   float,floatplacement=H
                   ]
-- Join subquery Q3: Inner join by payer-payee across txs
def joinAcrossTx(tfIn, tfOut):
  N = len(tfIn); M = len(tfOut)
  i=0; j=0
  while (i<N and j<M):
    if (tfIn[i].timing < tfOut[j].timing):
      if(i==N) or (tfIn[i+1].timing > tfOut[j].timing):
        emit(tfIn[i],tfOut[j])
        i+=1;  j+=1
      else:
        i+=1
    else:
      j+=1
\end{lstlisting}



==> text/misc/lst_q31.tex <==
\ignore{
\definecolor{mygreen}{rgb}{0,0.6,0}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={(*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{purple},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{HTML}{C42043}
\definecolor{backcolour}{HTML}{F2F2F2}
\definecolor{bookColor}{cmyk}{0,0,0,0.90}  
\color{bookColor}

\lstset{upquote=true}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{codepurple},
    numberstyle=\numberstyle,
    stringstyle=\color{blue},
    basicstyle=\footnotesize\ttfamily,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=10pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
}
\lstset{style=mystyle}

\begin{lstlisting}[caption=Subquery Q3,
                   linerange={1-21},
                   firstnumber=1,
                   deletekeywords={[2]INT},
                   morekeywords={clustered},
                   framesep=8pt,
                   xleftmargin=40pt,
                   framexleftmargin=40pt,
                   frame=tb,
                   framerule=0pt, 
                   label=sql:uniswap:q3,
                   float,floatplacement=H
                   ]
//Join subquery Q3: Inner join by payer-payee across txs
void joinAcrossTx(Call[] tfIn, Call[] tfOut){
  int i=0, j=0;
  while (i < tfIn.length & j < tfOut.length){
    int k = findMatch(tfIn[i], tfOut, true);
    if(k != 0) {i++; if(k == j) j++; continue;}
    k = findMatch(tfOut[j], tfIn, false);
    if(k != 0) {j++; if(k == i) i++; continue;}
    i++; j++;
}}

int findMatch(Call ele, Call[] list, Boolean downwards){
  int p1 = ..., p2 = ...;
  while(downwards ? p1++ < list.length : p1-- > 0){
    if(list[p1].val == ele.val) {emit(p1); return p1;}
    else if(list[p1].val > ele.val) continue;
    while(downwards ? p2++ < list.length : p2-- > 0){
      if(list[p1].val+list[p2].val == ele.val){
        emit(p1,p2); return p1;
}}}}
\end{lstlisting}



==> text/misc/lst_sql.tex <==
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{HTML}{C42043}
\definecolor{backcolour}{HTML}{F2F2F2}
\definecolor{bookColor}{cmyk}{0,0,0,0.90}  
\color{bookColor}

\lstset{upquote=true}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{codepurple},
    numberstyle=\numberstyle,
    stringstyle=\color{blue},
    basicstyle=\footnotesize\ttfamily,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=10pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
}
\lstset{style=mystyle}

\ignore{

\newcommand\numberstyle[1]{%
    \footnotesize
    \color{codegray}%
    \ttfamily
    \ifnum#1<10 0\fi#1 |%
}
}


\begin{lstlisting}[ language=SQL,
                    deletekeywords={IDENTITY},
                    deletekeywords={[2]INT},
                    morekeywords={clustered},
                    framesep=8pt,
                    xleftmargin=40pt,
                    framexleftmargin=40pt,
                    frame=tb,
                    framerule=0pt, 
                    caption={Filter query for Uniswap-V2},
                    label=sql:uniswap,
                    float,floatplacement=H ]
-- Select the candidate set of swaps' transferIn 
SELECT * AS T1
FROM CallTable
WHERE callee_func IN ("transfer", "transferFrom") AND data.pay_to IN SET_POOL_UNISWAP

-- Select possible causes 
SELECT * AS T2
FROM CallTable
WHERE callee_func == ("swap", "addLiquidity")

-- Union the two sets to find swaps
T1 UNION T2
ORDER BY txID, call_seq
\end{lstlisting}


==> text/misc/lst_sql2.tex <==
\begin{lstlisting}[ language=SQL,
                    deletekeywords={IDENTITY},
                    deletekeywords={[2]INT},
                    morekeywords={clustered},
                    framesep=8pt,
                    xleftmargin=40pt,
                    framexleftmargin=40pt,
                    frame=tb,
                    framerule=0pt, 
                    caption={SQL query for Uniswap-V2},
                    label=sql:uniswapv2:2,
                    float,floatplacement=H ]
SELECT * AS T1_SINGLETX
FROM CallTable
WHERE callee_func IN ("wrappedSwap", "wrappedAddLiquidity")

SELECT * AS T2_MULTITX
FROM CallTable
WHERE txID NOT IN (SELECT txID FROM T1_SINGLETX)

SELECT * AS T3_TFTOPOOL
FROM T2_MULTITX
WHERE callee_func IN ("transfer", "transferFrom") AND data.pay_to IN SET_POOL_UNISWAP

-- Select possible causes
SELECT * AS T4_CALLPOOL
FROM T2_MULTITX
WHERE callee_func == ("swap", "addLiquidity")
    
-- Union the two sets to find swaps
SELECT *
FROM T3_TFTOPOOL, T4_CALLPOOL
WHERE T3_TFTOPOOL.data.pay_to == T4_CALLPOOL.data.pay_to AND T3_TFTOPOOL.data._amount == T4_CALLPOOL.data._amount
AND T4_CALLPOOL.callee_func == "swap"
ORDER BY txID, call_seq

SELECT *
FROM T3_TFTOPOOL AS T31, T3_TFTOPOOL AS T32, T4_CALLPOOL
WHERE T31.data.pay_to == T4_CALLPOOL.data.pay_to AND 
T32.data.pay_to == T4_CALLPOOL.data.pay_to AND 
AND T4_CALLPOOL.callee_func == "addLiquidity"
ORDER BY txID, call_seq
\end{lstlisting}


==> text/misc/lst_sql3.tex <==
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{HTML}{C42043}
\definecolor{backcolour}{HTML}{F2F2F2}
\definecolor{bookColor}{cmyk}{0,0,0,0.90}  
\color{bookColor}

\lstset{upquote=true}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{codepurple},
    numberstyle=\numberstyle,
    stringstyle=\color{blue},
    basicstyle=\footnotesize\ttfamily,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=10pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
}
\lstset{style=mystyle}

\begin{lstlisting}[ language=SQL,
                    deletekeywords={IDENTITY},
                    deletekeywords={[2]INT},
                    morekeywords={clustered},
                    framesep=8pt,
                    xleftmargin=40pt,
                    framexleftmargin=40pt,
                    frame=tb,
                    framerule=0pt, 
                    caption={Subquery Q1 (SQL)},
                    label=sql:uniswapv2:2,
                    float,floatplacement=H ]
-- Join subquery Q1: Inner join by payer-payee in a single tx
SELECT * as results_atomic1
FROM table_tfIn INNER JOIN table_tfOut
ON table_tfIn.txID = table_tfOut.txID AND table_tfIn.payee == table_tfOut.payer AND table_tfIn.val = table_tfOut.val
\end{lstlisting}


==> text/misc/lst_sql_bancorx.tex <==
\ignore{
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{HTML}{C42043}
\definecolor{backcolour}{HTML}{F2F2F2}
\definecolor{bookColor}{cmyk}{0,0,0,0.90}  
\color{bookColor}

\lstset{upquote=true}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{codepurple},
    numberstyle=\numberstyle,
    stringstyle=\color{blue},
    basicstyle=\footnotesize\ttfamily,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=10pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
}
\lstset{style=mystyle}

\newcommand\numberstyle[1]{%
    \footnotesize
    \color{codegray}%
    \ttfamily
    \ifnum#1<10 0\fi#1 |%
}

}


\begin{lstlisting}[ language=SQL,
                    deletekeywords={IDENTITY},
                    deletekeywords={[2]INT},
                    morekeywords={clustered},
                    framesep=8pt,
                    xleftmargin=40pt,
                    framexleftmargin=40pt,
                    frame=tb,
                    framerule=0pt, 
                    caption={SQL query for BancorX},
                    label=sql:bancorx,
                    float,floatplacement=H ]
-- Select the candidate set of swaps' transferIn 
SELECT * AS T1
FROM Ethereum.CallTable
WHERE callee_func IN ("xTransfer") AND callee_contract IN SET_ETHADDR_BANCORX

-- Select possible causes 
SELECT * AS T2
FROM EOS.CallTable
WHERE callee_func == ("reportTx") AND callee_contract IN SET_EOSADDR_BANCORX

-- Union the two sets to find swaps
SELECT * 
FROM T1 OUTER JOIN T2
ON T1.txID == T2.data.txID AND T1.data.pay_to == T2.data.pay_to AND T1.data._amount == T2.data._amount
\end{lstlisting}


==> text/misc/lst_sql_filter.tex <==
\begin{lstlisting}[ language=SQL,
                    deletekeywords={IDENTITY},
                    deletekeywords={[2]INT},
                    morekeywords={clustered},
                    framesep=8pt,
                    xleftmargin=40pt,
                    framexleftmargin=40pt,
                    frame=tb,
                    framerule=0pt, 
                    caption={SQL query for Uniswap-V2},
                    label=sql:uniswapv2:2,
                    float,floatplacement=H ]
-- 1. Filter-Stage Queries
SELECT * AS T1_SINGLETX
FROM CallTable
WHERE callee_func IN ("wrappedSwap", "wrappedAddLiquidity")

SELECT * AS T2_MULTITX
FROM CallTable
WHERE txID NOT IN (SELECT txID FROM T1_SINGLETX)

SELECT * AS T3_TFIN
FROM T2_MULTITX
WHERE callee_func IN ("transfer", "transferFrom") AND data.pay_to IN SET_POOL_UNISWAP

-- Select possible causes
SELECT * AS T4_TFOUT
FROM T2_MULTITX
WHERE callee_func == ("swap", "addLiquidity")
    
-- 2. Join-Stage Queries: Join by payer-payee
SELECT *
FROM T3_TFIN, T4_TFOUT
WHERE T3_TFIN.data.pay_to == T4_TFOUT.data.pay_to AND T3_TFIN.data._amount == T4_TFOUT.data._amount
AND T4_TFOUT.callee_func == "swap"
ORDER BY txID, call_seq

-- 2. Join-Stage Queries: Optimistic similarity join
SELECT *
FROM T3_TFIN AS T31, T3_TFIN AS T32, T4_TFOUT
WHERE T31.data.pay_to == T4_TFOUT.data.pay_to AND 
T32.data.pay_to == T4_TFOUT.data.pay_to AND 
AND T4_TFOUT.callee_func == "addLiquidity"
ORDER BY txID, call_seq
\end{lstlisting}


==> text/old/paper.tex <==
\section{Introduction}

Swapping the ownership of crypto assets between accounts is an essential DeFi application. For instance, decentralized exchange or DEX supports the swap business on a single blockchain. DEX is among the most popular DeFi applications on deployed blockchains, notably Uniswap-V2 on Ethereum. For another instance, cross-chain swaps increases the liquidity of crypto assets and receive increasing popularity in practice.

Atomicity is the key correctness property of any swap, which states a swap should be executed in an all-or-nothing manner without being interleaved with other swaps. There are existing trustless protocols that guarantee atomicity by design, such as atomic cross-chain swaps (ACCS~\cite{DBLP:conf/podc/Herlihy18}). However, these protocols are slow and costly, causing multiple rounds of transactions, leaving them with limited adoption in practice. Practical swaps rely on either the faith of good behavior of trusted third-parties or the flawless program implementation of smart contracts. Take Uniswap-V2 as an example. Uniswap-V2's a composable automatic market maker (AMM), consisting of the frontend router layer and backend liquidity pools. It is designed to enforce swap atomicity at the router layer. In deployment, a router can be materialized on-chain as a smart contract (e.g., Uniswap-V2's default router smart contract or others implementing the 0x protocols) or off-chain operated by asset owners. With off-chain routers, the atomicity of swaps is left in the hands of trusted third-parties. Besides DEX, the deployed cross-chain swaps also widely include custodians in their protocol, who are trusted to send tokens on one blockchain when they receive tokens from the trader on another blockchain.

This work examines the atomicity assumption made in deployed crypto-asset swaps and conducts measurements to uncover the incidents of atomicity violation. We use the notions of atomicity anomalies~\cite{DBLP:conf/podc/Herlihy18} as the measurement goals. We propose data analysis on the traces of transactions and function calls in relevant blockchains. Our principled approach is to select from the traces the sets of candidate transfer calls in swaps and then to join the sets on certain conditions to discover swaps of atomicity and anomalies. Ideally, atomicity anomalies can be detected by outer joins when the function call traces are stored in relational databases. However, the anomaly detection is complicated in practice by a number of factors such as interference of other workflows than swaps in a DEX (e.g., Uniswap-V2's \texttt{addLiquidity}), special behavior of tokens (e.g., self-changing balances), et al. We propose two-phase data analysis on relational trace database, in which the first stage runs an SQL query to select and union candidate transfers, and the second stage runs a state machine that checks the validity or atomicity of the selected swaps.

We conduct two case studies using our general method above, respectively on Uniswap-V2 as a representative single-chain DEX and BancorX as a cross-chain swap service. We report the uncovered cases of atomicity anomalies and the delays between transfers in atomic swaps. The results show the anomalous swaps in Uniswap-V2 where two swaps can be interleaved in execution. This can be exploited to exchange rates during a swap and gain illicit profit. On BancorX, we discover atomicity anomalies in which the trader transfers her asset to the counterparty but never receives her exchanged asset (i.e., the \textsc{UNDERWATER} anomaly as defined in \S~\ref{sec:model}). We further inspect the uncovered cases that show the anomalies are caused by the insufficient confirmations from the custodians. The BancorX results also show the significant delay between two transfers of a swap (e.g., as long as 20 hours).

\section{Data Models and Definitions}
\label{sec:model}

\noindent
{\bf Transfer}: 
Given two accounts (blockchain addresses) $t_S$ and $t_R$, a transfer $tf$, denoted by $\langle{}t_S,t_R,c,v,b,d,txid\rangle{}$, sends value $v$ in currency $c$ from sender account $t_S$ to receiver account $t_R$. This transfer occurs on blockchain $b$ and is carried out by the transaction of hash $txid$. $d$ is the ``data'' field of the transaction, which includes information related to smart-contract function invocation. 

\noindent
{\bf Swap}: 
A (valid) swap consists of two transfers that can be ``matched'' on the conditions of their senders, receivers and the equality of their value. That is, a swap's two transfers $tf_1$ and $tf_2$ meet the following conditions:

\begin{eqnarray}
\begin{cases}
tf_1.t_S& \text{= } tf_2.t_R \\
tf_1.t_R&  \text{= } tf_2.t_S
\end{cases}
\label{eqn:atomic:match}
\end{eqnarray}

A swap can be materialized on a single blockchain (i.e., $tf_1.b==tf_2.b$)  or multiple blockchains(i.e., $tf_1.b\neq{}tf_2.b$) . The former type of swap is carried out by a DEX on a single blockchain, the latter type of swap is carried out cross-chain protocols.

\begin{figure}[!ht]
  \begin{center}
    \subfloat[Swap anomalies]{%
\includegraphics[width=0.075\textwidth]{figures/atomicity2.eps}
\label{fig:atomicity}
    }%
\hspace{0.5in}
    \subfloat[Workflow]{%
\includegraphics[width=0.125\textwidth]{figures/workflow.eps}
\label{fig:workflow}
    }%
  \end{center}%\vspace{-0.15in}
  \caption{Modeling swaps}
\label{fig:swaps}
\end{figure}

The exchange rate of the swap is defined as $r$=$\frac{tf_1.v}{tf_2.v}$, which can be determined differently on different platforms.

\noindent
{\bf Atomicity and anomalies}: A swap is \textsc{ATOMIC} or \textsc{A} if the two transfers meet the condition defined in Equations~\ref{eqn:atomic:match} and the timing difference of the two transfers is within a timeout threshold $tt$.

A swap is a \textsc{FREERIDER} or \textsc{F} if it only has $tf_2$ but not a matching $tf_1$, that is, $\langle{}-,tf_2\rangle{}$. In other words, the account $tf_2.t_R$ receives value in $tf_2$, yet without paying anything (i.e., without $tf_1$). 

Relaxing the condition, a swap $\langle{}tf_1,tf_2\rangle{}$ is a \textsc{DISCOUNT} or \textsc{D} if $\frac{tf_1.v}{tf_2.v}<r$ where $r$ is the market exchange rate between currencies $tf_1.c$ and $tf_2.c$. 

A swap is an \textsc{UNDERWATER} or \textsc{U} if it only has $tf_1$ but not a matching $tf_2$. In other words, the account $tf_1.t_S$ pays valuable in her own currency in transfer $tf_1$, yet without receiving anything (i.e., without $tf_2$). 

A swap $\langle{}tf_1,tf_2\rangle{}$ is an \textsc{OVERCHARGE} or \textsc{O} if $\frac{tf_1.v}{tf_2.v}>r$ where $r$ is the market exchange rate between currencies $tf_1.c$ and $tf_2.c$. 

Figure~\ref{fig:atomicity} illustrates the relationship of swaps of different types. 

\section{General Transaction Analysis}
\label{sec:generalmethod}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Trace database schema: Transaction and call tables.}
\label{tab:schema}\centering{
\begin{tabularx}{0.46\textwidth}{ |r<{\ttfamily}|X| }
  \hline
   Attributes & Meaning \\ \hline
   \multicolumn{2}{l}{TxTable}    \\ \hline
   msg.sender & The account sending this transaction\\ \hline
   txID & Transaction ID\\ \hline
   \multicolumn{2}{l}{CallTable}    \\ \hline
   caller & Caller account \\ \hline
   callee\_contract & Callee smart contract\\ \hline
   callee\_func& Callee function name\\ \hline
   data & Function-specific data, including argument list (ref. Table~\ref{tab:api})\\ \hline
   gas\_price & Gas price \\ \hline
   gas & Maximal Gas allowed to run this call \\ \hline
   call\_seq & Call sequence number \\ \hline
   txID & ID of the transaction triggering this call\\ \hline
\end{tabularx}
}
\end{table}

\input{text/lst1.tex}

To discover the cases of atomicity anomalies, we start from a ``trace'' database consisting of a transaction table and a function-call table. The data schema of these two tables is illustrated in Table~\ref{tab:schema}, where a transaction record has the primary key of \texttt{txID} and attributes including \texttt{msg.sender}, \texttt{gas\_price}, et al. A function-call record has \texttt{caller}, \texttt{callee\_contract}, \texttt{callee\_func}, \texttt{gas}, \texttt{txID}, et al. The specific meanings of these attributes are described in Table~\ref{tab:schema}. Particularly, the \texttt{data} attribute stores the argument list of the function call. The \texttt{call\_seq} is an attribute that indicates the function call's position in the call tree initiated by the same transaction. A caller's sequence number is the prefix of callee's sequence number. For instance, consider a statement in function \texttt{foo} calls function \texttt{bar}. Let's say the sequence number of function call to \texttt{foo} is `032'. Then the sequence number of the call to bar can be `0320'.

Our goal is to discover all incidents of atomicity anomalies from the trace database. The general idea is to {\it select from the CallTable the two candidate sets, respectively for the first transfer and second transfer in a swap, and then joins these two sets before checking the swaps' validity.} 
Materializing this idea on different underling exchanges, we obtain a data analytical workflow that consists of concrete SQL queries and state-machine checking logic, as in Figure~\ref{fig:workflow}.

\section{Case study: Uniswap-V2}
\subsection{Approach}

\begin{figure*}[htbp!]
  \begin{center}
    \subfloat[Uniswap-V2 protocol for swapping tokens]{%
\includegraphics[width=0.4\textwidth]{figures/protocol_uniswap.eps}
      \label{fig:uniswap:protocol}%
    }%
    \hspace{0.3in}%
    \subfloat[Trace database]{%
\includegraphics[width=0.1\textwidth]{figures/protocol_uniswap2.eps}
      \label{fig:uniswap:db}%
    }%
    \hspace{0.35in}%
    \subfloat[Automata checking atomicity (of single-tx swaps).]{%
\includegraphics[width=0.3\textwidth]{figures/automata.eps}
      \label{fig:uniswap:check}%
    }%
  \end{center}%\vspace{-0.15in}
  \caption{Modeling Uniswap-V2: The protocol, trace database and atomicity-checking automata.}\label{fig:uniswap}\vspace{-0.10in}
\end{figure*}

\input{text/lst_sql.tex}

\noindent
{\bf Preliminary of Uniswap-V2}: Uniswap-V2, as a composable AMM, runs two types of smart contracts: A frontend ``router'' smart contract that exposes a collection of user-friendly APIs and a series of backend smart contracts, each providing a liquidity pool for a pair of tokens. 

The key functionality of Uniswap-V2 is swapping the ownership of two tokens between a trader and a Uniswap pool. Figure~\ref{fig:uniswap:protocol} illustrates an example function-call graph in which a trader exchanges her \texttt{mToken} with Uniswap's pool for \texttt{tToken}. The process involves two transactions. In transaction \ballnumber{1}, the trader calls the \texttt{mToken} smart contract to \texttt{approve} Uniswap-V2's router smart contract spending her account. Then, in transaction \ballnumber{2}, the trader calls the Router's function \texttt{wrappedSwap}, which runs a series of internal calls, including \texttt{transferFrom} (\ballnumber{21}), \texttt{swap} (\ballnumber{22}), \texttt{getBalance} (\ballnumber{221}), and \texttt{transfer} (\ballnumber{222}), as shown in the figure.

Another functionality in Uniswap-V2 (not shown in Figure~\ref{fig:uniswap:protocol}) is allowing traders to make deposit into the liquidity pool. Given a pool, the trader deposit the two supported tokens at their current ratio and receive a certain amount of LP tokens in return. For instance, the trader can call \texttt{mToken}'s \texttt{transfer} and \texttt{tToken}'s \texttt{transfer}, at certain ratio, before calling Uniswap-V2's router contract's \texttt{addLiquidity} function.


\noindent
{\bf Design challenges}: Recall that finding swaps of atomicity and anomalies entails identifying the set of transferIn and transferOut events. On Uniswap-V2, a naive approach of finding transferIn is to select the \texttt{transfer} or \texttt{transferFrom} calls whose receivers are one of Uniswap-V2's liquidity pools.
However, in Uniswap-V2, such a \texttt{transfer} call is possible not only in a \texttt{swapToken} workflow but also in a \texttt{addLiquidity} workflow.
Identifying \texttt{transferFrom} calls without knowing their causes can lead to false positives. For instance, a \texttt{transfer} call paying a liquidity pool in a valid \texttt{addLiquidity} workflow can be mistaken to be a \texttt{transfer} call in an invalid \texttt{swapToken} workflow exhibiting the \textsc{UNDERWATER} anomaly.

To solve the problem, our strategy is to select the \texttt{transfer} calls in both \texttt{swapToken} and \texttt{addLiquidity} workflows during the SQL query and to distinguish the two cases using state-machine checks. To do so, our SQL query needs to capture the calls of function \texttt{addLiquidity}. 

\ignore{
a naive approach of finding transferOut is to select the \texttt{transfer} calls sent from one of Uniswap-V2's liquidity pools and sent to the pools' supported token. However, in Uniswap-V2, \texttt{transfer} calls sent by a liquidity pool can not only be in a \texttt{swapToken} protocol but also in a \texttt{addLiquidity} protocol, leading to false positives by the naive approach. To overcome the challenge, we instead use the calls to a pool's \texttt{swap} function to identify transferOut.

--To find atomicity anomalies, one can follow the SQL query ``template'' described in \S~\ref{XX} by first finding the candidates of transferIn and those of transferOut before joining the sets. To find the transferIn (transferOut), the naive approach is to select the transfers whose senders (receivers) are one of the Uniswap-V2's liquidity pools. This approach works well, if the DEX only supports one function of \texttt{swap}, and all the transfers issued to the DEX are relevant to \texttt{swap}.

However, Uniswap-V2's \texttt{addLiquidity} workflow also involves sending \texttt{transfer} calls to a liquidity pool, which confuses the naive approach. For instance, such a \texttt{transfer} call can be part of the \texttt{swap} protocol as in Figure~\ref{XX} or equally likely be part of the \texttt{addLiquidity} protocol. Without attributing a  \texttt{transfer} call to the right protocol can result failure of detecting \texttt{swap}s and/or introduce false positives
}

\noindent
{\bf Proposed trace analytics}: The overall analytics consists of three stages, an SQL query to prepare a table of candidate call records, an automata to find swaps executed in single transactions and to check their atomicity, and an automata to do the same for multi-transaction swaps.

{\it 1. SQL query}: 
Our SQL query for Uniswap-V2 is in Listing~\ref{sql:uniswap}, where intermediary result \texttt{T1} stores the candidate set of swaps' transferIn events by directly selecting the \texttt{transfer} calls that could be matched to a \texttt{swapToken} workflow or a \texttt{addLiquidity} workflow. Intermediary result \texttt{T2} stores the candidate set of calls to a target pool's \texttt{swap}s and \texttt{addLiquidity}s. The third query union the two intermediate results ordered first by transaction ID and then by call sequence number.

{\it 2. Automata for single-tx swaps}: 
The SQL query result is then fed into an automata finding swaps and checking their atomicity. The automata for single-transaction swaps is described in Figure~\ref{fig:uniswap:check}. Specifically, the SQL query result is a table of calls of three functions, \texttt{swap}, \texttt{addLiquidity}, and \texttt{transfer} (or \texttt{transferFrom}). These call records are ordered by transaction ID and then by their call sequence numbers. The automata in Figure~\ref{fig:uniswap:check} combines the state machines of both \texttt{wf\_swapToken} and \texttt{wf\_addLiquidity} workflows, where $tf_X$ refers to a \texttt{transfer} call that pays to a target liquidity pool.
Only when the automata ends up in the green state, no error is thrown. Particularly, State $2$/$4$/$6$ may refer to the atomicity anomaly \textsc{U}/\textsc{F}/\textsc{I}. \textsc{I} means the two swaps are executed interleaved, such as swap1.transferIn, swap2.transferIn, swap2.transferOut, and swap1.transferOut.

{\it 3. Automata for multi-tx swaps}: The single-transaction automata find valid \texttt{swaps} (i.e., atomic swaps) and \texttt{addLiquidity} workflows and remove them from the table. After that, we run another automata to check the validity of multi-transaction swaps.

This method can capture atomic swaps (\textsc{A}) and anomalies (including \textsc{U}, \textsc{F}, \textsc{O}, and \textsc{D}).

%YYY

\noindent
{\bf Example}: Consider the example in Figure~\ref{fig:uniswap:protocol} where a trader swaps her \texttt{mToken}s with Uniswap-V2 for \texttt{tToken}s. The trace database stores two transactions and six calls as in Figure~\ref{fig:uniswap:db}. Running the SQL query (Listing~\ref{sql:uniswap}) on this database results in intermediary table $T1$ containing \ballnumber{21} and table $T2$ containing \ballnumber{22}. Table $T3$ contains the union-ed result $\{\ballnumber{21}, \ballnumber{22}\}$, which passes the atomicity check of single-transaction swaps.

\ignore{
YYY: Correctness analysis:

For anomalies, we first find all the transactions that invoke the \texttt{transfer} function in any token smart contracts that are registered in Uniswap and transfer tokens to the corresponding pair smart contracts. For each identified deposit transaction, suppose it corresponds to the pair smart contract say $P$. We then check the trace of swap calls received by $P$ and find the one matching the deposit function based on the three conditions (W1/W2/W3).
}

\subsection{Results}

\input{text/eval_uniswap.tex}

\input{text/case_bancorx.tex}

\section{Conclusion}
This paper presents a measurement study to uncover the atomicity anomalies in deployed DEX and cross-chain swaps.



==> text/old/paper2.tex <==
\section{Data Models and Definitions}
\label{sec:model}

\noindent
{\bf Transfer}: 
Given two accounts (blockchain addresses) $ts$ and $tr$, a transfer $tf$, denoted by $\langle{}ts,tr,c,v,b,d,txID\rangle{}$, sends value $v$ in currency $c$ from sender account $ts$ to receiver account $tr$. This transfer occurs on blockchain $b$ and is carried out by the transaction of hash $txID$. $d$ is the ``data'' field of the transaction, which includes information related to smart-contract function invocation. 

\begin{table}[!htbp] %force in current page, disable float.
\caption{Data schema: Input trace tables (transactions and function calls) and intermediate transfer tables.}
\label{tab:schema}\centering{
\begin{tabularx}{0.46\textwidth}{ |r<{\ttfamily}|X| }
  \hline
   Attributes & Meaning \\ \hline
   \multicolumn{2}{l}{Input: TxTable}    \\ \hline
   msg.sender & The account sending this transaction\\ \hline
   txID & Transaction ID\\ \hline
   \multicolumn{2}{l}{Input: CallTable}    \\ \hline
   caller & Caller account \\ \hline
   callee\_contract & Callee smart contract\\ \hline
   callee\_func& Callee function name\\ \hline
   data & Function-specific data, including argument list (ref. Table~\ref{tab:api})\\ \hline
   gas\_price & Gas price \\ \hline
   gas & Maximal Gas allowed to run this call \\ \hline
   call\_seq & Call sequence number \\ \hline
   txID & ID of the transaction triggering this call\\ \hline
   \multicolumn{2}{l}{Intermediary: TfInTable and TfOutTable}    \\ \hline
   $payer$ & Payer account \\ \hline
   $payee$ & Payee account \\ \hline
   $currency$ & Currency/token \\ \hline
   $val$ & Value (in the units of $c$)\\ \hline
   $bkc$ & The running blockchain\\ \hline
   $data$ & Function specific data, including argument list \\ \hline
   $txID$ & ID of the current transaction \\ \hline
\end{tabularx}
}
\end{table}

\input{text/lst1.tex}

\noindent
{\bf Swap}: 
A (valid) swap consists of two transfers, respectively named $tfIn$ and $tfOut$, that can be ``matched'' on the conditions of their senders, receivers and the equality of their value. That is, a swap's two transfers $tfIn$ and $tfOut$ meet the following conditions:

\begin{eqnarray}
\begin{cases}
tfIn.payer& \text{= } tfOut.payee \\
tfIn.payee&  \text{= } tfOut.payer
\end{cases}
\label{eqn:atomic:match}
\end{eqnarray}

A swap can be materialized on a single blockchain (i.e., $tfIn.bkc==tfOut.bkc$)  or multiple blockchains(i.e., $tfIn.bkc\neq{}tfOut.bkc$) . The former type of swap is carried out by a DEX on a single blockchain, the latter type of swap is carried out cross-chain protocols.


The exchange rate of the swap is defined as $r$=$\frac{tfIn.val}{tfOut.val}$, which can be determined differently on different platforms.

\noindent
{\bf Atomicity and anomalies}: A swap is \textsc{ATOMIC} or \textsc{A} if the two transfers meet the condition defined in Equations~\ref{eqn:atomic:match} and the timing difference of the two transfers is within a timeout threshold $tt$.

A swap is a \textsc{FREERIDER} or \textsc{F} if it only has $tfOut$ but not a matching $tfIn$, that is, $\langle{}-,tfOut\rangle{}$. In other words, the account $tfOut.payee$ receives value in $tfOut$, yet without paying anything (i.e., without $tfIn$). 

Relaxing the condition, a swap $\langle{}tfIn,tfOut\rangle{}$ is a \textsc{DISCOUNT} or \textsc{D} if $\frac{tfIn.val}{tfOut.val}<r$ where $r$ is the market exchange rate between currencies $tfIn.currency$ and $tfOut.currency$. 

A swap is an \textsc{UNDERWATER} or \textsc{U} if it only has $tfIn$ but not a matching $tfOut$. In other words, the account $tfIn.payer$ pays valuable in her own currency in transfer $tfIn$, yet without receiving anything (i.e., without $tfOut$). 

A swap $\langle{}tfIn,tfOut\rangle{}$ is an \textsc{OVERCHARGE} or \textsc{O} if $\frac{tfIn.val}{tfOut.val}>r$ where $r$ is the market exchange rate between currencies $tfIn.currency$ and $tfOut.currency$. 

Figure~\ref{fig:atomicity} illustrates the relationship of swaps of different types. 

\section{Generic Trace Analysis Framework}
\label{sec:generic}

\begin{figure*}
\centering
  \subfloat[Swaps atomicity and anomalies]{%
    \includegraphics[width=0.06\textwidth]{figures/atomicity.eps}
    \label{fig:atomicity}
  }
  \hspace{0.25in}
  \subfloat[Trace analysis workflow to find swaps of atomicity and violations]{%
    \includegraphics[width=0.4\textwidth]{figures/workflow2.eps}
    \label{fig:workflow}
  }
  \hspace{0.25in}
  \subfloat[Join analysis]{%
    \includegraphics[width=0.275\textwidth]{figures/workflow3.eps}
    \label{fig:workflow3}
  }
\caption{Swap definition and overall analysis workflow}
\end{figure*}

\noindent{\bf Input database}:
The starting point of our analysis is a database storing raw traces of transactions and function calls on one or multiple blockchains. The data schema of each table is described in Table~\ref{tab:schema}, where a transaction record has the primary key of \texttt{txID} and has several attributes including \texttt{msg.sender}, \texttt{gas\_price}, et al. A function-call record has \texttt{caller}, \texttt{callee\_contract}, \texttt{callee\_func}, \texttt{gas}, \texttt{txID}, et al. The specific meanings of these attributes are described in Table~\ref{tab:schema}. 

Particularly, the \texttt{data} attribute stores the argument list of the function call. The \texttt{call\_seq} is an attribute that indicates the function call's position in the call tree initiated by the same transaction. Given a caller-callee pair, the caller's sequence number is the prefix of the callee's sequence number. For instance, consider a statement in function \texttt{foo} calls function \texttt{bar}. Let's say the sequence number of function call to \texttt{foo} is `032'. Then the sequence number of the call to bar can be `0320'.

\noindent{\bf Data analysis}:
The data analysis workflow is illustrated in Figure~\ref{fig:workflow}. It first selects from the initial database the candidates of $tfIn$'s and $tfOut$'s, producing two intermediary tables. It then joins the two tables to produce the results of atomic swaps and swaps violating atomicity. 

Specifically, the first step selects relevant function calls from the database based on DApp-specific conditions. For instance, in Uniswap-V2, it selects as $tfIn$ candidates any ERC20 tokens' transfer calls with receivers being Uniswap-V2's registered liquidity pools). It selects as $tfOut$ candidates calls to Uniswap-V2 specific functions, namely \texttt{swap}.
The two intermediary tables (i.e., $tfIn$ and $tfOut$) follow the data schema defined in Table~\ref{tab:schema}. 

The second step joins the two intermediary tables by running a series of subqueries and iteratively updating the two tables, as shown in Figure~\ref{fig:workflow3}. Specifical subqueries are described below.

{\it The first subquery Q1} joins the two tables on the equality of transaction ID (i.e., the two function calls occur in the same transaction), the matching of $tfIn$'s payee and $tfOut$'s payer (i.e., Equation~\ref{eqn:atomic:match}) and optionally, the equality of value being transfered. This is materialized an SQL join query as in Listing~\ref{sql:uniswapv2:2}. It identifies atomic swaps by finding the one-to-one mappings from the inner-join results, that is, one $tfIn$ candidate matching exactly one $tfOut$ candidate and vice versa. It removes the $tfIn$ and $tfOut$ records in identified atomic swaps from the two intermediary tables.
\input{text/lst_sql.tex}
\input{text/lst_sql3.tex}

{\it The second subquery Q2} then joins transfer calls based on their execution order (in the same transaction). The heuristics is that smart contracts are executed in a single thread, and a $tfIn$ call would match a subsequent $tfOut$ call in the execution order. For instance, consider a set of transfer calls, $tfIn_1,tfIn_2,tfOut_3,tfOut_4$. If they are executed in the order of $tfIn_1,tfOut_3,tfIn_2,tfOut_4$, they are joined as two atomic swaps, $\langle{}tfIn_1,tfOut_3\rangle{}$ and $\langle{}tfIn_2,tfOut_4\rangle{}$. If they are executed in the order of $tfIn_1,tfIn_2,tfOut_3,tfOut_4$, they are joined as two swaps $\langle{}tfIn_1,tfOut_4\rangle{}$ and $\langle{}tfIn_2,tfOut_3\rangle{}$\footnote{In this case, it is possible that $tfIn_1$ matches $tfOut_3$, instead of $tfOut_2$. The ground truth is that YYYJiaqi.}, producing interleaved execution anomaly. 

To materialize the heuristics, we propose an algorithm that replays the selected function calls in their execution order (e.g., by traversing the function call sequences/graph) and conducts the matching: By maintaining a stack as in List~\cite{XXX}, it pushes an entry to the stack upon a $tfIn$ call and pops the top entry from the stack upon a $tfOut$ call. By this means, it matches the current $tfOut$ call to the predecessor $tfIn$ call(s).

{\it The third subquery Q3} joins the transfer calls across transactions based on the timing. Intuitively, when $tfIn$ and $tfOut$ occur in two different transactions, an invariant must hold, that is, the $tfIn$ transaction must happen before the $tfOut$ transaction. 

\input{text/lst_q31.tex}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.225\textwidth]{figures/join_problem.eps}
\caption{Join problem}
\label{fig:joinproblem}
\end{figure}

{\bf Design goal}: We formulate the research to discover atomicity anomalies that manifest in mismatches (between tfIn and tfOut records). We aim at designing join algorithms that take as input the tfIn and tfOut tables and produce atomic swaps and anomalies. The particular design goal is that 1) the algorithm should be able to actual swap anomalies, and 2) the found anomalies should not be the artifacts caused by the defect of our algorithm.

We use an example to illustrate the design goals. Suppose there are two $tfIn$ calls and three $tfOut$ calls, with their value and timestamps shown as in Figure~\ref{fig:joinproblem}. For instance, $\langle{}50,3\rangle$ is a $tfIn$ call that transfers value $50$ at timestamp $3$. One possible mapping P1 is
$\langle{}50,1\rangle\leftrightarrow{}{\langle{}40,2\rangle,\langle{}10,5\rangle}$ and 
$\langle{}50,3\rangle\leftrightarrow{}\langle{}50,4\rangle$, which produce no anomalies. Another possible mapping P2 is $\langle{}50,1\rangle\leftrightarrow{}\langle{}50,4\rangle$, which leaves $\langle{}50,3\rangle$ unable to match $\langle{}40,2\rangle$, as the $tfIn$ call cannot occur before any $tfOut$ calls. While P2 produces swap anomalies, these are caused by the defect of the mapping schemes, as they can be avoided if the algorithm selects the mapping scheme P1. The goal of algorithm design is to produce the necessary cases of anomalies by selecting the mapping schemes producing the minimal cases of anomalies.

Ideal algorithm: Ideally, one can generate the $tfIn$ and $tfOut$ tables' powersets and run a cross-product to check all possible combinations. However, the powerset of a set of $n$ records is $2^n$, and the ideal algorithm does not scale even for a small $n$ (e.g., 40).

{\bf Proposed greedy algorithm}: To achieve the design goals in both avoiding artifacts of anomalies and achieving efficiency, we limit the target cases of one-to-$m$ mappings (with $m\leq{}2$), instead of the generic many-to-many mappings. This is based on the observation that in real-life traces, most atomic swaps do not include more than two $tfIn$ or $tfOut$ calls.

We propose a greedy algorithm to join transfer calls across transactions, described by $joinAcrossTx$ in Listing~\ref{label=sql:uniswap:q3}. Briefly, the algorithm maintains two pointers to respectively iterate through the input tables. During the iteration, given a specific pair of $tfIn$ call $c_i$ and $tfOut$ call $c_j$, it first tries to find one or two $tfOut$ calls that match $c_i$ (i.e., the invocation to $findMatch()$ in Line 5). If that fails, it then tries to find one or two $tfIn$ calls that match $c_j$ (i.e., the invocation to $findMatch()$ in Line 07). Inside the $findMatch$ function, it runs a nested loop to iterate through the provided list, and it stops upon the first hit is found.

{\bf Correctness analysis}: Why it can early stop? XXX

---

Besides them, there can be unmatched cases in the join results, for instance, multiple $tfIn$ candidates matched to one $tfOut$ candidate. We run further DApp-specific conditions to join them, before drawing the final conclusion on swap atomicity. 

\section{Case study: Uniswap-V2}
\subsection{Approach}
\begin{figure*}[htbp!]
  \begin{center}
    \subfloat[Uniswap-V2 protocol for swapping tokens]{%
\includegraphics[width=0.4\textwidth]{figures/protocol_uniswap.eps}
      \label{fig:uniswap:protocol}%
    }%
    \hspace{0.3in}%
    \subfloat[Trace database]{%
\includegraphics[width=0.3\textwidth]{figures/protocol_uniswap2.eps}
      \label{fig:uniswap:db}%
    }%
  \end{center}%\vspace{-0.15in}
  \caption{Modeling Uniswap-V2: The protocol, trace database and atomicity-checking automata.}\label{fig:uniswap}
\end{figure*}

\input{text/lst_sql.tex}

\noindent
{\bf Preliminary of Uniswap-V2}: Uniswap-V2, as a composable AMM, runs two types of smart contracts: A frontend ``router'' smart contract that exposes a collection of user-friendly APIs and a series of backend smart contracts, each providing a liquidity pool for a pair of tokens. 

The key workflow of Uniswap-V2 is swapping the ownership of two tokens between a trader and a Uniswap pool. Figure~\ref{fig:uniswap:protocol} illustrates an example function-call graph in which a trader exchanges her \texttt{mToken} with Uniswap's pool for \texttt{tToken}. 
This involves with two essential function calls: \ballnumber{1'} The trader first invokes \texttt{transfer} function in the \texttt{mToken} smart contract (which is the $tfIn$ call). \ballnumber{2'} The trader then invokes Uniswap-V2's liquidity pool's \texttt{swap} function as the $tfOut$ call, which further invokes \texttt{tToken}'s \texttt{transfer} function (\ballnumber{2'1}).

Another workflow in Uniswap-V2 (not shown in Figure~\ref{fig:uniswap:protocol}) is that a trader makes deposit in the liquidity pool. Specifically, the trader deposits in a pool the two supported tokens at their current ratio and receives LP tokens in return. For instance, the trader can call \texttt{mToken}'s \texttt{transfer} function and \texttt{tToken}'s \texttt{transfer}, at a certain rate, before invoking Uniswap-V2 liquidity pool's \texttt{mint} function.

Note that the trader in the above scheme can be materialized as an EOA (externally owned account) or a smart-contract account. For a trader EOA, the function calls issued by the trader (e.g., \ballnumber{1'} and \ballnumber{2'}) are ``external'' and encoded in dedicated transactions. For a smart-contract trader (e.g., Uniswap-V2 routing smart contract or a smart contract instantiating the 0x protocol), the function calls issued by the trader are internal calls.

\noindent{\bf Design challenge}: A straightforward approach is to apply the generic trace analysis described in \S~\ref{sec:generic} to the case of Uniswap-V2. However, matters are complicated by the presence of \texttt{addLiquidity} workflow. For instance, in Figure~\ref{XXX}, a \texttt{transfer} call that pays Uniswap-V2's liquidity pool can be part of a \texttt{swap} workflow, or equally likely, be part of an \texttt{addLiquidity} workflow. These two cases need to be distinguished in order to identify potential swaps. Otherwise, false positives (of swap anomalies) may occur. For instance, a \texttt{transfer} call paying Uniswap-V2's liquidity pool in an \texttt{addLiquidity} workflow may be mistaken to be a $tfIn$ call in a \texttt{swap} workflow, without finding $tfOut$ and leading to a false positive of \textsc{UNDERWATER} anomaly. 

---

To solve the problem, our strategy is to select the \texttt{transfer} calls in both \texttt{swapToken} and \texttt{addLiquidity} workflows during the SQL query and to distinguish the two cases using state-machine checks. To do so, our SQL query needs to capture the calls of function \texttt{addLiquidity}. 

---

For measurement, we find the cases of atomic swaps and match the two transfer transactions. To do so, given the known smart contracts of Uniswap's liquidity pools, we first locate all transactions invoking these smart contracts' \texttt{swap} function. The swap function has an argument (``to'' as listed in XXX) which refers to the user's address. We then leverage this information to find a transaction that W1) is sent from the user (of the ``to'' address), W2) is sent to the mToken, and W3) transfers tokens to Uniswap's pair smart contract. If there are multiple matching transactions, we further check XXX?

function swap(uint amount0Out, uint amount1Out, address to, bytes calldata data);

The above method is able to identify the violation incident (V1): Given a \texttt{swap} invocation, it cannot find a \texttt{transfer} invocation to mToken that meets the above three conditions in the entire Ethereum transaction history. 

For V2, we first find all the transactions that invoke the \texttt{transfer} function in any token smart contracts that are registered in Uniswap and transfer tokens to the corresponding pair smart contracts. For each identified deposit transaction, suppose it corresponds to the pair smart contract say $P$. We then check the trace of swap calls received by $P$ and find the one matching the deposit function based on the three conditions (W1/W2/W3).

\subsubsection{Results}
\input{text/eval_uniswap.tex}

\clearpage

%\input{text/lst_sql2.tex}
%\input{text/lst_sql_filter.tex}

\subsection{EOS}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.275\textwidth]{figures/protocol_pegged_eos.eps}
\caption{EOS}
\label{fig:protocol:eos}
\end{figure}

\clearpage

\section{Measurement Studies on Cross-chain Swaps}
In this section, we describe the measurement study on cross-chain token swaps to uncover the case of atomicity violations. We first describe a general model of cross-chain swaps and how it is instantiated in actual swaps in practice. We then describe the methods specific to measuring different cross-chain swaps. 

\begin{figure}[!ht]
\centering
\includegraphics[width=0.275\textwidth]{figures/protocol_pegged.eps}
\caption{The general model of cross-chain swaps}
\label{fig:protocol:general}
\end{figure}

\subsection{Modelling Cross-chain Swaps}
\label{sec:model:crosschain}

In general, a cross-chain swap works among four parties. As shown in Figure~\ref{fig:protocol:general}, a {\it user} initially holds cryptocurrency or tokens, say A, on the {\it source blockchain}, and a {\it custodian} holds the pegged token B on the {\it destination blockchain}, which also supports smart contracts. It swaps the user's token A with the custodian's token B. To do so, the protocol generally runs in three steps: \ballnumber{1} The user sends a transaction to the source blockchain to transfer his token A to the custodian. \ballnumber{2} The custodian gets notified, through a communication channel, of the user's transaction. \ballnumber{3} The custodian sends a transaction to the destination blockchain to transfer a certain amount of token B to the user's account. 

Different actual cross-chain swaps instantiates the above model, notably for applications such as pegged tokens.
\subsection{Measurement Methods of wBTC}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.325\textwidth]{figures/protocol_pegged_wbtc.eps}
\caption{The WBTC protocol}
\label{fig:protocol:wbtc}
\end{figure}

WBTC is a popular pegged token on Ethereum that is backed by Bitcoin on a one-to-one rate. In WBTC, there is a smart contract on Ethereum (destination blockchain) called Token Factory. Step \ballnumber{2} consists of two substeps: The user first invokes the Factory's function \texttt{addRequest($btx$)} where $btx$ is the hash of the user's Bitcoin transaction. The custodian watching Ethereum's event stream gets notified of the invocation to \texttt{addRequest($btx$)} invokes the smart contract's function \texttt{requestConfirm($btx$)} which further verifies the Bitcoin deposit and mints the same amount of WBTC under the user's account. Note that function \texttt{addRequest($btx$)} sent by the user is necessary for the custodian to verify the Bitcoin deposit. Figure~\ref{fig:protocol:wbtc} shows the WBTC's protocol to mint a token on Ethereum.

To pair the collateral deposit and token mint in WBTC, we exploit the following fact: 1) The address of WBTC's Factory smart contract is publicly known , and 2) The Step \ballnumber{3}'s function \texttt{requestConfirm} contains the hash of Bitcoin deposit transaction. Specifically, to a deposit and token mint (i.e., measurement goal M0), we start by collecting the transactions calling WBTC's \texttt{requestConfirm}, then locate the corresponding Bitcoin transaction hashes, and finally verifies the inclusion of such transactions in the Bitcoin's blockchain. 

In WBTC, the type-V1 atomicity violation is materialized as the absence of a Bitcoin deposit in the presence of a WBTC mint. V1 is verified by the failure of observing Bitcoin deposit inclusion.  The type-V2 violation cannot be verified in our method XXX.  

\clearpage

\input{text/case_bancorx.tex}



==> text/old/v10_intro_ndss23submission.tex <==
\section{Introduction}

Recent years have witnessed the rise of Decentralized Finance (DeFi) on blockchains. A prominent class of DeFi applications is Decentralized Exchange (DEX) that allows a trader account to swap their assets from one type of tokens to another. 
On Ethereum, deployed DEX instances including Uniswap~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer} all run AMM protocols or automated market maker, which account for more than $95\%$ of the DEX activities all time~\cite{me:etherscan:topdex}, attracting hundreds of millions of transactions today (as of July, 2022). Other than token swap, an AMM\footnote{We use the terms AMM and DEX interchangeably in this paper.} supports liquidity addition/removal in which a liquidity-provider account deposits tokens as a reserve for subsequent token swaps.

AMM can be misused. A well studied class of AMM misuses are sandwich attacks and arbitrage~\cite{DBLP:conf/sp/DaianGKLZBBJ20,DBLP:journals/corr/abs-2101-05511,DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2105-02784,DBLP:conf/sp/ZhouQCLG21}. In both attacks, the attacker account extracts illicit value by sending multiple transactions in a crafted order. Recent research has shown the large scale of sandwich attacks and arbitrage on Ethereum~\cite{DBLP:journals/corr/abs-2101-05511,DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2105-02784,DBLP:conf/sp/ZhouQCLG21}. 
Another AMM misuse is to list scam tokens~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21} that impersonate other tokens to trick their traders. In these known misuse patterns, each attack is composed of multiple AMM operations, such as a cycle of token swaps in arbitrage~\cite{DBLP:journals/corr/abs-2105-02784} and two transactions that frontrun and backrun a victim transaction in a sandwich attack~\cite{DBLP:journals/corr/abs-2101-05511}.
%scam tokens by short-lived span of AMM operations~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21}, etc.

\begin{figure}[b!ht]
\begin{center}
\includegraphics[width=0.425\textwidth]{figures/workflow7.eps}
\end{center}
\caption{Transaction-analysis workflow to 1) discover AMM operation atomicity violations and 2) detect attack instances in theft and lost tokens.}
\label{fig:workflow7}
\end{figure}

\vspace{2pt}\noindent\textbf{Discovering atomicity violations}. 
This work aims to study a different class of AMM misuses: atomicity violations. Specifically, an AMM operation, be it a token swap or liquidity management, should execute a sequence of token deposits and withdrawals in an all-or-nothing manner (i.e., atomic operation execution). Violation of the operation atomicity could imply the presence of security risks or even attacks. For instance, executing a token swap by a standalone withdrawal (i.e., without the matching deposit) could indicate an incident of theft in which a thief withdraws value without making any deposit to the AMM. For another instance, a token swap by a standalone deposit (without a matching withdrawal) could mean an adversarial AMM denying the withdrawal request from the trader who has made a deposit.
Note that atomicity violation is different from the known AMM misuses that manifest in multi-operation sequences and do not entail the violation of individual operations' atomicity.

By connecting together and analyzing over $60$ million transactions on Ethereum and Binance Smart Chain (BSC), to our surprise, we find that atomicity violations widely exist among deployed AMM services: 
Committing these violations are the most popular services, including Uniswap V2~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer}.
In total, they have performed more than $74$ thousand AMM operations violating atomicity, which exhibit various patterns including standalone token deposit, standalone withdrawal, account mismatch, and value mismatch.

%To understand the nature of the atomicity violations, that is, whether they occur by accident or are committed intentionally, we formulate the following hypothesis: 1) The atomicity violations in which the deposited value is below the value withdrawn could indicate token thefts in which a thief account attacks by extracting value from a victim AMM or trader account. 2) The atomicity violations in which the deposited value exceeds the value withdrawn could indicate AMM denial of service in which a victim trader depositing value is declined of withdrawal service. Specifically, we focus on the lost-token risks in which the victim trader deposits tokens by mistakes.

\vspace{2pt}\noindent\textbf{Understanding atomicity violations}. 
We aim to understand the nature of the atomicity violations, whether they are accidents or intentional crimes. While different atomicity violations can be attributed to different threats (e.g., denial of service mentioned above), we mainly focus on the prominent cases of token theft in our measurement result.

Detecting theft from the atomicity violations is challenging. This is because the ground truth often includes off-chain activities unaccounted for.
%which are unobservable. 
For instance, when attributing a standalone withdrawal to theft, one has to know that the party making the deposit to accounts and the party withdrawing from the accounts are controlled by two distinct physical entities, which is known to be an intractable problem with only on-chain data; known heuristics such as address clustering~\cite{DBLP:conf/fc/Victor20,DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:conf/sp/HuangALIBMLLSM18,DBLP:books/daglib/0040621} do not apply here (see \S~\ref{sec:discoveryproblem} for detail).

To address this challenge, we focus on making sense of the accounts' on-chain behaviors and matching them to the rational attack strategies we identify through analyzing the AMM protocols. For instance, a rational thief in fear of being frontrun by competing thieves would send crafted transactions with the minimal deposit-to-withdrawal delay, which can indicate the occurrence of an attack. For another instance, to avoid the failure of theft, a careful thief would check on-chain states extensively (e.g., token balances) before committing the theft; these pre-attack operations (e.g., calling token function \texttt{balanceOf}) could indicate an intentional theft. We propose an algorithm to capture the account behavior with such indicators and automatically detect thefts.

Overall, our method is an end-to-end transaction-analysis pipeline, depicted in Figure~\ref{fig:workflow7}, which first discovers atomicity violations and then detects and characterizes theft attacks.

%We found in practice the exploitable deposits can be created in a variety of unexpected application scenarios, including free token giveaways (i.e., airdropping), tokens redistributing fees to privileged shareholder accounts, tokens bearing interest, tokens that can adjust or rebase total supply, buggy smart contracts, and unsafe user interface that executes a swap in two separate transactions, etc. 

\vspace{2pt}\noindent\textbf{Findings}. 
On the Ethereum mainnet and BSC fork, we discover $55$ thousand theft attacks mounted by $258$ distinct attacker accounts, inflicting a loss of more than $3.88$ million USD stolen from $978$ victim accounts.
Each attack instance we found matches at least one indicator. 
As the measurement results show, real-world thieves exploit the undefined behavior in the AMM protocols, such as rebasing token supply, token interest and other non-standard token features, to successfully withdraw value. Interestingly, the attackers {\it adapt} their behavior to different exploits: When the attacker is to extract value from interest-bearing tokens, she waits long enough, typically hundreds of Ethereum blocks, for the interest to accumulate and to become profitable. To steal other kinds of deposits, such as token rebase, the same attacker instead wastes no time extracting the illicit value, typically within one or two blocks, to prevent frontrunning.

%One cause of the atomicity violations is that certain non-standard token operations unspecified in the AMM protocols (e.g., rebasing token supply and interest-bearing tokens) are mistreated as token deposit that allows subsequent token withdrawal to succeed. This manifests in standalone withdrawals. Another cause is that certain token deposits are not intended for withdrawal (e.g., airdrop and token lost-and-found), which results in standalone deposits.

We further study attackers' and victims' behavior by tracking their money flow and their actions to create/destroy smart contracts. Our study uncovers the systematic criminal activities: the crime bosses use mixer services to hide their identities while sending commissions and instructions. After the attack, the money is sent to various DeFi services to maximize illicit profit. Exploit smart contracts are widely used to improve attack success rates.

From the violations that are not attributed to theft, we further detect the instance of potential denial of service. Particularly, we formulate the problem of detecting lost tokens where the deposits are made by mistake, and the AMM refuses to return the tokens. We propose threat indicators by assuming the victim accounts' rational behavior after lost tokens. Our measurement result on Ethereum confirms the existence of lost tokens on Uniswap V3, Curve and Balancer (inflicting a total value of $57,000$ USD lost unfairly by these AMMs). We note that the atomicity violations could imply other threats than theft and lost tokens, and a comprehensive study is left for future research. 
%is out of the scope of this work.

\vspace{2pt}\noindent\textbf{Mitigation}. 
%why it is hard to design secure AMM in practice?
Our empirical study shows that all six popular AMM services (i.e., Uniswap V2/V3, Pancakeswap, Sushiswap, Balancer, and Curve) are vulnerable to either the threat of theft or DoS like lost tokens. This unsatisfactory state of affairs in practice is not by accident: Designing a secure AMM is fundamentally difficult. As detailed in \S~\ref{sec:causeanalysis}, as a token deposit only entails calling the token smart contract, the AMM smart contract is unaware of the depositor's information and is left with no ground to enforce any permission upon token withdrawal, which causes theft.

%It reveals a fundamental design challenge in securing AMM where the AMM smart contract with limited information needs to recognize token deposits of various intentions.

To mitigate the risks, we have made the first attempt to design secure AMM protocols that require rewriting and redeployment of smart contracts. To mitigate token thefts, the secure AMM prohibits exploitable token deposits for security at the expense of more restrictive interfaces in AMM operations. To avoid lost tokens, the AMM smart contract is extended with a BtcRelay~\cite{me:btcrelay,DBLP:conf/aft/DaveasKKZ20} such as the capability to verify the transaction requesting token returns. 
Besides, we propose mitigation schemes retrofittable to a deployed AMM instance without upgrading the smart contracts. These schemes harden the security of an off-chain infrastructure and application-layer smart contracts on top of AMMs.

\vspace{2pt}\noindent\textbf{Contributions}. Our contributions are outlined below: 


\vspace{2pt}\noindent$\bullet$\textit{ New findings}. We discover a total of $3.88$ million USD worth of stolen value by measuring and analyzing atomicity violations on six popular AMM services on Ethereum and BSC. 

The discovered token theft attacks uncover the previously unknown patterns of extractable value (e.g., token rebase, interest, airdrop, buggy application smart contracts) and expose the adaptive attack strategies that occur offline and otherwise would have been hidden. We further study the criminal infrastructures and campaigns mounted to systematically prepare, execute and finalize the theft attacks.

\vspace{2pt}\noindent$\bullet$\textit{ New techniques}. We develop an end-to-end analytical pipeline to detect atomicity violations and relevant attacks from Ethereum transaction traces, including an efficient join algorithm and various heuristics to automatically discover and cross-check token theft and lost tokens. 

\noindent
{\bf Roadmap}: \S~\ref{sec:background} introduces the background of transactions, tokens and AMM. The discovery of atomicity violations is in \S~\ref{sec:detectviolatingswap}. Threat model is formulated in \S~\ref{sec:understanding}. Detection of theft attacks is presented in \S~\ref{sec:attack}. Detection of lost tokens is in \S~\ref{sec:losttokens}. 
Countermeasures are presented in \S~\ref{sec:mitigate}. Related work is in \S~\ref{sec:rw}. Bug disclosure is in \S~\ref{sec:disclosure} with the conclusion in \S~\ref{sec:conclude}.

\section{Background}
\label{sec:background}

Ethereum blockchain supports two types of addresses: An externally owned account (EOA), which is an Ether owner's public key, and a contract account (CA), which refers to the immutable memory address to which the smart contract is deployed on miners. An Ethereum transaction is a binding between its sender address and receiver address.

Most widely deployed tokens on Ethereum are fungible tokens in which each unit is interchangeable with and indistinguishable from any other unit. ERC20 is the most adopted standard of fungible tokens on Ethereum. ERC20 functions include \texttt{transfer} which allows a token owner to transfer her tokens to another account, \texttt{approve} which allows an owner to delegate the spending of her tokens to another delegatee account, \texttt{transferFrom} that allows a delegatee account to spend tokens on behalf of the original owner under the approved token limit, \texttt{balanceOf} that allows anyone to get an account's token balance, etc.

An AMM or automated market maker is a dominant form of decentralized exchange (DEX) deployed on Ethereum blockchains. An AMM runs one or multiple ``pools'' in smart contracts. An AMM pool owns two tokens, say $T_0$ and $T_1$. An AMM pool minimally supports two operations: 1) token swap between a trader account and the pool smart contract, and 2) liquidity addition/removal between a provider account and the pool smart contract. The trader and liquidity provider can be either an EOA or a CA.

In a token-swap operation, the trader deposits $dx$ units of token $T_0$ to the pool's account and receives from the pool $dy$ units of token $T_1$. The AMM internally determines the token exchange rate (or value of $dy$) by enforcing the invariant on some function. For instance, Uniswap is a constant-product market maker where the invariant function is the product of the two token balance.

In an add-liquidity operation, the liquidity provider deposits $dx$ units of token $T_0$, deposits $dy$ units of token $T_1$, and withdraws a certain amount of ``base'' tokens $T_{\texttt{LP}}$. A remove-liquidity workflow is the reverse of add-liquidity, in that the liquidity provider deposits tokens $T_{\texttt{LP}}$ and withdraws tokens $T_0$ and $T_1$ at a certain ratio.


\begin{table}[!htbp] %force in current page, disable float.
\centering{\small
\begin{tabularx}{0.5\textwidth}{ |l|X|l| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
Layer & $swapToken$ & $addLiquidity$ \\ \hline
Uniswap V2
& $T_0$.\texttt{transfer}() & $T_0$.\texttt{transfer}() \\ 
& $p$.\texttt{swap}() & $T_1$.\texttt{transfer}() \\ 
 & & $p$.\texttt{mint}() \\ 
\cline{2-3}
& $*$.\texttt{transferFrom}() & $*$.\texttt{transferFrom}() \\ 
& $p$.\texttt{swap}() & $*$.\texttt{transferFrom}() \\ 
 & & $p$.\texttt{mint}() \\ 
\hline
Uniswap V3
& $p$.\texttt{swap}() & $p$.\texttt{mint}() \\ 
\hline
Balancer
& $p$.\texttt{swapExactAmountIn}() & $p$.\texttt{joinpool}() \\ 
\hline
Curve
& $p$.\texttt{exchange}() & $p$.\texttt{add\_liquidity}() \\ 
\hline
\end{tabularx}
}
\caption{AMM protocols' API in $swapToken$ and $addLiquidity$ operations. $T_0$/$p$/$*$ represent deposited token/pool/arbitrary smart contract.}
\label{tab:uniswapv2:api}
\end{table}









%------------------old version---------------------------



==> text/old/v10_paper3_ndss23submission.tex <==
\vspace{-0.15in}
\section{Discovering Atomicity Violations}
\label{sec:detectviolatingswap}
\label{sec:mmalgo}

\noindent
{\bf Data model}: 
In an AMM, each operation, be it token swap or liquidity management, consists of token deposits and withdrawals. A token deposit is a value transfer to an AMM pool where the transfer can be done by either 1) directly calling the token's \texttt{transfer} function or 2) calling the token's \texttt{approve} function followed by the pool calling \texttt{transferFrom} function.
A token withdrawal is a value transfer from the pool by the pool calling the token's \texttt{transfer} function.

\noindent
{\bf Atomicity specification}: 
%The AMM protocol specifies what function calls are acceptable to be a token deposit (and withdrawal); for instance, in Uniswap V2, a token deposit is a call to a token's \texttt{transfer} function can be a token deposit. A call to a pool's \texttt{swap} function can be a token withdrawal. 
An AMM operation executes a sequence of token deposits and withdrawals; the correctness means the atomic operation execution. Without loss of generality, we use token swap as an example in the description, while the extension to liquidity operations is straightforward. Given a token swap, we call the account calling the deposit function by the depositor and the account receiving the token withdrawal by the withdrawer.

\vspace{-0.15in}
\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/anomalies.eps}
\end{center}
\caption{Atomic operations (token swaps) and violations.}
\vspace{-0.2in}
\label{fig:swaps}
\end{figure}

\begin{itemize}[leftmargin=0.5cm]
%\setlength{\itemindent}{-1em}
\item
An atomic token swap consists of a token deposit of one token worth value $v$ and a withdrawal of another token worth the same value. The depositor and withdrawer accounts are either the same or match a function call if both deposit and withdrawal are in the same transaction. 

\item
{\bf Atomicity violation I} is a standalone withdrawal that does not match any token deposit.

\item
{\bf Atomicity violation II} is a standalone deposit that does not match any token withdrawal. 

\item
{\bf Atomicity violation III} is an account mismatch in which the depositor and withdrawer accounts in a sequence of otherwise matched deposits and withdrawals do not match. For instance, as shown in Figure~\ref{fig:swaps}, the deposit is issued from Account Alice, and the withdrawal is from Bob.

\item
{\bf Atomicity violation IV} is a lower-value deposit in which the deposited value is lower than the value withdrawn.

\item
{\bf Atomicity violation V} is a higher-value deposit in which the deposited value is higher than the value withdrawn. Both Violations IV and V are cases of value mismatch.
\end{itemize}

Figure~\ref{fig:swaps} shows five atomicity violation patterns and the atomic case of a token swap.

%We believe atomicity violation implies anomalous activities. For instance, a standalone withdrawal could imply value theft where the withdrawer is able to extract value from the AMM pool without depositing any value. A violation-III token swap implies theft in which the withdrawer is able to extract value from a victim depositor. For another example, a standalone deposit could imply lost tokens where a trader makes a mistake depositing value but is unable to withdraw it.

\noindent
{\bf Input data}:
Our input data is raw blockchain transactions, including function calls and log events by smart contracts. We obtain the transaction data by crawling Ethereum exploration services including \url{Etherscan.io}~\cite{me:etherscan}, \url{BSCscan.io}~\cite{me:bscscan} and relevant BigQuery datasets~\cite{me:bigquery:ethereumdataset}. 
We only use the event log emitted from the AMM pool smart contract (which we assume is trusted), such as Uniswap V2's pool.
From the raw input data, we attribute the \texttt{transfer}/\texttt{transferFrom} calls to token deposits and withdrawals as described. Besides, we collect the invocations to relevant functions, such as \texttt{swap} in Uniswap V3 in Table~\ref{tab:uniswapv2:api}; from there, we can filter out the deposits and withdrawals that are mapped to atomic operations. 
We also use the pool's events to reconstruct the mapping between deposit value and withdrawal value in the withdrawal record.

\noindent
{\bf Design challenge}:
A naive way of finding atomicity violations is to filter out atomic operations by extensively joining token deposits with withdrawals. Because an atomic AMM operation can contain an arbitrary number of deposits and withdrawals, the naive join needs to be built on the {\it powerset} of token deposits and withdrawals, which is extremely expensive and unscalable (Note that the powerset of $n$ deposits/withdrawals is of $2^n$ elements).
To avoid inefficiency, our observation is that due to Ethereum's single-threaded execution model, a token deposit can be matched only to a subsequent withdrawal before the next deposit occurs. This property allows to join token deposits and withdrawals based on their timings and makes it possible for linear-time search.

\noindent
{\bf The algorithm} takes as input a list of function calls representing token deposits and withdrawals. In the first round, the algorithm equi-joins the function-call records by their transaction IDs. If the deposits and withdrawals in the same transaction also match in value, it emits them as an atomic operation before removing them from the list. If the value does not match, the algorithm merges the intra-transaction deposits and withdrawals into one virtual record (e.g., a deposit of value equal to the originally deposited value deducted by the withdrawn value).

In the second round, the algorithm joins deposits and withdrawals across transactions. It linearly scans the list of deposits and withdrawals sorted by time: For two consecutive deposits, say $d1$ and $d2$, it finds any subset of all withdrawals between $d1$ and $d2$ that matches $d1$ in value. For each match, the algorithm removes the deposit and withdrawals from the list before emitting an atomic operation. The algorithm then reverses the process; that is, for two consecutive withdrawals, it finds a set of deposits between the two withdrawals that match the earlier withdrawal in value.

In the third round, the algorithm linearly scans the remaining list and emits the token deposits and withdrawals as either value mismatch or standalone operations. The pseudocode is in Appendix~\ref{sec:algorithm:detect}.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.3\textwidth]{figures/join_problem2.eps}
\caption{Matchmaking deposits and withdrawals: Matched cases are in green boxes, and mismatches are rendered in red, including standalone withdrawal (I), standalone deposits (II), and deposits of lower value (IV). In the figure, \texttt{tf}/\texttt{tff} refer to functions \texttt{transfer}/\texttt{transferFrom}.}
\vspace{-0.1in}
\label{fig:joinproblem}
\end{figure}

\noindent
{\bf Example}: We show an example of running the atomicity violation discovery algorithm in Uniswap V2. Uniswap V2 supports token deposits by both \texttt{transfer} and \texttt{transferFrom}. It also supports token withdrawals by \texttt{swap} (in $swapToken$) and by \texttt{mint} (in $addLiquidity$). We collect the corresponding function-call records for token deposits and withdrawals. Figure~\ref{fig:joinproblem} shows the collected deposits and withdrawals, ordered by time. 
In the first round, the algorithm identifies and filters out atomic operations by linking deposits and withdrawals through transaction ID, which is \texttt{tff1}-\texttt{swap1}. In the second round, it then matches token deposits and withdrawals by timing. For instance, \texttt{tf2} and \texttt{tf3} are matched to \texttt{mint1} by value, which leads to an atomic $addLiquidity$ operation. In the last round, the algorithm emits the mismatches in the remaining list. Specifically, \texttt{tf4} is mapped to \texttt{swap3}, but their value does not match, thus producing a case of Violation IV. Then there are two standalone operations left in the list, that is, \texttt{tf1} (Violation II) and \texttt{swap2} (I).

%{\it An example}: Figure~\ref{fig:joinproblem} shows how token deposits to a Uniswap pool are matched to token withdrawals from the same pool. The data records storing deposits/withdrawals are aligned and sorted by time. The figure shows two matched cases (i.e., two green boxes). Three mismatch cases are discovered: On the timeline, the first \textsc{transfer} is a standalone deposit (i.e., II). The second \textsc{swap} is a standalone token withdrawal (I). In the red box is a pair of deposits and withdrawals whose value does not match (i.e., IV).

\begin{table}[!htbp] %force in current page, disable float.
\caption{Discovered atomicity violations on top DEXes: value is presented in the unit of million USD, and the number of transactions violating atomicity (i.e., \#tx) is presented in the unit of a thousand.}
\label{tab:swapsviolating}\centering{\scriptsize
\begin{tabularx}{0.5\textwidth}{ |l|l|l|l|l|l|l||X| } %X is stretching to \textwidth, while c is to match with text width in cell.
\hline
 & Atomic & I & II & III & IV & V & \#tx ($10^3$) \\ \hline
Uniswap-V2 & $618*10^6$ & {\color{red} \bf $1.26$} & $.36$ & {\bf$.49$} & $.09$ & {\color{red} \bf $3.64$} & $212$ \\ \hline
Sushiswap & $.17*10^6$ & {$\approx{}0$} & {$.03$} & {\bf$.064$} & $\approx{}0$ & $0$ & $.33$ \\ \hline
Pancakeswap & $73*10^6$ & {$.53$} & $.12$ & {\bf$.05$} & $.99$ & $0$ & $452$ \\ \hline
Uniswap-V3 & $5.3*10^4$ & $0$ & {$.17$} & $0$ & $0$ & $0$ & $.17$\\  \hline
Balancer
& $1.3*10^4$ & $0$ & {$.74$} & $0$ & $0$ & $0$ & $6.9$ \\ \hline
Curve
& $1.3*10^5$ & $0$ & $\approx{}0$ & $0$ & $0$ & $0$ & $\approx{}0$\\ \hline 
\end{tabularx}
}
\end{table}

\noindent
{\bf Results}: We conduct the measurement and transaction analysis on all six DEX services.
In particular, we set the minimal $Z\%$ value difference to determine match/mismatch. If a deposit (withdrawal) has $Z\%$ higher value than the paired withdrawal (deposit), it is considered a mismatched case (IV/V/). A rule of thumb is to set $Z\%=10\%$ on our dataset, which helps remove the negative cases, such as fees charged by tokens and router smart contracts.
For each DEX, we report the number of swaps and their total value under each category. 
To estimate the value in a violating operation $tx$, we use the exchange rate between the token $T$ and one of the three USD-pegged stablecoins (i.e., $USDT$, $USDC$, and $DAI$). Specifically, we find from the three Uniswap-V2 pools (i.e., $T$-$USDC$, $T$-$USDT$, and $T$-$DAI$) the swap transaction say $tx'$ that occurs at the nearest time to $tx$. We use the exchange rate in $tx'$ to estimate the value of token $T$ in transaction $tx$.
 
The majority of swaps, about $97.9\%$, are atomic in the result. Among the rest that violates atomicity, there are two significant sources (in red): Violation I and V in Uniswap V2. Cases violating V are caused by the high token fees charged by some AMM pools. Cases violating I are caused by some non-standard token deposits, as will be discussed in \S~\ref{sec:profitabledeposits}.

\section{Formulating Threats from Atomicity Violations}
\label{sec:understanding}
\label{sec:causeanalysis}

This section formulates two threats from the discovered atomicity violation. We characterize AMM protocols, formulate the threat model, and present a brief security analysis. At last, we describe some profitable deposits found empirically.

\subsection{Characterizing AMM protocols}

An AMM service consists of pool smart contracts and token smart contracts. A pool smart contract needs to support essential AMM operations, including token swaps and liquidity addition/removal. In addition, a responsible AMM pool also needs to handle the ``error'' case where tokens are deposited to the pool by mistake (e.g., users using the wrong interface) and need to be returned. 

\begin{table}[!htbp] %force in current page, disable float.
  \caption{Characterization of AMM protocols. ``Lost'' refers to lost tokens.}
  \label{tab:ammprofile}
  \centering{
  \begin{tabularx}{0.475\textwidth}{ |X|c|c|c|c| }
  \hline
Design & Uniswap V2 & Uniswap V3 & Balancer & Curve \\ \hline
Deposit by \texttt{transfer} 
& \cmark & \xmark & \xmark & \xmark \\ \hline
Risks
& Theft & Lost & Lost & Lost \\ \hline
  \end{tabularx}
}
\end{table}

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.3\textwidth]{figures/uniswapv2-dilemma.eps}
\end{center}
\caption{The AMM service supporting token deposit-by-\texttt{transfer}; the functions are specific to the example of Uniswap V2.}
\label{fig:uniswapv2model}
\end{figure}

Each AMM operation internally consists of a series of token deposits and withdrawals. A token deposit can be made by two mechanisms, considering the ERC20 token standard. 1) A trader account may call token $ T_0$'s \texttt{transfer} function to deposit tokens to the pool's account. We call this mechanism deposit-by-\texttt{transfer}. Figure~\ref{fig:uniswapv2model} shows an example AMM accepting deposit-by-\texttt{transfer} in which the depositor first externally calls $T_0$’s \texttt{transfer} to deposit tokens, and the pool then calls token $T_1$’s \texttt{transfer} to withdraw tokens and to complete the token swap. 2) Alternatively, a trader account may first call token $ T_0$'s \texttt{approve} to delegate the spending right to the pool smart contract, and then the pool smart contract calls $ T_0$'s \texttt{transferFrom} to complete the deposit. We call this design by deposit-by-\texttt{transferFrom}.

We characterize the AMM protocols by their support of deposit-by-\texttt{transfer}. The characterization result is presented in Table~\ref{tab:ammprofile}, where the Uniswap V2 family support deposit-by-\texttt{transfer} (and also deposit-by-\texttt{transferFrom}), and the other AMMs don’t support deposit-by-\texttt{transfer}.

\subsection{Threat Model}

\noindent{\bf Token theft}: Against an AMM (that supports deposit-by-\texttt{transfer}), an adversarial trader monitors certain on-chain states and sends crafted transactions to call AMM operations. The attack is successful if the crafted transactions are able to withdraw more value than deposited from the AMM pool. The attacker's capability includes monitoring certain blockchain states in both mempool and included blocks, determining a ``pending'' AMM state in value is deposited but is not withdrawn yet, and sending crafted transactions to frontrun other withdrawal transactions. The victim can be the AMM pool itself or another account that deposited value to the pool; for the latter, the account can be a trader (e.g., in $P_4)$ or other non-standard depositors such as token issuers calling rebase (in $P_1$). 

\noindent{\bf Lost tokens}: On an AMM (that does not support deposit-by-\texttt{transfer}), a victim trader makes a deposit to the AMM pool using the unsupported \texttt{transfer} mechanism. This deposit by mistake can be made by the trader accidentally or being intentionally tricked by an external attacker. Having received the deposit, the adversarial AMM pool does not return it to the trader, resulting in permanently lost tokens.

\subsection{Security Analysis}

We present a brief security analysis, in theory, to shed light on why the two threats would succeed in practice. In the next two sections (\S~\ref{sec:attack} and \S~\ref{sec:losttokens}), we conduct empirical studies to detect the two attack instances from discovered atomicity violation cases.

\noindent
{\bf Theft on AMM supporting deposit-by-\texttt{transfer}}: This case applies to Uniswap V2-based services, including Uniswap V2, Pancakeswap, and Sushiswap. In these AMM services, consider a token swap operation in which token deposit and withdrawal are made in two separate transactions, as shown in Figure~\ref{fig:uniswapv2model}. The deposit transaction $tx_1$ in the figure {\it only} calls the token smart contract, and the withdrawal transaction $tx_2$ calls the AMM pool smart contract. Due to the ERC20 standard, the token smart contract does not record the depositor information on-chain in $tx_1$. When the pool handles the withdrawal transaction $tx_2$, it cannot find depositor information on-chain and thus is unable to exercise any access control (or permissions) on who can withdraw the deposited value. We call this vulnerability by {\bf permissionless withdrawal}. In practice, all Uniswap V2's pool smart contracts support permissionless withdrawal. They detect token deposits by tracking the pool account's balance update and allow the first request that comes to withdraw the value. The withdrawn value can be up to the amount of the deposited value.

An AMM pool that allows permissionless withdrawal exposes the trader to the risk of token thefts. Because no permission is checked, the deposited value can be extracted by another transaction $ tx'_1$ sent by an adversary frontrunning $tx_1$. $ tx'_1$ can be sent by a human adversary or a bot.

\noindent
{\bf Lost tokens on AMM not supporting deposit-by-\texttt{transfer}}: This case applies to all AMM protocols other than Uniswap V2. A mistaken token deposit is normally by the trader externally calling the token smart contract's \texttt{transfer} function. Because the AMM pool does not recognize \texttt{transfer}, it can not take any action upon receiving such a deposit. The tokens are thus lost by the adversarial AMM.

Based on the observation above, we hypothesize atomicity violations with more deposited value than withdrawn, that is, I, III, and IV, in the Uniswap V2-based AMM services, are instances of token theft attacks. We present our study to detect thefts in Uniswap V2 in \S~\ref{sec:attack}. We also hypothesize atomicity violations with less deposited value than withdrawn, that is, II and V, in the other AMM services, including Uniswap V3, Balancer, and Curve, are instances of lost tokens. We present our empirical study to detect lost tokens in these services in \S~\ref{sec:losttokens}.

\subsection{Profitable Deposits}
\label{sec:profitabledeposits}

We describe some profitable deposits found in our measurement result. We use Uniswap V2 as an example to show why such deposits are profitable and can be stolen in theft.

\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.475\textwidth]{figures/victimpatterns.eps}
\end{center}
\caption{Patterns of profitable deposits: $R$ is the router smart contract (part of the pool), $T_0$/$T_1$ are the two tokens in the target liquidity pool. Both $P_1$ and $P_2$ are non-standard mechanisms that update token balance.}
\vspace{-0.15in}
\label{fig:patterns}
\end{figure}

\subsubsection{Token Supply Rebase (Pattern $P_1$)}
\label{sec:cases:rebase}

In many real-world tokens, the account balance can be changed by non-standard operations beyond token transfer. We describe an example of {\it token rebase}. Token balance can be elastically adjusted by token issuers for purposes such as stabilizing the token's exchange rates against other tokens. In practice, token rebase is such a non-standard balance-changing function, supported in some widely used tokens, such as AMPL~\cite{me:ampl:token}. When a token, say $T_0$, is rebased, a Uniswap's relevant pool, say for tokens $T_0$ and $T_1$, could have its $T_0$ balance increased. Uniswap falsely assumes that this balance increase is due to some accounts that swap token $T_0$ for token $T_1$. Uniswap's pool would mistakenly admit anyone who requests to withdraw token $T_1$ after the rebase of $T_0$.

\ignore{
{\it Token shareholder}: 
As another example, there are tokens that charge ``tax'' to average owner accounts and redistribute the ``tax'' income among privileged accounts of shareholders. Specifically, these tokens support two kinds of owners, average owner, and token shareholders. When there is a transfer, the token smart contract charges a certain amount of fees. The fees are redistributed to the privileged accounts of token shareholders. Thus, a transfer between average accounts would update the balance of all shareholders' accounts. In a Uniswap's pool of token types $T_0$ and $T_1$, if the pool's account in $T_0$ is a shareholder, any transfers in $T_0$ would increase the pool's balance and create a profitable opportunity.
 
Furthermore, even when the pool receives a token deposit, the deposit may not be intended as a part of the swap. For instance, airdrop is a common practice to promote the use of a new token type, in which token issuers periodically give away newly minted tokens to the current token owners (e.g., in Tokens MILK2~\cite{me:token:milk2} and 3Cs~\cite{me:token:3cs}). When a token, say $T_0$, is airdropped into a Uniswap's pool, the pool holding tokens $T_0$ and $T_1$ would mistakenly treat the transfer as a part of swap from token $T_0$ to $T_1$. Thus, the pool would admit anyone's request to withdraw token $T_1$ after airdrop of token $T_0$ to the pool's account.
}

In general, these non-standard token operations allow for updating the pool's balance but do not intend to withdraw the same value from the pool. We name the pattern $P_1$.

\subsubsection{Interest-bearing Tokens ($P_2$)}
Beyond $P_1$, there are implicit approaches to updating the balance. Many tokens are bearing interest. That is, the balance in the token smart contract increases at a certain rate as time goes by. Suppose a Uniswap pool is of token $T_0$ and $T_1$ where $T_0$ is interest bearing. Similar to $P_1$, the Uniswap pool observing the increase of token $T_0$ would admit the withdrawal of token $T_1$ by anyone who requests it, including a value-extracting attacker. We call this attacker's pattern by $P_2$, which is different from $P_1$. In $P_2$, the attacker simply waits long enough to harvest the extractable value from token interest. 

\subsubsection{External Transfer for Deposit ($P_3$)}

In Uniswap, a trader can externally call token $ T_0$'s transfer function to make a deposit so that she can withdraw token $T_1$ in a separate transaction. We call the pattern of a victim trader sending a transaction to externally transfer token $T_0$ by $P_3$. When $P_3$ occurs, a malicious account can send the withdrawal transaction ahead of the victim's one to claim the value in the pool. This attack is possible because a Uniswap pool receiving a deposit of $T_0$ will approve the next withdrawal of token $T_1$, no matter who sends it. 

\subsubsection{Buggy Router Contracts ($P_4$)}

In the above three patterns, the victim may externally call token $ T_0$'s functions. In the fourth pattern $P_4$, the trader delegates the handling of the swap to a router smart contract that is buggy and violates atomicity. After the trader EOA's transaction, the router smart contract successfully completes the deposit of Token $T_0$ but fails at requesting the withdrawal of Token $T_1$. Thus, anyone who requests the token withdrawal in the next transaction, including an attacker EOA, would succeed in extracting the value illicitly. 

\section{Detecting Token Thefts}
\label{sec:attack}

\subsection{The Detection Problem}
\label{sec:discoveryproblem}

\noindent{\bf Theft detection}: 
The detected atomicity violations, especially I, III, and IV, could present the value that {\it can} be extracted by real-world attackers. However, whether the value is {\it actually} extracted by the attackers, or equivalently, whether the violation operations are actual attack instances, is a different problem. 

Consider as an example that a token issuer sends a vulnerable rebase transaction to a pool's token, followed by a withdrawal transaction sent by account $A$ (i.e., $P_1$). $A$ may or may not be the token issuer. The former case is not an attack, as the token issuer, aware of the risky rebase, sends the withdrawal to remedy the risk. The latter case may be an attack. In other situations, including $P_3$ and $P_4$, a atomicity violation can also be attributed differently.
\ignore{
For instance, in $P_1$, after a token issuer sends an exploitable rebase transaction, it is equally likely one of the following cases occur: 1) the token issuer, aware of rebase being exploitable, quickly sends a swap request herself to claim the value in the Uniswap pool. 2) An attacker observing the occurrence of rebase operation calls the liquidity pool to withdraw the value there. The former case is not an attack, while the latter one is. In other cases, the same applies: In $P_3$, if the trader sends another transaction to withdraw the value in token $T_1$ right after the transaction of depositing $T_0$, it is a benign case. But if it is an attacker account that withdraws after the external deposit, it constitutes an attack. In $P_4$, if the trader observes the router exception and immediately send a ``make-up'' transaction to claim the value herself, it is a benign case. But if it is a third-party ill-intended account that sends the withdrawal transaction, it constitutes an attack.
}

Distinguishing attacks from benign cases entails checking two essential conditions: {\bf 1) Whether two accounts are controlled by two distinct physical users}: It cannot be an attack if the trader account who makes the profitable deposit in token $T_0$ is controlled by the same physical user with the account who succeed in withdrawing the value in token $T_1$. 
Thus, attack detection becomes the problem of linking two blockchain accounts of the same physical user, which is known to be an intractable problem if the only information known is on-chain data.
{\bf 2) What's a transaction sender's intention}: That is, whether a withdrawal transaction is intended as an attack. Even when the withdrawer and depositor accounts are not the same physical user, they can be friends in  real life, which makes the swap non-attack. Thus, it entails detecting the depositor account's intention in sending the withdrawal request, which, however, can be hidden opaque and pose challenges to detection.

\noindent
{\bf Feasibility of existing approaches}: 
On checking Condition 1), there are existing works that tackle the recovery of account linkage by heuristics specific to Bitcoin's UTXO model~\cite{DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13}. The only work for Ethereum~\cite{DBLP:conf/fc/Victor20} presents a linkage heuristic exploiting some DEXes deposit addresses. Specifically, on order book-based DEXes (i.e., IDEX and EtherDelta), trader Alice swapping token $T_0$ for $T_1$ can specify the so-called deposit address who receives $T_1$. Assuming a swap is normal, the sharing of deposit addresses by two traders implies that the two traders are controlled by the same physical user. This work is different from our attack detection problem, where the deposit address heuristic is to detect the case that two accounts are linked, while our problem is to detect if two accounts are unlinked. More importantly, the deposit address heuristic works only under the assumption of normal swaps, while our work deals with atomicity violations. Given an atomicity-violating swap, the deposit address of a swap refers to the attacker. Thus, when an attacker targets two victim traders, it could appear that two traders share the same deposit address. In this attack, the two victim traders do not have to be linked to the same off-chain user.

On checking Condition 2), there are existing works on threat intelligence on blockchains by characterizing attackers' behavior~\cite{DBLP:conf/uss/SuSDL0XL21}. However, their targets are program-level attacks such as reentrancy attacks, and their attack strategies don't apply to the DEX context of this work.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.4\textwidth]{figures/indicators.eps}
\end{center}
\caption{Rational attack strategies (A1/A2/A3).}
\label{fig:indicators}
\end{figure}

\subsection{The Detection Method}

We discover attacks by designing attack strategies specifically for different profitable deposits and use them as attack indicators to match the observable attacker behavior on-chain. 

\noindent
{\bf Design rationale: Attack strategies}: Recall that each atomicity-violating swap involves a profitable deposit followed by a withdrawal that reaps the profit. An attacker needs to strategically send the withdrawal to ensure high success rates by properly monitoring the profitable deposits. We consider three attack strategies:

\begin{itemize}[leftmargin=0.5cm]
%\setlength{\itemindent}{0em}
\item
 {\bf A1) Aggressive attacker (monitoring deposits)}: The attacker directly monitors the mempool for the profitable deposits. In this strategy, the attacker monitors different cases of profitable deposits, such as $P_1$/$P_2$/$P_3$/$P_4$. The attacker launches a node joining the Ethereum blockchain network and monitors the node's mempool so that the profitable-deposit transaction can be detected as soon as they are propagated in the blockchain network. 

Strategy A1 entails the attacker customizing the monitored conditions to different causes. It minimizes the time window between the exploited deposit and withdrawal and ensures a high success rate in the presence of competitors.

\item{\bf A2)
The general-purpose attacker (monitoring pool)}: The attacker monitors the Ethereum's smart contract state to check if the pool is profitable. For instance, when a rebase transaction is executed in the blockchain, it could increase the balance in the token smart contract and leave the reserve in the pool smart contract unchanged. By detecting the difference between token balance and reserve, the attacker ensures sending a withdrawal can succeed.

Strategy A2 is generalizable to different profitable deposits, in the sense that the attacker monitors a single condition that all different profitable deposits will trigger. However, this strategy works only after the profitable deposit transaction is executed and included in the blockchain. So an aggressive attacker (A1) can frontrun a general-purpose attacker (A2).

\item{\bf A3)
Scavenger trader}: The trader randomly and aggressively sends attack transactions in the hope of luckily extracting the profit. The delay between the withdrawal and victim deposit can be arbitrary. 
\end{itemize}

\noindent
{\bf Proposed attack indicators}: 
An account's strategy, which normally occurs in the blackbox off-chain state, is not directly observable from the on-chain traces. We distill observable information and design indicators to infer attack strategies.

To begin with, an aggressive attacker monitoring the off-chain mempool states cannot be observed from the on-chain traces. Likewise, a general-purpose attacker who may choose to issue RPC calls to read on-chain data is also unobservable. For these cases, we collect the gap between the block, including deposit transactions, and the block including the exploit withdrawal transactions, as the metric to infer the presence of an attack and further the attack strategies. For instance, if the block gap is always $0$, it indicates the case is exclusively an aggressive attack. If the deposit is token interest and the block gap is always large, it indicates an aggressive attack exploiting token interest. Otherwise, if the block gap is randomly distributed, it is likely a scavenger trader. Based on the heuristics, we propose several indicators listed below. We defer the description of proposed theft-detection algorithm and additional indicators to Appendix~\ref{appd:extraindicators}.

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I1: An account whose withdrawal transactions occur consistently within $X_1$ blocks after profitable deposits (i.e., block gap smaller than $X_1$) and whose victim deposits are not caused by token interests (i.e., not $P_2$) is likely to be an attacker. Formally, 
$$
I_1\leq{}X_1
$$
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I2:
An account whose withdrawal transactions occur consistently more than $X_2$ blocks after profitable deposits (i.e., block gap larger than $X_2$) and whose victim deposits are based on token interests is likely to be an attacker. Formally, 
$$
I_1\geq{}X_2
$$
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I12:
An account whose ratio between indicator I2 and I1 is larger than $X_{21}$ is likely an attacker. 
Intuitively, it shows the attacker's intentional adaptive strategies in exploiting deposits of different patterns.
Formally,
$$
\frac{I_2}{I_1}\geq{}X_{21}
$$
}}\end{center}

In practice, many accounts use delegate smart contracts on-chain to relay their payload (of malicious withdrawals). The delegate smart contracts make attack strategies observable. We propose the following indicators to take advantage of this fact. 

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I4:
An account who attempts to withdraw through a smart contract that checks both pool reserves (i.e., calling \texttt{pool.getReserves()}) and token balances (calling \texttt{erc20token.balanceOf()}) is likely a general-purpose attacker. Note that this indicator does not require the smart contract to actually withdraw the token $T_1$. 
}}\end{center}

The intuition of the above indicator is that a general-purpose attacker uses the pool's \texttt{getReserves()} function and token's \texttt{balanceOf()} function to obtain the token reserve and balance, respectively. This shows the account's intention to calculate pool profitability and indicates a general-purpose attacker. 
%Note that the indicator is not necessary (i.e., causing false negatives), as a general-purpose attacker can issue RPC queries to read reserves and balances, leaving no trace on-chain.

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I5: An account whose withdrawal transactions exclude any token deposit is likely to be an attacker.
%An account whose withdrawal transactions also include token deposits is likely to be a scavenger trader, even though the withdrawal is of higher value than the deposit.
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I6:
Standalone withdrawal that extract value from deposit patterns $P_1$ and $P_2$ indicate an attacker, because the value in $P_1$ and $P_2$ is intended for AMM pools, not for external accounts. This intuition is materialized into the formula below:
$$
\frac{|P_1|+|P_2|}{\sum_{i}{|P_i|}}>X_7
$$
}}\end{center}

\subsection{Results}

\subsubsection{Validation using Ground Truth}

\noindent{\bf Establishing ground-truth}:
We search the Internet sites, including Google, Twitter, and Reddit. Our searches include the candidate attacker accounts (i.e., mules in Table~\ref{tab:attackerview}) and keywords such as ``attack, vulnerable, scam, frontrunning, bot, arbitrager, MEV, bots.'' Besides, we check the candidate account's tags on Etherscan and if they are security sensitive.
Out of the $142$ suspected accounts from our results (described next in \S~\ref{sec:theftinstances}), we found $9$ accounts are complained about on the Internet, and $2$ accounts are tagged as MEV bots on Etherscan. 
The ground-truth accounts are presented in Table~\ref{tab:attackerview}, and the full detail of ground truth data collection is in Appendix~\ref{sec:groundtruth}.

\begin{table}[!htbp] %force in current page, disable float.
\caption{Detection parameters extracted from the ground-truth data}
\label{tab:parameters}\centering{
\begin{tabularx}{0.4\textwidth}{ |X|l|l|l|l|l| }
  \hline
  Parameters & $X_1$ & $X_2$ & $X_{12}$ & $X_4$ & $X_7$ \\ \hline
  Value & $617$ & $19.28$ & $1$ & $97.5\%$ & $69.2\%$ \\ \hline
\end{tabularx}
}
\end{table}

\noindent{\bf Result validation}: Recall that our detection method is parameterized. We use the ground truth data to set the parameters so that all the ground-truth accounts can be detected positive under these parameters. The ``trained'' parameters are listed in Table~\ref{tab:parameters}. 
For instance, account $0x0c08545df4939ef46c1364b5930e840739667467$'s $I2$ meets the condition ($I2<2$) and account $0xEA674fdDe714fd979de3EdF0F56AA9716B898ec8$ meets the condition that $\frac{I2}{I1}=686/0.5=1372>19.2$.

\subsubsection{Detected Attack Instances}
\label{sec:theftinstances}

\begin{table*}[h]
  \caption{Detected theft instances by accounts: Ground truth and test data. Bold are strong cases suggesting the account is an attacker. Victims include normal accounts and token issuers.}
\label{tab:attackerview}
  \centering{\scriptsize
  \begin{tabular}{|p{6.7cm}|p{1.0cm}|p{2.3cm}|p{0.4cm}|p{0.5cm}|p{0.5cm}|p{1.4cm}|p{0.2cm}|p{0.5cm}|p{0.5cm}|}
  \hline
  Accounts & Value & {Deposit} & \multicolumn{6}{c|}{Attack indicators} & Label \\
  \cline{4-9}
  (Mules) & $10^3$ USD & patterns &I1 & I2 &I12 & I4 & I5 &I6&\\ \hline
  \multicolumn{10}{|l|}{Ground truth data} \\
  \hline
  $0x9799b475dec92bd99bbdd943013325c36157f383$ & 556 & 33$P_1$,4$P_2$,6$P_4$    &422       &371        &0.88  & 0                  &\xmark      &86\% & A3\\
  \hline
  $0x0c08545df4939ef46c1364b5930e840739667467$ & 101 & 3$P_1$,1$P_4$            &{\bf 1.5} &           &0     & 0                  &\xmark      &75\%& A2 \\
  \hline
  $0x56178a0d5f301baf6cf3e1cd53d9863437345bf9$ & 101 & 53$P_1$,4$P_2$,2$P_3$,2$P_4$ &13    & 1574      &{\bf121}   & 0                  &\xmark      &93\%& A1 \\
  \hline
  $0x0000000000007f150bd6f54c40a34d7c3d5e9f56$ & 11 & 15$P_2$                   &          &96         &$\infty$& 15 ({\bf 100\%}) &\xmark      &100\%&   \\
  \hline
  $0x7c651d7084b4ba899391d2d4d5d3d47fff823351$ & 1.8 & 2$P_1$                   &68        &           &0     & 0                  &\xmark      &100\%&  \\
  \hline
  $0x00000000e84f2bbdfb129ed6e495c7f879f3e634$ & 0.5 & 9$P_1$,4$P_3$            &{\bf 1.1} &           &0     & 0                  &{\bf \cmark}&69\%&   \\
  \hline
  $0xca850b6833ef86ef0484c6be74b06d61b39df031$ & 0.5 & 40$P_3$                  &{\bf 1.4} &           &0     & 39 ({\bf 98\%})    &\xmark      &0\%&   \\
  \hline
  $0x17e8ca1b4798b97602895f63206afcd1fc90ca5f$ & 0 & 1$P_1$                     &3061      &           &0     & 0                  &{\bf \cmark}&100\%&   \\
  \hline
  $0xf90e98f3d8dce44632e5020abf2e122e0f99dfab$ & 0 & 1$P_1$                     &1402      &           &0     & 0                  &\xmark      &100\%&   \\
  \hline
  $0x42d0ba0223700dea8bca7983cc4bf0e000dee772$ & 0.5 & 1$P_3$                   &{\bf 0}   &           &0     & 1  ({\bf 100\%})   &{\bf \cmark}&0\%&   \\
  \hline
  $0xEA674fdDe714fd979de3EdF0F56AA9716B898ec8$ & 0.2 & 2$P_1$,5$P_2$            &{\bf 0.5} &686        &{\bf1372}& 6 ({\bf 86\%})   &{\bf \cmark}&100\%&   \\
  \hline
  $0x000000000025d4386f7fb58984cbe110aee3a4c4$ & 0.2 & 1$P_1$                   &38        &           &0     & 1  ({\bf 100\%})   &\xmark      &100\%&   \\
  \hline
  $0xD224cA0c819e8E97ba0136B3b95ceFf503B79f53$ & 0.1 & 3$P_2$,1$P_3$            &32        &617  &19    & 4  ({\bf 100\%})   &\xmark      &75\%&   \\
  \hline
  $0xb8aaed2e3117fa589eb05b0d7d0c8469d9e41ec5$ & 0.1 & 1097$P_1$                &351       &           &0     & 0                  &\xmark      &100\%&   \\
  \hline
  $0x829BD824B016326A401d083B33D092293333A830$ & 0.1 & 5$P_2$                   &          &696  &$\infty$ & 5  ({\bf 100\%})   &\xmark      &100\%&   \\
  \hline
  \multicolumn{10}{|l|}{Test data} \\
  \hline
  $0x2a2e25ad00faac024f6a8d8cdc0fc698fbda71b7$ & 239 & $32P_1$                  &{\bf 0.03}&           &0     & 32 ({\bf 100\%})   &{\bf \cmark}&100\%& A1\\
  \hline
  $0xdb40ea5b6d0ef9e45c00c194345b44765a53dd19$ & 113 & $12P_1,2P_2,3P_3$        &{\bf 2.5} &665  &{\bf266}   & 17 ({\bf 100\%})   &{\bf \cmark}&82\%& A1 \\
  \hline
  $0xb6bf45f59b94d31af2b51a5547ef17ff81672743$ & 20 & $1091P_1,131P_2,9P_4$     &224       &600  &2.7   & 1231 ({\bf 100\%}) &{\bf \cmark}&99\%& A2\\
  \hline
  $0xc762e15cfbf392f4346ee7e8466ca595e571382b$ & 16 & $64P_1,6P_2,13P_4$        &{\bf 3.0} & 5.3       &1.8   & 83 ({\bf 100\%})   &{\bf \cmark}&84\%& A2\\
  \hline
  $0xa32d3f8a970ab3222ffa1c89cb910abf7b7201d0$ & 6 & $208P_2$                   &          &942 &$\infty$ & 208 ({\bf 100\%})  &{\bf \cmark}&100\%& A2\\
  \hline
\end{tabular}%
}
\end{table*}
  


We present our analysis result in Table~\ref{tab:attackerview} which characterizes the most frequent accounts involved in atomicity violations. The metrics include value stolen, causes, attacker indicators, the number of pools attacked, the number of victim accounts, and the label whether the account is an attacker. From the table, we analyze the attackers' strategy of several selected accounts.

\noindent
{\bf Case 1: Agg. attacker (A1) w. zero block gap}: Account $0x2a2e$ is involved in $32$ atomicity violations and gains more than $2.39*10^5$ USD worth of illicit tokens. All $32$ swaps from this account are sent via a smart contract which checks the pool's profitability before withdrawal (I4). In terms of timing, the malicious withdrawals are always sent in the same block with the risky, profitable deposit. We believe account $0x2a2e$ aggressively monitors the mempool for the target tokens' rebase transactions and if found, sends withdrawals immediately to ``backrun'' the deposits and claim the value.

\noindent
{\bf Case 2: General attacker (A2) w. off-chain monitoring}: Account $0x0c08$ has withdrawn four times and grabbed tokens of $1.01*10^5$ USD. The account directly and externally calls Uniswap pool's swap function to withdraw without checking pool profitability on-chain. The withdrawals are included in exactly one block after the one that includes the risky deposit. We believe Account $ 0x0c08$'s strategy is to monitor the pool profitability from an off-chain vantage point and to immediately send withdrawal by external calls. Because the account monitors the pool profitability instead of the cause (risky deposit), it has to wait until the inclusion of risky deposit that updates the pool state to be profitable. This explains why the inclusion of withdrawal has to be one block after the block including the risky deposit.

\noindent
{\bf Case 3: Agg. attacker (A1) stealing interest}: Both Accounts $0xdb40$ and $0x5617$ have extracted value from interest-bearing tokens. Their block gaps are large ($665$ and $1574$, respectively). Given that there are enough samples, this consistent behavior shows both accounts' attack strategy to wait long enough for the token interest to accumulate and for the extractable value to be large enough before acting on it.

\noindent
{\bf Case 4: Adapting strategies}: For all accounts with indicators I1 and I2 in the table, it is clear that the block gaps for different causes (I1 and I2) differ: The block gaps for non-interest causes are consistently much shorter than those for token interests. It implies that the attackers are aware of the situation (which causes them to exploit) and tailor their strategies to it.

\noindent
{\bf Case 5: Scavenger trader (A3)}: Account $0x9799$ is unlikely an intentional attacker: First, it does not read the token balance or check the pool's profitability before the withdrawal. Second, the block gap between the profitable deposit and malicious withdrawal is large, at hundreds of blocks apart. In addition, the smart contract Account $0x9799$ relays her withdrawal requests also make deposit to the pool. All these indicators show that $0x9799$ is a scavenger trader.

\subsubsection{Block Gaps}

\begin{figure}[!ht]
  \begin{center}
    \subfloat[Block gaps and the number of competing attackers]{%
\includegraphics[width=0.245\textwidth]{figures/figure_allrebase_blockdif.eps}
\label{fig:blockdif_1}
    }%
    %\hspace{-0.2cm}%
    \subfloat[Block gaps and value stolen]{%
\includegraphics[width=0.245\textwidth]{figures/figure_value_blockdif.eps}
\label{fig:blockdif_2}
    }%
  \end{center}
  \caption{Block gaps and affecting factors}\label{fig:complex}\vspace{-0.10in}
\end{figure}

Recall that each theft attack runs in two transactions: The first transaction that creates extractable value, and the second transaction that withdraws the value and steals it. Given each detected attack (described in the previous subsection), we measure the gap of the two blocks that include the attack's two transactions, namely block gap. We further report two metrics: the number of competing attackers and the value stolen. For each profitable deposit transaction, say $tx$, we find transactions sent by competing attackers. Here, a competing attacker either directly sends a transaction to withdraw the extractable value created by $tx$ but fails or sends a transaction to read the token balance and pool reserve (which shows the intention to withdraw the value). 

We report the block gaps with the varying number of competitors in Figure~\ref{fig:blockdif_1}. A larger dot in a X/Y coordinate in the figure represents more attacks found with the same X/Y value. The result shows that when there are many competing attackers, the block gap tends to be small. This could be explained: Because the first attacker wins, the more attackers there are, the earlier the withdrawal transaction is sent, namely a smaller block gap.
The result also shows that with few competing attackers comes a large range of block gaps.

We then report the block gaps with varying value stolen in Figure~\ref{fig:blockdif_2}. The result shows that when the stolen value is large, the block gap tends to be small. A possible explanation is that the higher extractable value gives the attacker more incentives to send the withdrawal transaction with a higher fee and to frontrun other potential thieves.
 
\subsubsection{Attacker/Victim Behavior over Time}

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_attacker_timeline.eps}
\end{center}
\caption{Attack timeline of top-10 attackers. In the Y axis, attacker accounts are ordered by the total value stolen.
Data from 07/09/2020 (block 10422671) - 06/29/2021 (block 12727620).}
\label{fig:attack}
\end{figure*}

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_victim_timeline.eps}
\end{center}
\caption{Attack timeline of top-10 victims. In the Y axis, victim accounts are ordered by the total value stolen.
Data from 07/29/2020 (block 10553883) - 01/10/2022 (block 13979019).}
\label{fig:victim}
\end{figure*}

We plot the timeline of the top-10 attackers' activities in Figure~\ref{fig:attack}. The attackers are ranked by the total value stolen, with attacker $0x9799$ being the top-1. Each dot represents a detected attack sent by the attacker's account. The size of the dot represents stolen value. Color represents the exploit pattern. The most successful attacker ($0x9799$) steals value through different causes (including rebase, airdrop, etc.) The attacker's activities last about 
$1.1*10^6$ blocks, which amount to six months. The second attacker ($0x2a2e$) concentrates all her attacks on a one-month span. She exploits exclusively the value created by rebase operations. The third attacker ($0xdb40$) mount attacks sporadically and target value created through two causes: Token interest and rebase operations. The ninth attacker exploits buggy smart contracts to gain illicit profit. The tenth attacker exclusively grabs the value from the token interest in a three-month period. As a result, most top attackers mount multiple attacks consistently, which shows the attacks are intended and not by accident.

We additionally study top victims' behavior. The victims are ranked by the value stolen. In Figure~\ref{fig:victim}, we plot in dots the transactions sent by victims whose deposits are stolen in identified attacks. Different color represents different causes. Additionally, in hollow green circles, we plot the normal transactions sent by the victims and related to Uniswap. The result shows that most victims change behavior after an attack/theft. For instance, victim accounts, including $0x0cd4$ and $0x80cc$, all stop using the vulnerable interface (e.g., partly error) to send a deposit after an attack. However, other victims can repeatedly create extractable value that gets stolen. For instance, account $0x66ac$ repeatedly airdrop tokens to the Uniswap pool, which gets stolen. 

\subsubsection{Value Received by Pools}

\begin{table}[!htbp] %force in current page, disable float.
\centering{
\begin{tabularx}{0.425\textwidth}{ |X|l|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
\hline
Value extracted by & Rebase ($P_1$) & External transfer ($P_3$) \\
\hline
External attackers & \$0.81M & \$0.50M \\
\hline
Pools (intended) & \$58.1M & \$1.22M \\
\hline
Pools (accidental) & \$0.65M & \$1.29M \\
\hline
\end{tabularx}
}
\caption{Extractable value and its destinations}
\label{tab:extractable_value}
\end{table}

\begin{figure}[!htbp]
\begin{center}
  \subfloat[Value created by rebase ($P_1$)]{%
     \includegraphics[width=0.245\textwidth]{figures/figure_rebase_seg.eps}
    \label{fig:moneyflow_1}
  }%
  \subfloat[Value created by external transfers ($P_3$): all pools are between token $XX$ and $WETH$, where $XX$ is the tick on the $x$ axis.]{%
    \includegraphics[width=0.245\textwidth]{figures/figure_underwater_seg.eps}
     \label{fig:moneyflow_2}
     }%
\end{center}
\caption{Extractable value received by the pool versus that by attacker accounts}\label{fig:complex}\vspace{-0.10in}
\end{figure}


Extractable value can be claimed by any account, including an external attacker and the pool itself. Our measurement result so far captures the former case. In this experiment, we measure the extractable value that goes to the pool.

A pool can claim extractable value by calling the \texttt{sync} function, which synchronizes the pool reserve and token balance. In Uniswap, there are three circumstances \texttt{sync} is called: a standalone call to \texttt{sync} in a transaction, \texttt{sync} called after a \texttt{swap} in the same transaction, \texttt{sync} called after an \texttt{addLiquidity} call in the same transaction. In the first case, tokens are sent to the pool intentionally (denoted by ``pool (intended)'' in the table and figures), and in the second and third cases, the pool receives deposit by accident (denoted by ``pool (accidental)''), because it is an irrelevant transaction to \texttt{sync} the reserve and token balance. Informally, we calculate the extractable value that goes to the pool in the following method: We obtain the value of the pool reserve before and after the transaction. We also parse the function call arguments from the transaction data field. We can cross-check the pre-state, post-state, and function arguments to detect the mismatch, which can be attributed to the extractable value. For instance, a normal \texttt{swap} in Uniswap does not change the product in AMM, and a spurious \texttt{swap} that the pool receives extractable value can be detected by the violation of product equality.

Using the above method, we measure the total extractable value claimed by the pool under different patterns, including $P_1$ and $P_3$. The result is presented in Table~\ref{tab:extractable_value}: The total value claimed by the pools is consistently more than $5\times$ of that by external attackers. This suggests ``room'' for the current Uniswap thief to increase their revenue. We further show the total extractable value by different pools/tokens. In Figure~\ref{fig:moneyflow_1}, we plot the extractable value created by different rebase-enabled tokens (Pattern $P_1$). 
Token $AMPL$ has the highest extractable value, most of which goes back to the pool by the token issuer intentionally calling \texttt{sync} function after each \texttt{rebase} call (the ``intended'' case). 
Token $BASE$ is the third highest in total extractable value and has the highest value stolen by external attackers. In Figure~\ref{fig:moneyflow_2}, we plot the extractable value created by external transfers (Pattern $P_3$) against different pools. Here, all the top-value pools we found are between token $WETH$ and another token. The most vulnerable pool is between Token $UNI$ and $WETH$, whose extractable value is $400$ thousand USD in total, among which the $10\%$ value is extracted by external attackers and the rest is mostly sent to the pool intentionally. Token $ YFill$'s value is exclusively extracted by external attackers. Token $ SUSHI$'s deposit is mostly claimed by the pool accidentally. 

\subsection{Characterizing Crimes}
\label{sec:behavior}

We further expand the scope of each attack instance by tracing the money flow and smart contract lineage. The goal is to uncover the attack business.

\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.495\textwidth]{figures/UniswapV2attacker3.eps}
\end{center}
\caption{Attack campaign template: Preparing, mounting, and wrapping up thefts.}
\label{fig:business}
\end{figure}

Given an attack instance with attacker accounts $\{A\}$, we construct an expanded attack graph by adding the following information: 1) the transactions that pay Ether or tokens to the attacker accounts, 2) the transactions that deploy the smart contracts used in the attack, and 3) the transactions that are sent by the mule accounts which receive the stolen tokens after the attack. These new transactions would add to the graph a set of new accounts, be it either the transaction sender or receiver. We iteratively apply this graph-expansion process until it reaches the ``hub-node'' accounts, which receive or send a large number of transactions (e.g., a popular DEX pool or mixer service). 
For instance, Figure~\ref{fig:business} shows an example of an expanded attack instance, with the attackers in the red box and the victims; the added accounts and transactions are outside the two boxes. 

\noindent
{\bf Attack ecosystem template}: We analyze the expanded attack graph in a template consisting of three phases: 1) attack preparation, 2) attack execution, and 3) attack wrap-up. Phase 2) is the core attack component, and Phases 1) and 3) are the expanded parts. In general, the actual boss often sits behind an exchange/mixer service, such as Tornado~\cite{me:tornado}, to hide its identity. In attack preparation (Phase 1), the boss sends commission in Ether to Attackers and Exploit developers. The Ether transfer can be relayed through the Mules. An Exploit developer writes an Exploit smart contract and deploys it to the blockchain. It then mounts the attack in the execution phase (Phase 2), exercising the strategies described previously (\S~\ref{sec:attack}). To wrap up a series of attacks (Phase 3), the mule receiving the stolen tokens transfers the tokens back to the boss. This is often done by swapping the stolen tokens to ETH (e.g., via DEX and wrapped tokens such as WETH) and by sending the ETH to the boss via a mixer service. In the attack wrap-up phase, the mule may transfer tokens to Investors to maximize the stolen value. 

\begin{table*}[h]
\caption{Attack ecosystem and attacker correlation: Red text shows the two attackers share the same developer of exploit smart contracts. AO represents the attack operator and EC is the exploit smart contract.
}
\label{tab:eco}
\centering{\small
    %\begin{tabular}{|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{1cm}|p{1.2cm}|}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \hline
    Accounts & \multicolumn{4}{c|}{Attack (S2)} & \multicolumn{2}{c|}{Preparation (S1)} & \multicolumn{2}{c|}{Wrap-up (S3)}  \\ \cline{2-9}
    (Mules) & \#AO & \#EC & Developer & Value ($10^3$ USD) & Commission & Mixer & DEX & Mixer \\
    \hline
     $0x9799$ & 5 %$0x4e53$, $0xac72$, $0xa084$, $0x5bb4$, $0xe929$ 
& 24 % $0x338c$, $0x3ac7$, $0x34a2$, $0x9a99$, $0x2927$, $0x536b$, $0xe9f8$, $0x684b$, $0x58a3$, $0x72bb$, $0xa8a2$, $0x72cb$, $0x2528$, $0xbf2d$, $0xadfc$, $0xd6a2$, $0x24af$, $0x1335$, $0xf367$, $0x94fc$, $0x5caf$,  $0x6332$, $0x3c3a$, $0x1233$	
& {\bf \color{red} $0x8641$} & 556 & \xmark  & \xmark  & \cmark  & \xmark \\
    \hline
    $0x2a2e$  & 1 %$0x2a2e$ 
& 1 %$0x5f5a$ 
& $0x2a2e$ & 239 & \cmark  & \xmark  & \cmark  & \cmark 
\\
    \hline
    $0xdb40$  & 5 %$0x64bc$, $0x62ae$, $0x3807$, $0x225c$, $0xdb40$ 
& 2 %$0x4dbc$, $0x4626$ 
& $0x4626$ & 113 & \cmark  & \cmark  & \cmark  & \cmark 
\\
    \hline
    $0x0c08$  & 1 %$0xfdee$ 
& 1 %$0x0c08$ 
& $0x0c08$ & 101 & \xmark  & \xmark  & \cmark  & \xmark 
\\
    \hline
    $0x5617$  & 4 %$0x3a51$, $0xf97b$, $0xbf3f$, $0xa1e6$ 
& 10 %$0xfb51$, $0x328d$, $0x8a14$, $0x0fc7$, $0x4ed5$, $0xb439$ ,$0x55a2$, $0x6ba3$ 
& \color{red}{$0x8641$} & 101 & \xmark  & \xmark  & \cmark  & \cmark 
\\
    \hline
    $0xb6bf$ & 1 %$0x675f$ 
& 2 %$0xb6bf$, $0x8526$ 
& $0x675f$ & 20 & \cmark  & \xmark  & \cmark  & \xmark 
\\
    \hline
    $0xc762$ & 1%$0xd0d0$ 
& 1%$0xc762$ 
& $0xd0d0$ & 16 & \cmark  & \cmark  & \cmark  & \cmark 
 \\
    \hline
    $0xa32d$ & 1%$0x7505$ 
& 1%$0xa32d$ 
& $0x7505$ & 6 & \cmark  & \xmark  & \xmark  & \xmark 
\\
    \hline  
    \end{tabular}%
}
\end{table*}

\ignore{
\begin{table}[h]
\caption{Attack ecosystem and attacker correlation: Red text shows the two attack instances are mounted using the exploit smart contracts developed by the same developer. AO represents attack operator and EC is exploit smart contract.
}
\label{tab:eco}
{\centering \scriptsize
    \begin{tabular}{|p{0.3cm}|p{1cm}|p{0.3cm}|p{0.3cm}|p{1cm}|p{0.7cm}|p{0.8cm}|p{.5cm}|}
    \hline
    Idx &Value ($10^3$~USD) & \#AO & \#EC & Developers & Mules & Deposits & Block gaps\\
    \hline
    1 & 552 & 5 %$0x4e53$, $0xac72$, $0xa084$, $0x5bb4$, $0xe929$ 
& 24 % $0x338c$, $0x3ac7$, $0x34a2$, $0x9a99$, $0x2927$, $0x536b$, $0xe9f8$, $0x684b$, $0x58a3$, $0x72bb$, $0xa8a2$, $0x72cb$, $0x2528$, $0xbf2d$, $0xadfc$, $0xd6a2$, $0x24af$, $0x1335$, $0xf367$, $0x94fc$, $0x5caf$,  $0x6332$, $0x3c3a$, $0x1233$	
& {\bf \color{red} $0x8641$} & $0x9799$ & $P_1$ & 121\\
    \hline
    2 & 101 & 1 %$0x2a2e$ 
& 1 %$0x5f5a$ 
& $0x2a2e$ & $0x2a2e$ 
& $P_1$ & 1\\
    \hline
    3 & 96 & 5 %$0x64bc$, $0x62ae$, $0x3807$, $0x225c$, $0xdb40$ 
& 2 %$0x4dbc$, $0x4626$ 
& $0x4626$ & $0xdb40$ 
& $P_1$ & 0\\
    \hline
    4 & 86 & 1 %$0xfdee$ 
& 1 %$0x0c08$ 
& $0x0c08$ & $0x0c08$ 
& $P_1$ & 1\\
    \hline
    5 & 67 & 4 %$0x3a51$, $0xf97b$, $0xbf3f$, $0xa1e6$ 
& 10 %$0xfb51$, $0x328d$, $0x8a14$, $0x0fc7$, $0x4ed5$, $0xb439$ ,$0x55a2$, $0x6ba3$ 
& \color{red}{$0x8641$} & $0x5617$ 
& $P_3$ & 2\\
    \hline
    6 & 48 & 1 %$0x675f$ 
& 2 %$0xb6bf$, $0x8526$ 
& $0x675f$ & $0x675f$ & $P_1$ & 0\\
    \hline
    7 & 29 & 1%$0xd0d0$ 
& 1%$0xc762$ 
& $0xd0d0$ & $0xd0d0$& $P_3$ & 1 \\
    \hline
    8 & 22 & 1%$0x7505$ 
& 1%$0xa32d$ 
& $0x7505$ & $0x7505$& $P_1$ & 0 \\
    \hline  
    \end{tabular}%
}
\end{table}
}


\noindent
{\bf Results}: We measure the attack behavior in terms of attack preparation, execution and wrap-up. We find different attacks mounted by the same mule account are consistent and thus present the aggregated results by mule accounts. The result is in Table~\ref{tab:eco}.

In the attack execution phase (S2), the result shows that attacks are systematic, typically with a mule associated with multiple attack operators (AO) and exploit smart contracts (EC). For instance, Mule $0x9799$ has mounted attacks through $5$ different operator EOAs and leveraged more than $24$ different exploit smart contracts. Her exploit contracts are developed by the same developer for another Mule $0x5617$ (in red in Table~\ref{tab:eco}); this implies an underground business of exploit contract development.

We further characterize the attack preparation (S1) and wrap-up (S3) on different mules. Under S1, Column ``Commission'' shows whether the mule's attack operators receive money used for mounting the attacks within 30 days before the attack. Column ``Mixer'' shows whether the attack commission comes from the anonymized crime boss hidden behind a mixer service, such as Tornado. Under S2, Column ``DEX'' shows whether the attacker interacts with a DEX service to exchange tokens or to maximize the illicit profit. Column ``Tornado'' shows whether the attacker eventually transfer money to the anonymized boss behind the mixer service. The result shows that different mules vary in their strategies in attack preparation and wrap-up. For instance, Mule $0x9799$ is quite simplistic in the sense that she only interacted with DEX and didn't involve any mixer service in her attacks. Mule $0xdb40$\footnote{The full address of $0xdb40$ is $0xdb40ea5b6d0ef9e45c00c194345b44765a53dd19$ and the account behavior is public on \url{https://etherscan.io/address/0xdb40ea5b6d0ef9e45c00c194345b44765a53dd19}.} and $0xc762$, on the other hand, are quite sophisticated and employ strategies involving mixer and DEX.

\section{Detecting Lost Tokens}
\label{sec:losttokens}

\noindent
{\bf Problem}:
We detect lost tokens out of standalone deposits (i.e., atomicity violation II). On the one hand, the incidents of lost tokens appear as standalone deposits. On the other hand, not every standalone deposit should be attributed to lost tokens. There are other causes, such as token giveaways, and administrative accounts calling privileged AMM operations. 

\noindent
{\bf Methods}: We propose two heuristics for detecting lost tokens. In the first heuristic, we assume the trader account calls an unsupported mechanism to deposit a token, finds the deposit fails, and switch to an alternative mechanism to retry the deposit. For instance, suppose an account deposits tokens using \texttt{transfer} in Uniswap V3, which does not accept \texttt{transfer}. The trader then switches to depositing the same value using \texttt{approve} before calling AMM operations such as \texttt{swap}. 
Based on the heuristics, we design the following indicator I8.

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I8:
Given a standalone deposit to an AMM pool, we find the transactions after the deposit from the same sender account. We filter out the transactions that are not issued to the same token with the deposit and the transactions that call the same token function with the deposit. The presence of such transactions given a deposit is an indicator of lost token.
}}\end{center}

In the second heuristic, the idea is that lost tokens must be deposited by an unprivileged AMM account. And a privileged account, such as an AMM administrator, is entitled to deposit value to an AMM pool, which is unlikely a mistaken deposit. We propose the indicator for lost token below:

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I9: An account that calls privileged AMM functions (e.g., \texttt{setSwapFee()} in Balancer) is an privileged account, and a standalone deposit sent by a privileged account is not attributed to lost tokens.
}}\end{center}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Aggregated results on lost tokens}
\label{tab:lost}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|l|l|l| }
  \hline
   AMM & \# txs & Total value (USD) & Block diff (avg) \\ \hline
   Uniswap-V3 & $20$ & $47928$ & $9013$ \\ \hline
   Balancer & $192$ & $7875$ & $6578$ \\ \hline
   Curve & $3$ & $905$ & $14533$ \\ \hline
\end{tabularx}
}
\end{table}


\noindent
{\bf Results}:
Using the method above, we detect $215$ instances of lost tokens on Uniswap V3, Balancer, and Curve, inflicting a total of lost tokens worth $56708$ USD, as shown in Table~\ref{tab:lost}. Given a standalone deposit, we calculate its value using the token price at the time of the deposit (by using nearest price with token WETH in Uniswap V2). We record the block difference between the standalone deposit and the follow-up deposit retry sent from the same account. It can be seen block difference on Uniswap V3 is about $371$ blocks which amounts to about $1.78$ hours. Detailed case analysis is in Appendix~\ref{sec:losttoken:cases}.

\section{Countermeasures}
\label{sec:mitigate}

As analyzed in \S~\ref{sec:understanding}, an AMM pool designer faces a dilemma, whether to support token deposit-by-\texttt{transfer}. Because to handle such a deposit, as in Uniswap V2, an AMM is susceptible to token theft, and not to handle the deposit, as in other AMM protocols, the AMM exposes their traders to the risk of lost tokens. In this section, we present countermeasures to bypass the design dilemma and against the two threats/risks. We present two mitigation paradigms: secure design of new AMM protocols that require redeployment of smart contracts and retrofittable hardening of deployed AMM services.

\subsection{Secure AMM Protocols}

We propose a secure protocol design for AMM pools. In our protocol, we follow Uniswap V3's design and require the AMM pool to accept only the deposits made by the \texttt{approve}-\texttt{transferFrom} workflow. By this means, the pool smart contract can keep track of swap-intended token deposits and thus can enforce permission checks on token withdrawal. That is, token withdrawal is granted only when its receiver is the same as the original depositor. By this means, it eradicates the risk of token thefts.

The risk of lost token is caused by the incapability of tracking token transfer history in the ERC20 standard. While changing ERC20 standard can help fix the issue, it is not practical given the large-scale deployment of ERC20 tokens on Ethereum. We propose a protocol to mitigate lost tokens with off-chain assistance. 

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.3\textwidth]{figures/mitigate_losttokens.eps}
\end{center}
\caption{Trustless design to mitigate lost token risks}
\label{fig:mitiglost}
\end{figure}

In our protocol, we assume a lost-and-found smart contract (called the service) that has the privilege to approve a request to return token deposits. Suppose a user Alice makes a mistake in depositing tokens to our AMM pool by calling the unsupported \texttt{transfer} function. The token deposit transaction is $tx1$. After finding the mistake, Alice may request a refund by contacting the lost-and-found service. Alice's request includes $tx1$ and enough blocks after $tx1$ (inclusively) to verifies $tx1$'s finality on Ethereum. Using the information, the service smart contract then verifies the finality of $tx1$ on Ethereum. It also checks various conditions, including whether it is the AMM pool that receives a token deposit from $tx1$ and the request is signed by Alice's secret key. If the conditions are met, the service calls a privileged function \texttt{returnToken} on the AMM pool. Figure~\ref{fig:mitiglost} presents our trustless lost-and-found protocol.

\subsection{Hardening Deployed AMM Services}

\noindent
{\bf Lost-and-found service off-chain}: We propose running a lost-and-found off-chain web service. This off-chain service monitors the on-chain state for profitability and collects extractable value ahead of actual attacks. To do so, the service takes an aggressive strategy by directly monitoring the vulnerable deposits (i.e., $P_1$, $P_3$, $P_4$) and withdrawing immediately upon discovery. For token interest $P_2$, the service monitors mempool for stealing transactions sent to the pools supporting token interests. Upon the discovery, the service sends transactions to frontrun the stealing transactions. 

In essence, this service performs the same functionality as thief attackers in discovering profitability opportunities on-chain, but it is benign in the sense that it stores the extracted value and allows victims to claim their tokens. Technically, given the value deposited by Account $V$, the service stores the value and allows $V$ or any other account with $ V$'s signature to claim the value.

\noindent
{\bf Fuzzing router smart contracts}: For the atomicity violations caused by buggy router contracts (i.e., $P_4$), one can mitigate the problem by developing more secure router smart contracts. Here, to ensure that the router calls deposit and withdrawal in all possible code paths, we fuzz the router smart contract using a fuzzing framework Echidna~\cite{DBLP:conf/issta/GriecoSCFG20}. Specifically, we develop a test oracle that defines swap atomicity and a smart contract rewriter to automatically insert the oracle to the target router smart contract. The test oracle records all the \texttt{transfer}/\texttt{transferFrom}/\texttt{swap} invocations and checks if there is a standalone invocation in the end of execution.   

\section{Related Work}
\label{sec:rw}

We survey the most relevant works and compare them against this one. Due to the space limit, we defer the extended related work to Appendix~\ref{appdx:rw}.

\noindent
{\bf DeFi attacks and BEV}: In DeFi, a primary class of attacks exploit Blockchain extractable value or BEV. BEV is the amount of value that can be extracted by reordering transactions. 
Torres, et al.~\cite{DBLP:conf/uss/TorresCS21} detect frontrunning attacks from Ethereum transactions by the attack signature being a pair of successful and failed transactions. Qin et al.~\cite{DBLP:journals/corr/abs-2101-05511} measure and characterize four BEV-exploiting attacks, including liquidation, sandwich attacks, arbitrage and transaction relay, on Ethereum. Wang, et al.~\cite{DBLP:journals/corr/abs-2105-02784} detect the instances of arbitrage on Uniswap-V2, by finding profitable cycles on the token-transfer graph. Zhou, et al.~\cite{DBLP:conf/sp/ZhouQCLG21} discover arbitrage opportunities by finding profitable cycles among token-token exchange rates in real time. Xia, et al.~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21} detect scam tokens listed on Uniswap V2 that impersonate other tokens to trick their traders; the attack signature is that the scam token's pool has a shorter-lived life span of transactions than the normal pools.

{\it This work's distinction to know BEV}: Arbitrage and sandwich attacks are two known patterns to extract BEV from AMM. In arbitrage, the profitable opportunities come from the difference in token exchange rates between AMM pools. In sandwich attacks, the profitable opportunities come from the imminent price changes caused by pending trades. 1) Both BEV attacks exploit or manipulate token prices. In both attacks, the attacker monitors certain conditions on the token prices to determine the timing of value extraction.
In this work, the ``extractable value'' stolen from the theft comes from the AMM design flaw that allows permissionless withdrawal. To extract the value, the attacker does not monitor token prices; instead, she monitors the presence of exploitable deposit (non-standard token deposit such as rebase) to determine when to extract the value.
2) In addition, in existing arbitrage and sandwich attacks, the attack success does not require breaking the atomicity of individual AMM operations. That is, a successful sandwich attack (or arbitrage attack) can be composed of a sequence of token swaps that are atomic. By contrast, the theft attacks studied in this work require breaking the atomicity of AMM operations.
Therefore, the theft attacks studied in this work are fundamentally different from the BEV-based attacks~\cite{DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2101-05511,DBLP:journals/corr/abs-2105-02784,DBLP:conf/sp/ZhouQCLG21}, due to their difference in causes and execution conditions. 

\noindent
{\bf Smart contract vulnerabilities and attacks}: Existing research has covered the automatic discovery of new smart-contract vulnerability~\cite{DBLP:conf/ccs/LuuCOSH16,DBLP:conf/uss/KruppR18} and detection of attack instances of known vulnerabilities~\cite{DBLP:conf/uss/ZhangZZL20,DBLP:conf/uss/ZhouYXCY020,DBLP:conf/uss/SuSDL0XL21,DBLP:conf/uss/0001L21}. These two lines of researches tackle generic program-level attacks such as reentrancy attacks and transaction ordering dependencies, which are not DeFi specific as in this work.

\section{Responsible Disclosure}
\label{sec:disclosure}

We have reported the discovered atomicity violations and the vulnerabilities to Uniswap's bug bounty program (\url{https://uniswap.org/bug-bounty}). The bugs have been confirmed. The bug-report detail is documented in the anonymized Google document~\cite{me:bugreport:defiant}. 

\section{Conclusion}
\label{sec:conclude}

This paper presents the first measurement study of atomicity violations and token theft attacks on popular AMMs on Ethereum. The study unearths more than $55$ thousand thefts and stolen tokens worth a total of $3.88$ million USD. It uncovers a range of previously unknown patterns of vulnerable deposits (e.g., token interest and supply adjustment), exposes real-world attackers' adaptive strategies to send malicious withdrawals, and reveals their systematic behavior in preparing, executing, and finalizing theft attacks. Finally, it presents mitigation schemes to design secure AMM protocols and to harden the deployed AMM services running immutable smart contracts.


==> text/old/v1_3_eval.tex <==

\section{Measurement Results}

\subsection{Single-chain Swaps: the Case of Uniswap}

\begin{figure}
\begin{center}
    \includegraphics[width=0.35\textwidth]{./expfigure/exp-uniswap1.eps}
    \caption{Uniswap TransferOut-TransferIn block difference distribution} \label{uniswap}
\end{center}
\end{figure}


We collect Uniswap's transactions from May 04, 2020 (i.e., Uniswap V2:factory's launch day) to July 08, 2021. With the method described in chapter~\ref{chap:2.1}, we explored the swap events violate the atomicity in $6627$ token pairs. We find $468$ swap transactions that cannot correspond to \textit{transfer} events. They satisfy P1 or P2. We further set $0\%$ amount deviation and $10$ block time deviation as the condition to classify matched or mis-matched TransferIn/Out. And we get $74$ P1 cases and $397$ P2 cases, all of the cases miss TransferIn. We count the time difference between TransferOut and TransferIn in P1 which shows the opportunity for the attacker to mount a frontrun attack(see figure ~\ref{uniswap}). $61$ out of $74$ P1 cases execute TransferIn and TransferOut in the same block while $13$ of them are in different blocks which lead to higher risk. The largest block difference reaches $10$ blocks which give the attacker $100$ seconds to arbitrage. After our analysis of the P2 instance, we found that the balance of token like aSUSD keeps changing which leads to the asynchronous between contract internally maintained balance and actual balance. Anyone can benefit from the feature that violates atomicity.


\subsection{Cross-chain Swaps}
\begin{figure}[!ht]
  \begin{center}
    \subfloat[Time interval T1-T2]{%
    \includegraphics[width=0.25\textwidth]{./expfigure/exp-wbtc2.eps}
    \label{wbtc2}
    }%
    \subfloat[Time interval T2-T3]{%
    \includegraphics[width=0.25\textwidth]{./expfigure/exp-wbtc1.eps}
    \label{wbtc1}
    }%
  \end{center}
  \caption{WTBC time distribution}
  \label{fig:complex}\vspace{-0.10in}
\end{figure}

\textbf{WBTC}: We summarize all the transactions from the deployment of \textit{WBTC: factory}: contract to July 08, 2020. We analyze a total of 99 cases. We verified that all the user’s requests and responses match each other by detecting each MintConfirmed event matches \textit{addRequest} event .  We report the time difference between two transactions in Fig.~\ref{wbtc1}. The result shows that in $49.5\%$ cases, WBTC server responses in $3$ hours after the user sends a request(i.e., T3-T2<$3$ hours). However, other cases show the server has a long response delay as much as $121$ hours. We also calculate the time difference between step1 and step2(e.g., T2-T1) for further research(Fig. ~\ref{wbtc2}), the figure shows that 57\% of users prefer sending requests in 4 hours after they deposit BTC on the server's wallet.


\begin{figure}[!ht]
  \begin{center}
    \subfloat[imBTC distribution in time interval T1-T3]{%
    \includegraphics[width=0.25\textwidth]{./expfigure/exp-imbtc.eps}
    \label{imbtc}
    }%
    \subfloat[tBTC distribution in time interval T1-T3]{%
    \includegraphics[width=0.25\textwidth]{./expfigure/exp-tbtc.eps}
    \label{tbtc}
    }%
  \end{center}
  \caption{Results of imBTC and tBTC}
\end{figure}

\textbf{imBTC}: We get the transaction history of imBTC token from Oct 25, 2019 to July 20, 2020. The number of records is 913. After analyzing with the method in chapter~\ref{chap:2.2}, we report the time difference distribution in interval T1-T3  in Figure ~\ref{imbtc}. The result shows that the delay of response is at least $4$ hours. $873$ out of $913$ cases complete the transaction in 4-6 hours. The largest response time for imBTC is $22$ hours.Compare to wBTC server, ImBTC transaction completion time is more concentrated and stable. However, the median time difference ($4.32$ hours) is longer than wbtc ($3.73$ hours). .

\textbf{tBTC}: We collected the transaction history data from May 17, 2020 to June 04, 2020 to display the information of T3-T1 for further research (see Figure ~\ref{tbtc}). The result shows $67\%$ of users send requests soon after they deposit bitcoin tokens ( $<5$ hours), others wait more than 5 hours, the median time for the complete transaction is $4.9$ hours . There is no advantage compared to WBTC and imBTC. The advantage of tBTC is the server will respond instantly after the user sends a request.

\begin{figure}  
\begin{center}
    \includegraphics[width=0.35\textwidth]{./expfigure/exp-binance1.eps}
    \caption{Binance distribution in time interval T2-T3} \label{Binance}
\end{center}
\end{figure}

\textbf{Binance}: We traverse the data from Feb 22, 2021 to June 15, 2021 in ethereum and binance network.We obtain 6194 matched pairs. Each pair includes 2 transactions. One is in Ethereum network with the following parameters {from: Address A1,to: Address B1, timestamp: t1, value: v1}. The other is in Binance network with the following parameters  {from: Address A2,to: Address B2,timestamp: t2,value: v2} where 1) Address A1=Address B2, 2) Address A2 and Address B2 belong to binance wallet set 3) absolute value of (T1-T2) less than $1$ hour. 4) v1=v2. So that we record the time difference distribution of T3-T2 (see Figure 4. The result shows $94.8$\% swap completed in 10 minutes. $9$ out of $6194$ cases take more than $50$ minutes. The median time difference is $29.3$ minutes which is more efficient compared to the bridge between BTC and Ethereum network.(Fig.~\ref{wbtc2})

\section{Conclusion}
This paper demonstrates several methods to measure atomicity over single-chain swaps and cross-chain swaps in blockchain networks. The result proposed evidence of violate atomicity in Uniswap history. At the same time, we measured several famous cross-chain swap bridges and discovered the risks when trading.

\clearpage


\begin{table}[!htbp] %force in current page, disable float.
\caption{Uniswap TransferOut-TransferIn block difference distribution}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c| }
  \hline
  Range of block delay & Number of cases  \\ \hline
  $0$ & 61 \\ \hline
  $1$ & 10 \\ \hline
  $2$ & 1 \\ \hline
  $3$ & 1 \\ \hline
  $>3$ & 1 \\ \hline
\end{tabularx}
}
\end{table}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Time difference of T2 and T3 in Binance bridge swap}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c| }
  \hline
  Time difference (minutes) & Number of cases  \\ \hline
  $[0,10)$ & 5873 \\ \hline
  $[10,20)$ & 219  \\ \hline
  $[20,30)$ & 39  \\ \hline
  $[30,40)$ & 33 \\ \hline
  $[40,50)$ & 21 \\ \hline
  $[50,60)$ & 9 \\ \hline
\end{tabularx}
}
\end{table}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Time difference of T2 and T1 in wbtc swap}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c| }
  \hline
  Time difference (hours) & Number of cases  \\ \hline
  $[0,1)$ & 59 \\ \hline
  $[1,2)$ & 15 \\ \hline
  $[2,3)$ & 3 \\ \hline
  $[3,4)$ & 8 \\ \hline
  $[4,5)$ & 1 \\ \hline
  $[5,6)$ & 0\\ \hline
  $[6,7)$ & 0\\ \hline
  $[7,8)$ & 1  \\ \hline
  $[8,12)$ & 1  \\ \hline
  $[12,24)$ & 7 \\ \hline
  $[24,infinite)$ & 9 \\ \hline
\end{tabularx}
}
\end{table}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Time difference of T3 and T2 in wBTC swap}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c| }
  \hline
  Time difference (hours) & Number of cases  \\ \hline
  $[0,1)$ & 11 \\ \hline
  $[1,2)$ & 17 \\ \hline
  $[2,3)$ & 22 \\ \hline
  $[3,4)$ & 7 \\ \hline
  $[4,5)$ & 3 \\ \hline
  $[5,6)$ & 7 \\ \hline
  $[6,7)$ & 5 \\ \hline
  $[7,8)$ & 3  \\ \hline
  $[8,12)$ & 8  \\ \hline
  $[12,24)$ & 9 \\ \hline
  $[24,infinite)$ & 7 \\ \hline
\end{tabularx}
}
\end{table}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Time difference of T3 and T1 in imBTC swap}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c| }
  \hline
  Time difference & Number of cases  \\ \hline
  $[0,4h)$ & 0 \\ \hline
  $[4h,4h10m)$ & 300 \\ \hline
  $[4h,4h30m)$ & 244 \\ \hline
  $[4h30m,5h)$ & 42 \\ \hline
  $[5h,6h)$ & 287 \\ \hline
  $[6h,infinite)$ & 40 \\ \hline
\end{tabularx}
}
\end{table}
\begin{table}[!htbp] %force in current page, disable float.
\caption{Time difference of T3 and T1 in tBTC swap}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c| }
  \hline
  Time difference & Number of cases  \\ \hline
  $[0,5h)$ & 95 \\ \hline
  $[5h,10h)$ & 26 \\ \hline
  $[10h,15h)$ & 0 \\ \hline
  $[15h,20h)$ & 14 \\ \hline
  $[20h,25h)$ & 7 \\ \hline
\end{tabularx}
}
\end{table}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Time difference of \texttt{xTransfer} and \texttt{reporttx} in Ethereum to EOS swap}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c| }
  \hline
  Time Difference (minutes) & Distribution ( * $100\%$)  \\ \hline
  $[0,2]$ & 1.06 \\ \hline
  $[2,3]$ & 19.34 \\ \hline
  $[3,4]$ & 35.13 \\ \hline
  $[4,5]$ & 24.84 \\ \hline
 $[5,6]$ & 11.59 \\ \hline
 $[6,10]$ & 6.1 \\ \hline
 $[10,60]$ & 0.74 \\ \hline
 $[60,600]$ & 0.82 \\ \hline
 $[600,1200]$ & 0.47 \\ \hline
\end{tabularx}
}
\end{table}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Time difference of transfer and reportTx in EOS to Ethereum swap}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c| }
  \hline
  Time Difference (minutes) & Distribution ( * $100\%$)  \\ \hline
  $[0,3]$ & 17.80 \\ \hline
  $[3,10]$ & 23.10 \\ \hline
  $[10,60]$ & 11.65 \\ \hline
  $[60,120]$ & 8.75 \\ \hline
 $[120,240]$ & 8.42 \\ \hline
 $[240,360]$ & 8.60 \\ \hline
 $[360,600]$ & 6.63 \\ \hline
 $[600,1200]$ & 5.71 \\ \hline
 $[1200,1440]$ & 4.96 \\ \hline
\end{tabularx}
}
\end{table}



==> text/old/v1_abstract.tex <==
Swapping crypto-assets is an essential business in DeFi and has been gaining traction on various blockchains today. The well functioning of swaps heavily relies on the atomicity property, that is, the swap is executed in an all-or-nothing manner without being interrupted or interleaved with other swaps. While a highly desirable feature by both DEX designers and asset owners, it is unclear how well real-world swap services on blockchains enforce the atomicity requirement.
				
This paper presents the first measurement study to uncover incidents violating atomicity. We systematically consider decentralized exchanges (DEX) on a single blockchain and the swaps across blockchains. For single-chain swaps, we measure Ethereum's most popular DEX, Uniswap-V2, and uncover two patterns in which atomicity can be violated. For cross-chain swaps, we measure the BancorX protocol in deployment between EOS and Ethereum. The results show interesting, previously unknown incidents that swaps end up executing a single transfer and the significant delay between two transfers of a swap (e.g., as long as 60 hours).


==> text/old/v1_paper.tex <==
\section{Measurement Methodology}
This section presents an abstract view of our measurement and analytical methods. Specifically, we consider as the input data a series of currency ``transfers'' that can be collected and reconstructed from public blockchains. We leave it to future sections to describe specific data collection methods on different blockchains. This section focuses on describing the data analytics on a database storing ``transfer'' records that detect and expose the incidents of atomic violations. 

\subsection{Data models}

{\bf Swaps}: A {\it swap} is to exchange the ownership of two assets/currencies between two trader accounts. A (normal) swap essentially consists of two {\it transfers}, each transferring one currency from a trader to another. 

Formally, given two accounts (blockchain addresses) $t_S$ and $t_R$, a transfer $tf$, denoted by $\langle{}t_S,t_R,c,v,b,d,txid\rangle{}$, sends value $v$ in currency $c$ from sender account $t_S$ to receiver account $t_R$. This transfer occurs on blockchain $b$ and is carried out by the transaction of hash $txid$. $d$ is the ``data'' field of the transaction, which includes information related to smart-contract function invocation. 

A (normal) swap is a pair of two transfers that can be ``matched''. Here, the matching conditions are defined on the two transfers' sender, receiver accounts and the equality of their value. That is, a swap $sp$ consists of two transfers $tf_1$ and $tf_2$, such that the following conditions are met.

\begin{eqnarray}
\begin{cases}
tf_1.t_S&=tf_2.t_R \\
tf_1.t_R&=tf_2.t_S
\end{cases}
\label{eqn:atomic:match}
\end{eqnarray}

A swap can be materialized on a single blockchain (i.e., $tf_1.b=tf_2.b$)  or multiple blockchains(i.e., $tf_1.b\neq{}tf_2.b$) . The former type of swap is carried out by a DEX on a single blockchain, the latter type of swap is carried out cross-chain protocols.


\begin{figure}
\centering
\includegraphics[width=0.325\textwidth]{figures/atomicity2.eps}
\caption{Swap atomicity and violation types (M, V1 and V2)}
\label{fig:atomicity}
\end{figure}

The exchange rate of the swap is defined as $r=\frac{tf_1.v}{tf_2.v}$, which can be determined differently on different platforms.

{\bf Atomicity and violations}: A swap is {\it atomic} if the two transfers meet the condition defined in Equations~\ref{eqn:atomic:match} and the timing difference of the two transfers is within a timeout threshold $tt$.

A swap is a {\it freerider} if it only has $tf_2$ but not a matching $tf_1$, that is, $\langle{}-,tf_2\rangle{}$. In other words, the account $tf_2.t_R$ receives value in $tf_2$, yet without paying anything (i.e., without $tf_1$). 

Relaxing the condition, a swap $\langle{}tf_1,tf_2\rangle{}$ is a {\it discount} if $tf_1.v/tf_2.v<r$ where $r$ is the market exchange rate between currencies $tf_1.c$ and $tf_2.c$. 

A swap is an {\it underwater} if it only has $tf_1$ but not a matching $tf_2$. In other words, the account $tf_1.t_S$ pays valuable in her own currency in transfer $tf_1$, yet without receiving anything (i.e., without $tf_2$). 

A swap $\langle{}tf_1,tf_2\rangle{}$ is a {\it overcharge} if $tf_1.v/tf_2.v>r$ where $r$ is the market exchange rate between currencies $tf_1.c$ and $tf_2.c$. 

Overall, we denote an atomic swap by $M$, a freeride or discount swap by violation type $V1$, and an underwater or overcharge swap by violation type $V2$. Figure~\ref{fig:atomicity} illustrates the relationship of swaps of different types. 

\subsection{Measurement Methodology}

Given the ``transfer'' database described above, we run data analysis to detect the incidents of atomicity violation. In principle, the data analysis is a self-join operation on the transfer data table: An inner join on the matching conditions of Equation~\ref{eqn:atomic:match} produces the results of atomic swaps. A left join produces both atomic swaps and violating swaps of type ``underwater.'' A right join produces both atomic swaps and violation swaps of type ``freeride.''

We apply the above method to analyze the actual cases of exchanges and blockchains, such as an AMM DEX on a single blockchain and pegged tokens across different blockchains. To do so, we use background knowledge to identify candidate transfer sets and narrow the search prior to joining. For most DEXs on a single blockchain, the smart contract addresses are known, and we can use the addresses to identify relevant transactions prior to joining. For cross-chain swaps, the addresses of custodian on at one blockchain are published, and the initial dataset can be similarly pruned.

However, in these real situations, the assumptions made in the ``idealistic'' analytical model presented in this section may not hold, such as cross-chain traders using different addresses on different blockchains and same-chain traders relying on unknown exchange rates; both falsify the matching conditions in Equation~\ref{eqn:atomic:match}. There are more similar challenges as introduced in \S~\ref{sec:intro}. We will describe our specific solutions in different exchanges in the next sections.

\section{Measurement Studies on DEX}
\subsection{Modeling DEX (On a Single Blockchain)}
\subsection{Measurement Method for Uniswap/AMM}
\begin{figure}[!ht]
\centering
\includegraphics[width=0.225\textwidth]{figures/protocol_uniswap.eps}
\caption{The Uniswap protocol}
\label{fig:protocol:uniswap}
\end{figure}

Uniswap, as a composable AMM, runs two types of smart contracts: A frontend ``router'' smart contract that exposes a collection of API functions to the end users and several backend smart contracts, each providing a liquidity pool for a pair of tokens. We focus on describing the backend ``pool'' smart contract. Minimally, a user interacts with a Uniswap ``liquidity pool'' smart contract to exchange tokens with its liquidity provider. For example, consider the exchange between token mToken and tToken, as shown in Figure~\ref{XXX}. In Step \ballnumber{1}, the user first sends a transaction to transfer mToken to the liquidity provider's account. Then in Step \ballnumber{2}, the user invokes the liquidity pool's \texttt{swap} function, which verifies the recipient of the user's deposit and prepares the transfer call in the next step (e.g., obtaining the exchange rate). In Step \ballnumber{3}, the liquidity pool transfers tToken to the user by calling the \texttt{transfer} function.

For measurement, we find the cases of atomic swaps and match the two transfer transactions. To do so, given the known smart contracts of Uniswap's liquidity pools, we first locate all transactions invoking these smart contracts' \texttt{swap} function. The swap function has an argument (``to'' as listed in XXX) which refers to the user's address. We then leverage this information to find a transaction that W1) is sent from the user (of the ``to'' address), W2) is sent to the mToken, and W3) transfers tokens to Uniswap's pair smart contract. If there are multiple matching transactions, we further check XXX?

function swap(uint amount0Out, uint amount1Out, address to, bytes calldata data);

The above method is able to identify the violation incident (V1): Given a \texttt{swap} invocation, it cannot find a \texttt{transfer} invocation to mToken that meets the above three conditions in the entire Ethereum transaction history. 

For V2, we first find all the transactions that invoke the \texttt{transfer} function in any token smart contracts that are registered in Uniswap and transfer tokens to the corresponding pair smart contracts. For each identified deposit transaction, suppose it corresponds to the pair smart contract say $P$. We then check the trace of swap calls received by $P$ and find the one matching the deposit function based on the three conditions (W1/W2/W3).

\subsection{Measurement Study on IDEX}
\begin{figure}[!ht]
\centering
\includegraphics[width=0.325\textwidth]{figures/protocol_idex.eps}
\caption{The IDEX protocol}
\label{fig:protocol:idex}
\end{figure}

\section{Measurement Studies on Cross-chain Swaps}
In this section, we describe the measurement study on cross-chain token swaps to uncover the case of atomicity violations. We first describe a general model of cross-chain swaps and how it is instantiated in actual swaps in practice. We then describe the methods specific to measuring different cross-chain swaps. 

\begin{figure}[!ht]
\centering
\includegraphics[width=0.275\textwidth]{figures/protocol_pegged.eps}
\caption{The general model of cross-chain swaps}
\label{fig:protocol:general}
\end{figure}

\subsection{Modelling Cross-chain Swaps}
\label{sec:model:crosschain}

In general, a cross-chain swap works among four parties. As shown in Figure~\ref{fig:protocol:general}, a {\it user} initially holds cryptocurrency or tokens, say A, on the {\it source blockchain}, and a {\it custodian} holds the pegged token B on the {\it destination blockchain}, which also supports smart contracts. It swaps the user's token A with the custodian's token B. To do so, the protocol generally runs in three steps: \ballnumber{1} The user sends a transaction to the source blockchain to transfer his token A to the custodian. \ballnumber{2} The custodian gets notified, through a communication channel, of the user's transaction. \ballnumber{3} The custodian sends a transaction to the destination blockchain to transfer a certain amount of token B to the user's account. 

Different actual cross-chain swaps instantiates the above model, notably for applications such as pegged tokens.
\subsection{Measurement Methods of wBTC}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.325\textwidth]{figures/protocol_pegged_wbtc.eps}
\caption{The WBTC protocol}
\label{fig:protocol:wbtc}
\end{figure}

WBTC is a popular pegged token on Ethereum that is backed by Bitcoin on a one-to-one rate. In WBTC, there is a smart contract on Ethereum (destination blockchain) called Token Factory. Step \ballnumber{2} consists of two substeps: The user first invokes the Factory's function \texttt{addRequest($btx$)} where $btx$ is the hash of the user's Bitcoin transaction. The custodian watching Ethereum's event stream gets notified of the invocation to \texttt{addRequest($btx$)} invokes the smart contract's function \texttt{requestConfirm($btx$)} which further verifies the Bitcoin deposit and mints the same amount of WBTC under the user's account. Note that function \texttt{addRequest($btx$)} sent by the user is necessary for the custodian to verify the Bitcoin deposit. Figure~\ref{fig:protocol:wbtc} shows the WBTC's protocol to mint a token on Ethereum.

To pair the collateral deposit and token mint in WBTC, we exploit the following fact: 1) The address of WBTC's Factory smart contract is publicly known , and 2) The Step \ballnumber{3}'s function \texttt{requestConfirm} contains the hash of Bitcoin deposit transaction. Specifically, to a deposit and token mint (i.e., measurement goal M0), we start by collecting the transactions calling WBTC's \texttt{requestConfirm}, then locate the corresponding Bitcoin transaction hashes, and finally verifies the inclusion of such transactions in the Bitcoin's blockchain. 

In WBTC, the type-V1 atomicity violation is materialized as the absence of a Bitcoin deposit in the presence of a WBTC mint. V1 is verified by the failure of observing Bitcoin deposit inclusion.  The type-V2 violation cannot be verified in our method XXX.  
\subsection{Measurement Methods of BSC Bridge}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.325\textwidth]{figures/protocol_pegged_bsc.eps}
\caption{The BSC Bridge protocol}
\label{fig:protocol:bsc}
\end{figure}


PeggedETH on Binance's Smart Chain (BSC) instantiates the model described in \S~\ref{sec:model:crosschain}. In Step \ballnumber{1}, the user transfers Ether to the custodian's Ethereum address. In Step \ballnumber{2}, the user sends RPC requests supported by the custodian's web service, namely \texttt{SwapCreateRequest}~\cite{XXX} that includes the Ethereum transaction hash and user account. The custodian will then check his Ether balance and if the balance increase is from the user. After varying the deposit is successfully included and finalized, the custodian sends a \texttt{transfer} call in Step \ballnumber{3} to give the user a certain amount of \texttt{PeggedETH} token. Figure~\ref{fig:protocol:bsc} depicts the BSC bridge's protocol to mint a PeggedETH token on Ethereum.

To reconstruct a swap and its pair of transfers (measurement goal M0), we exploit the fact that the user (re)uses the same address across Ethereum and BSC. That is, {\it the ``from'' address of Ethereum \texttt{transfer} in Step \ballnumber{1} equals the ``to'' address of BSC \texttt{transfer} in Step \ballnumber{3}.} 

Specifically, given the custodian's known address $C$ (obtained from the web), we first locate all the ``mint'' transactions $tx_1$'s on BSC that are sent from $C$, then obtain the users' address (reused on BSC and Ethereum) from $tx_1$s' receiver address, and finally find the deposit transactions $tx_2$s on Ethereum that are sent from the users. 

If there are multiple $tx_2$'es sent from the user, I filter that with same value and 1 hour time difference. If find 2 matched, I'll choose the one with shorter time difference

In the case of V1 and V2, our method can neither find the relevant transactions nor verify the existence… YYY
\subsection{Measurement Methods of BancorX}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.325\textwidth]{figures/protocol_pegged_bancorx.eps}
\caption{The BancorX protocol}
\label{fig:protocol:bancorx}
\end{figure}


BancorX works ``symmetrically'' between two blockchains both supporting smart contracts. Specifically, in Step \ballnumber{1}, the user makes the deposit on the ``source'' smart contract by calling its function \texttt{xTransfer}. In Step \ballnumber{2}, the custodian watches the ``source'' blockchain's transaction history and get notified of \texttt{xTransfer} sent in the previous step. In Step \ballnumber{3}, the custodian invokes the ``destination'' smart contract's function \texttt{reportTx} that mints the pegged token under the user's account. In practice, between a pair of blockchains, the protocol can be executed in two directions, say from Ethereum to EOS (as shown in in Figure~\ref{fig:protocol:bancorx}) and from EOS to Ethereum.

To match the deposit and mint in a swap operation (measurement goal M1), we exploit that the \texttt{reportTx} function's argument (i.e., $\_txId$~\cite{XXX}) refers to the hash of transaction invoking \texttt{xTransfer}, thus making it possible to link the two functions in a swap.
Specifically, a swap's two smart contracts' addresses are initially known~\cite{XXX:bancorxoneos}. We first locate the transactions invoking \texttt{xTransfer} on the source blockchain and the transactions invoking \texttt{reportTx} on the destination blockchain. We then join the two transaction sets by matching each destination transaction's $\_txId$ with a source transaction. This method can capture atomic swaps (M1) and atomicity violations V1 and V2.

\input{text/lst1.tex}

\input{text/v1_3_eval.tex}


==> text/old/v2_lst_sql.tex <==
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{HTML}{C42043}
\definecolor{backcolour}{HTML}{F2F2F2}
\definecolor{bookColor}{cmyk}{0,0,0,0.90}  
\color{bookColor}

\lstset{upquote=true}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{codepurple},
    numberstyle=\numberstyle,
    stringstyle=\color{blue},
    basicstyle=\footnotesize\ttfamily,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=10pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
}
\lstset{style=mystyle}

\newcommand\numberstyle[1]{%
    \footnotesize
    \color{codegray}%
    \ttfamily
    \ifnum#1<10 0\fi#1 |%
}

\begin{lstlisting}[ language=SQL,
                    deletekeywords={IDENTITY},
                    deletekeywords={[2]INT},
                    morekeywords={clustered},
                    framesep=8pt,
                    xleftmargin=40pt,
                    framexleftmargin=40pt,
                    frame=tb,
                    framerule=0pt, 
                    caption={SQL query for Uniswap-V2},
                    label=sql:uniswap,
                    float,floatplacement=H ]
-- Select the candidate set of swaps' transferIn 
SELECT * AS T1
FROM CallTable
WHERE callee_func IN ("transfer", "transferFrom") AND data.pay_to IN SET_POOL_UNISWAP

-- Select possible causes 
SELECT * AS T2
FROM CallTable
WHERE callee_func == ("swap", "addLiquidity")

-- Union the two sets to find swaps
T1 UNION T2
ORDER BY txID, call_seq
\end{lstlisting}


==> text/old/v2_paper_defi21.tex <==
\section{Introduction}

Swapping the ownership of crypto assets between accounts is an essential DeFi application. For instance, decentralized exchange or DEX supports the swap business on a single blockchain. DEX is among the most popular DeFi applications on deployed blockchains, notably Uniswap-V2 on Ethereum. For another instance, cross-chain swaps increases the liquidity of crypto assets and receive increasing popularity in practice.

Atomicity is the key correctness property of any swap, which states a swap should be executed in an all-or-nothing manner without being interleaved with other swaps. There are existing trustless protocols that guarantee atomicity by design, such as atomic cross-chain swaps (ACCS~\cite{DBLP:conf/podc/Herlihy18}). However, these protocols are slow and costly, causing multiple rounds of transactions, leaving them with limited adoption in practice. Practical swaps rely on either the faith of good behavior of trusted third-parties or the flawless program implementation of smart contracts. Take Uniswap-V2 as an example. Uniswap-V2's a composable automatic market maker (AMM), consisting of the frontend router layer and backend liquidity pools. It is designed to enforce swap atomicity at the router layer. In deployment, a router can be materialized on-chain as a smart contract (e.g., Uniswap-V2's default router smart contract or others implementing the 0x protocols) or off-chain operated by asset owners. With off-chain routers, the atomicity of swaps is left in the hands of trusted third-parties. Besides DEX, the deployed cross-chain swaps also widely include custodians in their protocol, who are trusted to send tokens on one blockchain when they receive tokens from the trader on another blockchain.

This work examines the atomicity assumption made in deployed crypto-asset swaps and conducts measurements to uncover the incidents of atomicity violation. We use the notions of atomicity anomalies~\cite{DBLP:conf/podc/Herlihy18} as the measurement goals. We propose data analysis on the traces of transactions and function calls in relevant blockchains. Our principled approach is to select from the traces the sets of candidate transfer calls in swaps and then to join the sets on certain conditions to discover swaps of atomicity and anomalies. Ideally, atomicity anomalies can be detected by outer joins when the function call traces are stored in relational databases. However, the anomaly detection is complicated in practice by a number of factors such as interference of other workflows than swaps in a DEX (e.g., Uniswap-V2's \texttt{addLiquidity}), special behavior of tokens (e.g., self-changing balances), et al. We propose two-phase data analysis on relational trace database, in which the first stage runs an SQL query to select and union candidate transfers, and the second stage runs a state machine that checks the validity or atomicity of the selected swaps.

We conduct two case studies using our general method above, respectively on Uniswap-V2 as a representative single-chain DEX and BancorX as a cross-chain swap service. We report the uncovered cases of atomicity anomalies and the delays between transfers in atomic swaps. The results show the anomalous swaps in Uniswap-V2 where two swaps can be interleaved in execution. This can be exploited to exchange rates during a swap and gain illicit profit. On BancorX, we discover atomicity anomalies in which the trader transfers her asset to the counterparty but never receives her exchanged asset (i.e., the \textsc{UNDERWATER} anomaly as defined in \S~\ref{sec:model}). We further inspect the uncovered cases that show the anomalies are caused by the insufficient confirmations from the custodians. The BancorX results also show the significant delay between two transfers of a swap (e.g., as long as 60 hours).

\section{Data Models and Definitions}
\label{sec:model}

\noindent
{\bf Transfer}: 
Given two accounts (blockchain addresses) $t_S$ and $t_R$, a transfer $tf$, denoted by $\langle{}t_S,t_R,c,v,b,d,txid\rangle{}$, sends value $v$ in currency $c$ from sender account $t_S$ to receiver account $t_R$. This transfer occurs on blockchain $b$ and is carried out by the transaction of hash $txid$. $d$ is the ``data'' field of the transaction, which includes information related to smart-contract function invocation. 

\noindent
{\bf Swap}: 
A (valid) swap consists of two transfers that can be ``matched'' on the conditions of their senders, receivers and the equality of their value. That is, a swap's two transfers $tf_1$ and $tf_2$ meet the following conditions:

\begin{eqnarray}
\begin{cases}
tf_1.t_S& \text{= } tf_2.t_R \\
tf_1.t_R&  \text{= } tf_2.t_S
\end{cases}
\label{eqn:atomic:match}
\end{eqnarray}

A swap can be materialized on a single blockchain (i.e., $tf_1.b==tf_2.b$)  or multiple blockchains(i.e., $tf_1.b\neq{}tf_2.b$) . The former type of swap is carried out by a DEX on a single blockchain, the latter type of swap is carried out cross-chain protocols.


\begin{figure}
\centering
\includegraphics[width=0.25\textwidth]{figures/atomicity.eps}
\caption{Swap atomicity and anomalies}
\label{fig:atomicity}
\end{figure}

The exchange rate of the swap is defined as $r$=$\frac{tf_1.v}{tf_2.v}$, which can be determined differently on different platforms.

\noindent
{\bf Atomicity and anomalies}: A swap is \textsc{ATOMIC} or \textsc{A} if the two transfers meet the condition defined in Equations~\ref{eqn:atomic:match} and the timing difference of the two transfers is within a timeout threshold $tt$.

A swap is a \textsc{FREERIDER} or \textsc{F} if it only has $tf_2$ but not a matching $tf_1$, that is, $\langle{}-,tf_2\rangle{}$. In other words, the account $tf_2.t_R$ receives value in $tf_2$, yet without paying anything (i.e., without $tf_1$). 

Relaxing the condition, a swap $\langle{}tf_1,tf_2\rangle{}$ is a \textsc{DISCOUNT} or \textsc{D} if $\frac{tf_1.v}{tf_2.v}<r$ where $r$ is the market exchange rate between currencies $tf_1.c$ and $tf_2.c$. 

A swap is an \textsc{UNDERWATER} or \textsc{U} if it only has $tf_1$ but not a matching $tf_2$. In other words, the account $tf_1.t_S$ pays valuable in her own currency in transfer $tf_1$, yet without receiving anything (i.e., without $tf_2$). 

A swap $\langle{}tf_1,tf_2\rangle{}$ is an \textsc{OVERCHARGE} or \textsc{O} if $\frac{tf_1.v}{tf_2.v}>r$ where $r$ is the market exchange rate between currencies $tf_1.c$ and $tf_2.c$. 

Figure~\ref{fig:atomicity} illustrates the relationship of swaps of different types. 

\section{General Transaction Analysis}
\label{sec:generalmethod}

\begin{figure}\centering
\includegraphics[width=0.325\textwidth]{figures/workflow.eps}
\caption{Workflow}\label{fig:workflow}\end{figure}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Trace database schema: Transaction and call tables.}
\label{tab:schema}\centering{
\begin{tabularx}{0.46\textwidth}{ |r<{\ttfamily}|X| }
  \hline
   Attributes & Meaning \\ \hline
   \multicolumn{2}{l}{TxTable}    \\ \hline
   msg.sender & The account sending this transaction\\ \hline
   txID & Transaction ID\\ \hline
   \multicolumn{2}{l}{CallTable}    \\ \hline
   caller & Caller account \\ \hline
   callee\_contract & Callee smart contract\\ \hline
   callee\_func& Callee function name\\ \hline
   data & Function-specific data, including argument list (ref. Table~\ref{tab:api})\\ \hline
   gas\_price & Gas price \\ \hline
   gas & Maximal Gas allowed to run this call \\ \hline
   call\_seq & Call sequence number \\ \hline
   txID & ID of the transaction triggering this call\\ \hline
\end{tabularx}
}
\end{table}

\input{text/lst1.tex}

To discover the cases of atomicity anomalies, we start from a ``trace'' database consisting of a transaction table and a function-call table. The data schema of these two tables is illustrated in Table~\ref{tab:schema}, where a transaction record has the primary key of \texttt{txID} and attributes including \texttt{msg.sender}, \texttt{gas\_price}, et al. A function-call record has \texttt{caller}, \texttt{callee\_contract}, \texttt{callee\_func}, \texttt{gas}, \texttt{txID}, et al. The specific meanings of these attributes are described in Table~\ref{tab:schema}. Particularly, the \texttt{data} attribute stores the argument list of the function call. The \texttt{call\_seq} is an attribute that indicates the function call's position in the call tree initiated by the same transaction. A caller's sequence number is the prefix of callee's sequence number. For instance, consider a statement in function \texttt{foo} calls function \texttt{bar}. Let's say the sequence number of function call to \texttt{foo} is `032'. Then the sequence number of the call to bar can be `0320'.

Our goal is to discover all incidents of atomicity anomalies from the trace database. The general idea is to {\it select from the CallTable the two candidate sets, respectively for the first transfer and second transfer in a swap, and then joins these two sets before checking the swaps' validity.} 
Materializing this idea on different underling exchanges, we obtain a data analytical workflow that consists of concrete SQL queries and state-machine checking logic, as in Figure~\ref{fig:workflow}.

\section{Case study: Uniswap-V2}
\subsection{Approach}

\begin{figure*}[htbp!]
  \begin{center}
    \subfloat[Uniswap-V2 protocol for swapping tokens]{%
\includegraphics[width=0.4\textwidth]{figures/protocol_uniswap.eps}
      \label{fig:uniswap:protocol}%
    }%
    \hspace{0.3in}%
    \subfloat[Trace database]{%
\includegraphics[width=0.1\textwidth]{figures/protocol_uniswap2.eps}
      \label{fig:uniswap:db}%
    }%
    \hspace{0.35in}%
    \subfloat[Automata checking atomicity (of single-tx swaps).]{%
\includegraphics[width=0.3\textwidth]{figures/automata.eps}
      \label{fig:uniswap:check}%
    }%
  \end{center}%\vspace{-0.15in}
  \caption{Modeling Uniswap-V2: The protocol, trace database and atomicity-checking automata.}\label{fig:uniswap}\vspace{-0.10in}
\end{figure*}

\input{text/lst_sql.tex}

\noindent
{\bf Preliminary of Uniswap-V2}: Uniswap-V2, as a composable AMM, runs two types of smart contracts: A frontend ``router'' smart contract that exposes a collection of user-friendly APIs and a series of backend smart contracts, each providing a liquidity pool for a pair of tokens. 

The key functionality of Uniswap-V2 is swapping the ownership of two tokens between a trader and a Uniswap pool. Figure~\ref{fig:uniswap:protocol} illustrates an example function-call graph in which a trader exchanges her \texttt{mToken} with Uniswap's pool for \texttt{tToken}. The process involves two transactions. In transaction \ballnumber{1}, the trader calls the \texttt{mToken} smart contract to \texttt{approve} Uniswap-V2's router smart contract spending her account. Then, in transaction \ballnumber{2}, the trader calls the Router's function \texttt{wrappedSwap}, which runs a series of internal calls, including \texttt{transferFrom} (\ballnumber{21}), \texttt{swap} (\ballnumber{22}), \texttt{getBalance} (\ballnumber{221}), and \texttt{transfer} (\ballnumber{222}), as shown in the figure.

Another functionality in Uniswap-V2 (not shown in Figure~\ref{fig:uniswap:protocol}) is allowing traders to make deposit into the liquidity pool. Given a pool, the trader deposit the two supported tokens at their current ratio and receive a certain amount of LP tokens in return. For instance, the trader can call \texttt{mToken}'s \texttt{transfer} and \texttt{tToken}'s \texttt{transfer}, at certain ratio, before calling Uniswap-V2's router contract's \texttt{addLiquidity} function.


\noindent
{\bf Design challenges}: Recall that finding swaps of atomicity and anomalies entails identifying the set of transferIn and transferOut events. On Uniswap-V2, a naive approach of finding transferIn is to select the \texttt{transfer} or \texttt{transferFrom} calls whose receivers are one of Uniswap-V2's liquidity pools.
However, in Uniswap-V2, such a \texttt{transfer} call is possible not only in a \texttt{swapToken} workflow but also in a \texttt{addLiquidity} workflow.
Identifying \texttt{transferFrom} calls without knowing their causes can lead to false positives. For instance, a \texttt{transfer} call paying a liquidity pool in a valid \texttt{addLiquidity} workflow can be mistaken to be a \texttt{transfer} call in an invalid \texttt{swapToken} workflow exhibiting the \textsc{UNDERWATER} anomaly.

To solve the problem, our strategy is to select the \texttt{transfer} calls in both \texttt{swapToken} and \texttt{addLiquidity} workflows during the SQL query and to distinguish the two cases using state-machine checks. To do so, our SQL query needs to capture the calls of function \texttt{addLiquidity}. 

\ignore{
a naive approach of finding transferOut is to select the \texttt{transfer} calls sent from one of Uniswap-V2's liquidity pools and sent to the pools' supported token. However, in Uniswap-V2, \texttt{transfer} calls sent by a liquidity pool can not only be in a \texttt{swapToken} protocol but also in a \texttt{addLiquidity} protocol, leading to false positives by the naive approach. To overcome the challenge, we instead use the calls to a pool's \texttt{swap} function to identify transferOut.

--To find atomicity anomalies, one can follow the SQL query ``template'' described in \S~\ref{XX} by first finding the candidates of transferIn and those of transferOut before joining the sets. To find the transferIn (transferOut), the naive approach is to select the transfers whose senders (receivers) are one of the Uniswap-V2's liquidity pools. This approach works well, if the DEX only supports one function of \texttt{swap}, and all the transfers issued to the DEX are relevant to \texttt{swap}.

However, Uniswap-V2's \texttt{addLiquidity} workflow also involves sending \texttt{transfer} calls to a liquidity pool, which confuses the naive approach. For instance, such a \texttt{transfer} call can be part of the \texttt{swap} protocol as in Figure~\ref{XX} or equally likely be part of the \texttt{addLiquidity} protocol. Without attributing a  \texttt{transfer} call to the right protocol can result failure of detecting \texttt{swap}s and/or introduce false positives
}

\noindent
{\bf Proposed trace analytics}: The overall analytics consists of three stages, an SQL query to prepare a table of candidate call records, an automata to find swaps executed in single transactions and to check their atomicity, and an automata to do the same for multi-transaction swaps.

{\it 1. SQL query}: 
Our SQL query for Uniswap-V2 is in Listing~\ref{sql:uniswap}, where intermediary result \texttt{T1} stores the candidate set of swaps' transferIn events by directly selecting the \texttt{transfer} calls that could be matched to a \texttt{swapToken} workflow or a \texttt{addLiquidity} workflow. Intermediary result \texttt{T2} stores the candidate set of calls to a target pool's \texttt{swap}s and \texttt{addLiquidity}s. The third query union the two intermediate results ordered first by transaction ID and then by call sequence number.

{\it 2. Automata for single-tx swaps}: 
The SQL query result is then fed into an automata finding swaps and checking their atomicity. The automata for single-transaction swaps is described in Figure~\ref{fig:uniswap:check}. Specifically, the SQL query result is a table of calls of three functions, \texttt{swap}, \texttt{addLiquidity}, and \texttt{transfer} (or \texttt{transferFrom}). These call records are ordered by transaction ID and then by their call sequence numbers. The automata in Figure~\ref{fig:uniswap:check} combines the state machines of both \texttt{wf\_swapToken} and \texttt{wf\_addLiquidity} workflows, where $tf_X$ refers to a \texttt{transfer} call that pays to a target liquidity pool.
Only when the automata ends up in the green state, no error is thrown. Particularly, State $2$/$4$/$6$ may refer to the atomicity anomaly \textsc{U}/\textsc{F}/\textsc{I}. \textsc{I} means the two swaps are executed interleaved, such as swap1.transferIn, swap2.transferIn, swap2.transferOut, and swap1.transferOut.

{\it 3. Automata for multi-tx swaps}: The single-transaction automata find valid \texttt{swaps} (i.e., atomic swaps) and \texttt{addLiquidity} workflows and remove them from the table. After that, we run another automata to check the validity of multi-transaction swaps.

This method can capture atomic swaps (\textsc{A}) and anomalies (including \textsc{U}, \textsc{F}, \textsc{O}, and \textsc{D}).

%YYY

\noindent
{\bf Example}: Consider the example in Figure~\ref{fig:uniswap:protocol} where a trader swaps her \texttt{mToken}s with Uniswap-V2 for \texttt{tToken}s. The trace database stores two transactions and six calls as in Figure~\ref{fig:uniswap:db}. Running the SQL query (Listing~\ref{sql:uniswap}) on this database results in intermediary table $T1$ containing \ballnumber{21} and table $T2$ containing \ballnumber{22}. Table $T3$ contains the union-ed result $\{\ballnumber{21}, \ballnumber{22}\}$, which passes the atomicity check of single-transaction swaps.

\ignore{
YYY: Correctness analysis:

For anomalies, we first find all the transactions that invoke the \texttt{transfer} function in any token smart contracts that are registered in Uniswap and transfer tokens to the corresponding pair smart contracts. For each identified deposit transaction, suppose it corresponds to the pair smart contract say $P$. We then check the trace of swap calls received by $P$ and find the one matching the deposit function based on the three conditions (W1/W2/W3).
}

\subsection{Results}

\input{text/eval_uniswap.tex}

\input{text/case_bancorx.tex}

\section{Conclusion}
This paper presents a measurement study to uncover the atomicity anomalies in deployed DEX and cross-chain swaps.


==> text/old/v3_intro.tex <==
\section{Introduction}

Recent years witness the rise and continued success of blockchains and their applications, enjoying large-scale real-world usage in domains like Decentralized Finance or DeFi. A foundational and essential DeFi function is Decentralized Exchange or DEX, which allows traders to swap their asset from one token to another. 
One of the most used types of DEX is an automatic market maker or AMM. For instance, the Uniswap is an AMM protocol that dominates more than $90\%$ of DEX market on Ethereum and attracts a total of $149$ million transactions as of Jan. 2022~\cite{me:etherscan:topdex}. In AMM, the trader sends value in one token to the AMM's liquidity-pool account who maintains token reserves and sends back the same value in another token to the owner.

Of ultimate importance to its customers is the DEX's security against the token-stealing attack, in which a malicious account can extract value and gain illicit profit from the tokens intended to be received by the original trader. To prevent illicit value extraction, swap atomicity is essential, that is, the two transfer operations in a swap should be executed in an all-or-nothing fashion. An anomalous swap violating the atomicity could present extractable value to attackers. For instance, an attacker observing anomalous swap whose execution gets interrupted in the middle can extract value from the pool running the interrupted state where one token is deposited and the other token is not withdrawn yet.

While the existing literature has examined DEX security against arbitrage~\cite{DBLP:journals/corr/abs-2103-02228}, front-running and scam tokens~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21}, these attacks do not necessarily violate the atomicity of individual swaps. It is an open research problem whether the theft-by-violating-atomicity attacks do exist and whether there are criminal ecosystems systematically operating these attacks?

This work detects swap anomalies and theft attacks by analyzing the transaction traces on today's dominating DEXs on Ethereum. Specifically, we focus on the four most popular AMM DEXs, that is, Uniswap-V2, Uniswap-V3, Sushiswap, and Pancakeswap. The former three account for more than $90\%$ DEX market share on the Ethereum mainnet all time, and the last one is the most popular DEX on Binance Smart Chain, an Ethereum forked network. For each DEX, we analyze its transaction trace to answer the following research questions: {\bf RQ1) Anomaly detection}: Whether there are anomalous swaps that violate atomicity definition? {\bf RQ2) Attack detection}: From the identified swap anomalies, whether there are attacks extracting illicit value from these anomalous swaps? Note that not every anomalous swap has to be an attack (e.g., anomalous swap can be caused by a pool charging high fees, which is not an attack). {\bf RQ3) Attacker behavior}: What are the identified attackers' behavior, in setting up the attacks, strategies to trigger the attacks, transferring stolen assets after attacks, etc? Together, we aim to detect value thefts on DEX and uncover the underground criminal ecosystem that systematically extract and harvest illicit profit from the anomalous swaps.

{\bf Proposed methods}: We propose an end-to-end trace analytics pipeline to systematically tackles the above three research questions. In the first step, we detect anomalies by joining records of transfer operations across transactions to find mismatches as anomalies. In particular, Uniswap-V2 support a swap across multiple transactions, and joining multiple transactions pose efficiency challenges. We propose an efficient linear join algorithm by leveraging the invariants in Uniswap-V2 program.

In the second step, we detect attack instances out of the swap anomalies identified from the previous step. A stealing attack is an anomalous swap that occurs between an attacker account and victim trader. It excludes the non-attack cases of swap anomalies such as swaps charged with high fees and swaps that occur between two accounts controlled by the same physical user off-chain. To detect attacks, we manually inspect the trace to identify several victim patterns that create profitable opportunities and analyze the attacker's transactions, to uncover their intents. 

---

\noindent
{\bf Method: Trace analytics}:
Our proposed approach is an end-to-end semi-automated data-analytical pipeline, starting from the raw Ethereum data (events and transactions). The pipeline consists of three essential components: anomaly detection, attack detection and characterization, and cause analysis. 

To detect swap anomalies, we construct DEX-relevant data records from the Ethereum raw data and join the records to find mismatches and anomalous swaps. 

An actual attack requires an anomalous swap to occur between two distinct  real-world entities (i.e. an attacker and victim). This is essentially to detect the real-world linkage between two Ethereum accounts which, however, is hidden in the blackbox off-chain states and is difficult to detect. To tackle the challenge, we propose to characterize involved accounts' behavior within and beyond the anomalous swaps. We propose several heuristic-based attack signatures and detect attacks by matching account behavior to at least two signatures. We additionally collect the attack ground truth through online user complaints and validate the detection method.

We collect the trace data of four major Uniswap-based DEX'es (aforementioned) and run our trace analysis pipeline. Our results are two-fold: 1) swap anomalies and causes, 2) attack instances, 3) attacker behavior and ecosystem. In addition, we present the four common causes of the swap anomalies.

\noindent
{\bf Findings: Swap anomalies and causes}
We find anomalous swaps worth more than 3XXX million USD on Uniswap-V2. These swap anomalies either run transfers in two separate transactions (Type-II swap) or are a standalone transfer in a dedicated transaction that does not match any other transaction (Type-III swap). Besides the normal causes such as high swap fees, our findings reveal some unexpected cases of atomicity violation: 

1) Many standalone swaps (Type-III) are caused by non-standard token behavior: That is, the DEX smart contract interacts with tokens via standard functions (e.g., in ERC20) but makes implicit assumptions on non-standard token behavior, which can be false. For instance, we found 1.26 million USD worth of Type-III swaps allow freeride and are caused by \texttt{rebase}, a non-standard but common token operation through which the token issuer updates the balance of all token holders to deal with real-world needs such as inflation. Rebase invalidates DEX's assumption that any balance updates of DEX's account is due to some in-progress swap. There are other non-standard token operations such as interest, airdrop, etc. that cause Type-III swap anomalies. 

2) Buggy DEX smart contracts that, in some code path (e.g., due to mishandling exceptions), violates swap atomicity or sets erroneous exchange value. We found there are 0.205 million USD swaps on Uniswap V2 and XXX USD worth of swaps on Uniswap V3 are due to this cause.

3) API misuse, where a Uniswap-V3 trader uses Uniswap-V2 API/workflow, which results in Type-IIXXX swap anomalies on Uniswap-V3.

\noindent
{\bf Attack detection and ecosystems}: 
Based on the swap anomalies, we detect XXX attack instances, accumulating a total of XXX USD worth of illicit money flow.

---

Contribution:

\noindent{\bf Findings}: We discover a total of three million USD worth of swaps that violate atomicity, by measuring four popular Uniswap services on Ethereum and BSC. 

We identify and characterize the attackers and victims involved in these anomalous swap activities to shed light on the underground ecosystem that strategically exploits atomicity violation to gain illicit profit.

We analyze the causes of swap anomalies, including non-standard token operations in rebase/interest and erroneous exception handling in router smart contracts. We design effective attacks by exploiting the different causes.

\noindent{\bf Discovery technology}: We propose an end-to-end analytical pipeline to detect attacks in Uniswap transaction traces. Specifically, we propose an efficient join algorithm to discover atomicity, and several heuristics/indicators to automatically detect attackers/victims from anomalous swaps.

\noindent{\bf Mitigation strategies}: For partly errors, we build a fuzzer with a test oracle to automate the testing of the router smart contracts to develop.




==> text/old/v3_paper3.tex <==
\section{Background}

\noindent
{\bf Preliminary: Ethereum}: Ethereum supports two types of addresses: an externally owned account (EOA), which is an Ether owner's public key, and a contract address, which is the memory address where the smart contract is deployed on individual miner nodes. An Ethereum transaction binds a sender's address to a receiver's address.

\noindent
{\bf Preliminary: Uniswap and DEXs}:
Uniswap is a decentralized exchange (DEX) protocol designed based on automated market maker (AMM). 
A decentralized exchange or DEX allows for a trader EOA to swap her token for another token. Uniswap is the dominant DEX protocol on Ethereum and is designed based on automated market maker (AMM). An AMM maintains token reserves in a so-called liquidity pool; liquidity providers, who are token owners, deposit their tokens to fill up the reserves, and the pool uses the current reserves to calculate token exchange rates, on demand, to serve swaps.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.4\textwidth]{figures/uniswap-layers.eps}
\end{center}
\caption{Uniswap system and smart contracts at three layers.}
\label{fig:uniswap:layers}
\end{figure}

\begin{table}[!htbp] %force in current page, disable float.
\centering{\small
\begin{tabularx}{0.5\textwidth}{ |l|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
Layer & Functions \\ \hline
Liquidity 
& $swap(amountOut, to)$ \\ \cline{2-2}
pool~\cite{me:uniswapv2:pool}
& $getReserves()$ \\ \cline{2-2}
& $addLiquidity(min\_liquidity, max\_tokens,\dots)$ \\ \hline
ERC20~\cite{me:erc20:api}
& $transfer(address recipient, uint256 amount)$ \\ \cline{2-2}
token & $balanceOf(address account)$ \\ \hline
\end{tabularx}
}
\caption{Uniswap V2's liquidity pools' API}
\label{tab:uniswapv2:api}
\end{table}

A Uniswap-based DEX is architectured in three layers of smart contracts, as shown in Figure~\ref{fig:uniswap:layers}: 
The central layer is the liquidity pool which stores the provider's tokens and protect them in the events of swap. The liquidity pool issues token transfers to the underlying token layer. The liquidity pool serves different DeFi smart contracts in the application on top. The primary application is the router smart contracts for DEX, which, trusted by trader EOAs, coordinates the execution of swaps. Here, we mainly consider Uniswap's Version 2 protocol, which is adopted in major DEXs on Ethereum, including UniswapV2, Sushiswap and Pancakeswap. 
%We discuss Uniswap's Version 3 protocol in Appendix~\ref{appdx:uniswapv3YYY}.
Uniswap Version 2's API functions are presented in Table~\ref{tab:uniswapv2:api}. 

Specifically, Uniswap supports two essential workflows: swap and addLiquidity. Consider a pool of two tokens $T0$ and $T1$. In swap, the trader EOA sends the request to the router which coordinates the issuance of the two transfer calls, that is, the router calls token $T0$ to transfer in and calls pool's swapV2 or swapV3 function to transfer out token $T1$. 

In the addLiquidity workflow, a liquidity provider EOA deposits the two tokens $T0$ and $T1$ at a certain rate, and receives a deposit certificate (called LP token). Note that in addLiquidity workflow, there are transfer function calls to tokens $T0$ and $T1$.

\noindent
{\bf Risky swaps and specification}: In general, a (normal) swap should consist of two token transfers, one transfer of token $T0$ from the trader to the pool and the other transfer of token $T1$ from the pool to the trader. Mapping the two transfers to transactions result in different swap types: 

\begin{itemize}
\item
Type-I swap (atomic): In a Type-I swap, the two token transfers occur in the same blockchain transaction, and their value matches w.r.t. the current exchange rate. We call this type of swap an atomic swap. 
\item
Type-II swap (risky): In a Type-II swap, the two token transfers occur in separate blockchain transactions. Their value matches w.r.t. the current exchange rate. 
\item
Type-III swap (risky): In a Type-III swap, there is only one standalone token transfer observed, that is, the pool transfers out token $T1$ to a trader without receiving explicit transfer-in of token $T0$. 
\end{itemize}


\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/anomalies.eps}
\end{center}
\caption{Swaps of three types: Type II and III are risky swaps.}
\label{fig:swaps}
\end{figure}


Type-I swap runs the two transfers atomically in one transaction and is unlikely to constitute a token theft. Type-II and Type-III swaps are risky and could imply theft/attacks (as defined next). Specifically, in the Type-II swap, a malicious trader EOA could try to extract the value in the pool after the transaction to send the first transfer and before the transaction that carries out the second transfer. In the Type-III swap, it is abnormal for the pool to send value to a potentially malicious trader without receiving their deposit token.

\noindent
{\bf Threat model}: The primary threat in this work is DEX-value theft among trader EOAs. A victim is a trader EOA who has deposited the token to the pool but is unable to withdraw the other token from the pool. An attacker is an EOA who aims at extracting value from the liquidity pool interacting with a victim trader. The attacker's capability is to monitor certain conditions on the DEX states in real-time, and upon the satisfaction of the conditions, send crafted transactions to the DEX to extract the value and claim it illicitly. 

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/workflow5.eps}
\end{center}
\caption{Workflow of data analytics to detect risky swaps and attacks, as well as to analyze attackers'/victims' behavior.}
\label{fig:workflow:overall}
\end{figure*}

\noindent
{\bf System overview}: Figure~\ref{fig:workflow:overall} shows the overall data-analytics pipeline. The input data is more than $43$ million transactions with their event log crawled from etherscan.io, internal call sequences crawled from Google BigQuery services~\cite{XXX}. The pipeline consists of three stages: 1) Detecting risky swaps, which joins and matchmakers token transfers to detect the risky swaps as defined above, 2) Discovering token-theft attacks, which characterizes the behavior of accounts involved in risky swaps against proposed attack patterns, and 3) Uncovering on-chain crimes, which expose the attacker strategies, criminal infrastructures and ecosystems. 

These three steps are described in \S~\ref{sec:detectriskyswap}, \S~\ref{sec:attack}, and \S~\ref{sec:behavior} in the rest of this paper.

\section{Detecting Risky Transactions}
\label{sec:detectriskyswap}

\ignore{
\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.35\textwidth]{figures/workflow4.eps}
\end{center}
\caption{Overall data-analytical workflow}
\label{fig:workflow}
\end{figure}
}

To detect risky swaps, we first prepare raw blockchain data (e.g., events and transactions) into DEX specific data records, and then match-make data records to find risky swaps.

\subsection{Data format}
\label{sec:model}

\noindent
{\bf Transfer}: In a transfer operation $tf=\langle{}sender,receiver,token,value,txID\rangle{}$, account $sender$ transfers $value$ in $token$ to account $receiver$ in a transaction of $txID$. The transfer call can be internal or external, where an internal transfer call is issued by a smart contract and an external call is issued by an EOA (external owner account).  

{\bf Swap}: 
A (normal) swap occurs between two accounts where account Alice transfers value to Bob in one token, and Bob transfers back the same value in another token to Alice. For the sake of simplicity, we consider the case of a swap of two transfers. 

A swap is atomic, if two transfers, say $deposit$ and $withdrawal$, match in sender/receiver and value. Specifically, 

\begin{eqnarray}
& \begin{cases}
deposit.sender &\text{= } withdrawal.receiver \\
deposit.receiver &\text{= } withdrawal.sender 
\label{eqn:atomic:tfmatch}
\end{cases} & \\
& deposit.value * rate \text{= } withdrawal.value &
\label{eqn:atomic:valmatch}
\end{eqnarray}

Note that $rate$ is the exchange rate between $deposit.token$ and $withdrawal.token$.


\subsection{Data Preparation}

The goal here is to prepare the raw blockchain data into the $deposit$-and-$withdrawal$ data schema used in Swap specification in \S~\ref{sec:model}. The raw blockchain data includes smart-contract events and function calls. We specifically select relevant information to Uniswap DEX.
Suppose the target is a liquidity pool and its two associated tokens (e.g., $tokenIn$ and $tokenOut$ as in Figure~\ref{fig:uniswap2}).
To reconstruct candidate the $deposit$ records, we select all the calls that invoke one of the two tokens' transfer/transferFrom/mint functions and that transfer tokens to the pool's account. A reconstructed record is $deposit(valIn, txID)$. 

To reconstruct candidate $withdrawal$ records, we select the calls to the pool's function \texttt{swapCall}/\texttt{addLiquidity}. We also collect the events emitted by the pool. In particular, the Uniswap pool's events contain the mapping between $valIn$ and $ valOut$, so that it can reconstruct records $withdraw(valIn,valOut,txID)$. 

Here, we include $addLiquidity$ as a $withdrawal$ candidate, because otherwise it could introduce false positives in our matchmaking step. 
Specifically, recall Figure~\ref{fig:uniswap2:addliquidity} where the \texttt{addLiquidity} workflow includes token transfers to the pool. 
Thus, a transfer call to TokenIn can be part of an \texttt{addLiquidity} workflow, and without distinguishing it to the case that it belongs to the \texttt{swap} workflow, the match-making step may mis-classify it as an underwater swap.

In summary, the data preparation produces two sets of data records. The first set contains the data records for $deposit$ candidates including the selected function calls to transfer, transferFrom and mint, as described above. The second set stores the $withdrawal$ candidates,  including the calls to functions swap and addLiquidity.

\subsection{Match-making Algorithm}
\label{sec:mmalgo}

\noindent{\bf Design goal \& design space}: The goal is to join the two traces in order to find the risky swaps that violate atomicity. On the one hand, as one withdrawal candidate (e.g., a swap) can match an arbitrary number of deposit candidates, in theory, the join operation should be done on the power-sets of deposit/withdrawal traces, which is clearly unscalable — for instance, the power-set of a $n$-record set has $2^n$ elements. On the other hand, if any approximation is applied to design more efficient join algorithm, one does not want to introduce false-positive risky swaps, that is, the artifacts that mis-detected by the join algorithm and that can be avoided in a more precise join algorithm. 

Our algorithm design leverages a key invariant we observe in Uniswap's smart contract to save the search complexity without producing false positives. Specifically, Uniswap's liquidity pool smart contract runs in a single thread, and a swap/addLiquidity, say $C$, must only match any transfers that occur before $C$ and after $C$'s predecessor call to swap or addLiquidity. This invariant greatly saves the search space of match and allows to linearly merge the two traces with entries ordered by time.

\lstset{style=mystyle}
\begin{lstlisting}[caption=Psuedocode to find mismatch,
                   linerange={1-30},
                   firstnumber=1,
                   deletekeywords={[2]INT},
                   morekeywords={clustered},
                   framesep=2pt,
                   xleftmargin=5pt,
                   framexleftmargin=5pt,
                   frame=tb,
                   framerule=0pt, 
                   label=code:findmismatch,
                   float,floatplacement=H
                   ]
//deposits and swapOrAddL are both ordered by time
def findMismatch(Record[] deposits, Record[] withdrawals):
    for joinedpair in joinByTxId(deposits, withdrawals):
        removeMatch(deposits, withdrawals, joinedpair.i1, joinedpair.i2, joinedpair.j1, joinedpair.j2);
    for joinedpair in joinByTemporalSimilarity(deposits, withdrawals):
        removeMatch(deposits, withdrawals, joinedpair.i1, joinedpair.i2, joinedpair.j1, joinedpair.j2);
   
def removeMatch(Record[] deposits, Record[] withdrawals, int i1, int i2, int j1, int j2){
    for s in powerset(deposits[i1 ... i2]):
        for t in powerset(withdrawals[j1 ... j2]):   
        if sumValue(s) ==  sumValue(t):
            deposits.markRemoval(s); 
            withdrawals.markRemoval(t); 
            return;
\end{lstlisting}

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.325\textwidth]{figures/automata3.eps}
\end{center}
\caption{Matchmaking algorithm in two steps that produces the Type-II and Type-III patterns that violate swap atomicity.}
\label{fig:automata}
\end{figure}

\noindent{\bf The algorithm}:
The proposed algorithm in Listing~\ref{code:findmismatch} takes as input the traces of deposit and withdrawal records and produces as output the risky swaps it finds. The algorithm internally runs in two rounds. In the first round, it equi-joins the deposit records with withdrawal records based on their transaction IDs. In each joined tuple, which is a set of deposit records and withdrawal records in the same transaction, it match the deposit and withdrawal records. In the removeMatch function, it finds a group of deposit records that match a group of withdrawal records in value. Specifically, if the deposit record has the same value with a withdrawal record in the same transaction, it constitutes a normal swap or addLiquidity operation, and the two records are removed from the two traces. If the value mismatches. it merges the two records into one, that is, the one with larger value. For instance, if a transfer of value 5 and a swap of value 8 are in the same transaction, it replaces the two records in the dataset with a merged swap record of value 8-5=3.

The second round runs a similar join-then-matchmaking process with the first round. The only difference is the join condition is temporal similarity, that is, a record withdrawal[i] joins deposit records that occur before withdrawal[i] and after withdrawal[i-1] (assuming deposit and withdrawal records are ordered in time). After the joined pair is produced, it runs the same match-making function and remove the matched cases.

After these rounds, what's left in the table are the mismatches.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.3\textwidth]{figures/join_problem2.eps}
\caption{Example on joining \texttt{swapEvent} and \texttt{deposit} records}
\label{fig:joinproblem}
\end{figure}

{\it An example}: In Figure~\ref{fig:joinproblem} shows two example traces of deposit and withdrawal records. The two traces are aligned and sorted by time. Assume each record is handled by a distinct transaction. The figure shows that two matched cases (in green). The first transfer tf1 is a standalone deposit (i.e., underwater) and the second swap is a standalone withdrawal (i.e., freeride). In the red shade is a pair of deposit and withdrawal whose value does not match (a discount).

\subsection{Results}

\begin{table*}[!htbp] %force in current page, disable float.
\caption{Risky swaps on Uniswap-based DEXs}
\label{tab:1}\centering{\footnotesize
\begin{tabularx}{0.8\textwidth}{ |X|c|c|c|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
  Swap types                & \# of \texttt{deposit} & \# of  \texttt{withdrawal} & Value/diff (\$M) & Causes \\ \hline
  \multicolumn{5}{|l|}{Uniswap V2}   \\  \hline
 Type-I  & $52.7*10^6$  & $52.7*10^6$   & $6.18*10^8$  & Atomic \\ \hline
 Type-II  & $762$  & $761$   & {\bf $0.486$}  & External transfer \\ \hline
 Type-II  & $35$  & $35$   & {\bf $0.205$}  & Router error \\ \hline
 Type-III (O) & $2.01*10^5$ & $2.01*10^5$ & $23.3$/$3.64$ & Fees \\ \hline
 Type-III (D) & $3879$ & $3879$ & {\bf $0.185$/$0.094$} & Rebase \\ \hline
 Type-III (F) & $4767$ & $0$ & {\bf $1.26$} & Rebase/interest \\  \hline
  \multicolumn{5}{|l|}{Pancakeswap}   \\  \hline
 Type-I  & $2.97*10^6$  & $2.97*10^6$   & $7.34*10^7$  & Atomic \\ \hline
 Type-II  & $364$  & $364$   & {\bf $0.047$/$1.4*10^{-4}$}  & \\ \hline
 Type-III (D) & $1.7*10^5$ & $1.7*10^5$ & {\bf $0.99$} & Rebase \\ \hline
 Type-III (F) & $0$ & $1.99*10^5$ & {\bf $0.53$} & Rebase \\ \hline
 Type-III (U) & $7.087*10^5$ & $0$ & {\bf $0.12$} & Airdrop (synced) \\ \hline
\\ \hline
\end{tabularx}
}
\end{table*}

We collect the traces of three UniswapV2-based DEX'es and analyze them using the methods described in \S~\ref{sec:mmalgo}. The three DEX'es are Uniswap V2 and Sushiswap, both on the Ethereum mainnet, as well as the Pancakeswap on Binance Smart Chain. We present the results in Table~\ref{tab:1}. 

For each DEX, we report the measured cases of atomic swaps (i.e., value matched), discount/overcharge (i.e., value mismatched), and freeload/underwater (i.e., standalone transfer). In particular, when matching records in the same transaction in value, we only report the case with value difference larger than 10\%; we are aware that most DEX routers charge fees lower than 10\%, which are normal use cases and less interesting in the sense of finding risky swaps. For each case, we report the number of transfers involved (including both deposit and withdrawal), as well as the total value. To estimate the value, we crawl the historical exchange rates reported by etherscan (\url{https://etherscan.io/tokens}) on the same day/hour of the reported swap. We also select high-value cases and report their causes.

In Table~\ref{tab:1}, on Uniswap V2, the majority of swaps, with total value of $618$ billion USD and in more than 0.5 billion Ethereum transactions (as in the third row of the table), are atomic ones, each of which is carried out by one transaction calling a router smart contract (recall Figure~\ref{fig:uniswap2}). Besides, as shown in the fourth row, there are $761$ atomic swaps, each of which is carried out by two or three transactions that directly call Uniswap's pool smart contract. The fifth row shows $35$ swaps that match in value but invoke a router smart contract with ``partly error.'' The case of ``partly error'' router smart contract is discussed in more details in \S~\ref{sec:partlyerror}.

On Uniswap V2, more than $20$ thousand swaps are overcharge, which are caused by the particularly high fees by the operating routers or tokens. For instance, some tokens enforce a fee scheme to penalize the token deposit and to encourage the withdrawal. 

3879 swaps are discount, where a trader account receives profit. A primary cause is a token's rebase operation that occurs before the swap, as will be described in details in \S~\ref{sec:rebase}.

In the eighth row, $4767$ swaps are standalone deposit operations  (i.e., Freeride) that directly call the liquidity pool's swap function. In total, they are worth $1.26$ million USD. The profit come from the tokens' non-standard rebase operation or interest behavior.

\subsection{Causes: Patterns of Profitable Deposit}

\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.475\textwidth]{figures/victimpatterns.eps}
\end{center}
\caption{Patterns of profitable deposits: $R$ is the router smart contract, $T0/T1$ are the two tokens in the target liquidity pool}
\label{fig:patterns}
\end{figure}

We describe several attack patterns that we discovered through manual inspection. Based on the patterns, we will then describe our generalizable methods to model attackers' intent and cluster attackers by behavior.

\subsubsection{Non-standard Token Balance Updates (Pattern P1)}
\label{sec:cases:rebase}

In many real-world tokens, account balance can be changed by non-standard operations beyond token transfer. We describe two examples. {\it Rebase}: For instance, token balance can be elastically adjusted by token issuers, for purposes such as to stabilize the token's exchange rates against other tokens. In practice, token rebase is such a non-standard balance-changing function, supported in some widely used tokens, such as AMPL~\cite{me:ampl:token}. When a token, say $T0$, is rebased, a Uniswap's relevant pool, say for tokens $T0$ and $T1$, could have its $T0$ balance increased. Uniswap falsely assumes that this balance increase is due to some account swap token $T0$ for token $T1$. Uniswap's pool would mistakenly admit anyone who requests to withdraw token $T1$ after the rebase of $T0$.

{\it Token shareholder}: Another example is tokens that charge fees to average trader and distribute the income of fees to shareholders. In this type of tokens, there are two types of token owners, average owner and token shareholders. When there is a transfer, the token smart contract charges a certain amount of fees. The fees are redistributed to the privileged accounts of token shareholders. Thus, a transfer between average accounts would update the balance of all shareholders' accounts. In a Uniswap's pool of token types $T0$ and $T1$, if the pool's account in $T0$ is a shareholder, any transfers in $T0$ would increase the pool's balance and create profitable opportunity.
 
Furthermore, even when the pool receives a token deposit, the deposit may not be intended as a part of swap. For instance, airdrop is a common practice to promote the use of new token type, in which token issuers periodically give away newly minted tokens to the current token owners (e.g., in Tokens XXX and XXX). When a token, say $T0$, is airdropped into a Uniswap's pool, the pool holding tokens $T0$ and $T1$ would mistakenly treat the transfer as a part of swap from token $T0$ to $T1$. Thus, the pool would admit anyone's request to withdraw token $T1$ after airdrop of token $T0$ to the pool's account.

In general, there can be an explicit token operation that increases the pool's balance of token $X$, but is not with the intention of swap value. Thus, an attacker observing the occurrence of such exploitable operation can strategically extract value from the pool and gain illicit profit. We name this attack pattern by P1. 

\subsubsection{Implicit Token Balance Updates (P2)}
Beyond P1, there are implicit approach to update balance. Many tokens are bearing interest. That is, the balance in the token smart contract increases at a certain rate as the time goes by. Suppose a Uniswap pool is of token $T0$ and $T1$ where $T0$ is interest bearing. Similar to P1, the Uniswap pool observing the increase of token $T0$ would admit the withdrawal of token $T1$ by anyone who requests it, including a value-extracting attacker. We call this attacker's pattern by P2, which is different from P1. In P2, the attacker simply waits for long enough to harvest the extractable value from token interest. 

\subsubsection{External Transfer for Deposit (P3)}

In Uniswap, a trader can externally call token $T0$'s transfer function to make deposit so that she can in a separate transaction withdraw token $T1$. We call the pattern of a victim trader sending a transaction to externally transfer token $T0$ by P3. When P3 occurs, a malicious account can send the withdraw transaction ahead of the victim's one, to claim the value in the pool.  This attack is possible because a Uniswap pool receiving a deposit of $T0$ will approve of the next withdrawal request of token $T1$, no matter who sends it. 

\subsubsection{Buggy Router Contracts (P4)}

In the above three patterns, the victim externally calls token $T0$'s functions. In the fourth pattern P4, the trader delegates the handling of swap to a router smart contract that is buggy and violates atomicity. After the trader EOA's transaction, the router smart contract successfully completes the deposit of Token $T0$ but fails at requesting the withdrawal of Token $T1$. Thus, anyone who requests the token withdrawal in the next transaction, including an attacker EOA, would succeed in grabbing the value illicitly. 

\section{Discovering Attacks}
\label{sec:attack}

\subsection{The Problem}

\noindent{\bf Formulating attack detection problem}: 
The detected risky swaps present value that {\it can} potentially be extracted and grabbed by attackers. However, whether the value is {\it actually} extracted by attackers, or equivalently, whether the risky swaps are actual attack instances, is a different problem. 

Consider as an example that a token issuer sends a vulnerable rebase transaction to a pool's token, followed by a withdrawal transaction sent by account $X$ (i.e., P1). It is equally likely that $X$ is the token issuer and that $X$ is not. The former case is not an attack, as the token issuer aware of the risky rebase sends the withdrawal to remedy the risk. The latter case may be an attack. For other situations including P3 and P4, the same applies that a risky swap can be attributed differently.
\ignore{
For instance, in P1, after a token issuer sends an exploitable rebase transaction, it is equally likely one of the following cases occur: 1) the token issuer aware of rebase being exploitable quickly sends a swap request herself to claim the value in the Uniswap pool. 2) An attacker observing the occurrence of rebase operation calls the liquidity pool to withdraw the value there. The former case is not an attack, while the latter one is. In other cases, the same apply: In P3, if the trader sends another transaction to withdraw the value in token $T1$ right after the transaction of depositing $T0$, it is a benign case. But if it is an attacker account who withdraws after the external deposit, it constitutes an attack. In P4, if the trader observing the router exception and immediately send a ``make-up'' transaction to claim the value herself, it is a benign case. But if it is a third-party ill-intended account who sends the withdrawal transaction, it constitutes an attack.
}

To distinguish the benign case and attack out of a risky swap, it entails checking two key conditions: {\bf 1) Account non-linkage}: Whether the trader account who made the original deposit in token $T0$ and the account who successfully withdraw the value in token $T1$ are controlled by the same user off-chain. In other words, this is a problem of deciding the non-linkage between two blockchain accounts, which is intractable with only the on-chain data. 
{\bf 2) Account intention}: Whether a blockchain account is ill-intended in a transaction. Even when the withdrawer and depositor accounts are not the same physical user, they can be friends in the real life, which makes the swap non-attack. Thus, it entails to detect the depositor account's intention in sending the withdraw request, which however can be hidden opaque and pose challenges to detection.

{\bf Feasibility of existing approaches}: 
On Challenge 1), there are existing works that tackle the recovery of account linkage by heuristics specific to Bitcoin's UTXO model~\cite{XXX}. The only work for Ethereum~\cite{XXX} presents a linkage heuristic exploiting some DEXs deposit addresses. Specifically, on order book-based DEXs (i.e., IDEX and EtherDelta), trader Alice swapping token $T0$ for $T1$ can specify the so-called deposit address who receives $T1$. Assuming a swap is normal, the sharing of deposit addresses by two traders implies that the two traders are controlled by the same physical user. This work is different from our attack detection problem, where the deposit address heuristic is to detect the case that two accounts are linked, while our problem is to detect if two accounts are unlinked. More importantly, the deposit address heuristic works only under the assumption of normal swaps, while our work deals with risky swaps. Given an risky swap, the deposit address of a swap refers to the attacker. Thus, when an attacker targets two victim traders, it could appear that two traders share the same deposit address. In this attack, the two victim traders do not have to be linked to the same off-chain user.

On Challenge 2), there are existing works on threat intelligence on blockchains by characterizing attackers' behavior~\cite{XXX/YYY}. However, their target attacks are program-level attacks such as reentrancy attacks, and the attack strategies recovered in the work are specific and don't apply to the DEX attacks in our work.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.4\textwidth]{figures/indicators.eps}
\end{center}
\caption{Attack strategies (A1/A2/A3) and indicators}
\label{fig:indicators}
\end{figure}

\subsection{Attack Discovery Approaches}

We discover attacks by designing attack strategies specifically for different profitable deposits and use them as attack indicators to match the observable attacker behavior on-chain. 

{\bf Design rationale: Attack strategies}: Recall that each risky swap involves with a profitable deposit followed by a withdrawal that reaps the profit. An attacker needs to strategically send the withdrawal to ensure high success rates by properly monitoring the profitable deposits. We consider the following three attack strategies:

\begin{itemize}
\item[A1)]
 {\bf Aggressive attacker (monitoring deposits)}: The attacker directly monitors the mempool for the profitable deposits. In this strategy, the attacker monitors different cases of profitable deposits, such as P1/P2/P3/P4. The attacker launch a node joining the Etheruem blockchain network and monitors the node's mempool so that the profitable-deposit transaction can be detected as soon as they are propagated in the blockchain network. 

Strategy A1 entails the attacker to customize the monitored conditions to different causes. It minimizes the time window between the profitable deposit and the exploit withdrawal, and can ensure high success ratio in the presence of competing attackers.

\item[A2)]{\bf 
General-purpose attacker (monitoring pool)}: The attacker monitors the Ethereum's smart contract state to check if the pool is profitable. For instance, when a rebase transaction is executed in the blockchain, it could increase the balance in the token smart contract and leave the reserve in the pool smart contract unchanged. By detecting the difference between token balance and reserve, the attacker ensures sending a withdrawal can succeed.

Strategy A2 is generalizable to different profitable deposits, in the sense that the attacker monitors a single condition that all different profitable deposits will trigger. However, this strategy works only after the profitable deposit transaction is executed and included in the blockchain. So an aggressive attacker (A1) can frontrun an general-purpose attacker (A2).

\item[A3)]{\bf 
Lucky trader}: The trader does not intentionally observe conditions on pool profitability but is lucky in grabbing the profit by inserting a withdrawal after the profitable deposit. The delay between the withdrawal and victim deposit can be arbitrary. 
\end{itemize}

{\bf Proposed attack indicators}: 
An account's strategy, which normally occur in the blackbox off-chain state, is not directly observable from the on-chain traces. We distill observable information and design indicators to infer attack strategies.

To start with, an aggressive attacker monitoring the off-chain mempool states cannot be observed from the on-chain traces. Likewise, a general-purpose attacker who may choose to issue RPC calls to read on-chain data is also unobservable. For these cases, we  collect the gap between the block including deposit transactions and the block including the exploit withdrawal transactions as the metric to infer the presence of an attack and further the attack strategies. For instance, if the block gap is always $0$, it indicates the case is exclusively an aggressive attack. If the deposit is token interest and the block gap is always large, it indicates an aggressive attack exploiting token interest. Otherwise, if the block gap is randomly distributed, it is likely to be a lucky trader. Based on the heuristics, we propose the following three indicators:

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I1) An account whose withdrawal transactions occur consistently within $G$ blocks after profitable deposits (i.e., block gap smaller than $G$) and whose victim deposits are non-interest is likely to be an attacker. 
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I2) An account whose withdrawal transactions occur consistently more than $G'$ blocks after profitable deposits (i.e., block gap larger than $G'$) and whose victim deposits are based on token interests is likely to be an attacker.
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I3) An account whose block gaps have large deviation is likely to be a lucky trader.
}}\end{center}

In practice, many accounts use delegate smart contracts on-chain to relay their payload (of malicious withdrawals). The delegate smart contracts make attack strategies observable. We propose the following indicators to take advantage of this fact. 

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I4) An account who attempts to withdraw through a smart contract that checks both pool reserves (i.e., calling $pool.getReserves()$) and token balances (calling $erc20token.balanceOf()$) is likely a general-purpose attacker. Note that this indicator does not require the smart contract to actually withdraw the token $T1$. 
}}\end{center}

The intuition of the above indicator is that a general-purpose attacker uses the pool's $getReserves()$ function and token's $balanceOf()$ function to obtain the token reserve and balance, respectively. This shows the account's intention to calculate pool profitability and is an indicator of general-purpose attacker. Note that this indicator is not sufficient (i.e., causing false positiv), as a general-purpose attacker can issue RPC queries to read reserves and balances, leaving no trace on-chain.

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I5) An account whose withdrawal transactions exclude any token deposit is likely to be an attacker.
 
An account whose withdrawal transactions also include token deposits is likely to be a lucky trader, even through the withdrawal is of higher value than the deposit.
}}\end{center}

At last, we propose a heuristic that intentional attackers would victimize a diverse set of accounts while a lucky trader may victimize a fixed type of accounts (e.g., in the same pool).

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I6) If an account sends withdrawals in a large number of risky swaps, the account is an attacker.
}}\end{center}


{\bf Attack discovery algorithm}: We materialize the indicators in a holistic attack discovery algorithm. The algorithm takes as input the detected risky swaps from the previous phase (\S~\ref{sec:detectriskyswap}) and produces the labels for swaps and accounts what attack strategies are used.

Specifically, recall that each risky swap consists of a profitable deposit and a (successful) withdrawal. We expand it by adding all the withdrawal attempts, no matter success or failure, on the same pool by calling its $getReserves$ or $swap$ functions between time $t_1$ and $t_2$ where $t_1$/$t_2$ is the time when the current/next deposit occurs. We ignore the atomic swaps (Type-I) between $t_1$ and $t_2$. Hence for each risky swap, we obtain a list of accounts who send the withdrawal or expended withdrawal attempt. For each account and each associated swap, the algorithm checks the indicators and reports the number of attacker labels the account is tagged with. In particular, indicator I1/I2 produces the block gap averaged over all the swaps the account is involved when the deposit is non-interest/interest. 

\lstset{style=mystyle}
\begin{lstlisting}[caption=Psuedocode to discover attacks,
                   linerange={1-30},
                   firstnumber=1,
                   deletekeywords={[2]INT},
                   morekeywords={clustered},
                   framesep=2pt,
                   xleftmargin=5pt,
                   framexleftmargin=5pt,
                   frame=tb,
                   framerule=0pt, 
                   label=code:discoverattacks,
                   float,floatplacement=H
                   ]
void AttackDiscovery(RiskySwap[] swaps, int th1, int th2){
  for(RiskySwap s in swaps){
  Mapping blockGaps;

  for(Account w in s.getWithdrawers())
    //I4
    if(isCA(w)) //I4
    if(findCall(w, s.getPool(), "getReserve").getTx().checkCall(w, s.getPool().getTokens(), "getBalance()")) emit(w, "Attacker");
    //I1
    Block depositTime=s.getDeposit().getBlock();
    Block withdrawTime=w.getBlock();
    blockGaps.getValue(w).add(withdrawTime - depositTime));
    //I2
    numberSwaps.getValue(w).increment();
  }

  for(Account w in blockGaps.keySet()){
    blockGap.getValue(w).divideBy(numberSwaps.getValue(w));
    if(blockGap.getValue(w) > th1) emit (w, "Attacker");
    if(numberSwaps.getValue(w) > th2) emit (w, "Attacker");
  }
}
\end{lstlisting}


\subsection{Results}

\begin{table*}[h]
\centering{\small
\begin{tabular}{|p{1.25cm}|p{1.5cm}|p{2.5cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}|p{1.0cm}|p{1.4cm}|p{1.4cm}|}
\hline
Accounts & Value & {Profitable} & \multicolumn{4}{c|}{Attack indicators} &\# pools &\# victims & Label \\
\cline{4-7}
 & ($10^3$ USD) & deposit &I1 & I2 & I4 & I6 &{~}&{~} & (strategy) \\
\hline
\multicolumn{10}{|l|}{\it Most frequently swapping account}\\
\hline 
0x9799 & 556	& $33*P1, 4*P2, 6*P4$        &422  &371   & 	0    & 43 	 & 4 &  0 + 7  & A3\\
\hline                                                    
0x2a2e & 239	& $32*P1$                         &0.03  &                    & 	32   & 32 	 & 1 &  0  + 3 & A1\\
\hline                                                    
0xdb40 & 113	& $12*P1, 2*P2, 3*P3$          &2.5   &665    & 	17   & 17 	 & 1 &   0 + 4 & \\
\hline                                                    
0x0c08 & 101    & $3*P1, 1*P4$                         &1.5    &                    & 	0    & 4 	 & 1 &  1 + 1  &  \\
\hline                                                    
0x5617 & 101	& $53*P1, 4*P2, 2*P3, 2*P4$ &13     &1574 & 	0    & 61 	 & 3 &  2 + 4  & \\
\hline                                                    
0xb6bf & 20     & $1091*P1, 131*P2, 9*P4$         &224   &600   & 	1231 & 1231   & 9 & 12 + 5  & \\
\hline                                                    
0xc762 &  16    & $64*P1, 6*P2, 13*P4$                 &3.0    &437     &  	83   & 83     & 19&  0 + 4  & \\
\hline                                                    
0xa32d & 6      & $208*P2$                        &                     &942 & 	208  & 208    &   &  0 + 0  & \\
\hline
\multicolumn{10}{|l|}{\it Least frequently swapping account}\\
\hline
0xc408 & .8 & $P1$  & 0 & &  1& 1 		&  &  0 + 1 & \\
\hline                                                    
0x02ef & .1	  &  $43*P1, 9*P4$  & 2.6 &  &  52 & 52 	     &  &  1 + 0 & \\
\hline                                                    
0x2839 & .04 & $P1$ & 0   &  &  0 & 1 	      &  &  0 + 1 & \\
\hline                                                    
0x042d & .03 & $P1$ & 130 &  &  0& 1 		 &  &  0 + 1 & \\
\hline                                                    
0x5b1b & .01 & $P1$ & 206 &  &  0 & 1	     	  &  &  0 + 1 & \\
\hline                                                    
0x6cea & .01 & $P1$ & 904 &  &  0 & 1  	  &  &  0 + 1 & \\
\hline                                                    
0xf39f & .01 & $P3$ & 0   &  &  0 & 1     	  &  &  1 + 0 & \\
\hline                                                    
\end{tabular}%
}
\caption{Attackers and their patterns}
\label{table:analysis}
\end{table*}


We present our analysis result in Table~\ref{tab:attackerview} which characterizes the most/least frequent accounts involved in risky swaps. The metrics include value stolen, causes, attacker indicators, the number of pools attacked, the number of victim accounts, and the label whether the account is an attacker.  From the table, we analyze the attacker strategy of several selected accounts.

{\bf Case 1: Agg. attacker (A1) w. zero block gap}: Account $0x2a2e$ is involved in $32$ risky swaps (I6) and gains more than $2.39*10^5$ USD worth of illicit tokens. All $32$ swaps from this account are sent via a smart contract which checks the pool's profitability before withdrawal (I4). In terms of timing, the malicious withdrawals are always sent in the same block with the risky, profitable deposit. We believe account $0x2a2e$ aggressively monitors the mempool for the target tokens' rebase transactions, and if found, sends withdrawal transactions immediately to ``backrun'' the deposits and claim the profit. 

{\bf Case 2: General attacker (A2) w. off-chain monitoring}: Account $0x0c08$ has withdrawn four times and grabbed tokens of $1.01*10^5$ USD. The account directly and externally calls Uniswap pool's swap function to withdraw, without checking pool profitability on-chain. The withdrawals are included in exactly one block after the one that includes the risky deposit. We believe Account $0x0c08$'s strategy is to monitor the pool profitability from an off-chain vantage point and to immediately send withdrawal by externally calls. Because the account monitors the pool profitability instead of the cause (risky deposit), it has to wait until the inclusion of risky deposit that updates the pool state to be profitable. This explains why the inclusion of withdrawal has to be one block after the one including the risky deposit.

{\bf Case 3: Agg. attacker (A1) stealing interest}: Both Accounts $0xdb40$ and $0x5617$ have extracted value from tokens supporting embedded interest. Their block gaps are constant (687 and 586, respectively) with zero deviation. Given that there are enough samples, this consistent behavior shows both accounts' attack strategy to wait long enough for the token interest to accumulate and for the extractable value to be large enough before acting on it.

{\bf Case 4: Adapting strategies}: For all accounts with indicators I1 and I2 in the table, it is clear that the block gaps for different causes (I1 and I2) differ: The block gaps for non-interest causes are consistently much shorter than those for token interests. It implies that the attackers are aware of the situation (which causes to exploit) and tailor their strategies to it.

{\bf Case 5: Lucky trader (A3)}: Account $0x9799$ is unlikely an intentional attacker: First, it does not read the token balance or check the pool's profitability before the withdrawal. Second, the block gap between profitable deposit and malicious withdrawal is large, at hundreds of blocks apart. In addition, the smart contract Account $0x9799$ relays her withdrawal requests also makes deposit to the pool. All these indicators show that $0x9799$ is unlikely an intentional attacker, but instead a lucky trader who gets profits by accidents.

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_attacker_timeline.eps}
\end{center}
\caption{Timeline of detected attacks.
Data from 07/09/2020 (block no. 10422671) - 06/29/2021 (block no. 12727620).}
\label{fig:attack}
\end{figure*}

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_victim_timeline.eps}
\end{center}
\caption{Timeline of detected victims. 
Data from 08/25/2020 (block no. 10731770) - 06/16/2021 (block no. 12645092).}
\label{fig:victim}
\end{figure*}

\section{Characterizing On-chain Crimes}
\label{sec:behavior}
\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/UniswapV2attacker3.eps}
\end{center}
\caption{Attack campaign template: Preparing, mounting and wrapping up theft attacks.}
\label{fig:business}
\end{figure}

We further expand the scope of each attack instance by tracing the money flow and smart contract lineage. The goal is to uncover the attack business.

Given an attack instance with attacker accounts $\{A\}$, we construct an expanded attack graph by adding the following information: 1) the transactions that pay Ether or tokens to the attacker accounts, 2) the transactions that deploy the smart contracts used in the attack, and 3) the transactions that are sent by the mule accounts who receive the stolen tokens after the attack. These new transactions would add into the graph a set of new accounts, be it either the transaction sender or receiver. We iteratively apply this graph-expansion process, until it reaches the ``hub-node'' accounts, which receive or send a large number of transactions (e.g., a popular DEX pool). 
For instance, Figure~\ref{fig:business} shows an example of expanded attack instance, with the attackers in the red box and the victims; the added accounts and transactions are outside the two boxes. 

{\bf Attack ecosystem template}: We analyze the expanded attack graph in a template consisting of three phases: 1) attack preparation, 2) attack execution, and 3) attack wrap-up. Phase 2) is the core attack component, and Phases 1) and 3) are the expanded  parts. In general, the actual Boss often sits behind an exchange/mixer service, such as Tornado~\cite{XXX}, to hide its identity. In  attack preparation (Phase 1), the Boss sends Ether to Attackers and Exploit developers to cover the basic operational costs of the attack. The Ether transfer can be relayed through the Mules. An Exploit developer writes an Exploit smart contract and deploys it to the blockchain. It then mounts the attack in the execution phase (Phase 2)w, exercising the strategies described previously (\S~\ref{XXX}). To wrap up a series of attacks (Phase 3), the mule receiving the stolen tokens transfers the tokens back to the Boss. This is often done by swapping the stolen tokens to ETH (e.g., via DEX and wrapped tokens such as WETH) and by sending the ETH to the Boss via a mixer service. In the attack wrap-up phase, the mule may transfer tokens to Investors to maximize the stolen value. 

{\bf Results}: YYY

\begin{table*}[h]
{\centering
    \begin{tabular}{|p{1cm}|p{1.4cm}|p{1.4cm}|p{1.4cm}|p{1.4cm}|p{1.2cm}|p{1.2cm}|p{1cm}|}
    \hline
    Attack indices &Value ($10^3$~USD) & \#Operators & \#ECs & Developers & Mules & Profitable deposits & Block gaps\\
    \hline
    1 & 552 & 5 %$0x4e53$, $0xac72$, $0xa084$, $0x5bb4$, $0xe929$ 
& 24 % $0x338c$, $0x3ac7$, $0x34a2$, $0x9a99$, $0x2927$, $0x536b$, $0xe9f8$, $0x684b$, $0x58a3$, $0x72bb$, $0xa8a2$, $0x72cb$, $0x2528$, $0xbf2d$, $0xadfc$, $0xd6a2$, $0x24af$, $0x1335$, $0xf367$, $0x94fc$, $0x5caf$,  $0x6332$, $0x3c3a$, $0x1233$	
& {\bf \color{red} $0x8641$} & $0x9799$ & P1 & 121\\
    \hline
    2 & 101 & 1 %$0x2a2e$ 
& 1 %$0x5f5a$ 
& $0x2a2e$ & $0x2a2e$ 
& P1 & 1\\
    \hline
    3 & 96 & 5 %$0x64bc$, $0x62ae$, $0x3807$, $0x225c$, $0xdb40$ 
& 2 %$0x4dbc$, $0x4626$ 
& $0x4626$ & $0xdb40$ 
& P1 & 0\\
    \hline
    4 & 86 & 1 %$0xfdee$ 
& 1 %$0x0c08$ 
& $0x0c08$ & $0x0c08$ 
& P1 & 1\\
    \hline
    5 & 67 & 4 %$0x3a51$, $0xf97b$, $0xbf3f$, $0xa1e6$ 
& 10 %$0xfb51$, $0x328d$, $0x8a14$, $0x0fc7$, $0x4ed5$, $0xb439$ ,$0x55a2$, $0x6ba3$ 
& \color{red}{$0x8641$} & $0x5617$ 
& P3 & 2\\
    \hline
    6 & 48 & 1 %$0x675f$ 
& 2 %$0xb6bf$, $0x8526$ 
& $0x675f$ & $0x675f$ & P1 & 0\\
    \hline
    7 & 29 & 1%$0xd0d0$ 
& 1%$0xc762$ 
& $0xd0d0$ & $0xd0d0$& P3 & 1 \\
    \hline
    8 & 22 & 1%$0x7505$ 
& 1%$0xa32d$ 
& $0x7505$ & $0x7505$& P1 & 0 \\
    \hline  
    \end{tabular}%
}
    \caption{Attack ecosystem and attacker correlation: Red text shows the two attack instances are mounted using the exploit smart contracts developed by the same developer.}
    \label{tab:eco}
    \end{table*}


\section{Attack Mitigation}

\subsection{Root Cause of the Vulnerability}

Uniswap's pool accepts deposit of Token $T0$ in any form, including the external transfer call directly sent from the trader EOA. As can be seen in Appendix \S~\ref{appendix:XXX}, this flexibility greatly simplifies the programming of router smart contract, esp. when interoperating with other DeFi services~\cite{me:uniswapv2:whitepaper}. In order to know the deposit amount, Uniswap tracks the difference between the $T0$  reserve in the pool contract and the pool's account balance in $T0$'s token contract. Upon observing the difference, the pool allows anyone, on a first-come-first-served basis, to withdraw token $T1$ of the same value with the deposit in token $T0$. 

The root cause of Uniswap's vulnerability is that the pool implicitly assumes that any deposit of token $T0$ to the pool's account is intended for swapping out token $T1$. The assumption fails in the risky-swap cases identified in this work, including token rebase, airdrop, interest, etc. which all update the token balance but are not intended for swapping. 


\section{Related Works}
\label{sec:rw}

This work is related to blockchain data analysis. We survey two bodies of related works, that is, blockchain-data analysis for attack detection and user de-anonymization.


{\bf Detecting Smart-Contract Program-level Attacks}: Attack detection on blockchain generally works as distilling the attack signatures from known vulnerabilities and attack patterns and matching certain representation of smart-contract execution (e.g., in transactions, function-call graph or instruction traces) against the attack signatures. There are known patterns of smart-contract program-level attacks, such as reentrancy attacks, transaction order dependency, etc. Existing works tackle the detection of program-level attacks on Ethereum-like blockchains. 
 
TxSpectror~\cite{DBLP:conf/uss/ZhangZZL20} records and replays Ethereum transactions into fine-grained EVM instruction traces, which are stored in datalog databases and queries to compare against the signatures of known attacks. Similarly, Zhou et al~\cite{DBLP:conf/uss/ZhouYXCY020} model the coarse-grained traces of smart contract function calls and match them against known attack signatures. At its core, two function calls are modeled, that is, smart contract creation/destroy and token transfers (money flow). Su et al~\cite{DBLP:conf/uss/SuSDL0XL21} uses reported attack instances to extract attack signatures, and it discovers new attacks as well as uncovers the attacker/victim behavior by systematically analyzing the Ethereum blockchain traces. Other similar work~\cite{DBLP:conf/uss/0001L21} detects the attack instances of known vulnerabilities.  

{\bf Detecting DeFi Protocol-level Attacks}: In addition to detecting program-level attacks, there are related works on detecting protocol-level attacks on deployed DeFi applications. Notable DeFi attack patterns include frontrunning, arbitrage, etc. 

Torres, et al.~\cite{DBLP:conf/uss/TorresCS21} detects front-running attacks by matching Ethereum transactions against a signature of success-failure transaction pair. Qin et al~\cite{DBLP:journals/corr/abs-2101-05511} systemizes different types of front-running attacks and measures the attacks and mitigations in the wild.

Front-running attacks are a class of attacks in which the attacker inserts a malicious transaction before the victim transaction to extract illicit profit (e.g., to win an auction bid unfairly). More generally, front-running is a class of MEV or miner extractable value, in which transaction order can be manipulated by a profit-driven miner to receive additional profit.

Arbitrage attacks work by an aggressive trader gain profit by exploiting difference of exchange rates across different DEXes/price oracles. Wang, et al~\cite{DBLP:journals/corr/abs-2105-02784} detects cyclic arbitrage on Uniswap-V2, by finding profitable cycles on token-transfer graph (nodes are tokens and edges are transfers). Similarly, Zhou, et al~\cite{DBLP:conf/sp/ZhouQCLG21} discovers profit-generating transitions in real time by finding cycles  and leveraging solvers.


{\bf User de-anonymization}: While blockchain accounts and their activities are visible, the linkage of accounts (which are public keys) with real-world identities is not directly observable. There are existing works to infer blockchain account linkage in efforts to deanonymize users. Specifically, there are three types of linkage information: 1) Whether a specific account is linked to a specific real-world user identity. Existing works~\cite{DBLP:conf/fc/KoshyKM14} monitor a blockchain network' traffic of transactions propagated from an IP and link the transaction sender's account with the IP. Other works~\cite{XXX} aggregate transaction volume of a given account and use background knowledge to link the account to real-world ID.

2) Whether two blockchain accounts are linked, as the sender and receiver, in a privacy-enhanced transaction. Mixing services are intended to break the sender-receiver linkage. There are existing works aimed at reconstructing the sender-receiver relation on transactions relayed through mixing services. In particular, address reuse is a heuristic to link transaction senders/receivers on Bitcoin like blockchains~\cite{DBLP:conf/uss/YousafKM19,DBLP:conf/uss/KalodnerMLGPCN20}.

3) Whether two blockchain accounts are shared by the same real-world user. On Bitcoin, transaction graph analysis~\cite{DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:books/daglib/0040621} are proposed to recover the account linkage. Particularly, address clustering heuristics are proposed. For instance, two accounts that are co-spent by a Bitcoin transaction or that involve a change are likely to be controlled by the same off-chain user. These address clustering heuristics are useful only in the context of Bitcoin's UTXO model. Address clustering is useful to uncover the money flow in online criminal activities such as ransomware payments on Bitcoin~\cite{DBLP:conf/sp/HuangALIBMLLSM18}. 

Of most relevance to this work is the address clustering techniques proposed to link Ethereum accounts~\cite{DBLP:conf/fc/Victor20}. Specifically, the observation is that some DEX'es support the deposit address, that is, trader Alice swapping token T0 for token T1 can specify a ``deposit'' address to receive T1. Multiple accounts using the same deposit address are likely to be the same off-chain user. 

This work is different from Ethereum account linkage. In this work, the attack detection problem is to verify whether two Ethereum accounts are from two off-chain users, which is different from detecting if two accounts are linked by the same off-chain user. Moreover, the Ethereum address clustering work~\cite{DBLP:conf/fc/Victor20} has to assume that the swap is atomic, normal one, so that they can attribute address sharing to the cause of the same off-chain user. By contrast, in this work, we do observe two sender accounts share the same deposit address, but they are caused by two victim accounts whose swaps are grabbed by the same attack account, as verified by our analysis of attacker/victim behavior.
\clearpage

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/uniswapV2vsV3-1year.eps}
\end{center}
\caption{Usage of Uniswap V2 and V3 over time}
\label{fig:use}
\end{figure}


\begin{table}[!htbp] %force in current page, disable float.
\caption{Uniswap V3's liquidity pools' API to support token swaps}
\label{tab:uniswapv3:api}\centering{\small
\begin{tabularx}{0.475\textwidth}{ |c|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
Version & Function signature \\ \hline
\multirow{2}{*}{V3} & pool.swap(to\_address, amountIn, Price, tokenIn, tokenOut, fee) \\ \cline{2-2}
& uniswapV3SwapCallback(amountIn, amountOut, tokenIn, tokenOut, fee) require(msg.sender == pool)
\\ \hline
\end{tabularx}
}
\end{table}




==> text/old/v4_intro.tex <==
\section{Introduction}

Recent years witnessed the rise of Decentralized Finance (DeFi), a class of smart-contract applications running on operational blockchains.
The most popular DeFi is Decentralized Exchange (DEX), which allows traders to swap their assets stored in one token with those in another token. Automated Market Maker (AMM) is a dominating DEX protocol. For instance, Uniswap~\cite{me:dex:uniswap} is an AMM-based DEX that dominates $90\%$ of the DEX market on Ethereum, and it has attracted a total of $149$ million transactions as of Jan. 2022~\cite{me:etherscan:topdex}\jiaqi{Q:Update the number to Apr. 2022. A:I don't have data from Janary to now of bigquery. I'm collecting the number of calls from bloxy but it takes time.}. An AMM maintains token reserves under the account of liquidity pool and allows a trader to directly exchange their tokens with the pool's reserves.

\vspace{2pt}\noindent\textbf{Risk in DEX}. Like any currency exchange system, of ultimate importance is the DEX's security against the threat of token thefts, in which an unauthorized party's account can extract value and steal tokens to be received by the original trader. To prevent such illicit value extraction, swap atomicity is essential: That is, the transaction transfer operations in a swap should be executed in an all-or-nothing manner. Violating swap atomicity could pose security risks to the trader. For instance, an attacker observing a swap whose execution gets interrupted could extract value from the pool at the pending state where one token has been deposited while the other token has not yet been withdrawn. 
%This risk can be more severe, in the presence of permissionless, composable DeFi protocols running on AMMs, as elaborated on in \S~\ref{YYY}.

While existing research has measured DEX security against arbitrage~\cite{DBLP:journals/corr/abs-2103-02228}, front-running and scam tokens~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21}, these attacks do not necessarily violate the atomicity of individual swaps. It remains an open research problem whether risky DEX transactions violating atomicity exist, if they exist how pervasive they are, whether any real-world attacks materialize such risks into actual value loss, and whether there is a criminal ecosystem behind the attacks. 

Our research is the first attempt to address these problems, by systematically analyzing Ethereum transaction traces. Specifically, we focus on the most popular operational instances of DEXes: Uniswap-V2~\cite{XXX}, Sushiswap~\cite{XXX}, and Pancakeswap~\cite{XXX}. The first two account for more than $83\%$ of the DEX market on the Ethereum mainnet all time, and the last one is the most popular DEX on Binance Smart Chain (BSC), an Ethereum network fork~\cite{XXX}. For each DEX, we look into its transaction trace to answer the following research questions: {\it RQ1) Risky swap detection}: Whether there are risky swaps that violate the atomicity property? {\it RQ2) Attack discovery}: From the identified risky swaps, are there any intentional attacks that extract illicit value?\ignore{Note that not every risky swap has to be an attack (e.g., risky swap can be caused by a pool charging high fees, which is not an attack).} {\it RQ3) Attacker behavior}: What are the attackers' behaviors, particularly how to set up the attacks, trigger the attacks and transfer stolen assets afterwards? Together, we aim to detect value thefts on DEX and uncover the underground criminal ecosystem that systematically harvests illicit profit from the risky swaps.

\vspace{2pt}\noindent\textbf{Our methodology}. In our research, we developed an end-to-end transaction-analytical pipeline to systematically detect risky swaps, discover attack instances and analyze the attacker/vicitm behavior. 
More specifically, our pipeline first detects risky swaps by linking the records of different transfer operations across transactions to find the mismatch between the token value transferred into a liquidity-pool account and that coming out of the account. A challenge here is that AMMs such as Uniswap-V2 support a swap across multiple transactions, and directly connecting these transactions together can be very inefficient (e.g., entailing cross-product on the transactions' powerset). So in our research, we developed an efficient linear algorithm that takes advantage of the invariant in the Uniswap-V2 program.

Based on the risky swaps, our approach further identifies attack instances. An actual token-theft attack occurs between two distinct accounts, being it a victim trader and an attacker. However, whether two blockchain addresses are linked (e.g., controlled by the same physical user) is unknown from on-chain information. This poses a new challenge that existing techniques such as address clustering~\cite{DBLP:conf/fc/Victor20,DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:conf/sp/HuangALIBMLLSM18,DBLP:books/daglib/0040621} do not solve (see \S~\ref{sec:discoveryproblem} for details).
To tackle the challenge, we inspected the causes of risky swaps, identified the patterns of exploitable deposits (described in the next paragraph), hypothesized possible attack strategies, and used them to indicate and discover theft attacks from the risky swaps.

%We further collected attack ground-truth data from online user complaints to validate the effectiveness of our indicator-based technique.

\vspace{2pt}\noindent\textbf{Our findings}. 
We analyzed more than $53/1.9/3$ million transactions on Uniswap V2/Sushiswap/Pancakeswap and found more than $9443$/$311$/$454871$\jiaqi{The number updated} risky swaps violating atomicity. 
We found risky swaps follow the same ``template’’ in which a vulnerable deposit operation that creates extractable value is followed by multiple withdrawal requests that attempt to claim and steal the value, among which one succeeds. 

We further inspected the extractable deposits and found in practice they can be created in a variety of unexpected application scenarios, such as free token giveaways (i.e., airdropping), privileged accounts that charge tax, tokens bearing interest, buggy router smart contracts, and unsafe user interface that allows a swap to be conducted in two separate transactions, etc. 
The root cause is that in these scenarios, someone makes deposit into a Uniswap’s pool but does not intend to withdraw tokens in return. When this occurs, Uniswap falsely assumes that any pool deposit must be part of a swap and makes it possible to withdraw or extract the deposited value by anyone who comes to claim it, including an attacker. 


\ignore{
Each risky swap consists of a profitable deposit transaction and multiple attempts to withdraw the value, out of which one succeeds. We inspected the profitable deposit transactions and uncovered unexpected patterns of violating atomicity: 1) Profitable deposit can be made by non-standard token operations that update balance, such as rebasing token supply (to stabilize token price), offering token interest, giving away free tokens in the so-called airdropping practice, etc. 
2) Another cause is mishandled smart-contract exceptions which occur after a successful deposit but before the withdrawal, leaving the pool in an incomplete state. 
3) The third cause is the unsafe user interface in which a swap is carried out by two transactions which are not well coordinated.
%where the majority of attacks exploit the non-standard token operations.
%The root causes of these violation cases range from buggy smart contracts, unsafe user interfaces, and false assumptions on unspecified token behavior (non-standard functions).
}

We studied the attack strategies to take advantage of these profitable-deposit patterns and used them as attack indicators. On the Ethereum mainnet and BSC fork, we discover $4.65*10^5$\jiaqi{The number updated} theft attacks from $258$ distinct attacker accounts, inflicting a loss of more than $3.7$ million USD stolen from $978$ victim traders.
Each attack instance we found matches more than one indicators. A range of interesting attack strategies were observed in practice. For instance, real-world attackers {\it adapt} to the deposit patterns exploited: When it is the token interest to steal, the attackers choose to wait long, typically hundreds of Ethereum blocks, for the interest to accumulate and to be profitable. For other types of deposits, the attacker chooses to send the withdrawal immediately, say within one or two blocks, in order to front-run other competing attackers.

We further studied the attackers' behavior by tracking their money flow and contract creation/destroy sequence. Our study uncovers the systematic criminal activities: the crime bosses use mixer services to hide their identities while sending commissions and instructions. After the attack, the money is sent to a variety of DeFi services to maximize the illicit profit. Exploit smart contracts are widely used to facilitate attacks to improve the attack success rates.

\vspace{2pt}\noindent\textbf{Contributions}. The contributions of the paper are outlined as follows: 

\vspace{2pt}\noindent$\bullet$\textit{ New findings}. We discovered a total of $3.5$ million USD worth of stolen value, by measuring and analyzing atomicity violations on three popular Uniswap services on Ethereum and BSC. 
The discovered token theft attacks uncover the previously unknown patterns of vulnerable deposits (e.g., token rebase, interest, airdrop, mishandled contract exception) and expose the malicious, adaptive withdrawal behavior that occurs offline and otherwise would have been hidden. We further studied the criminal infrastructures and campaigns mounted to systematically prepare, execute and finalize the theft attacks.

\vspace{2pt}\noindent$\bullet$\textit{ New techniques}. We developed an end-to-end analytical pipeline to detect attacks from Uniswap transaction traces, including an efficient join algorithm for detecting atomicity violation, and approaches to automatically discover and cross-check token theft attacks. 
%XXX: Also we propose mitigation schemes including a fuzzer and test oracle to automatically detect mishandled exceptions in smart contracts.

Overall, this work leads to the findings that shed light on the current and future underground ecosystem that strategically exploits the atomicity violation to gain illicit profit.


\noindent
{\bf Roadmap}: \S~\ref{sec:background} introduces the background of Uniswap, defines risky swaps and describes the threat model. The first step in our analysis pipeline, that is, detecting risky swaps, is presented in \S~\ref{sec:detectriskyswap}. The second step, discovering attacks, is described in \S~\ref{sec:attack}. The third step, characterizing on-chain crimes, is in \S~\ref{sec:behavior}. 
Mitigation schemes are presented in \S~\ref{sec:mitigate}. Related work is described in \S~\ref{sec:rw}. Responsible disclosure is discussed in \S~\ref{sec:disclosure} with the conclusion in \S~\ref{sec:conclude}. 

%In Appendices are full related works in Appendix~\ref{sec:rw:extra}, 




==> text/old/v4_paper3.tex <==
\section{Background}
\label{sec:background}

\noindent
{\bf Preliminary: Ethereum \& Uniswap}: Ethereum supports two types of addresses: an externally owned account (EOA), which is an Ether owner's public key, and a contract address, which is the memory address where the smart contract is deployed on individual miner nodes. An Ethereum transaction binds a sender's address to a receiver's address.

A decentralized exchange or DEX supports the swapping of a trader EOA's token of one type for another token type. Uniswap is the dominant DEX protocol on Ethereum and is designed based on an automated market maker (AMM). An AMM maintains token reserves in a so-called liquidity pool; the token owners, called liquidity providers, deposit their tokens to fill up the reserves, and the pool uses the current reserves to calculate token exchange rates, on demand, to serve swaps.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.4\textwidth]{figures/uniswap-layers.eps}
\end{center}
\caption{Uniswap system and smart contracts at three layers.}
\label{fig:uniswap:layers}
\end{figure}

\begin{table}[!htbp] %force in current page, disable float.
\centering{
\begin{tabularx}{0.5\textwidth}{ |X|X|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
Layer & $Swap$ workflow & $addL.$ workflow \\ \hline
Router & \texttt{swapWrap}\yuzhe{XXX} & \texttt{addLiquidity}\yuzhe{XXX} \\ \hline
Liquidity pool~\cite{me:uniswapv2:pool}
& \texttt{swap}(amountOut, to) & \texttt{mint}(to\_address), \texttt{burn}(to\_address) \\ 
\hline
ERC20
& \multicolumn{2}{|l|}{\texttt{transfer}(trader,amountOut)} \\ 
token~\cite{me:erc20:api} & \multicolumn{2}{|l|}{\texttt{transferFrom}(trader,pool,amountOut)}\\ 
 & \multicolumn{2}{|l|}{\texttt{balanceOf}(account)} \\ \hline
\end{tabularx}
}
\caption{Uniswap-V2's liquidity pools' API: $addL.$ represents $addLiquidity$ workflow.}
\label{tab:uniswapv2:api}
\end{table}

The Uniswap protocol architects a DEX in three layers of smart contracts, as in Figure~\ref{fig:uniswap:layers}: 
The central layer is the liquidity pool, as described, which receives requests from the upper-layer router smart contracts and sends requests to transfer tokens in the underlying token smart contracts. The router smart contract is trusted by a trader EOA and is responsible for protecting their tokens when executing token swaps. The liquidity pool is responsible for protecting liquidity providers' token reserves during swaps. There are other DeFi smart contracts that may use the pool as a price oracle. 
Here, we mainly consider Uniswap's Version 2 (V2) protocol, which is adopted in major DEXes on Ethereum networks, including Uniswap-V2~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2} and Pancakeswap~\cite{me:pancakeswap:1}. 
%We discuss Uniswap's Version 3 (V3) protocol in Appendix~\ref{appdx:uniswapv3YYY}.
The API functions in Uniswap-V2's pools and ERC20 tokens are presented in Table~\ref{tab:uniswapv2:api}. 

More specifically, Uniswap's pool supports two essential workflows: swap and manage liquidity.
In a {\it swap} workflow, a trader EOA calls the router, which works with the liquidity pool to jointly coordinate the issuance of deposit and withdrawal (i.e., transferring token $T0$ into the pool's account and transferring token $T1$ out of its account).

A liquidity provider EOA can call function \texttt{addLiquidity} to a pool by depositing tokens $T0$ and $T1$ at a certain rate. The provider receives a deposit certificate (called LP token). Thus, an $addLiquidity$ workflow also includes the invocations of token's \texttt{transfer} functions.

\noindent
{\bf Risky swaps and specification}: In general, a (normal) swap should consist of two token transfers, one transfer of token $T0$ from the trader to the pool and the other transfer of token $T1$ from the pool to the trader. Mapping the two transfers to transactions result in different swap types: 

\begin{itemize}[leftmargin=0cm]
%\setlength{\itemindent}{-1em}
\item
Type-I swap (atomic): In a Type-I swap, the two token transfers occur in the same blockchain transaction, and their value matches w.r.t. the current exchange rate. We call this type of swap an atomic swap. 
\item
Type-II swap (risky): In a Type-II swap, the two token transfers occur in separate blockchain transactions. Their value matches w.r.t. the current exchange rate. 
\item
Type-III swap (risky): In a Type-III swap, there is only one standalone token transfer observed, that is, the pool transfers out token $T1$ to a trader without receiving explicit transfer-in of token $T0$. 

In a Type-III swap, a deposit (withdrawal) can not be attributed to a withdrawal (deposit). This can be caused by a standalone deposit that does not match any subsequent withdrawal (a sub-case we call Underwater or U), or by a standalone withdrawal that does not match any previous deposit (sub-case Freeride or F), or by a pair of deposit and withdrawal where the deposited value exceeds the withdrawn value  (sub-case Overcharge or O), or by a pair of deposit and withdrawal where the withdrawn value exceeds the deposited value (sub-case Discount or D). 
\end{itemize}


\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/anomalies.eps}
\end{center}
\caption{Swaps of three types: Type II and III are risky swaps.}
\label{fig:swaps}
\end{figure}


Type-I swap runs the two transfers atomically in one transaction and is unlikely to constitute a token theft. Type-II and Type-III swaps are risky and could imply theft/attacks (as defined next). Specifically, in the Type-II swap, a malicious trader EOA could try to extract the value in the pool after the transaction that sends the first transfer and before the transaction that carries out the second transfer. In the Type-III swap, it is abnormal for the pool to send value to a potentially malicious trader without receiving their deposit token.

\noindent
{\bf Threat model}: The primary threat in this work is DEX-value theft among trader EOAs. A victim is a trader EOA who has deposited the token to the pool but is unable to withdraw the other token from the pool. An attacker is an EOA who aims at extracting value from the liquidity pool interacting with a victim trader. The attacker's capability is to monitor certain conditions on the DEX states in real-time, and upon the satisfaction of the conditions, send crafted transactions to the DEX to extract the value and claim it illicitly. 

\ignore{
\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/workflow5.eps}
\end{center}
\caption{Workflow of data analytics to detect risky swaps and attacks, as well as to analyze attackers'/victims' behavior.}
\label{fig:workflow:overall}
\end{figure*}
}

\noindent
{\bf System overview}: Recall the transaction-analytical pipeline overview in Figure~\ref{fig:workflow:overall}. The input data is more than $43$ million transactions with their event log crawled from \url{etherscan.io}, internal call sequences crawled from Google BigQuery services~\cite{me:bigquery:ethereumdataset}. The pipeline consists of three stages: 1) Detecting risky swaps, which joins and matchmakers token transfers to detect the risky swaps as defined above, 2) Discovering token-theft attacks, which characterizes the behavior of accounts involved in risky swaps against proposed attack patterns, and 3) Uncovering on-chain crimes, which exposes the attack strategies, criminal infrastructures and ecosystems. 
The three steps are described in \S~\ref{sec:detectriskyswap}, \S~\ref{sec:attack}, and \S~\ref{sec:behavior}.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.325\textwidth]{figures/automata3.eps}
\end{center}
\caption{Matchmaking in two rounds to detect risky swaps (Type-II and Type-III swaps).}
\label{fig:automata}
\end{figure}

\section{Detecting Risky Swaps}
\label{sec:detectriskyswap}

\label{sec:mmalgo}

{\bf Input data}:
Our input data is raw blockchain transactions including function-call sequences and logged smart contract events, which are accessible from Ethereum exploration web services~\cite{me:bigquery:ethereumdataset} and \url{etherscan.io}. Particularly, we only consider (and hence trust) the event log of liquidity-pool smart contract. 

{\bf Design goals and challenges}:
We aim at finding the incidents of risky swaps (Type II and Type III as previously defined) from the blockchain traces. A naive algorithm design is to reconstruct data records representing individual deposits and withdrawals, and to conduct matchmaking between them. The data records left unmatched are risky swaps (specifically, Type III swaps). However, there are challenges: 1) If we only consider the invocations of token \texttt{transfer} for deposits and withdrawals, false positives will be introduced in the results. For instance, the \texttt{transfer} calls serving $addLiquidity$ workflow will not match any withdrawal in a swap and can be falsely introduced in the detection result (as an artifact). 2) In theory, an atomic swap can contain an arbitrary number of deposits and withdrawals, as long as their total value matches. Matchmaking for this general case can be extremely unscalable. That is, the matchmaking should join the {\it powerset} of deposits and the powerset of withdrawals, and the powerset of $n$ deposits/withdrawals is of $2^n$ elements. 

Our goal is to design an efficient and effective detection algorithm that does not introduce false positives in the results. To do so, our key observation is two-fold: 1) Perform matchmaking on both swap and add/remove liquidity data. 2) Uniswap's pool executes deposits and withdrawals in a single thread, thus a deposit can only be matched to a subsequent withdrawal before the next deposit. This greatly saves the search space and makes it possible to run the matchmaking in a linear time. 

{\bf The algorithm}:
Given the raw blockchain data (transactions and events), we first reconstruct deposit and withdrawal records. A deposit record is constructed by the invocations of a pool's tokens' \texttt{transfer}/\texttt{transferFrom}/$mint$ functions where the pool's account is the token receiver. A candidate withdrawal record is constructed by the invocations of a pool's \texttt{swap} or \texttt{addLiquidity} function. We also use the pool's events to reconstruct the mapping between deposit value and withdrawal value in the withdrawal record.

After the data preparation, the algorithm runs in two rounds of matchmaking. In the first round, it equi-joins the $deposit$ records with $withdrawal$ records by their transaction IDs. The join conditions also include the equality of value in both records. It also considers the case of addLiquidity. If matched, it emits the pair as a Type-I swap (or matched addLiquidity) and removes it from the current dataset.

In the second round, it conducts matchmaking across transactions. Based on the linear algorithm design, it scans through the $deposit$/$withdrawal$ records sorted by time; for each two consecutive $deposit$ records, it matches the earlier $deposit$ record with the powerset of all $withdrawal$ records falling in this period. We also run the reserved process where $deposit$ records between two consecutive $withdrawal$ records are matched. For each match, it emits the matched records as a Type-II swap (or matched \texttt{addLiquidity}) and removes them from the current dataset. In the end, what's left in the dataset are Type-III swaps. 
%Figure~\ref{fig:joinproblem} depicts the matchmaking process, and t
The pseudocode is in Appendix \S~\ref{sec:algorithm:detect}.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.3\textwidth]{figures/join_problem2.eps}
\caption{Matchmaking deposits and withdrawals: addL is function call \texttt{addLiquidity} and tf is function call \texttt{transfer}.}
\label{fig:joinproblem}
\end{figure}

{\it An example}: In Figure~\ref{fig:joinproblem} shows two example traces of deposit and withdrawal records. The two traces are aligned and sorted by time. Assume each record is handled by a distinct transaction. The figure shows two matched cases (in green). The first transfer $tf1$ is a standalone deposit (i.e., Underwater) and the second swap is a standalone withdrawal (Freeride). In the red shade is a pair of deposit and withdrawal whose value does not match (Discount).

\subsection{Results}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Swaps (Types I, II, III) on Uniswap-V2-based DEXes; in red are risky swaps exposing extractable value to attackers.}
\label{tab:swapsrisky}\centering{\footnotesize
\begin{tabularx}{0.5\textwidth}{ |l|l|l|l|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
  Swap types & \#$deposit$ & \#$withdrawal$ & Value/diff (\$M) & Causes \\ \hline
  \multicolumn{5}{|l|}{Uniswap-V2~\cite{me:dex:uniswap,Adams2020UniswapVC} (on Ethereum mainnet)}   \\  \hline
 I  & $52.7*10^6$  & $52.7*10^6$   & $6.18*10^8$  & Atomic \\ \hline
 II  & $762$  & $761$   & {\bf $0.486$}  & \textcolor{red}{External transfer} \\ \hline
 II  & $35$  & $35$   & {\bf $0.205$}  & \textcolor{red}{Router bug} \\ \hline
 III (O) & $2.01*10^5$ & $2.01*10^5$ & $23.3$/$3.64$ & Fees \\ \hline
 III (D) & $3879$ & $3879$ & {\bf $0.185$/$0.094$} & \textcolor{red}{Rebase} \\ \hline
 III (F) & $4767$ & $0$ & {\bf $1.26$} & \textcolor{red}{Rebase/interest} \\  \hline
   \multicolumn{5}{|l|}{Pancakeswap~\cite{me:pancakeswap:1} (on Binance Smart Chain~\cite{me:bsc:1})}   \\  \hline
 I  & $2.97*10^6$  & $2.97*10^6$   & $7.34*10^7$  & Atomic \\ \hline
 II  & $364$  & $364$   & {\bf $0.047$}  & \\ \hline
 III (D) & $1.7*10^5$ & $1.7*10^5$ & {\bf $1.16$/$0.99$} & \textcolor{red}{Rebase} \\ \hline
 III (F) & $0$ & $2.82*10^5$ & {\bf $0.53$} & \textcolor{red}{Rebase} \\ \hline
 III (U) & $2507$ & $0$ & {\bf $0.12$} & \textcolor{red}{Airdrop (sync'd)} \\ \hline
  \multicolumn{5}{|l|}{Sushiswap (on Ethereum mainnet)~\cite{me:sushiswap:1,me:sushiswap:2}}   \\  \hline
 I  & $3.73*10^6$  & $3.73*10^6$   & $1.69*10^5$  & Atomic \\ \hline
 II  & $16$  & $16$   & {\bf $0.064$}  & \\ \hline
 III (D) & $57$ & $57$ & {\bf $51$/$7.6*10^{-3}$} & \textcolor{red}{Rebase/interest} \\ \hline
 III (F) & $0$ & $193$ & {\bf $0.82*10^{-3}$} & \textcolor{red}{Rebase} \\ \hline
 III (U) & $61$ & $0$ & {\bf $2.9*10^{-2}$} & \textcolor{red}{Bug/Airdrop} \\ \hline
\end{tabularx}
}
\end{table}

We analyze the traces of three Uniswap-based DEXes using the methods described previously. The three DEXes are Uniswap-V2, Sushiswap and the Pancakeswap. 
In particular, we set the minimal $10\%$ value difference to determine match/mismatch. If a deposit (withdrawal) has $10\%$ higher value than the paired withdrawal (deposit), it is considered a mismatched case (Type-III). $10\%$ is empirically set as most tokens and routers charge less than $10\%$ fees.
For each DEX, we report the number of swaps and their total value under each category. 
To estimate the value, we crawl the historical exchange rates reported by etherscan (\url{https://etherscan.io/tokens}) on the same day/hour of the reported swap. The results are presented in Table~\ref{tab:swapsrisky}.

It can be seen that the majority of swaps, about $97.9\%$, are atomic (Type-I). The rest are risky swaps (Type-II and Type-III) worth a total of 26.2 million USD, among which the majority are caused by high fees as we inspected. We inspected the rest of risky swaps, which are more interesting and expose four exploitable deposit patterns.

\ignore{
In Table~\ref{tab:swaprisky}, on Uniswap-V2, the majority of swaps, with total value of $618$ billion USD and in more than 0.5 billion Ethereum transactions (as in the third row of the table), are atomic ones, each of which is carried out by one transaction calling a router smart contract (recall Figure~\ref{fig:uniswap2}). Besides, as shown in the fourth row, there are $761$ atomic swaps, each of which is carried out by two or three transactions that directly call Uniswap's pool smart contract. The fifth row shows $35$ swaps that match in value but invoke a router smart contract with ``partly error.'' The case of ``partly error'' router smart contract is discussed in more details in \S~\ref{sec:partlyerror}.

On Uniswap-V2, more than $20$ thousand swaps are overcharge, which are caused by the particularly high fees by the operating routers or tokens. For instance, some tokens enforce a fee scheme to penalize the token deposit and to encourage the withdrawal. 

3879 swaps are discount, where a trader account receives profit. A primary cause is a token's rebase operation that occurs before the swap, as will be described in details in \S~\ref{sec:rebase}.

In the eighth row, $4767$ swaps are standalone deposit operations  (i.e., Freeride) that directly call the liquidity pool's swap function. In total, they are worth $1.26$ million USD. The profit come from the tokens' non-standard rebase operation or interest behavior.
}

%\subsubsection{Causes: Patterns of Profitable Deposit}

\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.475\textwidth]{figures/victimpatterns.eps}
\end{center}
\caption{Patterns of profitable deposits: $R$ is the router smart contract, $T0$/$T1$ are the two tokens in the target liquidity pool}
\label{fig:patterns}
\end{figure}

\subsubsection{Non-standard Balance Updates (Cause $P_1$)}
\label{sec:cases:rebase}

In many real-world tokens, account balance can be changed by the non-standard operations beyond token transfer. We describe two examples. {\it Rebase}: For instance, token balance can be elastically adjusted by token issuers, for purposes such as to stabilize the token's exchange rates against other tokens. In practice, token rebase is such a non-standard balance-changing function, supported in some widely used tokens, such as AMPL~\cite{me:ampl:token}. When a token, say $T0$, is rebased, a Uniswap's relevant pool, say for tokens $T0$ and $T1$, could have its $T0$ balance increased. Uniswap falsely assumes that this balance increase is due to some accounts that swap token $T0$ for token $T1$. Uniswap's pool would mistakenly admit anyone who requests to withdraw token $T1$ after the rebase of $T0$.

{\it Token shareholder}: 
As another example, there are tokens that charge ``tax'' to average owner accounts and redistribute the ``tax'' income among privileged accounts of shareholders. Specifically, these tokens support two kinds of owners, average owner and token shareholders. When there is a transfer, the token smart contract charges a certain amount of fees. The fees are redistributed to the privileged accounts of token shareholders. Thus, a transfer between average accounts would update the balance of all shareholders' accounts. In a Uniswap's pool of token types $T0$ and $T1$, if the pool's account in $T0$ is a shareholder, any transfers in $T0$ would increase the pool's balance and create a profitable opportunity.
 
Furthermore, even when the pool receives a token deposit, the deposit may not be intended as a part of swap. For instance, airdrop is a common practice to promote the use of a new token type, in which token issuers periodically give away newly minted tokens to the current token owners (e.g., in Tokens MILK2~\cite{me:token:milk2} and 3Cs~\cite{me:token:3cs}). When a token, say $T0$, is airdropped into a Uniswap's pool, the pool holding tokens $T0$ and $T1$ would mistakenly treat the transfer as a part of swap from token $T0$ to $T1$. Thus, the pool would admit anyone's request to withdraw token $T1$ after airdrop of token $T0$ to the pool's account.

In general, these non-standard token operations allow to update the pool's balance but do not intend to withdraw the same value from the pool. We name this pattern of extractable value by $P_1$.

%In general, there can be an explicit token operation that increases the pool's balance of token $X$, but is not with the intention of swap value. Thus, an attacker observing the occurrence of such an exploitable operation can strategically extract value from the pool and gain illicit profit. We name this attack pattern by $P_1$. 

\subsubsection{Implicit Token Balance Updates ($P_2$)}
Beyond $P_1$, there are implicit approaches to update the balance. Many tokens are bearing interest. That is, the balance in the token smart contract increases at a certain rate as the time goes by. Suppose a Uniswap pool is of token $T0$ and $T1$ where $T0$ is interest bearing. Similar to $P_1$, the Uniswap pool observing the increase of token $T0$ would admit the withdrawal of token $T1$ by anyone who requests it, including a value-extracting attacker. We call this attacker's pattern by $P_2$, which is different from $P_1$. In $P_2$, the attacker simply waits long enough to harvest the extractable value from token interest. 

\subsubsection{External Transfer for Deposit ($P_3$)}

In Uniswap, a trader can externally call token $T0$'s transfer function to make deposit so that she can in a separate transaction withdraw token $T1$. We call the pattern of a victim trader sending a transaction to externally transfer token $T0$ by $P_3$. When $P_3$ occurs, a malicious account can send the withdraw transaction ahead of the victim's one, to claim the value in the pool.  This attack is possible because a Uniswap pool receiving a deposit of $T0$ will approve of the next withdrawal of token $T1$, no matter who sends it. 

\subsubsection{Buggy Router Contracts ($P_4$)}

In the above three patterns, the victim may externally call token $T0$'s functions. In the fourth pattern $P_4$, the trader delegates the handling of swap to a router smart contract that is buggy and violates atomicity. After the trader EOA's transaction, the router smart contract successfully completes the deposit of Token $T0$ but fails at requesting the withdrawal of Token $T1$. Thus, anyone who requests the token withdrawal in the next transaction, including an attacker EOA, would succeed in grabbing the value illicitly. 

\section{Discovering Attacks}
\label{sec:attack}

\subsection{The Problem}
\label{sec:discoveryproblem}

\noindent{\bf Formulating attack detection problem}: 
The detected risky swaps present value that {\it can} potentially be extracted and grabbed by attackers. However, whether the value is {\it actually} extracted by attackers, or equivalently, whether the risky swaps are actual attack instances, is a different problem. 

Consider as an example that a token issuer sends a vulnerable rebase transaction to a pool's token, followed by a withdrawal transaction sent by account $X$ (i.e., $P_1$). $X$ may or may not be the token issuer. The former case is not an attack, as the token issuer aware of the risky rebase sends the withdrawal to remedy the risk. The latter case may be an attack. For other situations including $P_3$ and $P_4$, the same applies that a risky swap can be attributed differently.
\ignore{
For instance, in $P_1$, after a token issuer sends an exploitable rebase transaction, it is equally likely one of the following cases occur: 1) the token issuer aware of rebase being exploitable quickly sends a swap request herself to claim the value in the Uniswap pool. 2) An attacker observing the occurrence of rebase operation calls the liquidity pool to withdraw the value there. The former case is not an attack, while the latter one is. In other cases, the same apply: In $P_3$, if the trader sends another transaction to withdraw the value in token $T1$ right after the transaction of depositing $T0$, it is a benign case. But if it is an attacker account who withdraws after the external deposit, it constitutes an attack. In $P_4$, if the trader observing the router exception and immediately send a ``make-up'' transaction to claim the value herself, it is a benign case. But if it is a third-party ill-intended account who sends the withdrawal transaction, it constitutes an attack.
}

Distinguishing attacks from benign cases entails checking two essential conditions: {\bf 1) Whether two accounts are controlled by two distinct physical users}: It cannot be an attack if the trader account who makes the profitable deposit in token $T0$ is controlled by the same physical user with the account who succeed in withdrawing the value in token $T1$. 
Thus, attack detection becomes the problem of linking two blockchain accounts of the same physical user, which is known to be an intractable problem if the only information known is on-chain data.
{\bf 2) What's a transaction sender's intention}: That is, whether a withdrawal transaction is intended as an attack. Even when the withdrawer and depositor accounts are not the same physical user, they can be friends in the real life, which makes the swap non-attack. Thus, it entails detecting the depositor account's intention in sending the withdraw request, which however can be hidden opaque and pose challenges to detection.

{\bf Feasibility of existing approaches}: 
On checking Condition 1), there are existing works that tackle the recovery of account linkage by heuristics specific to Bitcoin's UTXO model~\cite{DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13}. The only work for Ethereum~\cite{DBLP:conf/fc/Victor20} presents a linkage heuristic exploiting some DEXes deposit addresses. Specifically, on order book-based DEXes (i.e., IDEX and EtherDelta), trader Alice swapping token $T0$ for $T1$ can specify the so-called deposit address who receives $T1$. Assuming a swap is normal, the sharing of deposit addresses by two traders implies that the two traders are controlled by the same physical user. This work is different from our attack detection problem, where the deposit address heuristic is to detect the case that two accounts are linked, while our problem is to detect if two accounts are unlinked. More importantly, the deposit address heuristic works only under the assumption of normal swaps, while our work deals with risky swaps. Given a risky swap, the deposit address of a swap refers to the attacker. Thus, when an attacker targets two victim traders, it could appear that two traders share the same deposit address. In this attack, the two victim traders do not have to be linked to the same off-chain user.

On checking Condition 2), there are existing works on threat intelligence on blockchains by characterizing attackers' behavior~\cite{DBLP:conf/uss/SuSDL0XL21}. However, their targets are program-level attacks such as reentrancy attacks, and their attack strategies don't apply to the DEX context of this work.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.4\textwidth]{figures/indicators.eps}
\end{center}
\caption{Attack strategies (A1/A2/A3) and indicators}
\label{fig:indicators}
\end{figure}

\subsection{The Approach}

We discover attacks by designing attack strategies specifically for different profitable deposits and use them as attack indicators to match the observable attacker behavior on-chain. 

{\bf Design rationale: Attack strategies}: Recall that each risky swap involves with a profitable deposit followed by a withdrawal that reaps the profit. An attacker needs to strategically send the withdrawal to ensure high success rates by properly monitoring the profitable deposits. We consider the following three attack strategies:

\begin{itemize}[leftmargin=0cm]
%\setlength{\itemindent}{0em}
\item
 {\bf A1) Aggressive attacker (monitoring deposits)}: The attacker directly monitors the mempool for the profitable deposits. In this strategy, the attacker monitors different cases of profitable deposits, such as $P_1$/$P_2$/$P_3$/$P_4$. The attacker launches a node joining the Ethereum blockchain network and monitors the node's mempool so that the profitable-deposit transaction can be detected as soon as they are propagated in the blockchain network. 

Strategy A1 entails the attacker to customize the monitored conditions to different causes. It minimizes the time window between the exploited deposit and withdrawal, and ensures a high success rate in the presence of competitors.

\item{\bf A2)
General-purpose attacker (monitoring pool)}: The attacker monitors the Ethereum's smart contract state to check if the pool is profitable. For instance, when a rebase transaction is executed in the blockchain, it could increase the balance in the token smart contract and leave the reserve in the pool smart contract unchanged. By detecting the difference between token balance and reserve, the attacker ensures sending a withdrawal can succeed.

Strategy A2 is generalizable to different profitable deposits, in the sense that the attacker monitors a single condition that all different profitable deposits will trigger. However, this strategy works only after the profitable deposit transaction is executed and included in the blockchain. So an aggressive attacker (A1) can frontrun a general-purpose attacker (A2).

\item{\bf A3)
Lucky trader}: The trader does not intentionally observe conditions on pool profitability but is lucky in grabbing the profit by inserting a withdrawal after the profitable deposit. The delay between the withdrawal and victim deposit can be arbitrary. 
\end{itemize}

{\bf Proposed attack indicators}: 
An account's strategy, which normally occurs in the blackbox off-chain state, is not directly observable from the on-chain traces. We distill observable information and design indicators to infer attack strategies.

To start with, an aggressive attacker monitoring the off-chain mempool states cannot be observed from the on-chain traces. Likewise, a general-purpose attacker who may choose to issue RPC calls to read on-chain data is also unobservable. For these cases, we  collect the gap between the block including deposit transactions and the block including the exploit withdrawal transactions as the metric to infer the presence of an attack and further the attack strategies. For instance, if the block gap is always $0$, it indicates the case is exclusively an aggressive attack. If the deposit is token interest and the block gap is always large, it indicates an aggressive attack exploiting token interest. Otherwise, if the block gap is randomly distributed, it is likely to be a lucky trader. Based on the heuristics, we propose the following three indicators:

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I1 (Strong): An account whose withdrawal transactions occur consistently within $G$ blocks after profitable deposits (i.e., block gap smaller than $G$) and whose victim deposits are non-interest is likely to be an attacker. 
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I2 (Strong):
Indicator I2) An account whose withdrawal transactions occur consistently more than $G'$ blocks after profitable deposits (i.e., block gap larger than $G'$) and whose victim deposits are based on token interests is likely to be an attacker.
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I3: 
An account whose withdrawal transactions appear an arbitrary number of blocks after the profitable deposits are likely to be a lucky trader.
In other words, an account whose block gaps have a large deviation is likely to be a lucky trader.
}}\end{center}

In practice, many accounts use delegate smart contracts on-chain to relay their payload (of malicious withdrawals). The delegate smart contracts make attack strategies observable. We propose the following indicators to take advantage of this fact. 

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I4 (Strong):
An account who attempts to withdraw through a smart contract that checks both pool reserves (i.e., calling \texttt{pool.getReserves()}) and token balances (calling \texttt{erc20token.balanceOf()}) is likely a general-purpose attacker. Note that this indicator does not require the smart contract to actually withdraw the token $T1$. 
}}\end{center}

The intuition of the above indicator is that a general-purpose attacker uses the pool's \texttt{getReserves()} function and token's \texttt{balanceOf()} function to obtain the token reserve and balance, respectively. This shows the account's intention to calculate pool profitability and is an indicator of general-purpose attacker. 
%Note that the indicator is not necessary (i.e., causing false negatives), as a general-purpose attacker can issue RPC queries to read reserves and balances, leaving no trace on-chain.

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I5: An account whose withdrawal transactions exclude any token deposit is likely to be an attacker.
 
An account whose withdrawal transactions also include token deposits is likely to be a lucky trader, even though the withdrawal is of higher value than the deposit.
}}\end{center}

At last, we propose a heuristic that intentional attackers would victimize a diverse set of accounts while a lucky trader may victimize a fixed type of accounts (e.g., in the same pool).

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I6: If an account sends withdrawals in a large number of risky swaps, the account is an attacker.
}}\end{center}


{\bf Attack discovery algorithm}: We materialize the indicators in a holistic attack discovery algorithm. The algorithm takes as input the detected risky swaps from the previous phase (\S~\ref{sec:detectriskyswap}) and produces the labels for swaps and accounts what attack strategies are used.

Specifically, recall that each risky swap consists of a profitable deposit and a (successful) withdrawal. We expand it by adding all the withdrawal attempts, no matter success or failure, on the same pool by calling its \texttt{getReserves} or \texttt{swap} functions between time $t_1$ and $t_2$ where $t_1$/$t_2$ is the time when the current/next deposit occurs. We ignore the atomic swaps (Type-I) between $t_1$ and $t_2$. Hence for each risky swap, we obtain a list of accounts who send the withdrawal or expanded withdrawal attempt. For each account and each associated swap, the algorithm checks the indicators and reports the number of attacker labels the account is tagged with. In particular, indicator I1/I2 produces the block gap averaged over all the swaps the account is involved when the deposit is non-interest/interest. 

\lstset{style=mystyle}
\begin{lstlisting}[caption=Pseudocode to discover attacks,
                   %linerange={1-30},
                   numbers=none,
                   %firstnumber=1,
                   deletekeywords={[2]INT},
                   morekeywords={clustered},
                   framesep=2pt,
                   xleftmargin=5pt,
                   framexleftmargin=5pt,
                   frame=tb,
                   framerule=0pt, 
                   label=code:discoverattacks,
                   float,floatplacement=H
                   ]
void AttackDiscovery(RiskySwap[] swaps, int th1, int th2){
  for(RiskySwap s in swaps){
  Mapping blockGaps;

  for(Account w in s.getWithdrawers())
    if(isCA(w)) //I4
      if(findCall(w, s.getPool(), "getReserve").getTx().checkCall(w, s.pool().tokens(), "balanceOf()")) 
        emit(w, "Attacker");
    //I1
    Block depositTime=s.getDeposit().getBlock();
    Block withdrawTime=w.getBlock();
    blockGaps.getValue(w).add(withdrawTime-depositTime));
    //I2
    numberSwaps.getValue(w).increment();
  }

  for(Account w in blockGaps.keySet()){
    blockGap.getValue(w).divideBy(numberSwaps.getValue(w));
    if(blockGap.getValue(w) > th1) emit (w, "Attacker");
    if(numberSwaps.getValue(w) > th2) emit (w, "Attacker");
}}
\end{lstlisting}


\subsection{Results}

\subsubsection{Detected Attacks}
\begin{table*}[h]
\caption{Attacker characterization: A victim can be a normal token owner (N) or token issuer (I). The numbers reported under I1-I6 columns are described next: Given an account $A$, I1 is the average block gap of $A$'s transactions matching $P_1$, $P_3$ and $P_4$; I2 is the average block gap of $A$'s transactions matching $P_2$; I3 means the deviation of the block gaps reported under I1 and I2; I4 is the number of $A$'s transactions that read both pool's reserves and token balances; I5 reports whether $A$ has sent at least one transaction to deposit before withdrawal; I6 reports the number of risky swaps. Bold are strong cases suggesting the account is an attacker.}
\label{tab:attackerview}
\centering{\footnotesize
\begin{tabular}{|p{1cm}|p{1.1cm}|p{2.1cm}|p{0.4cm}|p{0.5cm}|p{0.5cm}|p{1.2cm}|p{0.2cm}|p{0.5cm}|p{0.8cm}|p{1.4cm}|p{1.1cm}|}
\hline
Accounts & Value & {Profitable} & \multicolumn{6}{c|}{Attack indicators} &\# pools &\# victims & Label \\
\cline{4-9}
(Mules) & ($10^3$ USD) & deposit &I1 & I2 & I3 & I4 & I5 & I6 & &normal/issuer & (strategy) \\ \hline 
$0x9799$ & 556 & $33P_1,4P_2,6P_4$ &422 &371 & 1290& 0 &N& 43 & 4 & 0/7 & A3\\
\hline 
$0x2a2e$ & 239 & $32P_1$ &{\bf 0.03} & &0.2 & 32 ({\bf 100\%}) &Y& 32 & 1 & 0 /3 & A1\\
\hline 
$0xdb40$ & 113 & $12P_1,2P_2,3P_3$ &{\bf 2.5} &{\bf 665} &2.0 & 17 ({\bf 100\%})&Y& 17 & 1 & 0/4 & A1 \\
\hline 
$0x0c08$ & 101 & $3P_1,1P_4$ &{\bf 1.5} & &0.7 & 0 &N& 4 & 1 & 1/1 & A2 \\
\hline 
$0x5617$ & 101 & $53P_1,4P_2,2P_3,2P_4$ &13 &{\bf 1574} &24 & 0 &N& 61 & 3 & 2/4 & A1 \\
\hline 
$0xb6bf$ & 20 & $1091P_1,131P_2,9P_4$ &224 &{\bf 600} &471 & 1231 ({\bf 100\%}) &Y& 1231 & 9 & 12/5 & A2\\
\hline 
$0xc762$ & 16 & $64P_1,6P_2,13P_4$ &{\bf 3.0} & 5.3 &437 & 83 ({\bf 100\%}) &Y& 83 & 19& 0/4 & A2\\
\hline 
$0xa32d$ & 6 & $208P_2$ & & {\bf 942} & & 208 ({\bf 100\%}) &Y& 208 & 1 & 0/0 & A2\\
\hline
\ignore{
\multicolumn{10}{|l|}{\it Least frequently swapping account}\\
\hline
0xc408 & .8 & $P_1$  & 0 & 1&  &&  N   &1 &  &  0 + 1 & \\
\hline                                                    
0x02ef & .1   &  $43P_1, 9P_4$  & 2.6  &&2.4  &  52&Y & 52       &  &  1 + 0 & \\
\hline                                                    
0x2839 & .04 & $P_1$ & 0   &0  &   &&N     &1    &  &  0 + 1 & \\
\hline                                                    
0x042d & .03 & $P_1$ & 130 &0  &  & 1    &N&  &  &  0 + 1 & \\
\hline                                                    
0x5b1b & .01 & $P_1$ & 206 &0  &   & 1   &N&      &  &  0 + 1 & \\
\hline                                                    
0x6cea & .01 & $P_1$ & 904 &0  &   & 1     &N& &  &  0 + 1 & \\
\hline                                                    
0xf39f & .01 & $P_3$ & 0   &0  &   & 1     &N&    &  &  1 + 0 & \\
\hline                                                    
}
\end{tabular}%
}
\end{table*}


We present our analysis result in Table~\ref{tab:attackerview} which characterizes the most frequent accounts involved in risky swaps. The metrics include value stolen, causes, attacker indicators, the number of pools attacked, the number of victim accounts, and the label whether the account is an attacker.  From the table, we analyze the attackers' strategy of several selected accounts.

{\bf Case 1: Agg. attacker (A1) w. zero block gap}: Account $0x2a2e$ is involved in $32$ risky swaps (I6) and gains more than $2.39*10^5$ USD worth of illicit tokens. All $32$ swaps from this account are sent via a smart contract which checks the pool's profitability before withdrawal (I4). In terms of timing, the malicious withdrawals are always sent in the same block with the risky, profitable deposit. We believe account $0x2a2e$ aggressively monitors the mempool for the target tokens' rebase transactions, and if found, sends withdrawal transactions immediately to ``backrun'' the deposits and claim the profit. 

{\bf Case 2: General attacker (A2) w. off-chain monitoring}: Account $0x0c08$ has withdrawn four times and grabbed tokens of $1.01*10^5$ USD. The account directly and externally calls Uniswap pool's swap function to withdraw, without checking pool profitability on-chain. The withdrawals are included in exactly one block after the one that includes the risky deposit. We believe Account $0x0c08$'s strategy is to monitor the pool profitability from an off-chain vantage point and to immediately send withdrawal by external calls. Because the account monitors the pool profitability instead of the cause (risky deposit), it has to wait until the inclusion of risky deposit that updates the pool state to be profitable. This explains why the inclusion of withdrawal has to be one block after the one including the risky deposit.

{\bf Case 3: Agg. attacker (A1) stealing interest}: Both Accounts $0xdb40$ and $0x5617$ have extracted value from interest bearing tokens. Their block gaps are large ($665$ and $1574$, respectively). Given that there are enough samples, this consistent behavior shows both accounts' attack strategy to wait long enough for the token interest to accumulate and for the extractable value to be large enough before acting on it.

{\bf Case 4: Adapting strategies}: For all accounts with indicators I1 and I2 in the table, it is clear that the block gaps for different causes (I1 and I2) differ: The block gaps for non-interest causes are consistently much shorter than those for token interests. It implies that the attackers are aware of the situation (which causes to exploit) and tailor their strategies to it.

{\bf Case 5: Lucky trader (A3)}: Account $0x9799$ is unlikely an intentional attacker: First, it does not read the token balance or check the pool's profitability before the withdrawal. Second, the block gap between profitable deposit and malicious withdrawal is large, at hundreds of blocks apart. In addition, the smart contract Account $0x9799$ relays her withdrawal requests also makes deposit to the pool. All these indicators show that $0x9799$ is unlikely an intentional attacker, but instead a lucky trader who gets profits by accidents.

\subsubsection{Block Gaps}

\begin{figure}[!ht]
  \begin{center}
    \subfloat[Block gaps and the number of competing attackers]{%
\includegraphics[width=0.245\textwidth]{figures/figure_allrebase_blockdif.eps}
\label{fig:blockdif_1}
    }%
    %\hspace{-0.2cm}%
    \subfloat[Block gaps and value stolen]{%
\includegraphics[width=0.245\textwidth]{figures/figure_value_blockdif.eps}
\label{fig:blockdif_2}
    }%
  \end{center}
  \caption{Block gaps and affecting factors}\label{fig:complex}\vspace{-0.10in}
\end{figure}

Recall that each of theft attack runs in two transactions: The first transaction that creates extractible value, and the second transaction that withdraws the value and steals it. Given each detected attack (described from the previous subsection), we measure the gap of the two blocks that respectively include the attack's two transactions, namely block gap. We further report two metrics, that is, the number of competing attackers and the value stolen. Particularly, for each profitable deposit transaction, say $tx$, we find transactions sent by competing attackers. Here, a competing attacker either directly sends a transaction to withdraw the extractible value created by $tx$ but fails, or sends a transaction to read the token balance and pool reserve (which shows the intention to withdraw the value). 

We report the block gaps with the varying number of competitors in Figure~\ref{fig:blockdif_1}. A larger dot in a X/Y coordinate in the figure represents more attacks found with the same X/Y value. The result shows that when there are many competing attackers, the block gap tends to be small. This could be explained: Because the first attacker wins, the more attackers there are, the earlier the withdraw transaction is sent, namely smaller block gap.
The result also shows that with few competing attackers comes a large range of block gaps.

We then report the block gaps with varying value stolen in Figure~\ref{fig:blockdif_2}. The result shows that when the stolen value is large, the block gap tends to be small. A possible explanation is that the higher extractible value gives the attacker more incentives to send the withdrawal transaction with higher fee and to frontrun other potential thieves.
 
\subsubsection{Attacker/Victim Behavior over Time}

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_attacker_timeline.eps}
\end{center}
\caption{Attack timeline of top-10 attackers. In the Y axis, attacker accounts are ordered by total value stolen.
Data from 07/09/2020 (block 10422671) - 06/29/2021 (block 12727620).}
\label{fig:attack}
\end{figure*}

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_victim_timeline.eps}
\end{center}
\caption{Attack timeline of top-10 victims. In the Y axis, victim accounts are ordered by total value stolen.
Data from 07/29/2020 (block 10553883) - 01/10/2022 (block 13979019).}
\label{fig:victim}
\end{figure*}

We plot the timeline of the top-10 attackers' activities in Figure~\ref{fig:attack}. The attackers are ranked by the total value stolen, with attacker $0x9799$ being the top-1. Each dot represents a detected attack sent by the attacker's account. The size of the dot represents stolen value. Color represents the exploit pattern. The most successful attacker ($0x9799$) steals value despite through different causes (including rebase, airdrop, etc.) The attacker's activities last about 
$1.1*10^6$ blocks, which amount to six months. The second attacker ($0x2a2e$) concentrates all her attacks to a one-month span. She exploits exclusively the value created by rebase operations. The third attacker ($0xdb40$) mount attacks sporadically and target value created through two causes: Token interest and rebase operations. The ninth attacker exploits partly errors to gain illicit profit. The tenth attacker exclusively grabs value from token interest in a three-month period. As a result, most top attackers mount multiple attacks consistently, which show the attacks are intended and not by accident.

We additionally study top victims' behavior. The victims are ranked by the value stolen. In Figure~\ref{fig:victim}, we plot in dots the transactions sent by victims whose deposit are stolen in identified attacks. Different color represents different causes. Additionally, in green hollow circles, we plot the normal transactions sent by the victims and related to Uniswap. The result shows that most victims change behavior after an attack/theft. For instance, victim accounts, including $0x0cd4$ and $0x80cc$, all stop using the vulnerable interface (e.g., partly error) to send deposit after an attack. However, other victims can repeatedly create extractible value that gets stolen. For instance, account $0x66ac$ repeatedly airdrop tokens to the Uniswap pool, which gets stolen. 

\subsubsection{Value Received by Pools}

\begin{table}[!htbp] %force in current page, disable float.
\centering{
\begin{tabularx}{0.4\textwidth}{ |l|l|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
\hline
Destination & Rebase ($P_1$) & External transfer ($P_3$) \\
\hline
External attackers & \$1.11M & \$0.32M \\
\hline
Pools & \$4.57M & \$1.19M \\
\hline
\end{tabularx}
}
\caption{Extractable value and its destinations}
\label{tab:extractable_value}
\end{table}
\begin{figure}[!htbp]
\begin{center}
  \subfloat[Value created by rebase ($P_1$)]{%
     \includegraphics[width=0.245\textwidth]{figures/figure_rebase_seg.eps}
    \label{fig:moneyflow_1}
  }%
  \subfloat[Value created by external transfers ($P_3$): all pools are between token $XX$ and $WETH$, where $XX$ is the tick on the $x$ axis.]{%
    \includegraphics[width=0.245\textwidth]{figures/figure_underwater_seg.eps}
     \label{fig:moneyflow_2}
     }%
\end{center}
\caption{Extractible value received by the pool versus that by attacker accounts}\label{fig:complex}\vspace{-0.10in}
\end{figure}


Extractible value can be claimed by any account, including an external attacker and the pool itself. Our measurement result so far captures the former case. In this experiment, we measure the extractible value that goes to the pool.

A pool can claim extractible value by calling the \texttt{sync} function, which synchronizes the pool reserve and token balance. In Uniswap, there are three circumstances \texttt{sync} is called: a standalone call to \texttt{sync} in a transaction, \texttt{sync} called after a \texttt{swap} in the same transaction, \texttt{sync} called after an \texttt{addLiquidity} call in the same transaction. Informally, we calculate the extractible value that goes to the pool in the following method: We obtain the value of pool reserve before and after the transaction. We also parse the function call arguments from the transaction data field. We can cross-check the pre-state, post-state and function arguments, to detect the mismatch, which can be attributed to the extractible value. For instance, a normal \texttt{swap} in Uniswap does not change the product in AMM, and a spurious \texttt{swap} that the pool receives extractible value can be detected by the violation of product equality.

Using the above method, we measure the total extractible value claimed by the pool under different patterns, including $P_1$ and $P_3$. The result is presented in Table~\ref{tab:extractable_value}: The total value claimed by the pools is consistently more than $3\times$ of that by external attackers. This suggests ``room'' for the current Uniswap thief to increase their revenue. We further show the total extractable value by different pools/tokens. In Figure~\ref{fig:moneyflow_1}, we plot the extractable value created by different rebase-enabled tokens (Pattern $P_1$). Token $AMPL$ has the most extractable value which is exclusively claimed back by the pool; very little value is claimed by external attackers -- this is due to that when token issuers call \texttt{rebase}, they also explicitly call Uniswap's \texttt{sync} function against the popular AMPL pools.\yuzhe{Double-check this sentence}. Token $BASE$ is the second highest in total extractable value and has the highest value stolen by attackers. In Figure~\ref{fig:moneyflow_2}, we plot the extractable value created by external transfers (Pattern $P_3$) against different pools. Here, the top-value pools we found are between token $WETH$ and another token. The most vulnerable pool is between token $ICE$ and $WETH$, whose extractable value accumulate to $4*10^5$ USD, among which $\frac{3}{4}$ is stolen by external attackers. For other pools, most extractable value is reclaimed by the pool.

\section{Characterizing Crimes}
\label{sec:behavior}

We further expand the scope of each attack instance by tracing the money flow and smart contract lineage. The goal is to uncover the attack business.

\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.495\textwidth]{figures/UniswapV2attacker3.eps}
\end{center}
\caption{Attack campaign template: Preparing, mounting and wrapping up theft attacks.}
\label{fig:business}
\end{figure}

Given an attack instance with attacker accounts $\{A\}$, we construct an expanded attack graph by adding the following information: 1) the transactions that pay Ether or tokens to the attacker accounts, 2) the transactions that deploy the smart contracts used in the attack, and 3) the transactions that are sent by the mule accounts who receive the stolen tokens after the attack. These new transactions would add into the graph a set of new accounts, be it either the transaction sender or receiver. We iteratively apply this graph-expansion process, until it reaches the ``hub-node'' accounts, which receive or send a large number of transactions (e.g., a popular DEX pool or mixer service). 
For instance, Figure~\ref{fig:business} shows an example of expanded attack instance, with the attackers in the red box and the victims; the added accounts and transactions are outside the two boxes. 

{\bf Attack ecosystem template}: We analyze the expanded attack graph in a template consisting of three phases: 1) attack preparation, 2) attack execution, and 3) attack wrap-up. Phase 2) is the core attack component, and Phases 1) and 3) are the expanded  parts. In general, the actual Boss often sits behind an exchange/mixer service, such as Tornado~\cite{me:tornado}, to hide its identity. In  attack preparation (Phase 1), the Boss sends commission in Ether to Attackers and Exploit developers. The Ether transfer can be relayed through the Mules. An Exploit developer writes an Exploit smart contract and deploys it to the blockchain. It then mounts the attack in the execution phase (Phase 2), exercising the strategies described previously (\S~\ref{sec:attack}). To wrap up a series of attacks (Phase 3), the mule receiving the stolen tokens transfers the tokens back to the Boss. This is often done by swapping the stolen tokens to ETH (e.g., via DEX and wrapped tokens such as WETH) and by sending the ETH to the Boss via a mixer service. In the attack wrap-up phase, the mule may transfer tokens to Investors to maximize the stolen value. 

\begin{table}[h]
\caption{Attack ecosystem and attacker correlation: Red text shows the two attackers share the same developer of exploit smart contracts. AO represents attack operator and EC is exploit smart contract.
}
\label{tab:eco}
\centering{\small
    %\begin{tabular}{|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{1cm}|p{1.2cm}|}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    Mules & \#AO & \#EC & Developer & Value ($10^3$ USD) \\
    \hline
     $0x9799$ & 5 %$0x4e53$, $0xac72$, $0xa084$, $0x5bb4$, $0xe929$ 
& 24 % $0x338c$, $0x3ac7$, $0x34a2$, $0x9a99$, $0x2927$, $0x536b$, $0xe9f8$, $0x684b$, $0x58a3$, $0x72bb$, $0xa8a2$, $0x72cb$, $0x2528$, $0xbf2d$, $0xadfc$, $0xd6a2$, $0x24af$, $0x1335$, $0xf367$, $0x94fc$, $0x5caf$,  $0x6332$, $0x3c3a$, $0x1233$	
& {\bf \color{red} $0x8641$} & 556 \\
    \hline
    $0x2a2e$  & 1 %$0x2a2e$ 
& 1 %$0x5f5a$ 
& $0x2a2e$ & 239
\\
    \hline
    $0xdb40$  & 5 %$0x64bc$, $0x62ae$, $0x3807$, $0x225c$, $0xdb40$ 
& 2 %$0x4dbc$, $0x4626$ 
& $0x4626$ & 113
\\
    \hline
    $0x0c08$  & 1 %$0xfdee$ 
& 1 %$0x0c08$ 
& $0x0c08$ & 101
\\
    \hline
    $0x5617$  & 4 %$0x3a51$, $0xf97b$, $0xbf3f$, $0xa1e6$ 
& 10 %$0xfb51$, $0x328d$, $0x8a14$, $0x0fc7$, $0x4ed5$, $0xb439$ ,$0x55a2$, $0x6ba3$ 
& \color{red}{$0x8641$} & 101
\\
    \hline
    $0xb6bf$ & 1 %$0x675f$ 
& 2 %$0xb6bf$, $0x8526$ 
& $0x675f$ & 20
\\
    \hline
    $0xc762$ & 1%$0xd0d0$ 
& 1%$0xc762$ 
& $0xd0d0$ & 16
 \\
    \hline
    $0xa32d$ & 1%$0x7505$ 
& 1%$0xa32d$ 
& $0x7505$ & 6
\\
    \hline  
    \end{tabular}%
}
\end{table}

\ignore{
\begin{table}[h]
\caption{Attack ecosystem and attacker correlation: Red text shows the two attack instances are mounted using the exploit smart contracts developed by the same developer. AO represents attack operator and EC is exploit smart contract.
}
\label{tab:eco}
{\centering \scriptsize
    \begin{tabular}{|p{0.3cm}|p{1cm}|p{0.3cm}|p{0.3cm}|p{1cm}|p{0.7cm}|p{0.8cm}|p{.5cm}|}
    \hline
    Idx &Value ($10^3$~USD) & \#AO & \#EC & Developers & Mules & Deposits & Block gaps\\
    \hline
    1 & 552 & 5 %$0x4e53$, $0xac72$, $0xa084$, $0x5bb4$, $0xe929$ 
& 24 % $0x338c$, $0x3ac7$, $0x34a2$, $0x9a99$, $0x2927$, $0x536b$, $0xe9f8$, $0x684b$, $0x58a3$, $0x72bb$, $0xa8a2$, $0x72cb$, $0x2528$, $0xbf2d$, $0xadfc$, $0xd6a2$, $0x24af$, $0x1335$, $0xf367$, $0x94fc$, $0x5caf$,  $0x6332$, $0x3c3a$, $0x1233$	
& {\bf \color{red} $0x8641$} & $0x9799$ & $P_1$ & 121\\
    \hline
    2 & 101 & 1 %$0x2a2e$ 
& 1 %$0x5f5a$ 
& $0x2a2e$ & $0x2a2e$ 
& $P_1$ & 1\\
    \hline
    3 & 96 & 5 %$0x64bc$, $0x62ae$, $0x3807$, $0x225c$, $0xdb40$ 
& 2 %$0x4dbc$, $0x4626$ 
& $0x4626$ & $0xdb40$ 
& $P_1$ & 0\\
    \hline
    4 & 86 & 1 %$0xfdee$ 
& 1 %$0x0c08$ 
& $0x0c08$ & $0x0c08$ 
& $P_1$ & 1\\
    \hline
    5 & 67 & 4 %$0x3a51$, $0xf97b$, $0xbf3f$, $0xa1e6$ 
& 10 %$0xfb51$, $0x328d$, $0x8a14$, $0x0fc7$, $0x4ed5$, $0xb439$ ,$0x55a2$, $0x6ba3$ 
& \color{red}{$0x8641$} & $0x5617$ 
& $P_3$ & 2\\
    \hline
    6 & 48 & 1 %$0x675f$ 
& 2 %$0xb6bf$, $0x8526$ 
& $0x675f$ & $0x675f$ & $P_1$ & 0\\
    \hline
    7 & 29 & 1%$0xd0d0$ 
& 1%$0xc762$ 
& $0xd0d0$ & $0xd0d0$& $P_3$ & 1 \\
    \hline
    8 & 22 & 1%$0x7505$ 
& 1%$0xa32d$ 
& $0x7505$ & $0x7505$& $P_1$ & 0 \\
    \hline  
    \end{tabular}%
}
\end{table}
}


{\bf Results}: 
We present the measurement results in Table~\ref{tab:eco}. It can be seen that each attacker is systematic, typically involving multiple attack operators and exploit smart contracts. For instance, the attacker using Mule $0x9799$ has mounted attacks through $5$ different operator EOAs and leveraged more than $24$ different exploit smart contracts. In addition, different attackers use the exploit smart contracts developed by the same developer (in red in Table~\ref{tab:eco}), implying an underground business of exploit contract development.

\section{Attack Mitigation}
\label{sec:mitigate}

We aim to mitigate theft attacks on deployed Uniswap DEXes. Because Ethereum is immutable and deployed smart contracts can not be patched, mitigation entails either 1) incrementally hardening the deployed DEX (on the mutable off-chain parts) or 2) deploying patched smart contracts but migrating traders to using the new contracts. In the following, we discuss both options for attack mitigation. 
We first discuss the root cause of the vulnerability.

\subsection{Root Cause of the Vulnerability}

Uniswap's pool accepts deposit of Token $T0$ in any form, including the external transfer call directly sent from the trader EOA. 
%As can be seen in Appendix \S~\ref{appendix:YYY}, 
This flexibility greatly simplifies the programming of router smart contract, esp. when interoperating with other DeFi services~\cite{me:uniswapv2:whitepaper}. In order to know the deposit amount, Uniswap tracks the difference between the $T0$  reserve in the pool contract and the pool's account balance in $T0$'s token contract. Upon observing the difference, the pool allows anyone, on a first-come-first-served basis, to withdraw token $T1$ of the same value with the deposit in token $T0$. 

The root cause of Uniswap's vulnerability is that the pool implicitly assumes that any deposit of token $T0$ to the pool's account is intended for swapping out token $T1$. The assumption fails in the risky-swap cases identified in this work, including token rebase, airdrop, interest, etc. which all update the token balance but are not intended for swapping. 

\subsection{\normalsize \bf Mitigation by Hardening Deployed DEX}

{\bf Lost-and-found service off-chain}: We propose running a lost-and-found off-chain web service. This off-chain service monitors the on-chain state for profitability and collects extractable value ahead of actual attacks. To do so, the service takes an aggressive strategy by directly monitoring the vulnerable deposits (i.e., $P_1$, $P_3$, $P_4$) and withdrawing immediately upon discovery. For token interest $P_2$, the service monitors mempool for stealing transactions sent to the pools supporting token interests. Upon the discovery, the service sends transactions to frontrun the stealing transactions. 

In essence, this service performs the same functionality with thief attackers in discovering profitability opportunities on-chain, but it is benign in the sense that it stores the extracted value and allows victims to claim their tokens. Technically, given value deposited by Account $V$, the service stores the value and allows $V$ or any other account with $V$'s signature to claim the value.

{\bf Fuzzing router smart contracts}: For the risky swaps using buggy router contracts (i.e., $P_4$), one can mitigate the problem by developing more secure router smart contracts. Here, to ensure that the router calls deposit and withdrawal in all possible code path, we fuzz the router smart contract using a fuzzing framework Echidna~\cite{DBLP:conf/issta/GriecoSCFG20}. Specifically, we develop a test oracle that defines swap atomicity and a smart contract rewriter to automatically insert the oracle to the target router smart contract. The test oracle records all the \texttt{transfer}/\texttt{transferFrom}/\texttt{swap} invocations and checks if there is a standalone invocation in the end of execution.   

\subsection{\normalsize \bf Mitigation by Patching Smart Contracts}

{\bf Challenge of migrating DEX liquidity providers}: Another direction to mitigate attacks is to develop patched smart contracts for an AMM pool and deploy them to new blockchain addresses. This approach entails migrating {\it both} liquidity providers and traders to the new pool smart contracts. Note that migrating only traders is insufficient, as the new pool without liquidity providers means a pool without sufficient reserves, which are less attractive to traders. However, in DEX, each liquidity provider is typically an average token owner who invests a small amount in the pool reserves (i.e., a non-professional, retail investor). Such retail provider making small investments would be deterred by the high transaction fees to migrate their invested tokens to a new pool smart contract.

In practice, the difficulty of migrating liquidity providers is real. Uniswap V3 protocol is developed and deployed on Ethereum mainnet. However, launched more than half a year (as of Feb. 2022), the V3's transaction volume lags behind and is still orders-of-magnitude lower than the V2's volume, as described in Appendix \S~\ref{sec:v3:use}. 
The difficulty of migrating providers to Uniswap V3 is corroborated by the user complaints online~\cite{me:migratev3:complaint1,me:migratev3:complaint2}. 

\section{Related Work}
\label{sec:rw}

This work is related to blockchain data analysis. We survey blockchain-data analysis for attack detection and user de-anonymization. 

{\bf Detecting Smart-Contract Program-level Attacks}: Attack detection on blockchain generally works as distilling the attack signatures from known vulnerabilities and attack patterns and matching certain representation of smart-contract execution (e.g., in transactions, function-call graph or instruction traces) against the attack signatures. There are known patterns of smart-contract program-level attacks, such as reentrancy attacks, transaction order dependency, etc. Existing works tackle the detection of program-level attacks on Ethereum-like blockchains. 
 
TxSpector~\cite{DBLP:conf/uss/ZhangZZL20} records and replays Ethereum transactions into fine-grained EVM instruction traces, which are stored in datalog databases and queries to compare against the signatures of known attacks. Similarly, Zhou et al~\cite{DBLP:conf/uss/ZhouYXCY020} model the coarse-grained traces of smart contract function calls and match them against known attack signatures. At its core, two function calls are modeled, that is, smart contract creation/destruction and token transfers (money flow). Su et al~\cite{DBLP:conf/uss/SuSDL0XL21} uses reported attack instances to extract attack signatures, and it discovers new attacks as well as uncovers the attacker/victim behavior by systematically analyzing the Ethereum blockchain traces. Other similar work~\cite{DBLP:conf/uss/0001L21} detects the attack instances of known vulnerabilities.  

{\bf Detecting DeFi Protocol-level Attacks}: In addition to detecting program-level attacks, there are related works on detecting protocol-level attacks on deployed DeFi applications. Notable DeFi attack patterns include frontrunning, arbitrage, etc. 

Torres, et al.~\cite{DBLP:conf/uss/TorresCS21} detects front-running attacks by matching Ethereum transactions against a signature of success-failure transaction pair. Qin et al~\cite{DBLP:journals/corr/abs-2101-05511} systematizes different types of front-running attacks and measures the attacks and mitigation in the wild.

Front-running attacks are a class of attacks in which the attacker inserts a malicious transaction before the victim transaction to extract illicit profit (e.g., to win an auction bid unfairly). More generally, front-running is a class of MEV or miner extractable value, in which transaction order can be manipulated by a profit-driven miner to receive additional profit.

Arbitrage attacks work by an aggressive trader gain profit by exploiting difference of exchange rates across different DEXes/price oracles. Wang, et al~\cite{DBLP:journals/corr/abs-2105-02784} detects cyclic arbitrage on Uniswap-V2, by finding profitable cycles on token-transfer graph (nodes are tokens and edges are transfers). Similarly, Zhou, et al~\cite{DBLP:conf/sp/ZhouQCLG21} discovers profit-generating transitions in real-time by finding cycles  and leveraging solvers.

{\bf User de-anonymization}: While blockchain accounts and their activities are visible, the linkage of accounts (which are public keys) with real-world identities is not directly observable. There are existing works to infer blockchain account linkage in efforts to deanonymize users. Specifically, there are three types of linkage information: 1) Whether a specific account is linked to a specific real-world user identity. Existing works~\cite{DBLP:conf/fc/KoshyKM14} monitor a blockchain network' traffic of transactions propagated from an IP and link the transaction sender's account with the IP. %Other works~\cite{XXX} aggregate transaction volume of a given account and use background knowledge to link the account to real-world ID.

2) Whether two blockchain accounts are linked, as the sender and receiver, in a privacy-enhanced transaction. Mixing services are intended to break the sender-receiver linkage. There are existing works aimed at reconstructing the sender-receiver relation on transactions relayed through mixing services. In particular, address reuse is a heuristic to link transaction senders/receivers on Bitcoin-like blockchains~\cite{DBLP:conf/uss/YousafKM19,DBLP:conf/uss/KalodnerMLGPCN20}.

3) Whether two blockchain accounts are shared by the same real-world user. On Bitcoin, transaction graph analysis~\cite{DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:books/daglib/0040621} is proposed to recover the account linkage. Particularly, address clustering heuristics are proposed. For instance, two accounts that are co-spent by a Bitcoin transaction or that involve a change are likely to be controlled by the same off-chain user. These address clustering heuristics are useful only in the context of Bitcoin's UTXO model. Address clustering is useful to uncover the money flow in online criminal activities such as ransomware payments on Bitcoin~\cite{DBLP:conf/sp/HuangALIBMLLSM18}. 

Of most relevance to this work is the address clustering techniques proposed to link Ethereum accounts~\cite{DBLP:conf/fc/Victor20}. Specifically, the observation is that some DEXes support the deposit address, that is, trader Alice swapping token T0 for token T1 can specify a ``deposit'' address to receive T1. Multiple accounts using the same deposit address are likely to be the same off-chain user. 

This work is different from Ethereum account linkage. In this work, the attack detection problem is to verify whether two Ethereum accounts are from two off-chain users, which is different from detecting if two accounts are linked by the same off-chain user. Moreover, the Ethereum address clustering work~\cite{DBLP:conf/fc/Victor20} has to assume that the swap is atomic, normal one, so that they can attribute address sharing to the cause of the same off-chain user. By contrast, in this work, we do observe two sender accounts share the same deposit address, but they are caused by two victim accounts whose swaps are grabbed by the same attack account, as verified by our analysis of attacker/victim behavior.


\section{Responsible Disclosure}
\label{sec:disclosure}

We have reported the discovered atomicity violations and the vulnerabilities to Uniswap's bug bounty program (\url{https://uniswap.org/bug-bounty}). The bugs have been confirmed. Further details on bug reporting are documented on the anonymized Google document (\url{https://shorturl.at/aADNY}). 

\section{Conclusion}
\label{sec:conclude}

This paper presents the first measurement study of atomicity violations and token theft attacks on popular Uniswap DEXes on Ethereum. The study unearths more than $4.65*10^5$ risky swaps violating atomicity and stolen tokens worthy of $3.5$ million USD. It specifically uncovers a range of previously unknown patterns of vulnerable deposits, exposes real-world attackers' adaptive withdrawal strategies, and their systematic behavior to prepare, execute, and wrap up the theft attacks. Finally, mitigation schemes are proposed to remedy the deployed DEXes running immutable smart contracts.


\section{Mitigation}
\subsection{The Vulnerability}

Recall that in an AMM, a trader interacts with a liquidity pool to swap tokens. Normally, the trader makes a deposit (in one token) to the pool's account and then withdraws the value from the pool (in another token). The pool needs to maintain a copy of token balances, namely reserves, which is essential in calculating and updating token-exchange rates.

\noindent
{\bf Why Uniswap-V2 is vulnerable?}: Uniswap-V2 materializes the above AMM architecture by the following design choice: It requires synchronizing the pool reserves against the token balances (i.e., the pool account's balance in the token smart contract). It (mis)uses the synchronized reserve, or more precisely, monitoring any reserve update, to infer token deposits, instead of directly tracking the deposits in the pool smart contract (i.e., deposits do not call any Uniswap-V2's procedures).  

While the design is intended to support flexible mechanisms of trader deposits including both standard token transfer and non-standard balance-updating operations, it sacrifices the security. Without directly tracking deposits, the pool smart contract does not know the sender accounts of deposits and is forced to accept any withdrawal without access control, that is, permissionless withdrawal. Without enforcing swap atomicity in the pool smart contract or in risky applications where value is deposited into pool's account without withdrawal, the permissionless withdrawal creates value-extraction opportunities, which can be seized by attackers who front-run legitimate traders, if any.

\noindent
{\bf Is Uniswap-V3 secure?}: Uniswap releases Version 3 (Uniswap-V3) since May 2021. V3 avoids permissionless withdrawal by directly tracking deposits, that is, having the pool's presence in handling a deposit operation.  Uniswap-V3 thus maintains the pool reserve updated only by trader deposits and excludes any other balance updates. That is, {\it Uniswap-V3's pool reserve is intentionally unsynchronized with the token contract's balance and does not reflect updates from rebase, interest, airdropping or other causes that fall under $P_1$ and $P_2$}. Uniswap-V3 uses this unsynchronized reserve to algorithmically determine token exchange rates, which is subject to a range of attacks in price manipulation, arbitrage, and even denial of service. While a full security analysis of Uniswap-V3 is out of the scope to this paper, refer to Appendix~\ref{sec:uniswapv3:attack} for a description of a denial-of-service attack that we discovered against Uniswap-V3. We demonstrate the success of the attack on a local Ethereum node running unmodified Uniswap-V3 smart contracts. The vulnerability is reported to the Uniswap bug-bounty program~\cite{me:bugreport:defiant}.

\noindent
{\bf How to secure AMM?}: We propose a secure design of AMM pool. In it, 1) the pool tracks deposits and records deposit senders, in order to enforce access controls on withdrawal. This avoids permissionless withdrawal and prevents extractable value. 2) The pool maintains token reserves and synchronizes them with token balances, so as to avoid arbitrage and price manipulation. Security analysis suggests that in this pool design, for the part of balance updates from the tracked deposits, the pool allows them to be withdrawn by the deposit senders. For untracked balance updates (e.g., rebase, airdropping, etc.), the pool simply synchronizes them into the pool reserve and does not allows anyone to withdraw.




==> text/old/v5_intro_ccs22.tex <==
\section{Introduction}


Recent years have witnessed the rise of Decentralized Finance (DeFi) applications on blockchains, among which the most popular one is Decentralized Exchange or DEX. A DEX allows trader accounts to swap, in a trustless fashion, their assets stored in one token with those in another token. In practice, Uniswap~\cite{me:dex:uniswap} is a DEX protocol with popular running instances on various Ethereum networks; these Uniswap instances have dominated more than $90\%$ of the DEX market share on Ethereum. 

\vspace{2pt}\noindent\textbf{Risk in DEX}. Like any currency exchange system, of ultimate importance is the DEX's security against the threat of token thefts, in which an unauthorized party's account can extract value and steal tokens to be received by the original trader. To prevent illicit value extraction, swap atomicity is essential: the token transfer operations in a swap should be executed in an all-or-nothing manner. Violating swap atomicity could pose security risks to the trader. For instance, an attacker observing a swap whose execution gets interrupted could extract value from the pool at the pending state where one token has been deposited while the other token has not yet been withdrawn. 
%This risk can be more severe in the presence of permissionless, composable DeFi protocols running on AMMs, as elaborated on in \S~\ref{YYY}.

While existing research has measured DEX security against arbitrage~\cite{DBLP:journals/corr/abs-2103-02228}, front-running and scam tokens~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21}, these attacks do not necessarily violate the atomicity of individual swaps. It remains an open research problem whether risky DEX transactions violating atomicity exist, and if they exist, how pervasive they are ({\it RQ1})? It is also currently unknown whether any attacks take place in the real world to materialize the risk into actual value loss ({\it RQ2})? Furthermore, if such theft attacks exist, what are attackers' and victims' behavior in preparing, conducting, and finalizing the attacks? Finally, whether there are underground criminal ecosystems that facilitate the thefts ({\it RQ3}).

\begin{figure}[b!ht]
\begin{center}
\includegraphics[width=0.26\textwidth]{figures/workflow6.eps}
\end{center}
\caption{Data-analytical workflow to detect, out of transaction and other blockchain data, risky swaps, theft attacks, and attackers/victims behavior to understand DeFi crimes. Risky swaps are those violating atomicity.}
\label{fig:workflow:overall}
\end{figure}

Our research is the first attempt to systematically address these open problems on top DEXes on Ethereum. These target DEX instances that dominate $90\%$ of the DEX market on Ethereum all run the Uniswap protocol~\cite{me:dex:uniswap}.
We develop an end-to-end transaction-analytical pipeline, as depicted in Figure~\ref{fig:workflow:overall}, to 1) detect risky swaps violating atomicity, 2) discover thefts, analyze attacker/victim behavior, and 3) uncover DeFi criminal ecosystems.

\vspace{2pt}\noindent\textbf{Our methodology}. 
More specifically, our pipeline first detects atomicity-violating swaps by joining the records of different token-transfer operations across transactions; the goal is to find the mismatch between the token value transferred into a DEX's pool account and that coming out of the account. The challenge here is that DEX such as Uniswap support a swap across multiple transactions, and directly joining these transactions together can be computationally expensive (e.g., entailing cross-product on all transactions' powerset). So in our research, we develop an efficient linear algorithm that takes advantage of the invariant observed from the Uniswap-V2's smart contract program.

Based on the violating swaps, our approach further identifies attack instances. An actual token-theft attack must occur between a victim trader and an attacker, that is, two distinct blockchain accounts that are not controlled by the same physical user. However, deciding whether two blockchain accounts are linked is intractable if the only information is on-chain data. Existing heuristics such as address clustering~\cite{DBLP:conf/fc/Victor20,DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:conf/sp/HuangALIBMLLSM18,DBLP:books/daglib/0040621} do not apply to the problem of discovering DEX thefts (see \S~\ref{sec:discoveryproblem} for details).

To work around the difficulty and to validate discovered attacks without the ground truth, our intuition is the following: {\it A systematic attacker would rationally analyze victim DEX's protocol/implementation and design well-founded strategies to maximize the attack success ratio or stolen value.}
We model such rational attackers, design several strategies, and use them as indicators to match candidate accounts' observable behavior on-chain. 
For instance, given that each risky swap consists of an exploitable deposit creating extractable value and a malicious withdrawal that claims the illicit value, a rational attacker would want to minimize the deposit-to-withdraw delay to front-run potential competing attackers. 
For another instance, a rational attacker would read DEX pool states (e.g., reserves and token balances) before the attack to check if the value has been extracted and avoid sending a transaction bound to fail.
%For another instance, for interest-bearing tokens where the longer it waits the more value can be extracted, a rational attacker would instead wait for longer delays before sending the malicious withdrawal. 
We propose an algorithm to discover thefts matching at least one indicator.

%To tackle the challenge, we inspected the causes of risky swaps, identified the patterns of exploitable deposits (described in the next paragraph), hypothesized possible attack strategies, and used them to indicate and discover theft attacks from the risky swaps.

%We further collected attack ground-truth data from online user complaints to validate the effectiveness of our indicator-based technique.

\vspace{2pt}\noindent\textbf{Our findings}. 
We use the above methods on the three most popular DEX instances: Uniswap-V2~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, and Pancakeswap~\cite{me:pancakeswap:1}. The first two account for more than $83\%$ of the DEX market on the Ethereum mainnet at all times, and the last one is the most popular DEX on Binance Smart Chain (BSC), an Ethereum network fork~\cite{me:bsc:1}. 
We analyze $53/1.9/3$ million transactions on Uniswap-V2/Sushiswap/Pancakeswap and found $210/0.3/1006$ thousand risky swaps are violating atomicity. 
%We found risky swaps follow the same ``template'' in which a vulnerable deposit operation that creates extractable value is followed by multiple withdrawal requests that attempt to claim and steal the value, among which one succeeds. 
We found in practice the exploitable deposits can be created in a variety of unexpected application scenarios, including free token giveaways (i.e., airdropping), tokens redistributing fees to privileged shareholder accounts, tokens bearing interest, tokens that can adjust or rebase total supply, buggy smart contracts, and unsafe user interface that executes a swap in two separate transactions, etc. 
The root cause is that the Uniswap protocol designer assumes that any deposit made into its pool is part of a swap and will be withdrawn, which does not hold in the above application scenarios; for instance, an airdrop that deposits to a DEX's account does not intend to withdraw.
%in these scenarios, someone makes a deposit into a Uniswap's pool but does not intend to withdraw tokens in return. When this occurs, Uniswap falsely assumes that any pool deposit must be part of a swap and makes it possible to withdraw or extract the deposited value by anyone who comes to claim it, including an attacker. 

We discover theft attacks where external attacker accounts extract the value created by the above vulnerable deposits in Uniswap pools. On the Ethereum mainnet and BSC fork, we discover $465$ thousand theft attacks mounted by $258$ distinct attacker accounts, inflicting a loss of more than $3.7$ million USD stolen from $978$ victim traders.
Each attack instance we found matches at least one indicator described above. Interesting attacker behavior was observed in practice. For instance, real-world attackers {\it adapt} to the different patterns of exploitable deposits and exhibit different behavior: When the attacker is to extract value from interest-bearing tokens, she waits long enough, typically hundreds of Ethereum blocks, for the interest to accumulate and to become profitable. To extract deposits of other patterns, the same attacker instead wastes no time extracting the illicit value, typically within one or two blocks.

We further study attackers' and victims' behavior by tracking their money flow and actions to create/destroy smart contracts. Our study uncovers the systematic criminal activities: the crime bosses use mixer services to hide their identities while sending commissions and instructions. After the attack, the money is sent to various DeFi services to maximize illicit profit. Exploit smart contracts are widely used to improve attack success rates.

We propose countermeasures to redesign secure DEX smart contracts by enforcing permissions on token withdrawal and tracking token deposits. The design trades off the support of flexible deposits for the security against thefts.
Given the observed difficulty of migrating liquidity out of a deployed DEX, we also propose countermeasures to harden an existing DEX by ensuring the security of off-chain parties and application-layer (or router) smart contracts.

\vspace{2pt}\noindent\textbf{Contributions}. This paper's contributions are outlined as follows: 

\vspace{2pt}\noindent$\bullet$\textit{ New findings}. We discover a total of $3.5$ million USD worth of stolen value by measuring and analyzing atomicity violations on three popular Uniswap services on Ethereum and BSC. 
The discovered token theft attacks uncover the previously unknown patterns of vulnerable deposits (e.g., token rebase, interest, airdrop, mishandled contract exception) and expose the malicious, adaptive withdrawal behavior that occurs offline and otherwise would have been hidden. We further study the criminal infrastructures and campaigns mounted to systematically prepare, execute and finalize the theft attacks.

\vspace{2pt}\noindent$\bullet$\textit{ New techniques}. We develop an end-to-end analytical pipeline to detect attacks from Uniswap transaction traces, including an efficient join algorithm for detecting atomicity violations and approaches to automatically discover and cross-check token theft attacks. 
%XXX: Also we propose mitigation schemes including a fuzzer and test oracle to automatically detect mishandled exceptions in smart contracts.

%This work leads to the findings that shed light on the current and future underground ecosystem that strategically exploits the atomicity violation to gain illicit profit.

\noindent
{\bf Roadmap}: \S~\ref{sec:background} introduces the background of Uniswap, defines risky swaps and describes the threat model. The first step in our analysis pipeline, that is, detecting risky swaps, is presented in \S~\ref{sec:detectriskyswap}. The second step, discovering attacks, is described in \S~\ref{sec:attack}. The third step, characterizing on-chain crimes, is in \S~\ref{sec:behavior}. 
Mitigation schemes are presented in \S~\ref{sec:mitigate}. Related work is described in \S~\ref{sec:rw}. Responsible disclosure is discussed in \S~\ref{sec:disclosure} with the conclusion in \S~\ref{sec:conclude}. 
\ignore{
}

%In Appendices are full related works in Appendix~\ref{sec:rw:extra}, 



==> text/old/v6_intro.tex <==
\section{Introduction}

Recent years witnessed the rise of Decentralized Finance (DeFi) applications on blockchains. In DeFi, the most popular application is the Decentralized Exchange (DEX) which allows a trader account to swap their assets from one token to another token. On Ethereum, the most popular DEX instances run AMM protocols or automated market maker; for instance, Uniswap, Curve, Balancer which are all AMM instances account for more than 99.9\% of the DEX market, attracting hundreds of millions of transactions as of this writing (2022). Other than token swap, an AMM also supports the operations of liquidity addition/removal in which a liquidity provider account deposits tokens to be used as reserve for token swaps.

AMM can be misused. In the existing literature, a well known class of AMM misuses are sandwich attacks and arbitrage. In both attacks, the attacker observes profitable conditions on blockchain and sends transactions, which calls AMM operations (e.g., token-swap or add-liquidity calls), in crafted order to extract the illicit profit. In particular, these exploits are multi-operational in the sense that the success of the exploit depends on how the invoked operations are ordered, and it assumes each individual operation is executed correctly. Recent research has shown the large scale of sandwich attacks and arbitrage on Ethereum~\cite{XXX}. Another class of AMM misuses are to create pools for scam tokens~\cite{XXX}; the misuses can also be detected by certain multi-operation patterns, such as being shorter-lived and less-used, as studied in \cite{XXX}. In summary, the known AMM misuses are based on how multiple AMM operations are composed into a crafted sequence, and the individual AMM operation is assumed to be correct.

This work aims to discover previously unknown AMM misuses and to measure their impacts on actual AMM instances. Instead of the known multi-operation misuses, we aim at uncovering atomicity violations of individual AMM operations, which are single-operation misuses. Specifically, an AMM operation typically consists of a sequence of token deposits and withdraws and atomicity requires that the token deposits and withdrawals are executed in an all-or-nothing fashion. In practice, however, the atomicity could be violated, such as standalone deposit (withdrawal) that does not match any token withdrawal (deposit).

\vspace{2pt}\noindent\textbf{Methodology}. 
%Method: 
To discover the misuses, our approach is to find the mismatch between an AMM's governing protocol and its use history (collected from Ethereum transactions). Specifically, our approach takes as input the AMM protocol specification and filtered transactions/events collected from blockchain exploration service(XXX). It produces the discovered AMM operations that violate the protocol specification. Internally, it joins the records of different token-transfer operations across transactions. To reduce the search space (e.g., a naive join would entail cross-product on all transactions' powerset), we develop an efficient linear algorithm that takes advantage of the invariant observed from the Uniswap-V2's smart contract program.

%\vspace{2pt}\noindent\textbf{Measurements and results}
We measure top AMMs on Ethereum including the instances of Uniswap family (Uniswap V2/V3, Sushiswap, Pancakeswap), Curve and Balancer. We found a variety of AMM mismatches such as standalone token deposits that do not match any withdrawal, and standalone token withdrawals that do not match to any deposits prescribed in the AMM protocol, etc. We manually analyze the causes of the AMM mismatches:

1) We found all AMM protocols except for Uniswap V2 choose not to handle token deposit by external \texttt{transfer} (i.e., the pool receiving tokens that are deposited by the original owner calling the ERC20 \texttt{transfer} function). In the case that token deposits are made by mistake, such noop AMM leaves no way for the depositor to retrieve the token back; in other words, the token is lost forever. We formulate the measurement study on lost tokens as described next.

2) The Uniswap V2 protocol accepts token deposits by external \texttt{transfer}. This design choice leaves the pool smart contract unable to track the original depositor and forces it to accept a token withdrawal without enforcing permission. This flawed design, which we call permissionless withdrawal, affects different workflows in a pool (including token swaps, liquidity addition/removal, and returning lost tokens) and has adverse impacts on all Uniswap V2 based instances (including Uniswap V2, Sushiswap and Pancakeswap).

The flawed design of permissionless withdrawal gives rise to a new class of extractable value (BEV) in which exploitable token deposits can be extracted by anyone who attempts to withdraw first. By studying relevant transactions, we reveal various patterns of exploitable deposits in practice that lead to actual token theft. These causes include both standard and non-standard token balance updates, interest-bearing tokens, and buggy AMM-caller smart contracts. 


XXX: We found in practice the exploitable deposits can be created in a variety of unexpected application scenarios, including free token giveaways (i.e., airdropping), tokens redistributing fees to privileged shareholder accounts, tokens bearing interest, tokens that can adjust or rebase total supply, buggy smart contracts, and unsafe user interface that executes a swap in two separate transactions, etc. 
%The root cause is that the Uniswap protocol designer assumes that any deposit made into its pool is part of a swap and will be withdrawn, which does not hold in the above application scenarios; for instance, an airdrop that deposits to a DEX's account does not intend to withdraw.
%in these scenarios, someone makes a deposit into a Uniswap's pool but does not intend to withdraw tokens in return. When this occurs, Uniswap falsely assumes that any pool deposit must be part of a swap and makes it possible to withdraw or extract the deposited value by anyone who comes to claim it, including an attacker. 


\vspace{2pt}\noindent\textbf{Measure token-thefts}. 
Based on the violating swaps, our approach further identifies attack instances. An actual token-theft attack must occur between a victim trader and an attacker, that is, two distinct blockchain accounts that are not controlled by the same physical user. However, deciding whether two blockchain accounts are linked is intractable if the only information is on-chain data. Existing heuristics such as address clustering~\cite{DBLP:conf/fc/Victor20,DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:conf/sp/HuangALIBMLLSM18,DBLP:books/daglib/0040621} do not apply to the problem of discovering DEX thefts (see \S~\ref{sec:discoveryproblem} for details).

To work around the difficulty and to validate discovered attacks without the ground truth, our intuition is the following: {\it A systematic attacker would rationally analyze victim DEX's protocol/implementation and design well-founded strategies to maximize the attack success ratio or stolen value.}
We model such rational attackers, design several strategies, and use them as indicators to match candidate accounts' observable behavior on-chain. 
For instance, given that each risky swap consists of an exploitable deposit creating extractable value and a malicious withdrawal that claims the illicit value, a rational attacker would want to minimize the deposit-to-withdraw delay to front-run potential competing attackers. 
For another instance, a rational attacker would read DEX pool states (e.g., reserves and token balances) before the attack to check if the value has been extracted and avoid sending a transaction bound to fail.
%For another instance, for interest-bearing tokens where the longer it waits the more value can be extracted, a rational attacker would instead wait for longer delays before sending the malicious withdrawal. 
We propose an algorithm to discover thefts matching at least one indicator.

%To tackle the challenge, we inspected the causes of risky swaps, identified the patterns of exploitable deposits (described in the next paragraph), hypothesized possible attack strategies, and used them to indicate and discover theft attacks from the risky swaps.

%We further collected attack ground-truth data from online user complaints to validate the effectiveness of our indicator-based technique.

\vspace{2pt}\noindent\textbf{Findings on token theft}. 
We use the above methods on the three most popular DEX instances: Uniswap-V2~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, and Pancakeswap~\cite{me:pancakeswap:1}. The first two account for more than $83\%$ of the DEX market on the Ethereum mainnet at all times, and the last one is the most popular DEX on Binance Smart Chain (BSC), an Ethereum network fork~\cite{me:bsc:1}. 
We analyze $53/1.9/3$ million transactions on Uniswap-V2/Sushiswap/Pancakeswap and found $210/0.3/1006$ thousand risky swaps are violating atomicity. 
%We found risky swaps follow the same ``template'' in which a vulnerable deposit operation that creates extractable value is followed by multiple withdrawal requests that attempt to claim and steal the value, among which one succeeds. 

We discover theft attacks where external attacker accounts extract the value created by the above vulnerable deposits in Uniswap pools. On the Ethereum mainnet and BSC fork, we discover $465$ thousand theft attacks mounted by $258$ distinct attacker accounts, inflicting a loss of more than $3.7$ million USD stolen from $978$ victim traders.
Each attack instance we found matches at least one indicator described above. Interesting attacker behavior was observed in practice. For instance, real-world attackers {\it adapt} to the different patterns of exploitable deposits and exhibit different behavior: When the attacker is to extract value from interest-bearing tokens, she waits long enough, typically hundreds of Ethereum blocks, for the interest to accumulate and to become profitable. To extract deposits of other patterns, the same attacker instead wastes no time extracting the illicit value, typically within one or two blocks.

We further study attackers' and victims' behavior by tracking their money flow and actions to create/destroy smart contracts. Our study uncovers the systematic criminal activities: the crime bosses use mixer services to hide their identities while sending commissions and instructions. After the attack, the money is sent to various DeFi services to maximize illicit profit. Exploit smart contracts are widely used to improve attack success rates.

We propose countermeasures to redesign secure DEX smart contracts by enforcing permissions on token withdrawal and tracking token deposits. The design trades off the support of flexible deposits for the security against thefts.
Given the observed difficulty of migrating liquidity out of a deployed DEX, we also propose countermeasures to harden an existing DEX by ensuring the security of off-chain parties and application-layer (or router) smart contracts.

\vspace{2pt}\noindent\textbf{Findings on lost tokens}. 

In summary, we develop an end-to-end transaction-analytical pipeline, as depicted in Figure 1, to 1) detect risky swaps violating atomicity, 2) discover thefts, analyze attacker/victim behavior, and 3) uncover DeFi criminal ecosystems.

\section{Background}

Ethereum blockchain supports two types of addresses: An externally owned account (EOA), which is an Ether owner's public key, and a contract account (CA), which refers to the immutable memory address to which the smart contract is deployed on miners. An Ethereum transaction is a binding between its sender address and receiver address.

An AMM or automated market maker is a dominant form of decentralized exchange (DEX) deployed on Ethereum blockchains. An AMM runs one or multiple ``pools'' in smart contracts on Ethereum blockchain. An AMM pool owns two tokens, say $T_0$ and $T_1$. An AMM pool minimally supports two workflows: 1) token swap between a trader account and the pool smart contract, and 2) liquidity addition/removal between a provider account and the pool smart contract. The trader and liquidity provider can be either an EOA or a CA.

In a token-swap workflow, the trader deposits $dx$ units of token $T_x$ to the pool's account and receives from the pool $dy$ units of token $T_y$. The AMM internally determines the token exchange rate (or value of $dy$) based on some constant function.

In an add-liquidity workflow, the liquidity provider deposits $dx$ units of token $T_\texttt{X}$, deposits $dy$ units of token $T_\texttt{Y}$, and withdraws a certain amount of ``base'' tokens $T_{\texttt{LP}}$. An remove-liquidity workflow is the reverse of add-liquidity, in that the liquidity provider deposits tokens $T_{\texttt{LP}}$ and withdraws tokens $T_\texttt{X}$ and $T_\texttt{Y}$ at a certain ratio.

{\bf AMM protocol specification}: 
%specifies how the AMM pool smart contract should interact with trader, provider and token smart contracts. 
An AMM protocol materializes the above model, particularly token deposits and withdrawals in supported workflows. Specifically, to deposit tokens $T_{\text{X}}$, a trader EOA can externally call the token's \texttt{transfer} function or call the token's \texttt{approve} function followed by the pool's call of the \texttt{transferFrom} function.

We characterize the top AMM protocols below:

\begin{table}[!htbp] %force in current page, disable float.
  \caption{Characterization of AMM protocols}
  \label{tab:policy}
  \centering{
  \begin{tabularx}{0.425\textwidth}{ |X|X|X|X|X| }
  \hline
& Uniswap V2 (incl. Sushiswap) & Uniswap V3 & Curve & Balancer \\ \hline
Deposit by external \texttt{transfer} 
& \cmark & \xmark & \xmark & \xmark \\ \hline
Return lost tokens
& \cmark & \xmark & \xmark & \xmark \\ \hline
Security risks
& EV & Lost tokens & Lost tokens & Lost tokens \\ \hline
  \end{tabularx}
}
\end{table}

\section{Background}
\label{sec:background}

\noindent
{\bf Preliminary: Ethereum \& Uniswap}: Ethereum supports two types of addresses: an externally owned account (EOA), which is an Ether owner's public key, and a contract address, which is the memory address where the smart contract is deployed on individual miner nodes. An Ethereum transaction binds a sender's address to a receiver's address.

A decentralized exchange or DEX supports the swapping of a trader EOA's token of one type for another token type. Uniswap is the dominant DEX protocol on Ethereum and is designed based on an automated market maker (AMM). An AMM maintains token reserves in a so-called liquidity pool; the token owners, called liquidity providers, deposit their tokens to fill up the reserves, and the pool uses the current reserves to calculate token exchange rates, on demand, to serve swaps.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.4\textwidth]{figures/uniswap-layers.eps}
\end{center}
\caption{Uniswap system and smart contracts at three layers.}
\label{fig:uniswap:layers}
\end{figure}

\begin{table}[!htbp] %force in current page, disable float.
\centering{
\begin{tabularx}{0.5\textwidth}{ |X|X|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
Layer & $Swap$ workflow & $addL.$ workflow \\ \hline
Router & \texttt{swap} (amountIn, amountOutMin, to\_addr) & \texttt{addLiquidity} (amountADesired, amountBDesired, amountAMin, amountBMin, to\_addr) \\ \hline
Liquidity pool~\cite{me:uniswapv2:pool}
& \texttt{swap}(amountOut, to\_addr) & \texttt{mint}(to\_addr), \texttt{burn}(to\_addr) \\ 
\hline
ERC20
  & \multicolumn{2}{|l|}{\texttt{transfer}(trader,amountOut)} \\ 
token~\cite{me:erc20:api} & \multicolumn{2}{|l|}{\texttt{transferFrom}(trader,pool,amountOut)}\\ 
 & \multicolumn{2}{|l|}{\texttt{balanceOf}(account)} \\ \hline
\end{tabularx}
}
\caption{Uniswap-V2's liquidity pools' API: $addL.$ represents $addLiquidity$ workflow.}
\label{tab:uniswapv2:api}
\end{table}

The Uniswap protocol architects a DEX in three layers of smart contracts, as in Figure~\ref{fig:uniswap:layers}: 
The central layer is the liquidity pool, as described, which receives requests from the upper-layer router smart contracts and sends requests to transfer tokens in the underlying token smart contracts. The router smart contract is trusted by a trader EOA and is responsible for protecting their tokens when executing token swaps. The liquidity pool is responsible for protecting liquidity providers' token reserves during swaps. There are other DeFi smart contracts that may use the pool as a price oracle. 
Here, we mainly consider Uniswap's Version 2 (V2) protocol, which is adopted in major DEXes on Ethereum networks, including Uniswap-V2~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2} and Pancakeswap~\cite{me:pancakeswap:1}. 
%We discuss Uniswap's Version 3 (V3) protocol in Appendix~\ref{appdx:uniswapv3YYY}.
The API functions in Uniswap-V2's pools and ERC20 tokens are presented in Table~\ref{tab:uniswapv2:api}. 

More specifically, Uniswap's pool supports two essential workflows: swap and manage liquidity.
In a {\it swap} workflow, a trader EOA calls the router, which works with the liquidity pool to jointly coordinate the issuance of deposit and withdrawal (i.e., transferring token $T0$ into the pool's account and transferring token $T1$ out of its account).

A liquidity provider EOA can call function \texttt{addLiquidity} to a pool by depositing tokens $T0$ and $T1$ at a certain rate. The provider receives a deposit certificate (called LP token). Thus, an $addLiquidity$ workflow also includes the invocations of token's \texttt{transfer} functions.

\noindent
{\bf Risky swaps and specification}: In general, a (normal) swap should consist of two token transfers, one transfer of token $T0$ from the trader to the pool and the other transfer of token $T1$ from the pool to the trader. Mapping the two transfers to transactions result in different swap types: 

\begin{itemize}[leftmargin=0cm]
%\setlength{\itemindent}{-1em}
\item
Type-I swap (atomic): In a Type-I swap, the two token transfers occur in the same blockchain transaction, and their value matches w.r.t. the current exchange rate. This type of swaps are atomic swaps. 
\item
Type-II swap (risky): In a Type-II swap, the two token transfers occur in separate blockchain transactions. Their value matches w.r.t. the current exchange rate. 
\item
Type-III swap (risky): In a Type-III swap, there is only one standalone token transfer observed, that is, the pool transfers out token $T1$ to a trader without receiving explicit transfer-in of token $T0$. 

In a Type-III swap, a deposit (withdrawal) can not be attributed to a withdrawal (deposit). This can be caused by a standalone deposit that does not match any subsequent withdrawal (a sub-case we call Underwater or U), or by a standalone withdrawal that does not match any previous deposit (sub-case Freeride or F), or by a pair of deposit and withdrawal where the deposited value exceeds the withdrawn value  (sub-case Overcharge or O), or by a pair of deposit and withdrawal where the withdrawn value exceeds the deposited value (sub-case Discount or D). 
\end{itemize}


\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/anomalies.eps}
\end{center}
\caption{Swaps of three types: Type II and III are risky swaps.}
\label{fig:swaps}
\end{figure}


Type-I swap runs the two transfers atomically in one transaction and is unlikely to constitute a token theft. Type-II and Type-III swaps are risky and could imply theft/attacks (as defined next). Specifically, in the Type-II swap, a malicious trader EOA could try to extract the value in the pool after the transaction that sends the first transfer and before the transaction that carries out the second transfer. In the Type-III swap, it is abnormal for the pool to send value to a potentially malicious trader without receiving their deposit token.

\noindent
{\bf Threat model}: The primary threat in this work is DEX-value theft among trader EOAs. A victim is a trader EOA who has deposited the token to the pool but is unable to withdraw the other token from the pool. An attacker is an EOA who aims at extracting value from the liquidity pool interacting with a victim trader. The attacker's capability is to monitor certain conditions on the DEX states in real-time, and upon the satisfaction of the conditions, send crafted transactions to the DEX to extract the value and claim it illicitly. 

\ignore{
\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/workflow5.eps}
\end{center}
\caption{Workflow of data analytics to detect risky swaps and attacks, as well as to analyze attackers'/victims' behavior.}
\label{fig:workflow:overall}
\end{figure*}
}

\noindent
{\bf System overview}: Recall the transaction-analytical pipeline overview in Figure~\ref{fig:workflow:overall}. The input data is more than $43$ million transactions with their event log crawled from \url{etherscan.io}, internal call sequences crawled from Google BigQuery services~\cite{me:bigquery:ethereumdataset}. The pipeline consists of three stages: 1) Detecting risky swaps, which joins and matchmakers token transfers to detect the risky swaps as defined above, 2) Discovering token-theft attacks, which characterizes the behavior of accounts involved in risky swaps against proposed attack patterns, and 3) Uncovering on-chain crimes, which exposes the attack strategies, criminal infrastructures and ecosystems. 
The three steps are described in \S~\ref{sec:detectriskyswap}, \S~\ref{sec:attack}, and \S~\ref{sec:behavior}.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.325\textwidth]{figures/automata3.eps}
\end{center}
\caption{Matchmaking in two rounds to detect risky swaps (Type-II and Type-III swaps).}
\label{fig:automata}
\end{figure}


\clearpage





==> text/old/v6_paper3_ccs22.tex <==
\section{Detecting Risky Swaps}
\label{sec:detectriskyswap}

\label{sec:mmalgo}

\noindent
{\bf Goal: Risky swaps}: In general, a (normal) swap should consist of two token transfers, one transfer of token $T0$ from the trader to the pool and the other transfer of token $T1$ from the pool to the trader. Mapping the two transfers to transactions result in different swap types: 

\begin{itemize}[leftmargin=0cm]
%\setlength{\itemindent}{-1em}
\item
Type-I swap (atomic): In a Type-I swap, the two token transfers occur in the same blockchain transaction, and their value matches w.r.t. the current exchange rate. This type of swaps are atomic swaps. 
\item
Type-II swap (risky): In a Type-II swap, the two token transfers occur in separate blockchain transactions. Their value matches w.r.t. the current exchange rate. 
\item
Type-III swap (risky): In a Type-III swap, there is only one standalone token transfer observed, that is, the pool transfers out token $T1$ to a trader without receiving explicit transfer-in of token $T0$. 

In a Type-III swap, a deposit (withdrawal) can not be attributed to a withdrawal (deposit). This can be caused by a standalone deposit that does not match any subsequent withdrawal (a sub-case we call Underwater or U), or by a standalone withdrawal that does not match any previous deposit (sub-case Freeride or F), or by a pair of deposit and withdrawal where the deposited value exceeds the withdrawn value  (sub-case Overcharge or O), or by a pair of deposit and withdrawal where the withdrawn value exceeds the deposited value (sub-case Discount or D). 
\end{itemize}


\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/anomalies.eps}
\end{center}
\caption{Swaps of three types: Type II and III are risky swaps.}
\label{fig:swaps}
\end{figure}


Type-I swap runs the two transfers atomically in one transaction and is unlikely to constitute a token theft. Type-II and Type-III swaps are risky and could imply theft/attacks (as defined next). Specifically, in the Type-II swap, a malicious trader EOA could try to extract the value in the pool after the transaction that sends the first transfer and before the transaction that carries out the second transfer. In the Type-III swap, it is abnormal for the pool to send value to a potentially malicious trader without receiving their deposit token.

\ignore{
\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/workflow5.eps}
\end{center}
\caption{Workflow of data analytics to detect risky swaps and attacks, as well as to analyze attackers'/victims' behavior.}
\label{fig:workflow:overall}
\end{figure*}
}


{\bf Input data}:
Our input data is raw blockchain transactions including function-call sequences and logged smart contract events, which are accessible from Ethereum exploration web services~\cite{me:bigquery:ethereumdataset} and \url{etherscan.io}. Particularly, we only consider (and hence trust) the event log of liquidity-pool smart contract. 

{\bf Design goals and challenges}:
We aim at finding the incidents of risky swaps (Type II and Type III as previously defined) from the blockchain traces. A naive algorithm design is to reconstruct data records representing individual deposits and withdrawals, and to conduct matchmaking between them. The data records left unmatched are risky swaps (specifically, Type III swaps). However, there are challenges: 1) If we only consider the invocations of token \texttt{transfer} for deposits and withdrawals, false positives will be introduced in the results. For instance, the \texttt{transfer} calls serving $addLiquidity$ workflow will not match any withdrawal in a swap and can be falsely introduced in the detection result (as an artifact). 2) In theory, an atomic swap can contain an arbitrary number of deposits and withdrawals, as long as their total value matches. Matchmaking for this general case can be extremely unscalable. That is, the matchmaking should join the {\it powerset} of deposits and the powerset of withdrawals, and the powerset of $n$ deposits/withdrawals is of $2^n$ elements. 

Our goal is to design an efficient and effective detection algorithm that does not introduce false positives in the results. To do so, our key observation is two-fold: 1) Perform matchmaking on both swap and add/remove liquidity data. 2) Uniswap's pool executes deposits and withdrawals in a single thread, thus a deposit can only be matched to a subsequent withdrawal before the next deposit. This greatly saves the search space and makes it possible to run the matchmaking in a linear time. 

{\bf The algorithm}:
Given the raw blockchain data (transactions and events), we first reconstruct deposit and withdrawal records. A deposit record is constructed by the invocations of a pool's tokens' \texttt{transfer}/\texttt{transferFrom}/$mint$ functions where the pool's account is the token receiver. A candidate withdrawal record is constructed by the invocations of a pool's \texttt{swap} or \texttt{addLiquidity} function. We also use the pool's events to reconstruct the mapping between deposit value and withdrawal value in the withdrawal record.

After the data preparation, the algorithm runs in two rounds of matchmaking. In the first round, it equi-joins the $deposit$ records with $withdrawal$ records by their transaction IDs. The join conditions also include the equality of value in both records. It also considers the case of addLiquidity. If matched, it emits the pair as a Type-I swap (or matched addLiquidity) and removes it from the current dataset.

In the second round, it conducts matchmaking across transactions. Based on our linear algorithm, it scans through the $deposit$/$withdrawal$ records sorted by time; for each two consecutive $deposit$ records, it matches the earlier $deposit$ record with the powerset of all $withdrawal$ records falling in this period. We also run the reserved process where $deposit$ records between two consecutive $withdrawal$ records are matched. For each match, it emits the matched records as a Type-II swap (or matched \texttt{addLiquidity}) and removes them from the current dataset. In the end, Type-III swaps are left in the dataset. 
%Figure~\ref{fig:joinproblem} depicts the matchmaking process, and t
The pseudocode is in Appendix~\ref{sec:algorithm:detect}.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.3\textwidth]{figures/join_problem2.eps}
\caption{Matchmaking deposits and withdrawals: Matched cases are in green boxes and mismatches are rendered in red (including Underwater, Freeride, and Discount). In the figure, \textsc{addL} refers to Uniswap function \textsc{addLiquidity}, and \textsc{tf} refers to token function \textsc{transfer}.}
\label{fig:joinproblem}
\end{figure}

{\it An example}: Figure~\ref{fig:joinproblem} shows how token deposits to a Uniswap pool are matched to token withdrawals from the same pool. The data records storing deposits/withdrawals are aligned and sorted by time. The figure show two matched cases (i.e., two green boxes). Three mismatch cases are discovered: On the timeline, the first \textsc{transfer} is a standalone deposit (i.e., Underwater). The second \textsc{swap} is a standalone token withdrawal (i.e., Freeride). In the red box is a pair of deposit and withdrawal whose value does not match (i.e., Discount).

\subsection{Results}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Swaps (Types I, II, III) on Uniswap-V2-based DEXes; in red are risky swaps exposing extractable value to attackers.}
\label{tab:swapsrisky}\centering{\footnotesize
\begin{tabularx}{0.5\textwidth}{ |l|l|l|l|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
  Swap types & \#$deposit$ & \#$withdrawal$ & Value/diff (\$M) & Causes \\ \hline
  \multicolumn{5}{|l|}{Uniswap-V2~\cite{me:dex:uniswap,Adams2020UniswapVC} (on Ethereum mainnet)}   \\  \hline
 I  & $52.7*10^6$  & $52.7*10^6$   & $6.18*10^8$  & Atomic \\ \hline
 II  & $762$  & $761$   & {\bf $0.486$}  & \textcolor{red}{External transfer} \\ \hline
 II  & $35$  & $35$   & {\bf $0.205$}  & \textcolor{red}{Router bug} \\ \hline
 III (O) & $2.01*10^5$ & $2.01*10^5$ & $23.3$/$3.64$ & Fees \\ \hline
 III (D) & $3879$ & $3879$ & {\bf $0.185$/$0.094$} & \textcolor{red}{Rebase} \\ \hline
 III (F) & $4767$ & $0$ & {\bf $1.26$} & \textcolor{red}{Rebase/interest} \\  \hline
   \multicolumn{5}{|l|}{Pancakeswap~\cite{me:pancakeswap:1} (on Binance Smart Chain~\cite{me:bsc:1})}   \\  \hline
 I  & $2.97*10^6$  & $2.97*10^6$   & $7.34*10^7$  & Atomic \\ \hline
 II  & $364$  & $364$   & {\bf $0.047$}  & \\ \hline
 III (D) & $1.7*10^5$ & $1.7*10^5$ & {\bf $1.16$/$0.99$} & \textcolor{red}{Rebase} \\ \hline
 III (F) & $0$ & $2.82*10^5$ & {\bf $0.53$} & \textcolor{red}{Rebase} \\ \hline
 III (U) & $2507$ & $0$ & {\bf $0.12$} & \textcolor{red}{Airdrop (sync'd)} \\ \hline
  \multicolumn{5}{|l|}{Sushiswap (on Ethereum mainnet)~\cite{me:sushiswap:1,me:sushiswap:2}}   \\  \hline
 I  & $3.73*10^6$  & $3.73*10^6$   & $1.69*10^5$  & Atomic \\ \hline
 II  & $16$  & $16$   & {\bf $0.064$}  & \\ \hline
 III (D) & $57$ & $57$ & {\bf $51$/$7.6*10^{-3}$} & \textcolor{red}{Rebase/interest} \\ \hline
 III (F) & $0$ & $193$ & {\bf $0.82*10^{-3}$} & \textcolor{red}{Rebase} \\ \hline
 III (U) & $61$ & $0$ & {\bf $2.9*10^{-2}$} & \textcolor{red}{Bug/Airdrop} \\ \hline
\end{tabularx}
}
\end{table}

We analyze the traces of three Uniswap-based DEXes using the methods described previously. The three DEXes are Uniswap-V2, Sushiswap and the Pancakeswap. 
In particular, we set the minimal $Z\%$ value difference to determine match/mismatch. If a deposit (withdrawal) has $Z\%$ higher value than the paired withdrawal (deposit), it is considered a mismatched case (Type-III). A rule of thumb is to set $Z\%=10\%$ on our dataset, which helps remove from the measurement results
negative cases, such as fees charged by tokens and router smart contracts.
For each DEX, we report the number of swaps and their total value under each category. 
To estimate the value, we crawl the historical exchange rates reported by etherscan (\url{https://etherscan.io/tokens}) on the same day/hour of the reported swap. The results are presented in Table~\ref{tab:swapsrisky}.

It can be seen that the majority of swaps, about $97.9\%$, are atomic (Type-I). The rest are risky swaps (Type-II and Type-III) worth a total of 26.2 million USD, among which the majority are caused by high fees. We inspect the rest of risky swaps, which are more interesting and find four exploitable deposit patterns.

\ignore{
In Table~\ref{tab:swaprisky}, on Uniswap-V2, the majority of swaps, with total value of $618$ billion USD and in more than 0.5 billion Ethereum transactions (as in the third row of the table), are atomic ones, each of which is carried out by one transaction calling a router smart contract (recall Figure~\ref{fig:uniswap2}). Besides, as shown in the fourth row, there are $761$ atomic swaps, each of which is carried out by two or three transactions that directly call Uniswap's pool smart contract. The fifth row shows $35$ swaps that match in value but invoke a router smart contract with ``partly error.'' The case of ``partly error'' router smart contract is discussed in more details in \S~\ref{sec:partlyerror}.

On Uniswap-V2, more than $20$ thousand swaps are overcharge, which are caused by the particularly high fees by the operating routers or tokens. For instance, some tokens enforce a fee scheme to penalize the token deposit and to encourage the withdrawal. 

3879 swaps are discount, where a trader account receives profit. A primary cause is a token's rebase operation that occurs before the swap, as will be described in details in \S~\ref{sec:rebase}.

In the eighth row, $4767$ swaps are standalone deposit operations  (i.e., Freeride) that directly call the liquidity pool's swap function. In total, they are worth $1.26$ million USD. The profit come from the tokens' non-standard rebase operation or interest behavior.
}

%\subsubsection{Causes: Patterns of Profitable Deposit}

\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.475\textwidth]{figures/victimpatterns.eps}
\end{center}
\caption{Patterns of profitable deposits: $R$ is the router smart contract, $T0$/$T1$ are the two tokens in the target liquidity pool}
\label{fig:patterns}
\end{figure}

\subsubsection{Non-standard Balance Updates (Cause $P_1$)}
\label{sec:cases:rebase}

In many real-world tokens, account balance can be changed by the non-standard operations beyond token transfer. We describe two examples. {\it Rebase}: For instance, token balance can be elastically adjusted by token issuers, for purposes such as to stabilize the token's exchange rates against other tokens. In practice, token rebase is such a non-standard balance-changing function, supported in some widely used tokens, such as AMPL~\cite{me:ampl:token}. When a token, say $T0$, is rebased, a Uniswap's relevant pool, say for tokens $T0$ and $T1$, could have its $T0$ balance increased. Uniswap falsely assumes that this balance increase is due to some accounts that swap token $T0$ for token $T1$. Uniswap's pool would mistakenly admit anyone who requests to withdraw token $T1$ after the rebase of $T0$.

{\it Token shareholder}: 
As another example, there are tokens that charge ``tax'' to average owner accounts and redistribute the ``tax'' income among privileged accounts of shareholders. Specifically, these tokens support two kinds of owners, average owner and token shareholders. When there is a transfer, the token smart contract charges a certain amount of fees. The fees are redistributed to the privileged accounts of token shareholders. Thus, a transfer between average accounts would update the balance of all shareholders' accounts. In a Uniswap's pool of token types $T0$ and $T1$, if the pool's account in $T0$ is a shareholder, any transfers in $T0$ would increase the pool's balance and create a profitable opportunity.
 
Furthermore, even when the pool receives a token deposit, the deposit may not be intended as a part of swap. For instance, airdrop is a common practice to promote the use of a new token type, in which token issuers periodically give away newly minted tokens to the current token owners (e.g., in Tokens MILK2~\cite{me:token:milk2} and 3Cs~\cite{me:token:3cs}). When a token, say $T0$, is airdropped into a Uniswap's pool, the pool holding tokens $T0$ and $T1$ would mistakenly treat the transfer as a part of swap from token $T0$ to $T1$. Thus, the pool would admit anyone's request to withdraw token $T1$ after airdrop of token $T0$ to the pool's account.

In general, these non-standard token operations allow to update the pool's balance but do not intend to withdraw the same value from the pool. We name this pattern of extractable value by $P_1$.

%In general, there can be an explicit token operation that increases the pool's balance of token $X$, but is not with the intention of swap value. Thus, an attacker observing the occurrence of such an exploitable operation can strategically extract value from the pool and gain illicit profit. We name this attack pattern by $P_1$. 

\subsubsection{Implicit Token Balance Updates ($P_2$)}
Beyond $P_1$, there are implicit approaches to update the balance. Many tokens are bearing interest. That is, the balance in the token smart contract increases at a certain rate as the time goes by. Suppose a Uniswap pool is of token $T0$ and $T1$ where $T0$ is interest bearing. Similar to $P_1$, the Uniswap pool observing the increase of token $T0$ would admit the withdrawal of token $T1$ by anyone who requests it, including a value-extracting attacker. We call this attacker's pattern by $P_2$, which is different from $P_1$. In $P_2$, the attacker simply waits long enough to harvest the extractable value from token interest. 

\subsubsection{External Transfer for Deposit ($P_3$)}

In Uniswap, a trader can externally call token $T0$'s transfer function to make deposit so that she can in a separate transaction withdraw token $T1$. We call the pattern of a victim trader sending a transaction to externally transfer token $T0$ by $P_3$. When $P_3$ occurs, a malicious account can send the withdraw transaction ahead of the victim's one, to claim the value in the pool.  This attack is possible because a Uniswap pool receiving a deposit of $T0$ will approve of the next withdrawal of token $T1$, no matter who sends it. 

\subsubsection{Buggy Router Contracts ($P_4$)}

In the above three patterns, the victim may externally call token $T0$'s functions. In the fourth pattern $P_4$, the trader delegates the handling of swap to a router smart contract that is buggy and violates atomicity. After the trader EOA's transaction, the router smart contract successfully completes the deposit of Token $T0$ but fails at requesting the withdrawal of Token $T1$. Thus, anyone who requests the token withdrawal in the next transaction, including an attacker EOA, would succeed in grabbing the value illicitly. 

\subsection{Root Cause Analysis}
We analyze AMM protocols to understand the root causes of atomicity violation. At a high level, each swap operation needs to take a token deposit and issue a token withdrawal. One of the key design choices is how an AMM pool recognizes a token deposit. A pool may accept an external token transfer as deposit, that is, a trader account externally calling token $T_0$'s \texttt{transfer} function. Alternatively, a pool may require the trader to first call $T_0$'s \texttt{approval} before the pool is allowed to call $T_0$'s \texttt{transferFrom} to complete the deposit. We characterize top AMMes in their supported deposit mechanism and present the result in Table~\ref{tab:ammprofile}. Most AMM protocols require the \texttt{approve}-\texttt{transferFrom} workflow, with the only exception of Uniswap V2.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.275\textwidth]{figures/uniswapv2-dilemma.eps}
\end{center}
\caption{Uniswap V2's design and the cause of permissionless withdraw.}
\label{fig:uniswapv2model}
\end{figure}

When an AMM pool supports deposit-by-external-\texttt{transfer}, the deposit and withdrawal in a swap could be executed in two separate transactions: As shown in Figure~\ref{fig:uniswapv2model}, the token-depositing transaction $tx_1$ calls the token smart contract, and the token-withdrawing transaction $tx_2$ calls the AMM pool smart contract. Because of the ERC20 standard, the account depositing $T0$ tokens is not recorded on-chain after $tx_1$, leaving the pool smart contract no way to enforce any permission on token withdrawal. A permissionless AMM exposes the trader to the risk of frontrunning where a malicious user or bot aggressively sends transactions to withdraw the value ahead of the benign trader. In practice, Uniswap V2's pool detects token deposit by tracking the pool's balance update and allows whoever comes the first to withdraw tokens with the same value to the balance update.

To avoid the security risk, an AMM pool can reject deposit-by-external-\texttt{transfer} in token swaps and liquidity management. However, in application scenarios such as token deposits by mistake, one cannot make any assumption on token deposit mechanisms. In reality, the most common way to mistakenly deposit tokens is to do so by externally calling \texttt{transfer}. When that occurs, a responsible pool needs to return the tokens. Now the AMM designer faces a design dilemma, that is, either to lock mistakenly deposited tokens, which makes the trader lose tokens forever, or to return the tokens, which exposes the trader to the risk of frontrunning.

We profile the existing AMMes: Uniswap V2 supports returning the mistakenly deposited tokens (using a function \texttt{skim}), while all other AMMes do not have the support. Overall, by design, Uniswap V2 based AMM instances are subject to token thefts and other AMMes expose their traders to the lost-token risk, as shown in Table~\ref{tab:ammprofile}.

\clearpage

\section{Discovering Token Thefts}
\label{sec:attack}

\subsection{The Problem}
\label{sec:discoveryproblem}

\noindent
{\bf Threat model}: The primary threat in this work is DEX-value theft among trader EOAs. A victim is a trader EOA who has deposited the token to the pool but is unable to withdraw the other token from the pool. An attacker is an EOA who aims at extracting value from the liquidity pool interacting with a victim trader. The attacker's capability is to monitor certain conditions on the DEX states in real-time, and upon the satisfaction of the conditions, send crafted transactions to the DEX to extract the value and claim it illicitly. 


\noindent{\bf Formulating attack detection problem}: 
The detected risky swaps present value that {\it can} potentially be extracted and grabbed by attackers. However, whether the value is {\it actually} extracted by attackers, or equivalently, whether the risky swaps are actual attack instances, is a different problem. 

Consider as an example that a token issuer sends a vulnerable rebase transaction to a pool's token, followed by a withdrawal transaction sent by account $X$ (i.e., $P_1$). $X$ may or may not be the token issuer. The former case is not an attack, as the token issuer aware of the risky rebase sends the withdrawal to remedy the risk. The latter case may be an attack. in other situations including $P_3$ and $P_4$, a risky swap can also be attributed differently.
\ignore{
For instance, in $P_1$, after a token issuer sends an exploitable rebase transaction, it is equally likely one of the following cases occur: 1) the token issuer aware of rebase being exploitable quickly sends a swap request herself to claim the value in the Uniswap pool. 2) An attacker observing the occurrence of rebase operation calls the liquidity pool to withdraw the value there. The former case is not an attack, while the latter one is. In other cases, the same apply: In $P_3$, if the trader sends another transaction to withdraw the value in token $T1$ right after the transaction of depositing $T0$, it is a benign case. But if it is an attacker account who withdraws after the external deposit, it constitutes an attack. In $P_4$, if the trader observing the router exception and immediately send a ``make-up'' transaction to claim the value herself, it is a benign case. But if it is a third-party ill-intended account who sends the withdrawal transaction, it constitutes an attack.
}

Distinguishing attacks from benign cases entails checking two essential conditions: {\bf 1) Whether two accounts are controlled by two distinct physical users}: It cannot be an attack if the trader account who makes the profitable deposit in token $T0$ is controlled by the same physical user with the account who succeed in withdrawing the value in token $T1$. 
Thus, attack detection becomes the problem of linking two blockchain accounts of the same physical user, which is known to be an intractable problem if the only information known is on-chain data.
{\bf 2) What's a transaction sender's intention}: That is, whether a withdrawal transaction is intended as an attack. Even when the withdrawer and depositor accounts are not the same physical user, they can be friends in the real life, which makes the swap non-attack. Thus, it entails detecting the depositor account's intention in sending the withdraw request, which however can be hidden opaque and pose challenges to detection.

{\bf Feasibility of existing approaches}: 
On checking Condition 1), there are existing works that tackle the recovery of account linkage by heuristics specific to Bitcoin's UTXO model~\cite{DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13}. The only work for Ethereum~\cite{DBLP:conf/fc/Victor20} presents a linkage heuristic exploiting some DEXes deposit addresses. Specifically, on order book-based DEXes (i.e., IDEX and EtherDelta), trader Alice swapping token $T0$ for $T1$ can specify the so-called deposit address who receives $T1$. Assuming a swap is normal, the sharing of deposit addresses by two traders implies that the two traders are controlled by the same physical user. This work is different from our attack detection problem, where the deposit address heuristic is to detect the case that two accounts are linked, while our problem is to detect if two accounts are unlinked. More importantly, the deposit address heuristic works only under the assumption of normal swaps, while our work deals with risky swaps. Given a risky swap, the deposit address of a swap refers to the attacker. Thus, when an attacker targets two victim traders, it could appear that two traders share the same deposit address. In this attack, the two victim traders do not have to be linked to the same off-chain user.

On checking Condition 2), there are existing works on threat intelligence on blockchains by characterizing attackers' behavior~\cite{DBLP:conf/uss/SuSDL0XL21}. However, their targets are program-level attacks such as reentrancy attacks, and their attack strategies don't apply to the DEX context of this work.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.4\textwidth]{figures/indicators.eps}
\end{center}
\caption{Attack strategies (A1/A2/A3) and indicators}
\label{fig:indicators}
\end{figure}

\subsection{The Approach}

We discover attacks by designing attack strategies specifically for different profitable deposits and use them as attack indicators to match the observable attacker behavior on-chain. 

{\bf Design rationale: Attack strategies}: Recall that each risky swap involves with a profitable deposit followed by a withdrawal that reaps the profit. An attacker needs to strategically send the withdrawal to ensure high success rates by properly monitoring the profitable deposits. We consider three attack strategies:

\begin{itemize}[leftmargin=0cm]
%\setlength{\itemindent}{0em}
\item
 {\bf A1) Aggressive attacker (monitoring deposits)}: The attacker directly monitors the mempool for the profitable deposits. In this strategy, the attacker monitors different cases of profitable deposits, such as $P_1$/$P_2$/$P_3$/$P_4$. The attacker launches a node joining the Ethereum blockchain network and monitors the node's mempool so that the profitable-deposit transaction can be detected as soon as they are propagated in the blockchain network. 

Strategy A1 entails the attacker to customize the monitored conditions to different causes. It minimizes the time window between the exploited deposit and withdrawal, and ensures a high success rate in the presence of competitors.

\item{\bf A2)
General-purpose attacker (monitoring pool)}: The attacker monitors the Ethereum's smart contract state to check if the pool is profitable. For instance, when a rebase transaction is executed in the blockchain, it could increase the balance in the token smart contract and leave the reserve in the pool smart contract unchanged. By detecting the difference between token balance and reserve, the attacker ensures sending a withdrawal can succeed.

Strategy A2 is generalizable to different profitable deposits, in the sense that the attacker monitors a single condition that all different profitable deposits will trigger. However, this strategy works only after the profitable deposit transaction is executed and included in the blockchain. So an aggressive attacker (A1) can frontrun a general-purpose attacker (A2).

\item{\bf A3)
Lucky trader}: The trader does not intentionally observe conditions on pool profitability but is lucky in grabbing the profit by inserting a withdrawal after the profitable deposit. The delay between the withdrawal and victim deposit can be arbitrary. 
\end{itemize}

{\bf Proposed attack indicators}: 
An account's strategy, which normally occurs in the blackbox off-chain state, is not directly observable from the on-chain traces. We distill observable information and design indicators to infer attack strategies.

To start with, an aggressive attacker monitoring the off-chain mempool states cannot be observed from the on-chain traces. Likewise, a general-purpose attacker who may choose to issue RPC calls to read on-chain data is also unobservable. For these cases, we  collect the gap between the block including deposit transactions and the block including the exploit withdrawal transactions as the metric to infer the presence of an attack and further the attack strategies. For instance, if the block gap is always $0$, it indicates the case is exclusively an aggressive attack. If the deposit is token interest and the block gap is always large, it indicates an aggressive attack exploiting token interest. Otherwise, if the block gap is randomly distributed, it is likely to be a lucky trader. Based on the heuristics, we propose the following three indicators:

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I1 (Strong): An account whose withdrawal transactions occur consistently within $G$ blocks after profitable deposits (i.e., block gap smaller than $G$) and whose victim deposits are non-interest is likely to be an attacker. 
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I2 (Strong):
Indicator I2) An account whose withdrawal transactions occur consistently more than $G'$ blocks after profitable deposits (i.e., block gap larger than $G'$) and whose victim deposits are based on token interests is likely to be an attacker.
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I3: 
An account whose withdrawal transactions appear an arbitrary number of blocks after the profitable deposits are likely to be a lucky trader.
In other words, an account whose block gaps have a large deviation is likely to be a lucky trader.
}}\end{center}

In practice, many accounts use delegate smart contracts on-chain to relay their payload (of malicious withdrawals). The delegate smart contracts make attack strategies observable. We propose the following indicators to take advantage of this fact. 

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I4 (Strong):
An account who attempts to withdraw through a smart contract that checks both pool reserves (i.e., calling \texttt{pool.getReserves()}) and token balances (calling \texttt{erc20token.balanceOf()}) is likely a general-purpose attacker. Note that this indicator does not require the smart contract to actually withdraw the token $T1$. 
}}\end{center}

The intuition of the above indicator is that a general-purpose attacker uses the pool's \texttt{getReserves()} function and token's \texttt{balanceOf()} function to obtain the token reserve and balance, respectively. This shows the account's intention to calculate pool profitability and is an indicator of general-purpose attacker. 
%Note that the indicator is not necessary (i.e., causing false negatives), as a general-purpose attacker can issue RPC queries to read reserves and balances, leaving no trace on-chain.

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I5: An account whose withdrawal transactions exclude any token deposit is likely to be an attacker.
 
An account whose withdrawal transactions also include token deposits is likely to be a lucky trader, even though the withdrawal is of higher value than the deposit.
}}\end{center}

At last, we propose a heuristic that intentional attackers would victimize a diverse set of accounts while a lucky trader may victimize a fixed type of accounts (e.g., in the same pool).

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I6: If an account sends withdrawals in a large number of risky swaps, the account is an attacker.
}}\end{center}


{\bf Attack discovery algorithm}: We materialize the indicators in a holistic attack discovery algorithm. The algorithm takes as input the detected risky swaps from the previous phase (\S~\ref{sec:detectriskyswap}) and produces the strategies an attack account takes.

Specifically, recall that each risky swap consists of a profitable deposit and a (successful) withdrawal. We expand it by adding all the withdrawal attempts, no matter success or failure, on the same pool by calling its \texttt{getReserves} or \texttt{swap} functions between time $t_1$ and $t_2$ where $t_1$/$t_2$ is the time when the current/next deposit occurs. We ignore the atomic swaps (Type-I) between $t_1$ and $t_2$. Hence for each risky swap, we obtain a list of accounts who send the withdrawal or expanded withdrawal attempt. For each account and each associated swap, the algorithm checks the indicators and reports the number of attacker labels the account is tagged with. In particular, indicator I1/I2 produces the average block gap over the account's swaps when the deposit is non-interest/interest. 

\lstset{style=mystyle}
\begin{lstlisting}[caption=Pseudocode to discover attacks,
                   %linerange={1-30},
                   numbers=none,
                   %firstnumber=1,
                   deletekeywords={[2]INT},
                   morekeywords={clustered},
                   framesep=2pt,
                   xleftmargin=5pt,
                   framexleftmargin=5pt,
                   frame=tb,
                   framerule=0pt, 
                   label=code:discoverattacks,
                   float,floatplacement=H
                   ]
void AttackDiscovery(RiskySwap[] swaps, int th1, int th2){
  for(RiskySwap s in swaps){
  Mapping blockGaps;

  for(Account w in s.getWithdrawers())
    if(isCA(w)) //I4
      if(findCall(w, s.getPool(), "getReserve").getTx().checkCall(w, s.pool().tokens(), "balanceOf()")) 
        emit(w, "Attacker");
    //I1
    Block depositTime=s.getDeposit().getBlock();
    Block withdrawTime=w.getBlock();
    blockGaps.getValue(w).add(withdrawTime-depositTime));
    //I2
    numberSwaps.getValue(w).increment();
  }

  for(Account w in blockGaps.keySet()){
    blockGap.getValue(w).divideBy(numberSwaps.getValue(w));
    if(blockGap.getValue(w) > th1) emit (w, "Attacker");
    if(numberSwaps.getValue(w) > th2) emit (w, "Attacker");
}}
\end{lstlisting}


\subsection{Results}

\subsubsection{Detected Attacks}
\begin{table*}[h]
\caption{Attacker characterization: A victim can be a normal token owner (N) or token issuer (I). The numbers reported under I1-I6 columns are described next: Given an account $A$, I1 is the average block gap of $A$'s transactions matching $P_1$, $P_3$ and $P_4$; I2 is the average block gap of $A$'s transactions matching $P_2$; I3 means the deviation of the block gaps reported under I1 and I2; I4 is the number of $A$'s transactions that read both pool's reserves and token balances; I5 reports whether $A$ has sent at least one transaction to deposit before withdrawal; I6 reports the number of risky swaps. Bold are strong cases suggesting the account is an attacker. Victims include normal accounts and token issuers.}
\label{tab:attackerview}
\centering{\footnotesize
\begin{tabular}{|p{5.3cm}|p{1.0cm}|p{1.9cm}|p{0.4cm}|p{0.5cm}|p{0.5cm}|p{1.2cm}|p{0.2cm}|p{0.5cm}|p{0.5cm}|p{0.7cm}|p{0.5cm}|}
\hline
Accounts & Value & {Profitable} & \multicolumn{6}{c|}{Attack indicators} &\# &\# & Label \\
\cline{4-9}
(Mules) & ($10^3$ USD) & deposit &I1 & I2 & I3 & I4 & I5 & I6 & pools & victims & \\ \hline
$0x9799b475dec92bd99bbdd943013325c36157f383$ & 556 & $33P_1,4P_2,6P_4$ &422 &371 & 1290& 0 &N& 43 & 4 & 0/7 & A3\\
\hline
$0x2a2e25ad00faac024f6a8d8cdc0fc698fbda71b7$ & 239 & $32P_1$ &{\bf 0.03} & &0.2 & 32 ({\bf 100\%}) &Y& 32 & 1 & 0 /3 & A1\\
\hline
$0xdb40ea5b6d0ef9e45c00c194345b44765a53dd19$ & 113 & $12P_1,2P_2,3P_3$ &{\bf 2.5} &{\bf 665} &2.0 & 17 ({\bf 100\%})&Y& 17 & 1 & 0/4 & A1 \\
\hline
$0x0c08545df4939ef46c1364b5930e840739667467$ & 101 & $3P_1,1P_4$ &{\bf 1.5} & &0.7 & 0 &N& 4 & 1 & 1/1 & A2 \\
\hline
$0x56178a0d5f301baf6cf3e1cd53d9863437345bf9$ & 101 & $53P_1,4P_2,2P_3,2P_4$ &13 &{\bf 1574} &24 & 0 &N& 61 & 3 & 2/4 & A1 \\
\hline
$0xb6bf45f59b94d31af2b51a5547ef17ff81672743$ & 20 & $1091P_1,131P_2,9P_4$ &224 &{\bf 600} &471 & 1231 ({\bf 100\%}) &Y& 1231 & 9 & 12/5 & A2\\
\hline
$0xc762e15cfbf392f4346ee7e8466ca595e571382b$ & 16 & $64P_1,6P_2,13P_4$ &{\bf 3.0} & 5.3 &437 & 83 ({\bf 100\%}) &Y& 83 & 19& 0/4 & A2\\
\hline
$0xa32d3f8a970ab3222ffa1c89cb910abf7b7201d0$ & 6 & $208P_2$ & & {\bf 942} & & 208 ({\bf 100\%}) &Y& 208 & 1 & 0/0 & A2\\
\hline
\ignore{
\multicolumn{10}{|l|}{\it Least frequently swapping account}\\
\hline
0xc408 & .8 & $P_1$  & 0 & 1&  &&  N   &1 &  &  0 + 1 & \\
\hline                                                    
0x02ef & .1   &  $43P_1, 9P_4$  & 2.6  &&2.4  &  52&Y & 52       &  &  1 + 0 & \\
\hline                                                    
0x2839 & .04 & $P_1$ & 0   &0  &   &&N     &1    &  &  0 + 1 & \\
\hline                                                    
0x042d & .03 & $P_1$ & 130 &0  &  & 1    &N&  &  &  0 + 1 & \\
\hline                                                    
0x5b1b & .01 & $P_1$ & 206 &0  &   & 1   &N&      &  &  0 + 1 & \\
\hline                                                    
0x6cea & .01 & $P_1$ & 904 &0  &   & 1     &N& &  &  0 + 1 & \\
\hline                                                    
0xf39f & .01 & $P_3$ & 0   &0  &   & 1     &N&    &  &  1 + 0 & \\
\hline                                                    
}
\end{tabular}%
}
\end{table*}


We present our analysis result in Table~\ref{tab:attackerview} which characterizes the most frequent accounts involved in risky swaps. The metrics include value stolen, causes, attacker indicators, the number of pools attacked, the number of victim accounts, and the label whether the account is an attacker.  From the table, we analyze the attackers' strategy of several selected accounts.

{\bf Case 1: Agg. attacker (A1) w. zero block gap}: Account $0x2a2e$ is involved in $32$ risky swaps (I6) and gains more than $2.39*10^5$ USD worth of illicit tokens. All $32$ swaps from this account are sent via a smart contract which checks the pool's profitability before withdrawal (I4). In terms of timing, the malicious withdrawals are always sent in the same block with the risky, profitable deposit. We believe account $0x2a2e$ aggressively monitors the mempool for the target tokens' rebase transactions, and if found, sends withdrawals immediately to ``backrun'' the deposits and claim the value.

{\bf Case 2: General attacker (A2) w. off-chain monitoring}: Account $0x0c08$ has withdrawn four times and grabbed tokens of $1.01*10^5$ USD. The account directly and externally calls Uniswap pool's swap function to withdraw, without checking pool profitability on-chain. The withdrawals are included in exactly one block after the one that includes the risky deposit. We believe Account $0x0c08$'s strategy is to monitor the pool profitability from an off-chain vantage point and to immediately send withdrawal by external calls. Because the account monitors the pool profitability instead of the cause (risky deposit), it has to wait until the inclusion of risky deposit that updates the pool state to be profitable. This explains why the inclusion of withdrawal has to be one block after the one including the risky deposit.

{\bf Case 3: Agg. attacker (A1) stealing interest}: Both Accounts $0xdb40$ and $0x5617$ have extracted value from interest bearing tokens. Their block gaps are large ($665$ and $1574$, respectively). Given that there are enough samples, this consistent behavior shows both accounts' attack strategy to wait long enough for the token interest to accumulate and for the extractable value to be large enough before acting on it.

{\bf Case 4: Adapting strategies}: For all accounts with indicators I1 and I2 in the table, it is clear that the block gaps for different causes (I1 and I2) differ: The block gaps for non-interest causes are consistently much shorter than those for token interests. It implies that the attackers are aware of the situation (which causes to exploit) and tailor their strategies to it.

{\bf Case 5: Lucky trader (A3)}: Account $0x9799$ is unlikely an intentional attacker: First, it does not read the token balance or check the pool's profitability before the withdrawal. Second, the block gap between profitable deposit and malicious withdrawal is large, at hundreds of blocks apart. In addition, the smart contract Account $0x9799$ relays her withdrawal requests also makes deposit to the pool. All these indicators show that $0x9799$ is unlikely an intentional attacker, but instead a lucky trader.

\subsubsection{Block Gaps}

\begin{figure}[!ht]
  \begin{center}
    \subfloat[Block gaps and the number of competing attackers]{%
\includegraphics[width=0.245\textwidth]{figures/figure_allrebase_blockdif.eps}
\label{fig:blockdif_1}
    }%
    %\hspace{-0.2cm}%
    \subfloat[Block gaps and value stolen]{%
\includegraphics[width=0.245\textwidth]{figures/figure_value_blockdif.eps}
\label{fig:blockdif_2}
    }%
  \end{center}
  \caption{Block gaps and affecting factors}\label{fig:complex}\vspace{-0.10in}
\end{figure}

Recall that each of theft attack runs in two transactions: The first transaction that creates extractable value, and the second transaction that withdraws the value and steals it. Given each detected attack (described from the previous subsection), we measure the gap of the two blocks that respectively include the attack's two transactions, namely block gap. We further report two metrics, that is, the number of competing attackers and the value stolen. Particularly, for each profitable deposit transaction, say $tx$, we find transactions sent by competing attackers. Here, a competing attacker either directly sends a transaction to withdraw the extractable value created by $tx$ but fails, or sends a transaction to read the token balance and pool reserve (which shows the intention to withdraw the value). 

We report the block gaps with the varying number of competitors in Figure~\ref{fig:blockdif_1}. A larger dot in a X/Y coordinate in the figure represents more attacks found with the same X/Y value. The result shows that when there are many competing attackers, the block gap tends to be small. This could be explained: Because the first attacker wins, the more attackers there are, the earlier the withdraw transaction is sent, namely smaller block gap.
The result also shows that with few competing attackers comes a large range of block gaps.

We then report the block gaps with varying value stolen in Figure~\ref{fig:blockdif_2}. The result shows that when the stolen value is large, the block gap tends to be small. A possible explanation is that the higher extractable value gives the attacker more incentives to send the withdrawal transaction with higher fee and to frontrun other potential thieves.
 
\subsubsection{Attacker/Victim Behavior over Time}

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_attacker_timeline.eps}
\end{center}
\caption{Attack timeline of top-10 attackers. In the Y axis, attacker accounts are ordered by total value stolen.
Data from 07/09/2020 (block 10422671) - 06/29/2021 (block 12727620).}
\label{fig:attack}
\end{figure*}

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_victim_timeline.eps}
\end{center}
\caption{Attack timeline of top-10 victims. In the Y axis, victim accounts are ordered by total value stolen.
Data from 07/29/2020 (block 10553883) - 01/10/2022 (block 13979019).}
\label{fig:victim}
\end{figure*}

We plot the timeline of the top-10 attackers' activities in Figure~\ref{fig:attack}. The attackers are ranked by the total value stolen, with attacker $0x9799$ being the top-1. Each dot represents a detected attack sent by the attacker's account. The size of the dot represents stolen value. Color represents the exploit pattern. The most successful attacker ($0x9799$) steals value despite through different causes (including rebase, airdrop, etc.) The attacker's activities last about 
$1.1*10^6$ blocks, which amount to six months. The second attacker ($0x2a2e$) concentrates all her attacks to a one-month span. She exploits exclusively the value created by rebase operations. The third attacker ($0xdb40$) mount attacks sporadically and target value created through two causes: Token interest and rebase operations. The ninth attacker exploits partly errors to gain illicit profit. The tenth attacker exclusively grabs value from token interest in a three-month period. As a result, most top attackers mount multiple attacks consistently, which show the attacks are intended and not by accident.

We additionally study top victims' behavior. The victims are ranked by the value stolen. In Figure~\ref{fig:victim}, we plot in dots the transactions sent by victims whose deposit are stolen in identified attacks. Different color represents different causes. Additionally, in green hollow circles, we plot the normal transactions sent by the victims and related to Uniswap. The result shows that most victims change behavior after an attack/theft. For instance, victim accounts, including $0x0cd4$ and $0x80cc$, all stop using the vulnerable interface (e.g., partly error) to send deposit after an attack. However, other victims can repeatedly create extractable value that gets stolen. For instance, account $0x66ac$ repeatedly airdrop tokens to the Uniswap pool, which gets stolen. 

\subsubsection{Value Received by Pools}

\begin{table}[!htbp] %force in current page, disable float.
\centering{
\begin{tabularx}{0.425\textwidth}{ |X|l|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
\hline
Value extracted by & Rebase ($P_1$) & External transfer ($P_3$) \\
\hline
External attackers & \$0.81M & \$0.50M \\
\hline
Pools (intended) & \$58.1M & \$1.22M \\
\hline
Pools (accidental) & \$0.65M & \$1.29M \\
\hline
\end{tabularx}
}
\caption{Extractable value and its destinations}
\label{tab:extractable_value}
\end{table}
\begin{figure}[!htbp]
\begin{center}
  \subfloat[Value created by rebase ($P_1$)]{%
     \includegraphics[width=0.245\textwidth]{figures/figure_rebase_seg.eps}
    \label{fig:moneyflow_1}
  }%
  \subfloat[Value created by external transfers ($P_3$): all pools are between token $XX$ and $WETH$, where $XX$ is the tick on the $x$ axis.]{%
    \includegraphics[width=0.245\textwidth]{figures/figure_underwater_seg.eps}
     \label{fig:moneyflow_2}
     }%
\end{center}
\caption{Extractable value received by the pool versus that by attacker accounts}\label{fig:complex}\vspace{-0.10in}
\end{figure}


Extractable value can be claimed by any account, including an external attacker and the pool itself. Our measurement result so far captures the former case. In this experiment, we measure the extractable value that goes to the pool.

A pool can claim extractable value by calling the \texttt{sync} function, which synchronizes the pool reserve and token balance. In Uniswap, there are three circumstances \texttt{sync} is called: a standalone call to \texttt{sync} in a transaction, \texttt{sync} called after a \texttt{swap} in the same transaction, \texttt{sync} called after an \texttt{addLiquidity} call in the same transaction. In the first case, tokens are sent to the pool intentionally (denoted by ``pool (intended)'' in the table and figures), and in the second and third cases, the pool receives deposit by accident (denoted by ``pool (accidental)''), because it is an irrelevant transaction to \texttt{sync} the reserve and token balance. Informally, we calculate the extractable value that goes to the pool in the following method: We obtain the value of pool reserve before and after the transaction. We also parse the function call arguments from the transaction data field. We can cross-check the pre-state, post-state and function arguments, to detect the mismatch, which can be attributed to the extractable value. For instance, a normal \texttt{swap} in Uniswap does not change the product in AMM, and a spurious \texttt{swap} that the pool receives extractable value can be detected by the violation of product equality.

Using the above method, we measure the total extractable value claimed by the pool under different patterns, including $P_1$ and $P_3$. The result is presented in Table~\ref{tab:extractable_value}: The total value claimed by the pools is consistently more than $5\times$ of that by external attackers. This suggests ``room'' for the current Uniswap thief to increase their revenue. We further show the total extractable value by different pools/tokens. In Figure~\ref{fig:moneyflow_1}, we plot the extractable value created by different rebase-enabled tokens (Pattern $P_1$). 
Token $AMPL$ has the highest extractable value, most of which goes back to the pool by the token issuer intentionally calling \texttt{sync} function after each \texttt{rebase} call (the ``intended'' case). 
Token $BASE$ is the third highest in total extractable value and has the highest value stolen by external attackers. In Figure~\ref{fig:moneyflow_2}, we plot the extractable value created by external transfers (Pattern $P_3$) against different pools. Here, all the top-value pools we found are between token $WETH$ and another token. The most vulnerable pool is between Token $UNI$ and $WETH$, whose extractable value is $400$ thousand USD in total, among which the $10\%$ value is extracted by external attackers and the rest is mostly sent to the pool intentionally. Token $YFill$'s value is exclusively extracted by external attackers. Token $SUSHI$'s deposit is mostly claimed by the pool accidentally. 

\subsection{Characterizing Crimes}
\label{sec:behavior}

We further expand the scope of each attack instance by tracing the money flow and smart contract lineage. The goal is to uncover the attack business.

\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.495\textwidth]{figures/UniswapV2attacker3.eps}
\end{center}
\caption{Attack campaign template: Preparing, mounting and wrapping up theft attacks.}
\label{fig:business}
\end{figure}

Given an attack instance with attacker accounts $\{A\}$, we construct an expanded attack graph by adding the following information: 1) the transactions that pay Ether or tokens to the attacker accounts, 2) the transactions that deploy the smart contracts used in the attack, and 3) the transactions that are sent by the mule accounts who receive the stolen tokens after the attack. These new transactions would add into the graph a set of new accounts, be it either the transaction sender or receiver. We iteratively apply this graph-expansion process, until it reaches the ``hub-node'' accounts, which receive or send a large number of transactions (e.g., a popular DEX pool or mixer service). 
For instance, Figure~\ref{fig:business} shows an example of expanded attack instance, with the attackers in the red box and the victims; the added accounts and transactions are outside the two boxes. 

{\bf Attack ecosystem template}: We analyze the expanded attack graph in a template consisting of three phases: 1) attack preparation, 2) attack execution, and 3) attack wrap-up. Phase 2) is the core attack component, and Phases 1) and 3) are the expanded  parts. In general, the actual Boss often sits behind an exchange/mixer service, such as Tornado~\cite{me:tornado}, to hide its identity. In  attack preparation (Phase 1), the Boss sends commission in Ether to Attackers and Exploit developers. The Ether transfer can be relayed through the Mules. An Exploit developer writes an Exploit smart contract and deploys it to the blockchain. It then mounts the attack in the execution phase (Phase 2), exercising the strategies described previously (\S~\ref{sec:attack}). To wrap up a series of attacks (Phase 3), the mule receiving the stolen tokens transfers the tokens back to the Boss. This is often done by swapping the stolen tokens to ETH (e.g., via DEX and wrapped tokens such as WETH) and by sending the ETH to the Boss via a mixer service. In the attack wrap-up phase, the mule may transfer tokens to Investors to maximize the stolen value. 

\begin{table*}[h]
\caption{Attack ecosystem and attacker correlation: Red text shows the two attackers share the same developer of exploit smart contracts. AO represents attack operator and EC is exploit smart contract.
}
\label{tab:eco}
\centering{\small
    %\begin{tabular}{|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{1cm}|p{1.2cm}|}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \hline
    Accounts & \multicolumn{4}{c|}{Attack (S2)} & \multicolumn{2}{c|}{Preparation (S1)} & \multicolumn{2}{c|}{Wrap-up (S3)}  \\ \cline{2-9}
    (Mules) & \#AO & \#EC & Developer & Value ($10^3$ USD) & Commission & Mixer & DEX & Mixer \\
    \hline
     $0x9799$ & 5 %$0x4e53$, $0xac72$, $0xa084$, $0x5bb4$, $0xe929$ 
& 24 % $0x338c$, $0x3ac7$, $0x34a2$, $0x9a99$, $0x2927$, $0x536b$, $0xe9f8$, $0x684b$, $0x58a3$, $0x72bb$, $0xa8a2$, $0x72cb$, $0x2528$, $0xbf2d$, $0xadfc$, $0xd6a2$, $0x24af$, $0x1335$, $0xf367$, $0x94fc$, $0x5caf$,  $0x6332$, $0x3c3a$, $0x1233$	
& {\bf \color{red} $0x8641$} & 556 & \xmark  & \xmark  & \cmark  & \xmark \\
    \hline
    $0x2a2e$  & 1 %$0x2a2e$ 
& 1 %$0x5f5a$ 
& $0x2a2e$ & 239 & \cmark  & \xmark  & \cmark  & \cmark 
\\
    \hline
    $0xdb40$  & 5 %$0x64bc$, $0x62ae$, $0x3807$, $0x225c$, $0xdb40$ 
& 2 %$0x4dbc$, $0x4626$ 
& $0x4626$ & 113 & \cmark  & \cmark  & \cmark  & \cmark 
\\
    \hline
    $0x0c08$  & 1 %$0xfdee$ 
& 1 %$0x0c08$ 
& $0x0c08$ & 101 & \xmark  & \xmark  & \cmark  & \xmark 
\\
    \hline
    $0x5617$  & 4 %$0x3a51$, $0xf97b$, $0xbf3f$, $0xa1e6$ 
& 10 %$0xfb51$, $0x328d$, $0x8a14$, $0x0fc7$, $0x4ed5$, $0xb439$ ,$0x55a2$, $0x6ba3$ 
& \color{red}{$0x8641$} & 101 & \xmark  & \xmark  & \cmark  & \cmark 
\\
    \hline
    $0xb6bf$ & 1 %$0x675f$ 
& 2 %$0xb6bf$, $0x8526$ 
& $0x675f$ & 20 & \cmark  & \xmark  & \cmark  & \xmark 
\\
    \hline
    $0xc762$ & 1%$0xd0d0$ 
& 1%$0xc762$ 
& $0xd0d0$ & 16 & \cmark  & \cmark  & \cmark  & \cmark 
 \\
    \hline
    $0xa32d$ & 1%$0x7505$ 
& 1%$0xa32d$ 
& $0x7505$ & 6 & \cmark  & \xmark  & \xmark  & \xmark 
\\
    \hline  
    \end{tabular}%
}
\end{table*}

\ignore{
\begin{table}[h]
\caption{Attack ecosystem and attacker correlation: Red text shows the two attack instances are mounted using the exploit smart contracts developed by the same developer. AO represents attack operator and EC is exploit smart contract.
}
\label{tab:eco}
{\centering \scriptsize
    \begin{tabular}{|p{0.3cm}|p{1cm}|p{0.3cm}|p{0.3cm}|p{1cm}|p{0.7cm}|p{0.8cm}|p{.5cm}|}
    \hline
    Idx &Value ($10^3$~USD) & \#AO & \#EC & Developers & Mules & Deposits & Block gaps\\
    \hline
    1 & 552 & 5 %$0x4e53$, $0xac72$, $0xa084$, $0x5bb4$, $0xe929$ 
& 24 % $0x338c$, $0x3ac7$, $0x34a2$, $0x9a99$, $0x2927$, $0x536b$, $0xe9f8$, $0x684b$, $0x58a3$, $0x72bb$, $0xa8a2$, $0x72cb$, $0x2528$, $0xbf2d$, $0xadfc$, $0xd6a2$, $0x24af$, $0x1335$, $0xf367$, $0x94fc$, $0x5caf$,  $0x6332$, $0x3c3a$, $0x1233$	
& {\bf \color{red} $0x8641$} & $0x9799$ & $P_1$ & 121\\
    \hline
    2 & 101 & 1 %$0x2a2e$ 
& 1 %$0x5f5a$ 
& $0x2a2e$ & $0x2a2e$ 
& $P_1$ & 1\\
    \hline
    3 & 96 & 5 %$0x64bc$, $0x62ae$, $0x3807$, $0x225c$, $0xdb40$ 
& 2 %$0x4dbc$, $0x4626$ 
& $0x4626$ & $0xdb40$ 
& $P_1$ & 0\\
    \hline
    4 & 86 & 1 %$0xfdee$ 
& 1 %$0x0c08$ 
& $0x0c08$ & $0x0c08$ 
& $P_1$ & 1\\
    \hline
    5 & 67 & 4 %$0x3a51$, $0xf97b$, $0xbf3f$, $0xa1e6$ 
& 10 %$0xfb51$, $0x328d$, $0x8a14$, $0x0fc7$, $0x4ed5$, $0xb439$ ,$0x55a2$, $0x6ba3$ 
& \color{red}{$0x8641$} & $0x5617$ 
& $P_3$ & 2\\
    \hline
    6 & 48 & 1 %$0x675f$ 
& 2 %$0xb6bf$, $0x8526$ 
& $0x675f$ & $0x675f$ & $P_1$ & 0\\
    \hline
    7 & 29 & 1%$0xd0d0$ 
& 1%$0xc762$ 
& $0xd0d0$ & $0xd0d0$& $P_3$ & 1 \\
    \hline
    8 & 22 & 1%$0x7505$ 
& 1%$0xa32d$ 
& $0x7505$ & $0x7505$& $P_1$ & 0 \\
    \hline  
    \end{tabular}%
}
\end{table}
}


{\bf Results}: We measure the attack behavior in terms of attack preparation, execution and wrap-up. We find different attacks mounted by the same mule account are consistent and thus present the aggregated results by mule accounts. The result is in Table~\ref{tab:eco}.

In the attack execution phase (S2), the result shows that attacks are systematic, typically with a mule associated with multiple attack operators (AO) and exploit smart contracts (EC). For instance, Mule $0x9799$ has mounted attacks through $5$ different operator EOAs and leveraged more than $24$ different exploit smart contracts. Her exploit contracts are developed by the same developer for another Mule $0x5617$ (in red in Table~\ref{tab:eco}); this implies an underground business of exploit contract development.

We further characterize the attack preparation (S1) and wrap-up (S3) on different mules. Under S1, Column ``Commission'' shows whether the mule's attack operators receive money used for mounting the attacks within 30 days before the attack. Column ``Mixer'' shows whether the attack commission comes from the anonymized crime boss hidden behind a mixer service, such as Tornado. Under S2, Column ``DEX'' shows whether the attacker interacts with a DEX service to exchange tokens or to maximize the illicit profit. Column ``Tornado'' shows whether the attacker eventually transfer money to the anonymized boss behind the mixer service. The result shows that different mules vary in their strategies in attack preparation and wrap-up. For instance, Mule $0x9799$ is quite simplistic in the sense that she only interacted with DEX and didn't involve any mixer service in her attacks. Mule $0xdb40$\footnote{The full address of $0xdb40$ is $0xdb40ea5b6d0ef9e45c00c194345b44765a53dd19$ and the account behavior is public on \url{https://etherscan.io/address/0xdb40ea5b6d0ef9e45c00c194345b44765a53dd19}.} and $0xc762$, on the other hand, are quite sophisticated and employ strategies involving mixer and DEX.

\section{Countermeasures}
\label{sec:mitigate}

This section presents two types of countermeasures, by patching the pool smart contracts and by hardening deployed DEX.

\subsection{Patching Pool Smart Contracts}

To mitigate the risk, one can patch a pool, deploy the patched smart contract to a new blockchain address, and convince traders to use the patched pool at the new address. The success of this approach relies on whether the new pool can attract existing and new liquidity providers. 

In this subsection, we discuss 1) how to design a secure AMM pool under token thefts, and 2) how practical it is to migrate liquidity providers from one DEX to another. In particular, Uniswap has launched Version V3 as a subsequent version of V2. Measuring the liquidity migration will help understand the relationship between V2 and V3 (i.e., are they suppose to co-exist or one replacing another). 

\subsubsection{Designing Secure AMM Pool}

To start with, we first review Uniswap-V2's vulnerability and analyze the root cause.

\noindent
{\bf Uniswap-V2's vulnerability}: Recall that in an AMM, a trader interacts with a liquidity pool to swap tokens. Normally, the trader makes a deposit (in one token) to the pool's account and then withdraws the value from the pool (in another token). The pool needs to maintain a copy of token balances, namely reserves, which is essential in calculating and updating token-exchange rates.

Uniswap-V2 materializes the above AMM architecture by the following design choice: It requires synchronizing the pool reserves against the token balances (i.e., the pool account's balance in the token smart contract). It (mis)uses the synchronized reserve, or more precisely, monitoring any reserve update, to infer token deposits, instead of directly tracking the deposits in the pool smart contract (i.e., deposits do not call any Uniswap-V2's procedures).  

While the design is intended to support flexible mechanisms of trader deposits including both standard token transfer and non-standard balance-updating operations, it sacrifices the security. Without directly tracking deposits, the pool smart contract does not know the sender accounts of deposits and is forced to accept any withdrawal without access control, that is, permissionless withdrawal. Without enforcing swap atomicity in the pool smart contract or in risky applications where value is deposited into pool's account without withdrawal, the permissionless withdrawal creates value-extraction opportunities, which can be seized by attackers who front-run legitimate traders, if any.

{\bf Secure AMM pool}: We propose a secure design of the AMM pool. In this design, the pool tracks deposit calls (i.e., let the pool be present in every deposit) and records the deposit senders. By this means, the pool can enforce that the deposit can only be withdrawn by the account making the deposit. This avoids the permissionless withdrawal in Uniswap-V2 and prevents creating extractable value.

Besides, our secure AMM pool retains the Uniswap-V2's design on synchronizing pool reserves with token balances, which is essential in preventing arbitrage and price manipulation.

Overall, our AMM pool keeps track of the two types of token-balance updates: 1) deposits and 2) other causes of balance updates, such as token rebasing and airdropping, that are not intended for swapping. The token balance added through deposit can only be withdrawn by the deposit account, and the token balance added in other means cannot be withdrawn. By this means, it prevents value extraction by arbitrary accounts. 

However, our secure AMM pool does sacrifice the flexibility of deposit supports. A trader cannot freely choose the deposit mechanism in doing a swap; for instance, if she directly transfers tokens to the pool's account, she will not be able to receive any value in return in our AMM pool.

{\bf Distinction to Uniswap-V3}: Our AMM pool is distinct from Uniswap-V3, a redesign of Uniswap pool deployed to the main net in May 2021. A key design in Uniswap-V3 is not to synchronize the pool reserve with token balance, which creates opportunities for arbitrage and denial of service. While a full security analysis of Uniswap-V3 pool is out of this paper's scope, we describe a vulnerability we discovered on Uniswap-V3 exploiting the unsynchronized pool reserve in Appendix~\ref{sec:uniswapv3:attack}. We demonstrate the success of the attack on a local Ethereum node running unmodified Uniswap-V3 smart contracts. The vulnerability is reported to the Uniswap bug-bounty program~\cite{me:bugreport:defiant}.

In deployment, we view Uniswap-V2 and V3 as two co-existing DEX instances, instead of one to replace the other. Because it is costly for liquidity providers to migrating their value from one DEX to another, as analyzed and measured below.

\subsubsection{Measuring Liquidity Migration}

\begin{figure}[!ht]
  \begin{center} 
    \subfloat[Number of migration transactions over all Uniswap-V2 pools]{%
       \includegraphics[width=0.24\textwidth]{figures/migration-amount-perday.eps} 
       \label{fig:migrate1}
    }%
    \subfloat[The percentage of migrated tokens on top-three Uniswap-V2 pools]{%
       \includegraphics[width=0.24\textwidth]{figures/remained-percentage.eps} 
       \label{fig:migrate3}
    }%
 \caption{Token/value migration out of Uniswap-V2}
  \end{center}
\end{figure}


The success of a patched pool relies on how much the new pool can attract enough liquidity from existing and new providers. It would be relatively easy for a new liquidity provider to use the patched smart contract. However, it would pose a challenge for existing ``small-business'' liquidity providers to migrate their investment from Uniswap-V2 to Uniswap-V3. The obstacle comes from the relatively high transaction fees compared to the small-volume assets owned by the non-professional, retail providers.

%Another direction to mitigate attacks is to develop patched smart contracts for an AMM pool and deploy them to new blockchain addresses. This approach entails migrating {\it both} liquidity providers and traders to the new pool smart contracts. Note that migrating only traders is insufficient, as the new pool without liquidity providers means a pool without sufficient reserves, which are less attractive to traders. However, in DEX, each liquidity provider is typically an average token owner who invests a small amount in the pool reserves (i.e., a non-professional, retail investor). Such retail provider making small investments would be deterred by the high transaction fees to migrate their invested tokens to a new pool smart contract.

In practice, the difficulty of migrating existing liquidity providers is real. We conducted a measurement study on the Uniswap-V2 using the method as follows: Given that Uniswap deployed a smart contract facilitating migration\footnote{Address of this smart contract is \url{https://etherscan.io/address/0xa5644e29708357803b5a882d272c41cc0df92b34\#code}.}, we collected all the transactions received by this smart contract, joined transaction hashes against the contract's event log, and extracted the contract-call arguments representing the migrated tokens and value. Figure~\ref{fig:migrate1} plots the number of migration transactions per day over time in a $481$-day period. The number of migration transactions spikes at $1839$ transactions on Day $125$ when Uniswap-V3 was launched, then quickly drop, and eventually remains below $9$ transactions per day after Day $250$.
Figure~\ref{fig:migrate3} plots the percentage of tokens remaining in the pool over time. Before Day $125$ when Uniswap-V3 is launched, all three pools have $100\%$ tokens. For all three pools, most drops of token reserves occur within $80$ days after the launch of Uniswap-V3, after which the remaining tokens in a pool become stabilized. The only exception is a dip that occurs around Day $480$ on Pool $USDT-WETH$. Eventually, the remaining tokens in the three pools ($USDC/UNI/USDT$) converges at $80\%/62\%/50\%$.
At last, the difficulty and high cost of migrating providers out of Uniswap-V2 is corroborated by online user complaints~\cite{me:migratev3:complaint1,me:migratev3:complaint2}. 

\subsection{Hardening Deployed DEXes}

{\bf Lost-and-found service off-chain}: We propose running a lost-and-found off-chain web service. This off-chain service monitors the on-chain state for profitability and collects extractable value ahead of actual attacks. To do so, the service takes an aggressive strategy by directly monitoring the vulnerable deposits (i.e., $P_1$, $P_3$, $P_4$) and withdrawing immediately upon discovery. For token interest $P_2$, the service monitors mempool for stealing transactions sent to the pools supporting token interests. Upon the discovery, the service sends transactions to frontrun the stealing transactions. 

In essence, this service performs the same functionality with thief attackers in discovering profitability opportunities on-chain, but it is benign in the sense that it stores the extracted value and allows victims to claim their tokens. Technically, given value deposited by Account $V$, the service stores the value and allows $V$ or any other account with $V$'s signature to claim the value.

{\bf Fuzzing router smart contracts}: For the risky swaps caused by buggy router contracts (i.e., $P_4$), one can mitigate the problem by developing more secure router smart contracts. Here, to ensure that the router calls deposit and withdrawal in all possible code path, we fuzz the router smart contract using a fuzzing framework Echidna~\cite{DBLP:conf/issta/GriecoSCFG20}. Specifically, we develop a test oracle that defines swap atomicity and a smart contract rewriter to automatically insert the oracle to the target router smart contract. The test oracle records all the \texttt{transfer}/\texttt{transferFrom}/\texttt{swap} invocations and checks if there is a standalone invocation in the end of execution.   

\section{Related Work}
\label{sec:rw}

This work is related to blockchain data analysis. We survey blockchain-data analysis for attack detection and user de-anonymization. 

{\bf Detecting Smart-Contract Program-level Attacks}: Attack detection on blockchain generally works as distilling the attack signatures from known vulnerabilities and attack patterns and matching certain representation of smart-contract execution (e.g., in transactions, function-call graph or instruction traces) against the attack signatures. There are known patterns of smart-contract program-level attacks, such as reentrancy attacks, transaction order dependency, etc. Existing works tackle the detection of program-level attacks on Ethereum-like blockchains. 
 
TxSpector~\cite{DBLP:conf/uss/ZhangZZL20} records and replays Ethereum transactions into fine-grained EVM instruction traces, which are stored in datalog databases and queries to compare against the signatures of known attacks. Similarly, Zhou et al~\cite{DBLP:conf/uss/ZhouYXCY020} model the coarse-grained traces of smart contract function calls and match them against known attack signatures. At its core, two function calls are modeled, that is, smart contract creation/destruction and token transfers (money flow). Su et al~\cite{DBLP:conf/uss/SuSDL0XL21} uses reported attack instances to extract attack signatures, and it discovers new attacks as well as uncovers the attacker/victim behavior by systematically analyzing the Ethereum blockchain traces. Other similar work~\cite{DBLP:conf/uss/0001L21} detects the attack instances of known vulnerabilities.  

{\bf Detecting DeFi Protocol-level Attacks}: In addition to detecting program-level attacks, there are related works on detecting protocol-level attacks on deployed DeFi applications. Notable DeFi attack patterns include frontrunning, arbitrage, etc. 

Torres, et al.~\cite{DBLP:conf/uss/TorresCS21} detects front-running attacks by matching Ethereum transactions against a signature of success-failure transaction pair. Qin et al~\cite{DBLP:journals/corr/abs-2101-05511} systematizes different types of front-running attacks and measures the attacks and mitigation in the wild.

Front-running attacks are a class of attacks in which the attacker inserts a malicious transaction before the victim transaction to extract illicit profit (e.g., to win an auction bid unfairly). More generally, front-running is a class of MEV or miner extractable value, in which transaction order can be manipulated by a profit-driven miner to receive additional profit.

Arbitrage attacks work by an aggressive trader gain profit by exploiting difference of exchange rates across different DEXes/price oracles. Wang, et al~\cite{DBLP:journals/corr/abs-2105-02784} detects cyclic arbitrage on Uniswap-V2, by finding profitable cycles on token-transfer graph (nodes are tokens and edges are transfers). Similarly, Zhou, et al~\cite{DBLP:conf/sp/ZhouQCLG21} discovers profit-generating transitions in real-time by finding cycles  and leveraging solvers.

{\bf User de-anonymization}: While blockchain accounts and their activities are visible, the linkage of accounts (which are public keys) with real-world identities is not directly observable. There are existing works to infer blockchain account linkage in efforts to deanonymize users. Specifically, there are three types of linkage information: 1) Whether a specific account is linked to a specific real-world user identity. Existing works~\cite{DBLP:conf/fc/KoshyKM14} monitor a blockchain network' traffic of transactions propagated from an IP and link the transaction sender's account with the IP. 
%Other works~\cite{XXX} aggregate transaction volume of a given account and use background knowledge to link the account to real-world ID.

2) Whether two blockchain accounts are linked, as the sender and receiver, in a privacy-enhanced transaction. Mixing services are intended to break the sender-receiver linkage. There are existing works aimed at reconstructing the sender-receiver relation on transactions relayed through mixing services. In particular, address reuse is a heuristic to link transaction senders/receivers on Bitcoin-like blockchains~\cite{DBLP:conf/uss/YousafKM19,DBLP:conf/uss/KalodnerMLGPCN20}.

3) Whether two blockchain accounts are shared by the same real-world user. On Bitcoin, transaction graph analysis~\cite{DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:books/daglib/0040621} is proposed to recover the account linkage. Particularly, address clustering heuristics are proposed. For instance, two accounts that are co-spent by a Bitcoin transaction or that involve a change are likely to be controlled by the same off-chain user. These address clustering heuristics are useful only in the context of Bitcoin's UTXO model. Address clustering is useful to uncover the money flow in online criminal activities such as ransomware payments on Bitcoin~\cite{DBLP:conf/sp/HuangALIBMLLSM18}. 

Of most relevance to this work is the address clustering techniques proposed to link Ethereum accounts~\cite{DBLP:conf/fc/Victor20}. Specifically, the observation is that some DEXes support the deposit address, that is, trader Alice swapping token T0 for token T1 can specify a ``deposit'' address to receive T1. Multiple accounts using the same deposit address are likely to be the same off-chain user. 

This work is different from Ethereum account linkage. In this work, the attack detection problem is to verify whether two Ethereum accounts are from two off-chain users, which is different from detecting if two accounts are linked by the same off-chain user. Moreover, the Ethereum address clustering work~\cite{DBLP:conf/fc/Victor20} has to assume that the swap is atomic, normal one, so that they can attribute address sharing to the cause of the same off-chain user. By contrast, in this work, we do observe two sender accounts share the same deposit address, but they are caused by two victim accounts whose swaps are grabbed by the same attack account, as verified by our analysis of attacker/victim behavior.


\section{Responsible Disclosure}
\label{sec:disclosure}

We have reported the discovered atomicity violations and the vulnerabilities to Uniswap's bug bounty program (\url{https://uniswap.org/bug-bounty}). The bugs have been confirmed. Further details on bug reporting are documented on the anonymized Google document~\cite{me:bugreport:defiant}. 

\section{Conclusion}
\label{sec:conclude}

This paper presents the first measurement study of atomicity violations and token theft attacks on popular Uniswap DEXes on Ethereum. The study unearths more than $465$ thousand thefts and stolen tokens worth of a total of $3.5$ million USD. It uncovers a range of previously unknown patterns of vulnerable deposits (e.g., token interest and supply adjustment), exposes real-world attackers' adaptive strategies to send malicious withdrawals, and reveals their systematic behavior in preparing, executing, and finalizing theft attacks. Finally, it presents mitigation schemes to remedy the deployed DEXes running immutable smart contracts.


==> text/old/v7_intro.tex <==
\section{Introduction}

Recent years witnessed the rise of Decentralized Finance (DeFi) on blockchains. A prominent class of DeFi applications is the Decentralized Exchange (DEX) which allows a trader account to swap their assets from one token to another. 
On Ethereum, deployed DEX instances including Uniswap~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer} all run AMM protocols or automated market maker, which account for more than $99.9\%$ of the DEX market, attracting hundreds of millions of transactions as of this writing (2022). Other than token swap, an AMM also supports liquidity addition/removal operations in which a liquidity provider account deposits tokens to be used as reserve for token swaps.

AMM can be misused. A well studied class of AMM misuses are sandwich attacks and arbitrage~\cite{DBLP:conf/sp/DaianGKLZBBJ20,DBLP:journals/corr/abs-2101-05511}. In both attacks, the attacker account extracts illicit value by sending transactions in crafted orders, where each transaction calls an AMM operation to either swap tokens or to manage liquidity. Recent research has shown the large scale of sandwich attacks and arbitrage on Ethereum~\cite{DBLP:journals/corr/abs-2101-05511}. 
Another AMM misuse is to list scam tokens~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21} that impersonate other tokens and trick their traders. Both AMM misuses can be detected by certain patterns on their traces of multiple AMM operations, such as arbitrage by profitable cycles of token swaps~\cite{DBLP:journals/corr/abs-2105-02784}, scam tokens by short-lived span of AMM operations~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21}, etc.

\begin{figure}[b!ht]
\begin{center}
\includegraphics[width=0.26\textwidth]{figures/workflow7.eps}
\end{center}
\caption{Data-analytical workflow to detect AMM operation atomicity violation, stolen tokens and theft attacks.}
\label{fig:workflow7}
\end{figure}




\vspace{2pt}\noindent\textbf{Discovering atomicity violations}. 
This work aims to discover previously unknown AMM misuses and to measure their impacts on actual AMM instances and blockchain networks. Instead of the known multi-operational misuses our goal is to uncover intra-operation misuses; more specifically, we measure whether an AMM operation executes token deposits and withdrawals in an all-or-nothing manner (i.e., the atomic execution). 
To our surprise, we find atomicity violation widely exist among deployed AMM instances: By extensively joining and analyzing 
$53/1.9/3$ million transactions relevant to UniswapV2~\cite{me:dex:uniswap,Adams2020UniswapVC}/Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}/Pancakeswap~\cite{me:pancakeswap:1} on Ethereum mainnet and Binance Smart Chain (BSC), we found $210/0.3/1006$ thousand instances executing AMM operations are violating atomicity. 
The study reveals various patterns of atomicity violation, such as standalone token deposits that match no withdrawal, standalone token withdrawal, the deposit-withdrawal pairs where the depositor does not match the withdrawer, and the pairs where the deposited value does not match the value withdrawn. 
One cause of the atomicity violations is that certain non-standard token operations unspecified in the AMM protocols (e.g., rebasing token supply and interest-bearing tokens) are mistreated as token deposit that allows subsequent token withdrawal to succeed. This manifests in standalone withdrawals. Another cause is that certain token deposits are not intended for withdrawal (e.g., airdrop and token lost-and-found), which results in standalone deposits.

\vspace{2pt}\noindent\textbf{Understanding atomicity violations}. 
We hypothesize the discovered atomicity violations could imply, among others, the presence of two security-critical scenarios: token thefts or lost tokens. In the former, an attacker account withdraws value from the AMM that belongs to others (e.g., victims being the pool or other traders). In the latter, a trader depositing tokens by mistake (or being tricked into doing so) cannot get the tokens back. 

We aim at detecting the incidents of token theft and lost tokens out of the atomicity violations. The detection is not easy, as the ground truth can lie in the account activities off-chain which are unobservable. For instance, in verifying an token theft instance, one has to know whether the depositor and withdrawer accounts are controlled by the same physical user, which is known to be an intractable problem if only the on-chain information is available; existing heuristics such as address clustering~\cite{DBLP:conf/fc/Victor20,DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:conf/sp/HuangALIBMLLSM18,DBLP:books/daglib/0040621} do not apply here (see \S~\ref{sec:discoveryproblem} for detail). 
%Likewise, for lost tokens, we analyze the trader's behavior in other relevant transactions. For instance, if a standalone token deposit is followed by another token deposit that uses different mechanism, the former is likely to be a deposit by mistake.

We develop an end-to-end transaction-analytical pipeline, depicted in Figure~\ref{fig:workflow7}, 1) to discover atomicity violations, 2) to detect theft and lost tokens, and 3) to uncover the attackers' systematic behavior in conducting these cyber-crimes.

%We found in practice the exploitable deposits can be created in a variety of unexpected application scenarios, including free token giveaways (i.e., airdropping), tokens redistributing fees to privileged shareholder accounts, tokens bearing interest, tokens that can adjust or rebase total supply, buggy smart contracts, and unsafe user interface that executes a swap in two separate transactions, etc. 

\vspace{2pt}\noindent\textbf{Findings}. 
We found the Uniswap V2 protocol (and all its running instances including Uniswap V2, Sushiswap, Pancakeswap) handles exploitable token deposits and are subject to token theft. All other AMM protocols refuse to handle exploitable token deposits and risk their traders under lost tokens. We thus detect token thefts on Uniswap V2 based instances and lost tokens on other instance.

We discover theft attacks where external attacker accounts extract the value created by the above vulnerable deposits in Uniswap pools. On the Ethereum mainnet and BSC fork, we discover $465$ thousand theft attacks mounted by $258$ distinct attacker accounts, inflicting a loss of more than $3.7$ million USD stolen from $978$ victim traders.
Each attack instance we found matches at least one indicator described above. Interesting attacker behavior was observed in practice. For instance, real-world attackers {\it adapt} to the different patterns of exploitable deposits and exhibit different behavior: When the attacker is to extract value from interest-bearing tokens, she waits long enough, typically hundreds of Ethereum blocks, for the interest to accumulate and to become profitable. To extract deposits of other patterns, the same attacker instead wastes no time extracting the illicit value, typically within one or two blocks.

We further study attackers' and victims' behavior by tracking their money flow and actions to create/destroy smart contracts. Our study uncovers the systematic criminal activities: the crime bosses use mixer services to hide their identities while sending commissions and instructions. After the attack, the money is sent to various DeFi services to maximize illicit profit. Exploit smart contracts are widely used to improve attack success rates.

We also detect, from the standalone deposits on Uniswap V3, the XXX incidents of lost tokens worth a total of XXX USD. Given a standalone deposit, our method to detect whether it results in lost token is whether it relies to deposit similar amount of tokens. 

\vspace{2pt}\noindent\textbf{Mitigation}. 
In our measurement study, all AMM instances are subject to either theft or lost tokens. This is not by accident. We attribute the security risk to the design dilemma and tradeoff between theft and lost tokens. We propose secure AMM protocols by prohibiting the theft-vulnerable deposit. To avoid lost tokens, we propose extending AMM with a BtcRelay like capability that verifies the inclusion of mistaken deposit transaction in the blockchain as a basis to approve token-return requests. Besides, we also propose mitigation schemes retrofitted over a deployed AMM instance where deployed smart contracts are immutable (or non-patchable). Our mitigation approach is by securing the off-chain infrastructure and the application-layer (router) smart contract.

\vspace{2pt}\noindent\textbf{Contributions}. This paper's contributions are outlined as follows: 

\vspace{2pt}\noindent$\bullet$\textit{ New findings}. We discover a total of $3.5$ million USD worth of stolen value by measuring and analyzing atomicity violations on three popular Uniswap services on Ethereum and BSC. 
The discovered token theft attacks uncover the previously unknown patterns of vulnerable deposits (e.g., token rebase, interest, airdrop, mishandled contract exception) and expose the malicious, adaptive withdrawal behavior that occurs offline and otherwise would have been hidden. We further study the criminal infrastructures and campaigns mounted to systematically prepare, execute and finalize the theft attacks.

\vspace{2pt}\noindent$\bullet$\textit{ New techniques}. We develop an end-to-end analytical pipeline to detect attacks from Uniswap transaction traces, including an efficient join algorithm for detecting atomicity violations and approaches to automatically discover and cross-check token theft attacks. 
%XXX: Also we propose mitigation schemes including a fuzzer and test oracle to automatically detect mishandled exceptions in smart contracts.

%This work leads to the findings that shed light on the current and future underground ecosystem that strategically exploits the atomicity violation to gain illicit profit.

\noindent
{\bf Roadmap}: \S~\ref{sec:background} introduces the background of Uniswap, defines risky swaps and describes the threat model. The first step in our analysis pipeline, that is, detecting risky swaps, is presented in \S~\ref{sec:detectriskyswap}. The second step, discovering attacks, is described in \S~\ref{sec:attack}. The third step, characterizing on-chain crimes, is in \S~\ref{sec:behavior}. 
Mitigation schemes are presented in \S~\ref{sec:mitigate}. Related work is described in \S~\ref{sec:rw}. Responsible disclosure is discussed in \S~\ref{sec:disclosure} with the conclusion in \S~\ref{sec:conclude}. 
\ignore{
}

\ignore{
\noindent
{\bf System overview}: 
To discover the misuses, our approach is to find the mismatch between an AMM's governing protocol and its use history (collected from Ethereum transactions). Specifically, our approach takes as input the AMM protocol specification and filtered transactions/events collected from blockchain exploration service (XXX). It produces the discovered AMM operations that violate the protocol specification. Internally, it joins the records of different token-transfer operations across transactions. To reduce the search space (e.g., a naive join would entail cross-product on all transactions' powerset), we develop an efficient linear algorithm that takes advantage of the invariant observed from the Uniswap-V2's smart contract program.

1) We found all AMM protocols except for Uniswap V2 choose not to handle token deposit by external \texttt{transfer} (i.e., a trader deposits a token to a pool's account by externally calling the ERC20 \texttt{transfer} function). This is shown in Table~\ref{tab:policy}. Users of these AMMes risk lost tokens, where tokens are deposited by mistake and the users can not retrieve them back. Such cases of standalone token deposits are found to widely exist on these AMMes, out of which we detect the lost-token cases. We verify the lost tokens by making sense of the same-trader behavior in other relevant transactions. For instance, we found on Uniswap V3, a standalone token deposit is commonly followed by the AMM's token swap, which indicates the trader mistakenly deposits tokens by using deprecated swap API. 

2) The Uniswap V2 protocol accepts token deposits by external \texttt{transfer}. This design choice leaves the pool smart contract unable to track the original depositor (see Figure~\ref{XXX}) and forces it to accept a token withdrawal without enforcing permission. This flawed design, which we call permissionless withdrawal, affects various AMM operations (including token swaps, liquidity addition/removal, and returning lost token) and has adverse impacts on all Uniswap V2 based instances (including Uniswap V2, Sushiswap and Pancakeswap). The permissionless withdrawal gives rise to a new class of token theft threats in which Alice's exploitable token deposit can be extracted by malicious trader Bob, if Bob sends the token-withdrawal transaction first. By studying relevant transactions, we reveal various patterns of exploitable deposits in practice that lead to actual token theft. These causes include both standard and non-standard token balance updates, interest-bearing tokens, and buggy AMM-caller smart contracts. 

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.325\textwidth]{figures/automata3.eps}
\end{center}
\caption{Matchmaking in two rounds to detect risky swaps (Type-II and Type-III swaps).}
\label{fig:automata}
\end{figure}
}


\section{Background}
\label{sec:background}

Ethereum blockchain supports two types of addresses: An externally owned account (EOA), which is an Ether owner's public key, and a contract account (CA), which refers to the immutable memory address to which the smart contract is deployed on miners. An Ethereum transaction is a binding between its sender address and receiver address.

An AMM or automated market maker is a dominant form of decentralized exchange (DEX) deployed on Ethereum blockchains. An AMM runs one or multiple ``pools'' in smart contracts. An AMM pool owns two tokens, say $T_0$ and $T_1$. An AMM pool minimally supports two operations: 1) token swap between a trader account and the pool smart contract, and 2) liquidity addition/removal between a provider account and the pool smart contract. The trader and liquidity provider can be either an EOA or a CA.

In a token-swap operation, the trader deposits $dx$ units of token $T_0$ to the pool's account and receives from the pool $dy$ units of token $T_1$. The AMM internally determines the token exchange rate (or value of $dy$) by enforcing the invariant on some function. For instance, Uniswap is a constant-product market maker where the invariant function is the product of the two token balance.

In an add-liquidity operation, the liquidity provider deposits $dx$ units of token $T_0$, deposits $dy$ units of token $T_1$, and withdraws a certain amount of ``base'' tokens $T_{\texttt{LP}}$. A remove-liquidity workflow is the reverse of add-liquidity, in that the liquidity provider deposits tokens $T_{\texttt{LP}}$ and withdraws tokens $T_0$ and $T_1$ at a certain ratio.

\begin{table}[!htbp] %force in current page, disable float.
\centering{\scriptsize
\begin{tabularx}{0.5\textwidth}{ |l|X|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
Layer & $swapT.$ workflow & $addL.$ workflow \\ \hline
Uniswap V2~\cite{me:uniswapv2:pool}
& $T_0$.\texttt{transfer}(trader,amountOut) & $T_0$.\texttt{transfer}(trader,amountOut) \\ 
& pool.\texttt{swap}(amountOut, to\_addr) & $T_1$.\texttt{transfer}(trader,amountOut) \\ 
 & & pool.\texttt{mint}(to\_addr) \\ 
\hline
Uniswap V3
& pool.\texttt{swapXXX}(amountOut, to\_addr) & pool.\texttt{addLXXX}(to\_addr) \\ 
\hline
\end{tabularx}
}
\caption{Uniswap V2/V3's API in $swapToken$ and $addLiquidity$ represents $addLiquidity$ workflow.}
\label{tab:uniswapv2:api}
\end{table}



==> text/old/v7_paper.tex <==
\section{Understanding Atomicity Violations}
\label{sec:detectviolatingswap}

\subsection{Discovering Atomicity Violations}
\label{sec:mmalgo}

\noindent
{\bf Data model}: 
In an AMM, each operation, be it token swap or liquidity management, consists of token deposits and withdrawals. Given a pool address, a token deposit is a value transfer to the pool where the transfer can be done by either 1) directly calling the token's \texttt{transfer} function or 2) calling the token's \texttt{approve} function followed by the pool calling \texttt{transferFrom} function.
A token withdrawal is a value transfer from the pool by the pool calling the token's \texttt{transfer} function.

\noindent
{\bf Atomicity specification}: 
%The AMM protocol specifies what function calls are acceptable to be a token deposit (and withdrawal); for instance, in Uniswap V2, a token deposit is a call to a token's \texttt{transfer} function can be a token deposit, and a call to a pool's \texttt{swap} function can be a token withdrawal. 
A correct execution of an AMM operation is a sequence of token deposits and withdrawals, meeting certain conditions. 
Here, we define the notion of atomic operation and the atomicity violating patterns. Without loss of generality, we use token swap as an example in description, while the extension to liquidity operations is straightforward. Given a token swap, we call the account calling the deposit function by the depositor and the account receiving the token withdrawal by the withdrawer.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/anomalies.eps}
\end{center}
\caption{Atomic swaps and violations.}
\label{fig:swaps}
\end{figure}

\begin{itemize}[leftmargin=0.5cm]
%\setlength{\itemindent}{-1em}
\item
An atomic token swap consists of a token deposit of one token worth value $v$ and a withdrawal of another token worth the same value. The depositor and withdrawer accounts are either the same or match a function call if both deposit and withdrawal are in the same transaction. 

\item
{\bf Atomicity violation I} is a standalone withdrawal that does not match any token deposit.

\item
{\bf Atomicity violation II} is a standalone deposit that does not match any token withdrawal. 

\item
{\bf Atomicity violation III} is account mismatch in which the depositor and withdrawer accounts in a sequence of otherwise matched deposits and withdrawals do not match. For instance, as shown in Figure~\ref{fig:swaps}, the deposit is issued from Account Alice and the withdrawal is from Bob.

\item
{\bf Atomicity violation IV} is lower-value deposit in which the deposited value is lower than the value withdrawn.

\item
{\bf Atomicity violation V} is higher-value deposit in which the deposited value is higher than the value withdrawn. Both Violations IV and V are cases of value mismatch.
\end{itemize}

Figure~\ref{fig:swaps} shows five atomicity violation patterns and the atomic case of a token swap.

%We believe atomicity violation implies anomalous activities. For instance, a standalone withdrawal could imply value theft where the withdrawer is able to extract value from the AMM pool without depositing any value. A violation-III token swap implies theft in which the withdrawer is able to extract value from a victim depositor. For another example, a standalone deposit could imply lost tokens where a trader makes a mistake depositing value but is unable to withdraw it.

{\bf Input data}:
Our input data is raw blockchain transactions including function calls and log events by smart contracts. We obtain the transaction data by crawling Ethereum exploration services including \url{Etherscan.io}~\cite{me:etherscan}, \url{BSCscan.io}~\cite{me:bscscan} and relevant BigQuery datasets~\cite{me:bigquery:ethereumdataset}. 
We only use the the event log emitted from the AMM pool smart contract (which we assume is trusted), such as Uniswap V2's pool.
From the raw input data, we attribute the \texttt{transfer}/\texttt{transferFrom} calls to token deposits and withdrawals as described. Besides, we collect the invocations to relevant functions, such as \texttt{swap} in Uniswap V3 in Table~\ref{tab:uniswapv2:api}; from there, we can filter out the deposits and withdrawals that are mapped to atomic operations. 
We also use the pool's events to reconstruct the mapping between deposit value and withdrawal value in the withdrawal record.

{\bf Design challenge}:
A naive way of finding atomicity violations is to filter out atomic operations by extensively joining token deposits with withdrawals. Because an atomic AMM operation can contain an arbitrary number of deposits and withdrawals, the naive join needs to be built on the {\it powerset} of token deposits and withdrawals, which is extremely expensive and unscalable (Note that the powerset of $n$ deposits/withdrawals is of $2^n$ elements).
To avoid the inefficiency, our observation is that due to Ethereum's single-threaded execution model, a token deposit can be matched only to a subsequent withdrawal before the next deposit occurs. This property allows to join token deposits and withdrawals based on their timings and makes it possible for linear-time search.

{\bf The algorithm} takes as input a list of function calls representing token deposits and withdrawals. In the first round, the algorithm equi-joins the function-call records by their transaction IDs. If the deposits and withdrawals in the same transaction also match in value, it emits them as an atomic operation before removing them from the list. If the value does not match, the algorithm merges the intra-transaction deposits and withdrawals into one virtual record (e.g., a deposit of value equal to the originally deposited value deducted by the withdrawn value).

In the second round, the algorithm joins deposits and withdrawals across transactions. It linearly scans the list of deposits and withdrawals sorted by time: For two consecutive deposits, say $d1$ and $d2$, it finds any subset of all withdrawals between $d1$ and $d2$ that matches $d1$ in value. For each match, the algorithm removes the deposit and withdrawals from the list before emitting an atomic operation. The algorithm then reverse the process, that is, for two consecutive withdrawals, it finds a set of deposits between the two withdrawal that match the earlier withdrawal in value.

In the third round, the algorithm linearly scan the remaining list and emits the token deposits and withdrawals as either value mismatch or standalone operations. The pseudocode is in Appendix~\ref{sec:algorithm:detect}.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.35\textwidth]{figures/join_problem2.eps}
\caption{Matchmaking deposits and withdrawals: Matched cases are in green boxes and mismatches are rendered in red, including standalone withdrawal (I), standalone deposits (II), and deposit of lower value (IV). In the figure, \texttt{tf}/\texttt{tff} refer to functions \texttt{transfer}/\texttt{transferFrom}.}
\label{fig:joinproblem}
\end{figure}

{\bf Example}: We show an example of running the atomicity violation discovery algorithm in Uniswap V2. Uniswap V2 supports token deposits by both \texttt{transfer} and \texttt{transferFrom}. It also supports token withdrawals by \texttt{swap} (in $swapToken$) and by \texttt{mint} (in $addLiquidity$). We collect the corresponding function-call records for token deposits and withdrawals. Figure~\ref{fig:joinproblem} shows the collected deposits and withdrawals, ordered by time. 
In the first round, the algorithm identifies and filters out atomic operations by linking deposits and withdrawals through transaction ID, which is \texttt{tff1}-\texttt{swap1}. In the second round, it then matches token deposits and withdrawals by timing. For instance, \texttt{tf2} and \texttt{tf3} are matched to \texttt{mint1} by value, which leads to an atomic $addLiquidity$ operation. In the last round, the algorithm emits the mismatches in the remaining list. Specifically, \texttt{tf4} is mapped to \texttt{swap3} but their value does not match, thus producing a case of Violation IV. Then there are two standalone operations left in the list, that is, \texttt{tf1} (Violation II) and \texttt{swap2} (I).

%{\it An example}: Figure~\ref{fig:joinproblem} shows how token deposits to a Uniswap pool are matched to token withdrawals from the same pool. The data records storing deposits/withdrawals are aligned and sorted by time. The figure show two matched cases (i.e., two green boxes). Three mismatch cases are discovered: On the timeline, the first \textsc{transfer} is a standalone deposit (i.e., II). The second \textsc{swap} is a standalone token withdrawal (I). In the red box is a pair of deposit and withdrawal whose value does not match (i.e., IV).

\begin{table}[!htbp] %force in current page, disable float.
\caption{Measured atomicity violations on top DEXes: value is presented in the unit of million USD, and the number of transactions violating atomicity (i.e., \#tx) is presented in the unit of a thousand.}
\label{tab:swapsviolating}\centering{\scriptsize
\begin{tabularx}{0.5\textwidth}{ |l|l|l|l|l|l|l||X| } %X is stretching to \textwidth, while c is to match with text width in cell.
\hline
 & Atomic & I & II & III & IV & V & \#tx ($10^3$) \\ \hline
Uniswap-V2 & $618*10^6$ & {\color{red} \bf $1.26$} & $.36$ & {\bf$.49$} & $.09$ & {\color{red} \bf $3.64$} & $212$ \\ \hline
Sushiswap & $.17*10^6$ & {$\approx{}0$} & {$.03$} & {\bf$.064$} & $\approx{}0$ & $0$ & $.33$ \\ \hline
Pancakeswap & $73*10^6$ & {$.53$} & $.12$ & {\bf$.05$} & $.99$ & $0$ & $452$ \\ \hline
Uniswap-V3 & $5.3*10^4$ & $0$ & {$.17$} & $0$ & $0$ & $0$ & $.17$\\  \hline
Balancer
& $1.3*10^4$ & $0$ & {$.74$} & $0$ & $0$ & $0$ & $6.9$ \\ \hline
Curve
& $1.3*10^5$ & $0$ & $\approx{}0$ & $0$ & $0$ & $0$ & $\approx{}0$\\ \hline 
\end{tabularx}
}
\end{table}

{\bf Results}: We conduct the measurement and transaction analysis on all six DEX services.
In particular, we set the minimal $Z\%$ value difference to determine match/mismatch. If a deposit (withdrawal) has $Z\%$ higher value than the paired withdrawal (deposit), it is considered a mismatched case (IV/V/). A rule of thumb is to set $Z\%=10\%$ on our dataset, which helps remove the negative cases, such as fees charged by tokens and router smart contracts.
For each DEX, we report the number of swaps and their total value under each category. 
To estimate the value in a violating operation $tx$, we use the exchange rate between the token $T$ and one of the three USD-pegged stablecoins (i.e., $USDT$, $USDC$ and $DAI$). Specifically, we find from the three Uniswap-V2 pools (i.e., $T$-$USDC$, $T$-$USDT$, and $T$-$DAI$) the swap transaction say $tx'$ that occurs at the nearest time to $tx$. We use the exchange rate in $tx'$ to estimate the value of token $T$ in transaction $tx$.

It can be seen that the majority of swaps, about $97.9\%$, are atomic. The rest are token swaps violating atomicity worth a total of 26.2 million USD, among which the majority are caused by high fees. 

\subsection{Interpreting Atomicity Violations}

\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.475\textwidth]{figures/victimpatterns.eps}
\end{center}
\caption{Patterns of profitable deposits: $R$ is the router smart contract, $T_0$/$T_1$ are the two tokens in the target liquidity pool}
\label{fig:patterns}
\end{figure}

\subsubsection{Non-standard Balance Updates (Pattern $P_1$)}
\label{sec:cases:rebase}

In many real-world tokens, account balance can be changed by the non-standard operations beyond token transfer. We describe two examples. {\it Rebase}: For instance, token balance can be elastically adjusted by token issuers, for purposes such as to stabilize the token's exchange rates against other tokens. In practice, token rebase is such a non-standard balance-changing function, supported in some widely used tokens, such as AMPL~\cite{me:ampl:token}. When a token, say $T_0$, is rebased, a Uniswap's relevant pool, say for tokens $T_0$ and $T_1$, could have its $T_0$ balance increased. Uniswap falsely assumes that this balance increase is due to some accounts that swap token $T_0$ for token $T_1$. Uniswap's pool would mistakenly admit anyone who requests to withdraw token $T_1$ after the rebase of $T_0$.

{\it Token shareholder}: 
As another example, there are tokens that charge ``tax'' to average owner accounts and redistribute the ``tax'' income among privileged accounts of shareholders. Specifically, these tokens support two kinds of owners, average owner and token shareholders. When there is a transfer, the token smart contract charges a certain amount of fees. The fees are redistributed to the privileged accounts of token shareholders. Thus, a transfer between average accounts would update the balance of all shareholders' accounts. In a Uniswap's pool of token types $T_0$ and $T_1$, if the pool's account in $T_0$ is a shareholder, any transfers in $T_0$ would increase the pool's balance and create a profitable opportunity.
 
Furthermore, even when the pool receives a token deposit, the deposit may not be intended as a part of swap. For instance, airdrop is a common practice to promote the use of a new token type, in which token issuers periodically give away newly minted tokens to the current token owners (e.g., in Tokens MILK2~\cite{me:token:milk2} and 3Cs~\cite{me:token:3cs}). When a token, say $T_0$, is airdropped into a Uniswap's pool, the pool holding tokens $T_0$ and $T_1$ would mistakenly treat the transfer as a part of swap from token $T_0$ to $T_1$. Thus, the pool would admit anyone's request to withdraw token $T_1$ after airdrop of token $T_0$ to the pool's account.

In general, these non-standard token operations allow to update the pool's balance but do not intend to withdraw the same value from the pool. We name this pattern of extractable value by $P_1$.

%In general, there can be an explicit token operation that increases the pool's balance of token $X$, but is not with the intention of swap value. Thus, an attacker observing the occurrence of such an exploitable operation can strategically extract value from the pool and gain illicit profit. We name this attack pattern by $P_1$. 

\subsubsection{Implicit Token Balance Updates ($P_2$)}
Beyond $P_1$, there are implicit approaches to update the balance. Many tokens are bearing interest. That is, the balance in the token smart contract increases at a certain rate as the time goes by. Suppose a Uniswap pool is of token $T_0$ and $T_1$ where $T_0$ is interest bearing. Similar to $P_1$, the Uniswap pool observing the increase of token $T_0$ would admit the withdrawal of token $T_1$ by anyone who requests it, including a value-extracting attacker. We call this attacker's pattern by $P_2$, which is different from $P_1$. In $P_2$, the attacker simply waits long enough to harvest the extractable value from token interest. 

\subsubsection{External Transfer for Deposit ($P_3$)}

In Uniswap, a trader can externally call token $T_0$'s transfer function to make deposit so that she can in a separate transaction withdraw token $T_1$. We call the pattern of a victim trader sending a transaction to externally transfer token $T_0$ by $P_3$. When $P_3$ occurs, a malicious account can send the withdraw transaction ahead of the victim's one, to claim the value in the pool.  This attack is possible because a Uniswap pool receiving a deposit of $T_0$ will approve of the next withdrawal of token $T_1$, no matter who sends it. 

\subsubsection{Buggy Router Contracts ($P_4$)}

In the above three patterns, the victim may externally call token $T_0$'s functions. In the fourth pattern $P_4$, the trader delegates the handling of swap to a router smart contract that is buggy and violates atomicity. After the trader EOA's transaction, the router smart contract successfully completes the deposit of Token $T_0$ but fails at requesting the withdrawal of Token $T_1$. Thus, anyone who requests the token withdrawal in the next transaction, including an attacker EOA, would succeed in grabbing the value illicitly. 

\subsection{Hypothesized Attacks}

\noindent
{\bf Threat model (token theft)}: 
An attacker trader sends one or multiple crafted transactions, at a right timing, to an AMM pool. The theft is successful if the attacker's transactions do not deposit tokens of any value and are able to receive positive value in return. The attacker has the capability of determining when to send the crafted transactions and monitoring on-chain states both in the mempool and in included blocks. The victim could be another trader who deposits value to the AMM pool or the AMM pool itself who receives value through various means (e.g., add liquidity or other non-standard ways as described above).

We hypothesize certain patterns of atomicity violations, including I, III and IV, are instances of token theft attacks. In these violating cases, either the deposited value exceeds the withdrawn value (i.e., I and IV), or the depositor account differs the withdrawer account. They are candidate signs of token theft. We present our validation study in the next section (\S~\ref{sec:attack}).

\noindent
{\bf Risk of lost tokens}: In violations II and V, the deposited value is under the withdrawn value. In these cases, the AMM pool appears to unfairly take value from the trader account. These cases can potentially indicate denial of AMM service. In this work, we particularly formulate the risk of lost tokens:

Suppose an account sending a token to an AMM smart contract by mistake. The token is lost if the account cannot find an AMM function to get the mistakenly deposited token back. 

\section{Detecting Token Thefts}
\label{sec:attack}

\subsection{The Detection Problem}
\label{sec:discoveryproblem}

\noindent{\bf Theft detection}: 
The detected atomicity violations, especially I, III, and IV, could present the value that {\it can} be extracted by real-world attackers. However, whether the value is {\it actually} extracted by the attackers, or equivalently, whether the violation operations are actual attack instances, is a different problem. 

Consider as an example that a token issuer sends a vulnerable rebase transaction to a pool's token, followed by a withdrawal transaction sent by account $X$ (i.e., $P_1$). $X$ may or may not be the token issuer. The former case is not an attack, as the token issuer aware of the risky rebase sends the withdrawal to remedy the risk. The latter case may be an attack. in other situations including $P_3$ and $P_4$, a risky swap can also be attributed differently.
\ignore{
For instance, in $P_1$, after a token issuer sends an exploitable rebase transaction, it is equally likely one of the following cases occur: 1) the token issuer aware of rebase being exploitable quickly sends a swap request herself to claim the value in the Uniswap pool. 2) An attacker observing the occurrence of rebase operation calls the liquidity pool to withdraw the value there. The former case is not an attack, while the latter one is. In other cases, the same apply: In $P_3$, if the trader sends another transaction to withdraw the value in token $T_1$ right after the transaction of depositing $T_0$, it is a benign case. But if it is an attacker account who withdraws after the external deposit, it constitutes an attack. In $P_4$, if the trader observing the router exception and immediately send a ``make-up'' transaction to claim the value herself, it is a benign case. But if it is a third-party ill-intended account who sends the withdrawal transaction, it constitutes an attack.
}

Distinguishing attacks from benign cases entails checking two essential conditions: {\bf 1) Whether two accounts are controlled by two distinct physical users}: It cannot be an attack if the trader account who makes the profitable deposit in token $T_0$ is controlled by the same physical user with the account who succeed in withdrawing the value in token $T_1$. 
Thus, attack detection becomes the problem of linking two blockchain accounts of the same physical user, which is known to be an intractable problem if the only information known is on-chain data.
{\bf 2) What's a transaction sender's intention}: That is, whether a withdrawal transaction is intended as an attack. Even when the withdrawer and depositor accounts are not the same physical user, they can be friends in the real life, which makes the swap non-attack. Thus, it entails detecting the depositor account's intention in sending the withdraw request, which however can be hidden opaque and pose challenges to detection.

{\bf Feasibility of existing approaches}: 
On checking Condition 1), there are existing works that tackle the recovery of account linkage by heuristics specific to Bitcoin's UTXO model~\cite{DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13}. The only work for Ethereum~\cite{DBLP:conf/fc/Victor20} presents a linkage heuristic exploiting some DEXes deposit addresses. Specifically, on order book-based DEXes (i.e., IDEX and EtherDelta), trader Alice swapping token $T_0$ for $T_1$ can specify the so-called deposit address who receives $T_1$. Assuming a swap is normal, the sharing of deposit addresses by two traders implies that the two traders are controlled by the same physical user. This work is different from our attack detection problem, where the deposit address heuristic is to detect the case that two accounts are linked, while our problem is to detect if two accounts are unlinked. More importantly, the deposit address heuristic works only under the assumption of normal swaps, while our work deals with risky swaps. Given a risky swap, the deposit address of a swap refers to the attacker. Thus, when an attacker targets two victim traders, it could appear that two traders share the same deposit address. In this attack, the two victim traders do not have to be linked to the same off-chain user.

On checking Condition 2), there are existing works on threat intelligence on blockchains by characterizing attackers' behavior~\cite{DBLP:conf/uss/SuSDL0XL21}. However, their targets are program-level attacks such as reentrancy attacks, and their attack strategies don't apply to the DEX context of this work.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.4\textwidth]{figures/indicators.eps}
\end{center}
\caption{Attack strategies (A1/A2/A3) and indicators}
\label{fig:indicators}
\end{figure}

\subsection{The Detection Method}

We discover attacks by designing attack strategies specifically for different profitable deposits and use them as attack indicators to match the observable attacker behavior on-chain. 

{\bf Design rationale: Attack strategies}: Recall that each risky swap involves with a profitable deposit followed by a withdrawal that reaps the profit. An attacker needs to strategically send the withdrawal to ensure high success rates by properly monitoring the profitable deposits. We consider three attack strategies:

\begin{itemize}[leftmargin=0.5cm]
%\setlength{\itemindent}{0em}
\item
 {\bf A1) Aggressive attacker (monitoring deposits)}: The attacker directly monitors the mempool for the profitable deposits. In this strategy, the attacker monitors different cases of profitable deposits, such as $P_1$/$P_2$/$P_3$/$P_4$. The attacker launches a node joining the Ethereum blockchain network and monitors the node's mempool so that the profitable-deposit transaction can be detected as soon as they are propagated in the blockchain network. 

Strategy A1 entails the attacker to customize the monitored conditions to different causes. It minimizes the time window between the exploited deposit and withdrawal, and ensures a high success rate in the presence of competitors.

\item{\bf A2)
General-purpose attacker (monitoring pool)}: The attacker monitors the Ethereum's smart contract state to check if the pool is profitable. For instance, when a rebase transaction is executed in the blockchain, it could increase the balance in the token smart contract and leave the reserve in the pool smart contract unchanged. By detecting the difference between token balance and reserve, the attacker ensures sending a withdrawal can succeed.

Strategy A2 is generalizable to different profitable deposits, in the sense that the attacker monitors a single condition that all different profitable deposits will trigger. However, this strategy works only after the profitable deposit transaction is executed and included in the blockchain. So an aggressive attacker (A1) can frontrun a general-purpose attacker (A2).

\item{\bf A3)
Lucky trader}: The trader does not intentionally observe conditions on pool profitability but is lucky in grabbing the profit by inserting a withdrawal after the profitable deposit. The delay between the withdrawal and victim deposit can be arbitrary. 
\end{itemize}

{\bf Proposed attack indicators}: 
An account's strategy, which normally occurs in the blackbox off-chain state, is not directly observable from the on-chain traces. We distill observable information and design indicators to infer attack strategies.

To start with, an aggressive attacker monitoring the off-chain mempool states cannot be observed from the on-chain traces. Likewise, a general-purpose attacker who may choose to issue RPC calls to read on-chain data is also unobservable. For these cases, we  collect the gap between the block including deposit transactions and the block including the exploit withdrawal transactions as the metric to infer the presence of an attack and further the attack strategies. For instance, if the block gap is always $0$, it indicates the case is exclusively an aggressive attack. If the deposit is token interest and the block gap is always large, it indicates an aggressive attack exploiting token interest. Otherwise, if the block gap is randomly distributed, it is likely to be a lucky trader. Based on the heuristics, we propose the following three indicators:

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I1 (Strong): An account whose withdrawal transactions occur consistently within $X_1$ blocks after profitable deposits (i.e., block gap smaller than $X_1$) and whose victim deposits are not caused by token interests (i.e., not $P_2$) is likely to be an attacker. Formally, 
$$
I_1\leq{}X_1
$$
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I2 (Strong):
An account whose withdrawal transactions occur consistently more than $X_2$ blocks after profitable deposits (i.e., block gap larger than $X_2$) and whose victim deposits are based on token interests is likely to be an attacker. Formally, 
$$
I_1\geq{}X_2
$$
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I12 (Strong):
An account whose ratio between indicator I2 and I1 is larger than $X_{21}$ is likely an attacker. 
Intuitively, it shows the attacker’s intentional adaptive strategies in exploiting deposits of different patterns.
Formally,
$$
\frac{I_2}{I_1}\geq{}X_{21}
$$
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I3: 
An account whose withdrawal transactions appear an arbitrary number of blocks after the profitable deposits are likely to be a lucky trader.
In other words, an account whose block gaps have a large deviation is likely to be a lucky trader.
}}\end{center}

In practice, many accounts use delegate smart contracts on-chain to relay their payload (of malicious withdrawals). The delegate smart contracts make attack strategies observable. We propose the following indicators to take advantage of this fact. 

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I4 (Strong):
An account who attempts to withdraw through a smart contract that checks both pool reserves (i.e., calling \texttt{pool.getReserves()}) and token balances (calling \texttt{erc20token.balanceOf()}) is likely a general-purpose attacker. Note that this indicator does not require the smart contract to actually withdraw the token $T_1$. 
}}\end{center}

The intuition of the above indicator is that a general-purpose attacker uses the pool's \texttt{getReserves()} function and token's \texttt{balanceOf()} function to obtain the token reserve and balance, respectively. This shows the account's intention to calculate pool profitability and is an indicator of general-purpose attacker. 
%Note that the indicator is not necessary (i.e., causing false negatives), as a general-purpose attacker can issue RPC queries to read reserves and balances, leaving no trace on-chain.

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I5: An account whose withdrawal transactions exclude any token deposit is likely to be an attacker.
 
An account whose withdrawal transactions also include token deposits is likely to be a lucky trader, even though the withdrawal is of higher value than the deposit.
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I7:
Standalone withdrawal that extract value from deposit patterns $P_1$ and $P_2$ indicate an attacker, because the value in $P_1$ and $P_2$ is intended for AMM pools, not for external accounts. This intuition is materialized into the formula below:
$$
\frac{|P_1|+|P_2|}{\sum_{i}{|P_i|}}>X_7
$$
}}\end{center}

{\bf Attack discovery algorithm}: We materialize the indicators in a holistic attack discovery algorithm. The algorithm takes as input the detected risky swaps from the previous phase (\S~\ref{sec:detectviolatingswap}) and produces the strategies an attack account takes.

Specifically, recall that each risky swap consists of a profitable deposit and a (successful) withdrawal. We expand it by adding all the withdrawal attempts, no matter success or failure, on the same pool by calling its \texttt{getReserves} or \texttt{swap} functions between time $t_1$ and $t_2$ where $t_1$/$t_2$ is the time when the current/next deposit occurs. We ignore the atomic swaps between $t_1$ and $t_2$. Hence for each risky swap, we obtain a list of accounts who send the withdrawal or expanded withdrawal attempt. For each account and each associated swap, the algorithm checks the indicators and reports the number of attacker labels the account is tagged with. In particular, indicator I1/I2 produces the average block gap over the account's swaps when the deposit is non-interest/interest. 

\lstset{style=mystyle}
\begin{lstlisting}[caption=Pseudocode to discover attacks,
                   %linerange={1-30},
                   numbers=none,
                   %firstnumber=1,
                   deletekeywords={[2]INT},
                   morekeywords={clustered},
                   framesep=2pt,
                   xleftmargin=5pt,
                   framexleftmargin=5pt,
                   frame=tb,
                   framerule=0pt, 
                   label=code:discoverattacks,
                   float,floatplacement=H
                   ]
void AttackDiscovery(AtomicityViolation[] swaps, int th1, int th2){
  for(AtomicityViolation s in swaps){
  Mapping blockGaps;

  for(Account w in s.getWithdrawers())
    if(isCA(w)) //I4
      if(findCall(w, s.getPool(), "getReserve").getTx().checkCall(w, s.pool().tokens(), "balanceOf()")) 
        emit(w, "Attacker");
    //I1
    Block depositTime=s.getDeposit().getBlock();
    Block withdrawTime=w.getBlock();
    blockGaps.getValue(w).add(withdrawTime-depositTime));
    //I2
    numberSwaps.getValue(w).increment();
  }

  for(Account w in blockGaps.keySet()){
    blockGap.getValue(w).divideBy(numberSwaps.getValue(w));
    if(blockGap.getValue(w) > th1) emit (w, "Attacker");
    if(numberSwaps.getValue(w) > th2) emit (w, "Attacker");
}}
\end{lstlisting}

\subsection{Results}

\subsubsection{Validation using Ground Truth}

We validate our indicator-based detection method by collecting and using ground-truth data. 

\begin{table}[!htbp] %force in current page, disable float.
\caption{Detection parameters extracted from the ground-truth data}
\label{tab:parameters}\centering{
\begin{tabularx}{0.425\textwidth}{ |X|c|c|c|c| }
  \hline
   $X_1$ & $X_2$ & $X_{12}$ & $X_4$ & $X_7$ \\ \hline
   $617$ & $19.28$ & $1$ & $97.5\%$ & $69.2\%$ \\ \hline
\end{tabularx}
}
\end{table}

\noindent{\bf Establishing ground-truth}:
We search the Internet sites including Google, twitter and reddit. Our searches include the candidate attacker accounts (i.e., mules in Table~\ref{tab:attackerview}) and keywords such as  ``attack, vulnerable, scam, frontrunning, bot, arbitrager, MEV, bots''. Besides, we check the candidate account's tags on Etherscan and if they are security sensitive.
Out of the $142$ suspected accounts from our results (described next in \S~\ref{sec:theftinstances}), we found $9$ accounts are complained about on the Internet and $2$ accounts are tagged as MEV bots on Etherscan. 
The ground-truth account are presented in Table~\ref{tab:attackerview}, and the full detail of ground truth data collection is in Appendix~\ref{sec:groundtruth}.

\noindent{\bf Detection method validation}: Recall that our detection method is parameterized. We use the ground truth data to set the parameters so that all the ground-truth accounts can be detected positive under these parameters. The ``trained'' parameters are listed in Table~\ref{tab:parameters}. 
For instance, account $0x0c08545df4939ef46c1364b5930e840739667467$'s $I2$ meets the condition ($I2<2$) and account $0xEA674fdDe714fd979de3EdF0F56AA9716B898ec8$ meets the condition that $\frac{I2}{I1}=686/0.5=1372>19.2$.

\subsubsection{Detected Attack Instances}
\label{sec:theftinstances}

\begin{table*}[h]
\caption{Attacker characterization: A victim can be a normal token owner (N) or token issuer (I). The numbers reported under I1-I6 columns are described next: Given an account $A$, I1 is the average block gap of $A$'s transactions matching $P_1$, $P_3$ and $P_4$; I2 is the average block gap of $A$'s transactions matching $P_2$; I3 means the deviation of the block gaps reported under I1 and I2; I4 is the number of $A$'s transactions that read both pool's reserves and token balances; I5 reports whether $A$ has sent at least one transaction to deposit before withdrawal; I6 reports the number of risky swaps. Bold are strong cases suggesting the account is an attacker. Victims include normal accounts and token issuers.}
\label{tab:attackerview}
\centering{\scriptsize
\begin{tabular}{|p{6.0cm}|p{1.0cm}|p{0.7cm}|p{0.4cm}|p{0.5cm}|p{0.5cm}|p{1.2cm}|p{0.2cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.7cm}|p{0.5cm}|}
\hline
Accounts & Value & {Ground} & \multicolumn{7}{c|}{Attack indicators} &\# &\# & Label \\
\cline{4-10}
(Mules) & $10^3$ USD & truth &I1 & I2 & I3 & I4 & I5 & I6 & I7 & pools & victims & \\ \hline
$0x9799b475dec92bd99bbdd943013325c36157f383$ & 556 & \cmark &422 &371 & 1290& 0 &N& 43 & \xmark & 4 & 0/7 & A3\\
\hline
$0x2a2e25ad00faac024f6a8d8cdc0fc698fbda71b7$ & 239 & \xmark &{\bf 0.03} & &0.2 & 32 ({\bf 100\%}) &Y& 32 & \xmark& 1 & 0 /3 & A1\\
\hline
$0xdb40ea5b6d0ef9e45c00c194345b44765a53dd19$ & 113 & \xmark &{\bf 2.5} &{\bf 665} &2.0 & 17 ({\bf 100\%})&Y& 17 & \xmark&1 & 0/4 & A1 \\
\hline
$0x0c08545df4939ef46c1364b5930e840739667467$ & 101 & \cmark &{\bf 1.5} & &0.7 & 0 &N& 4 & \xmark& 1 & 1/1 & A2 \\
\hline
$0x56178a0d5f301baf6cf3e1cd53d9863437345bf9$ & 101 & \cmark &13 &{\bf 1574} &24 & 0 &N& 61 & \cmark & 3 & 2/4 & A1 \\
\hline
$0xb6bf45f59b94d31af2b51a5547ef17ff81672743$ & 20 & \xmark &224 &{\bf 600} &471 & 1231 ({\bf 100\%}) &Y& 1231 &  \cmark & 9 & 12/5 & A2\\
\hline
$0xc762e15cfbf392f4346ee7e8466ca595e571382b$ & 16 & \xmark &{\bf 3.0} & 5.3 &437 & 83 ({\bf 100\%}) &Y& 83 & \xmark& 19& 0/4 & A2\\
\hline
$0xa32d3f8a970ab3222ffa1c89cb910abf7b7201d0$ & 6 & \xmark & & {\bf 942} & & 208 ({\bf 100\%}) &Y& 208 & \xmark& 1 & 0/0 & A2\\
\hline
\end{tabular}%
}
\end{table*}

We present our analysis result in Table~\ref{tab:attackerview} which characterizes the most frequent accounts involved in risky swaps. The metrics include value stolen, causes, attacker indicators, the number of pools attacked, the number of victim accounts, and the label whether the account is an attacker.  From the table, we analyze the attackers' strategy of several selected accounts.

{\bf Case 1: Agg. attacker (A1) w. zero block gap}: Account $0x2a2e$ is involved in $32$ risky swaps (I6) and gains more than $2.39*10^5$ USD worth of illicit tokens. All $32$ swaps from this account are sent via a smart contract which checks the pool's profitability before withdrawal (I4). In terms of timing, the malicious withdrawals are always sent in the same block with the risky, profitable deposit. We believe account $0x2a2e$ aggressively monitors the mempool for the target tokens' rebase transactions, and if found, sends withdrawals immediately to ``backrun'' the deposits and claim the value.

{\bf Case 2: General attacker (A2) w. off-chain monitoring}: Account $0x0c08$ has withdrawn four times and grabbed tokens of $1.01*10^5$ USD. The account directly and externally calls Uniswap pool's swap function to withdraw, without checking pool profitability on-chain. The withdrawals are included in exactly one block after the one that includes the risky deposit. We believe Account $0x0c08$'s strategy is to monitor the pool profitability from an off-chain vantage point and to immediately send withdrawal by external calls. Because the account monitors the pool profitability instead of the cause (risky deposit), it has to wait until the inclusion of risky deposit that updates the pool state to be profitable. This explains why the inclusion of withdrawal has to be one block after the one including the risky deposit.

{\bf Case 3: Agg. attacker (A1) stealing interest}: Both Accounts $0xdb40$ and $0x5617$ have extracted value from interest bearing tokens. Their block gaps are large ($665$ and $1574$, respectively). Given that there are enough samples, this consistent behavior shows both accounts' attack strategy to wait long enough for the token interest to accumulate and for the extractable value to be large enough before acting on it.

{\bf Case 4: Adapting strategies}: For all accounts with indicators I1 and I2 in the table, it is clear that the block gaps for different causes (I1 and I2) differ: The block gaps for non-interest causes are consistently much shorter than those for token interests. It implies that the attackers are aware of the situation (which causes to exploit) and tailor their strategies to it.

{\bf Case 5: Lucky trader (A3)}: Account $0x9799$ is unlikely an intentional attacker: First, it does not read the token balance or check the pool's profitability before the withdrawal. Second, the block gap between profitable deposit and malicious withdrawal is large, at hundreds of blocks apart. In addition, the smart contract Account $0x9799$ relays her withdrawal requests also makes deposit to the pool. All these indicators show that $0x9799$ is unlikely an intentional attacker, but instead a lucky trader.

\subsubsection{Block Gaps}

\begin{figure}[!ht]
  \begin{center}
    \subfloat[Block gaps and the number of competing attackers]{%
\includegraphics[width=0.245\textwidth]{figures/figure_allrebase_blockdif.eps}
\label{fig:blockdif_1}
    }%
    %\hspace{-0.2cm}%
    \subfloat[Block gaps and value stolen]{%
\includegraphics[width=0.245\textwidth]{figures/figure_value_blockdif.eps}
\label{fig:blockdif_2}
    }%
  \end{center}
  \caption{Block gaps and affecting factors}\label{fig:complex}\vspace{-0.10in}
\end{figure}

Recall that each of theft attack runs in two transactions: The first transaction that creates extractable value, and the second transaction that withdraws the value and steals it. Given each detected attack (described from the previous subsection), we measure the gap of the two blocks that respectively include the attack's two transactions, namely block gap. We further report two metrics, that is, the number of competing attackers and the value stolen. Particularly, for each profitable deposit transaction, say $tx$, we find transactions sent by competing attackers. Here, a competing attacker either directly sends a transaction to withdraw the extractable value created by $tx$ but fails, or sends a transaction to read the token balance and pool reserve (which shows the intention to withdraw the value). 

We report the block gaps with the varying number of competitors in Figure~\ref{fig:blockdif_1}. A larger dot in a X/Y coordinate in the figure represents more attacks found with the same X/Y value. The result shows that when there are many competing attackers, the block gap tends to be small. This could be explained: Because the first attacker wins, the more attackers there are, the earlier the withdraw transaction is sent, namely smaller block gap.
The result also shows that with few competing attackers comes a large range of block gaps.

We then report the block gaps with varying value stolen in Figure~\ref{fig:blockdif_2}. The result shows that when the stolen value is large, the block gap tends to be small. A possible explanation is that the higher extractable value gives the attacker more incentives to send the withdrawal transaction with higher fee and to frontrun other potential thieves.
 
\subsubsection{Attacker/Victim Behavior over Time}

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_attacker_timeline.eps}
\end{center}
\caption{Attack timeline of top-10 attackers. In the Y axis, attacker accounts are ordered by total value stolen.
Data from 07/09/2020 (block 10422671) - 06/29/2021 (block 12727620).}
\label{fig:attack}
\end{figure*}

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_victim_timeline.eps}
\end{center}
\caption{Attack timeline of top-10 victims. In the Y axis, victim accounts are ordered by total value stolen.
Data from 07/29/2020 (block 10553883) - 01/10/2022 (block 13979019).}
\label{fig:victim}
\end{figure*}

We plot the timeline of the top-10 attackers' activities in Figure~\ref{fig:attack}. The attackers are ranked by the total value stolen, with attacker $0x9799$ being the top-1. Each dot represents a detected attack sent by the attacker's account. The size of the dot represents stolen value. Color represents the exploit pattern. The most successful attacker ($0x9799$) steals value despite through different causes (including rebase, airdrop, etc.) The attacker's activities last about 
$1.1*10^6$ blocks, which amount to six months. The second attacker ($0x2a2e$) concentrates all her attacks to a one-month span. She exploits exclusively the value created by rebase operations. The third attacker ($0xdb40$) mount attacks sporadically and target value created through two causes: Token interest and rebase operations. The ninth attacker exploits partly errors to gain illicit profit. The tenth attacker exclusively grabs value from token interest in a three-month period. As a result, most top attackers mount multiple attacks consistently, which show the attacks are intended and not by accident.

We additionally study top victims' behavior. The victims are ranked by the value stolen. In Figure~\ref{fig:victim}, we plot in dots the transactions sent by victims whose deposit are stolen in identified attacks. Different color represents different causes. Additionally, in green hollow circles, we plot the normal transactions sent by the victims and related to Uniswap. The result shows that most victims change behavior after an attack/theft. For instance, victim accounts, including $0x0cd4$ and $0x80cc$, all stop using the vulnerable interface (e.g., partly error) to send deposit after an attack. However, other victims can repeatedly create extractable value that gets stolen. For instance, account $0x66ac$ repeatedly airdrop tokens to the Uniswap pool, which gets stolen. 

\subsubsection{Value Received by Pools}

\begin{table}[!htbp] %force in current page, disable float.
\centering{
\begin{tabularx}{0.425\textwidth}{ |X|l|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
\hline
Value extracted by & Rebase ($P_1$) & External transfer ($P_3$) \\
\hline
External attackers & \$0.81M & \$0.50M \\
\hline
Pools (intended) & \$58.1M & \$1.22M \\
\hline
Pools (accidental) & \$0.65M & \$1.29M \\
\hline
\end{tabularx}
}
\caption{Extractable value and its destinations}
\label{tab:extractable_value}
\end{table}
\begin{figure}[!htbp]
\begin{center}
  \subfloat[Value created by rebase ($P_1$)]{%
     \includegraphics[width=0.245\textwidth]{figures/figure_rebase_seg.eps}
    \label{fig:moneyflow_1}
  }%
  \subfloat[Value created by external transfers ($P_3$): all pools are between token $XX$ and $WETH$, where $XX$ is the tick on the $x$ axis.]{%
    \includegraphics[width=0.245\textwidth]{figures/figure_underwater_seg.eps}
     \label{fig:moneyflow_2}
     }%
\end{center}
\caption{Extractable value received by the pool versus that by attacker accounts}\label{fig:complex}\vspace{-0.10in}
\end{figure}


Extractable value can be claimed by any account, including an external attacker and the pool itself. Our measurement result so far captures the former case. In this experiment, we measure the extractable value that goes to the pool.

A pool can claim extractable value by calling the \texttt{sync} function, which synchronizes the pool reserve and token balance. In Uniswap, there are three circumstances \texttt{sync} is called: a standalone call to \texttt{sync} in a transaction, \texttt{sync} called after a \texttt{swap} in the same transaction, \texttt{sync} called after an \texttt{addLiquidity} call in the same transaction. In the first case, tokens are sent to the pool intentionally (denoted by ``pool (intended)'' in the table and figures), and in the second and third cases, the pool receives deposit by accident (denoted by ``pool (accidental)''), because it is an irrelevant transaction to \texttt{sync} the reserve and token balance. Informally, we calculate the extractable value that goes to the pool in the following method: We obtain the value of pool reserve before and after the transaction. We also parse the function call arguments from the transaction data field. We can cross-check the pre-state, post-state and function arguments, to detect the mismatch, which can be attributed to the extractable value. For instance, a normal \texttt{swap} in Uniswap does not change the product in AMM, and a spurious \texttt{swap} that the pool receives extractable value can be detected by the violation of product equality.

Using the above method, we measure the total extractable value claimed by the pool under different patterns, including $P_1$ and $P_3$. The result is presented in Table~\ref{tab:extractable_value}: The total value claimed by the pools is consistently more than $5\times$ of that by external attackers. This suggests ``room'' for the current Uniswap thief to increase their revenue. We further show the total extractable value by different pools/tokens. In Figure~\ref{fig:moneyflow_1}, we plot the extractable value created by different rebase-enabled tokens (Pattern $P_1$). 
Token $AMPL$ has the highest extractable value, most of which goes back to the pool by the token issuer intentionally calling \texttt{sync} function after each \texttt{rebase} call (the ``intended'' case). 
Token $BASE$ is the third highest in total extractable value and has the highest value stolen by external attackers. In Figure~\ref{fig:moneyflow_2}, we plot the extractable value created by external transfers (Pattern $P_3$) against different pools. Here, all the top-value pools we found are between token $WETH$ and another token. The most vulnerable pool is between Token $UNI$ and $WETH$, whose extractable value is $400$ thousand USD in total, among which the $10\%$ value is extracted by external attackers and the rest is mostly sent to the pool intentionally. Token $YFill$'s value is exclusively extracted by external attackers. Token $SUSHI$'s deposit is mostly claimed by the pool accidentally. 

\subsection{Characterizing Crimes}
\label{sec:behavior}

We further expand the scope of each attack instance by tracing the money flow and smart contract lineage. The goal is to uncover the attack business.

\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.495\textwidth]{figures/UniswapV2attacker3.eps}
\end{center}
\caption{Attack campaign template: Preparing, mounting and wrapping up theft attacks.}
\label{fig:business}
\end{figure}

Given an attack instance with attacker accounts $\{A\}$, we construct an expanded attack graph by adding the following information: 1) the transactions that pay Ether or tokens to the attacker accounts, 2) the transactions that deploy the smart contracts used in the attack, and 3) the transactions that are sent by the mule accounts who receive the stolen tokens after the attack. These new transactions would add into the graph a set of new accounts, be it either the transaction sender or receiver. We iteratively apply this graph-expansion process, until it reaches the ``hub-node'' accounts, which receive or send a large number of transactions (e.g., a popular DEX pool or mixer service). 
For instance, Figure~\ref{fig:business} shows an example of expanded attack instance, with the attackers in the red box and the victims; the added accounts and transactions are outside the two boxes. 

{\bf Attack ecosystem template}: We analyze the expanded attack graph in a template consisting of three phases: 1) attack preparation, 2) attack execution, and 3) attack wrap-up. Phase 2) is the core attack component, and Phases 1) and 3) are the expanded  parts. In general, the actual Boss often sits behind an exchange/mixer service, such as Tornado~\cite{me:tornado}, to hide its identity. In  attack preparation (Phase 1), the Boss sends commission in Ether to Attackers and Exploit developers. The Ether transfer can be relayed through the Mules. An Exploit developer writes an Exploit smart contract and deploys it to the blockchain. It then mounts the attack in the execution phase (Phase 2), exercising the strategies described previously (\S~\ref{sec:attack}). To wrap up a series of attacks (Phase 3), the mule receiving the stolen tokens transfers the tokens back to the Boss. This is often done by swapping the stolen tokens to ETH (e.g., via DEX and wrapped tokens such as WETH) and by sending the ETH to the Boss via a mixer service. In the attack wrap-up phase, the mule may transfer tokens to Investors to maximize the stolen value. 

\begin{table*}[h]
\caption{Attack ecosystem and attacker correlation: Red text shows the two attackers share the same developer of exploit smart contracts. AO represents attack operator and EC is exploit smart contract.
}
\label{tab:eco}
\centering{\small
    %\begin{tabular}{|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{1cm}|p{1.2cm}|}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \hline
    Accounts & \multicolumn{4}{c|}{Attack (S2)} & \multicolumn{2}{c|}{Preparation (S1)} & \multicolumn{2}{c|}{Wrap-up (S3)}  \\ \cline{2-9}
    (Mules) & \#AO & \#EC & Developer & Value ($10^3$ USD) & Commission & Mixer & DEX & Mixer \\
    \hline
     $0x9799$ & 5 %$0x4e53$, $0xac72$, $0xa084$, $0x5bb4$, $0xe929$ 
& 24 % $0x338c$, $0x3ac7$, $0x34a2$, $0x9a99$, $0x2927$, $0x536b$, $0xe9f8$, $0x684b$, $0x58a3$, $0x72bb$, $0xa8a2$, $0x72cb$, $0x2528$, $0xbf2d$, $0xadfc$, $0xd6a2$, $0x24af$, $0x1335$, $0xf367$, $0x94fc$, $0x5caf$,  $0x6332$, $0x3c3a$, $0x1233$	
& {\bf \color{red} $0x8641$} & 556 & \xmark  & \xmark  & \cmark  & \xmark \\
    \hline
    $0x2a2e$  & 1 %$0x2a2e$ 
& 1 %$0x5f5a$ 
& $0x2a2e$ & 239 & \cmark  & \xmark  & \cmark  & \cmark 
\\
    \hline
    $0xdb40$  & 5 %$0x64bc$, $0x62ae$, $0x3807$, $0x225c$, $0xdb40$ 
& 2 %$0x4dbc$, $0x4626$ 
& $0x4626$ & 113 & \cmark  & \cmark  & \cmark  & \cmark 
\\
    \hline
    $0x0c08$  & 1 %$0xfdee$ 
& 1 %$0x0c08$ 
& $0x0c08$ & 101 & \xmark  & \xmark  & \cmark  & \xmark 
\\
    \hline
    $0x5617$  & 4 %$0x3a51$, $0xf97b$, $0xbf3f$, $0xa1e6$ 
& 10 %$0xfb51$, $0x328d$, $0x8a14$, $0x0fc7$, $0x4ed5$, $0xb439$ ,$0x55a2$, $0x6ba3$ 
& \color{red}{$0x8641$} & 101 & \xmark  & \xmark  & \cmark  & \cmark 
\\
    \hline
    $0xb6bf$ & 1 %$0x675f$ 
& 2 %$0xb6bf$, $0x8526$ 
& $0x675f$ & 20 & \cmark  & \xmark  & \cmark  & \xmark 
\\
    \hline
    $0xc762$ & 1%$0xd0d0$ 
& 1%$0xc762$ 
& $0xd0d0$ & 16 & \cmark  & \cmark  & \cmark  & \cmark 
 \\
    \hline
    $0xa32d$ & 1%$0x7505$ 
& 1%$0xa32d$ 
& $0x7505$ & 6 & \cmark  & \xmark  & \xmark  & \xmark 
\\
    \hline  
    \end{tabular}%
}
\end{table*}

\ignore{
\begin{table}[h]
\caption{Attack ecosystem and attacker correlation: Red text shows the two attack instances are mounted using the exploit smart contracts developed by the same developer. AO represents attack operator and EC is exploit smart contract.
}
\label{tab:eco}
{\centering \scriptsize
    \begin{tabular}{|p{0.3cm}|p{1cm}|p{0.3cm}|p{0.3cm}|p{1cm}|p{0.7cm}|p{0.8cm}|p{.5cm}|}
    \hline
    Idx &Value ($10^3$~USD) & \#AO & \#EC & Developers & Mules & Deposits & Block gaps\\
    \hline
    1 & 552 & 5 %$0x4e53$, $0xac72$, $0xa084$, $0x5bb4$, $0xe929$ 
& 24 % $0x338c$, $0x3ac7$, $0x34a2$, $0x9a99$, $0x2927$, $0x536b$, $0xe9f8$, $0x684b$, $0x58a3$, $0x72bb$, $0xa8a2$, $0x72cb$, $0x2528$, $0xbf2d$, $0xadfc$, $0xd6a2$, $0x24af$, $0x1335$, $0xf367$, $0x94fc$, $0x5caf$,  $0x6332$, $0x3c3a$, $0x1233$	
& {\bf \color{red} $0x8641$} & $0x9799$ & $P_1$ & 121\\
    \hline
    2 & 101 & 1 %$0x2a2e$ 
& 1 %$0x5f5a$ 
& $0x2a2e$ & $0x2a2e$ 
& $P_1$ & 1\\
    \hline
    3 & 96 & 5 %$0x64bc$, $0x62ae$, $0x3807$, $0x225c$, $0xdb40$ 
& 2 %$0x4dbc$, $0x4626$ 
& $0x4626$ & $0xdb40$ 
& $P_1$ & 0\\
    \hline
    4 & 86 & 1 %$0xfdee$ 
& 1 %$0x0c08$ 
& $0x0c08$ & $0x0c08$ 
& $P_1$ & 1\\
    \hline
    5 & 67 & 4 %$0x3a51$, $0xf97b$, $0xbf3f$, $0xa1e6$ 
& 10 %$0xfb51$, $0x328d$, $0x8a14$, $0x0fc7$, $0x4ed5$, $0xb439$ ,$0x55a2$, $0x6ba3$ 
& \color{red}{$0x8641$} & $0x5617$ 
& $P_3$ & 2\\
    \hline
    6 & 48 & 1 %$0x675f$ 
& 2 %$0xb6bf$, $0x8526$ 
& $0x675f$ & $0x675f$ & $P_1$ & 0\\
    \hline
    7 & 29 & 1%$0xd0d0$ 
& 1%$0xc762$ 
& $0xd0d0$ & $0xd0d0$& $P_3$ & 1 \\
    \hline
    8 & 22 & 1%$0x7505$ 
& 1%$0xa32d$ 
& $0x7505$ & $0x7505$& $P_1$ & 0 \\
    \hline  
    \end{tabular}%
}
\end{table}
}


{\bf Results}: We measure the attack behavior in terms of attack preparation, execution and wrap-up. We find different attacks mounted by the same mule account are consistent and thus present the aggregated results by mule accounts. The result is in Table~\ref{tab:eco}.

In the attack execution phase (S2), the result shows that attacks are systematic, typically with a mule associated with multiple attack operators (AO) and exploit smart contracts (EC). For instance, Mule $0x9799$ has mounted attacks through $5$ different operator EOAs and leveraged more than $24$ different exploit smart contracts. Her exploit contracts are developed by the same developer for another Mule $0x5617$ (in red in Table~\ref{tab:eco}); this implies an underground business of exploit contract development.

We further characterize the attack preparation (S1) and wrap-up (S3) on different mules. Under S1, Column ``Commission'' shows whether the mule's attack operators receive money used for mounting the attacks within 30 days before the attack. Column ``Mixer'' shows whether the attack commission comes from the anonymized crime boss hidden behind a mixer service, such as Tornado. Under S2, Column ``DEX'' shows whether the attacker interacts with a DEX service to exchange tokens or to maximize the illicit profit. Column ``Tornado'' shows whether the attacker eventually transfer money to the anonymized boss behind the mixer service. The result shows that different mules vary in their strategies in attack preparation and wrap-up. For instance, Mule $0x9799$ is quite simplistic in the sense that she only interacted with DEX and didn't involve any mixer service in her attacks. Mule $0xdb40$\footnote{The full address of $0xdb40$ is $0xdb40ea5b6d0ef9e45c00c194345b44765a53dd19$ and the account behavior is public on \url{https://etherscan.io/address/0xdb40ea5b6d0ef9e45c00c194345b44765a53dd19}.} and $0xc762$, on the other hand, are quite sophisticated and employ strategies involving mixer and DEX.

\section{Detecting Lost Tokens}
\label{sec:losttokens}

\noindent
{\bf Problem}:
We detect lost tokens out of standalone deposits (i.e., atomicity violation II). On the one hand, the incidents of lost tokens appear as a standalone deposit. On the other hand, not every standalone deposit should be attributed to lost tokens. There are other causes such as token giveaway (e.g., airdrop) and administrative accounts calling privileged AMM operations. 

\noindent
{\bf Methods}: We propose two heuristics for detecting lost tokens. In the first heuristic, we assume the trader account calls an unsupported mechanism to deposit a token, finds the deposit fails, and switch to an alternative mechanism to retry the deposit. For instance, suppose an account deposits tokens using \texttt{transfer} in Uniswap V3 which does not accept \texttt{transfer}. The trader then switches to depositing the same value using \texttt{approve} before calling AMM operations such as \texttt{swap}. 
Based on the heuristics, we design the following indicator I8.

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I8:
Given a standalone deposit to an AMM pool, we find the transactions after the deposit from the same sender account. We filter out the transactions that are not issued to the same token with the deposit and the transactions that call the same token function with the deposit. The presence of such transactions given a deposit is an indicator of lost token.
}}\end{center}

In the second heuristic, the idea is that lost tokens must be deposited by an unprivileged AMM account. And a privileged account, such as an AMM administrator, is entitled to deposit value to an AMM pool, which is unlikely a mistaken deposit. We propose the indicator for lost token below:

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator I9: An account that calls privileged AMM functions (e.g., \texttt{setSwapFee()} in Balancer) is an privileged account, and a standalone deposit sent by a privileged account is not attributed to lost tokens.
}}\end{center}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Aggregated results on lost tokens}
\label{tab:lost}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|l|l|l| }
  \hline
   AMM & \# txs & Total value (USD) & Block diff (avg) \\ \hline
   Uniswap-V3 & $20$ & $47928$ & $9013$ \\ \hline
   Balancer & $192$ & $7875$ & $6578$ \\ \hline
   Curve & $3$ & $905$ & $14533$ \\ \hline
\end{tabularx}
}
\end{table}


\noindent
{\bf Results}:
Using the method above, we detect $215$ instances of lost tokens on Uniswap V3, Balancer and Curve, inflicting a total of lost tokens worth $56708$ USD, as shown in Table~\ref{tab:lost}. Given a standalone deposit, we calculate its value using the token price at the time of the deposit (by using nearest price with token WETH in Uniswap V2). We record the block difference between the standalone deposit and the follow-up deposit retry sent from the same account. It can be seen block difference on Uniswap V3 is about $371$ blocks which amount to about $1.78$ hours. Detailed case analysis is in Appendix~\ref{sec:losttoken:cases}.

\section{Countermeasures}
\label{sec:mitigate}

We first analyze the root cause of existing AMMs' insecurity in token theft and lost tokens.
%
Then, we present a secure design of AMM in defense of token theft and avoid lost tokens.
%
Third, we discuss strategies to incrementally harden a deployed AMM instance under insecure protocol design.

\subsection{Root Causes of AMM Insecurity}
\label{sec:causeanalysis}
We analyze AMM protocols to understand the root causes of atomicity violation. 
We identify two security-critical design choices in an AMM protocol: D1) How the AMM pool recognizes a token deposit? and D2) How the AMM pool handles a deposit by mistake? 

\noindent
{\bf Design choice D1: Deposit mechanism}: 
Each AMM operation, be it token swap or liquidity acquisition/removal, consists of a series of token deposits and withdrawals. An AMM pool may be designed to accept a token transfer as deposit, that is, a trader account externally calling token $T_0$'s \texttt{transfer} function in a token swap. We call this design by deposit-by-\texttt{transfer}. Alternatively, a pool may require the trader to first call $T_0$'s \texttt{approval} before the pool is allowed to do the \texttt{transferFrom} to complete the deposit. 
We call the design by deposit-by-\texttt{transferFrom}.

\begin{table}[!htbp] %force in current page, disable float.
  \caption{Characterization of AMM protocols: ``US2/US3/Ce/Br'' represent Uniswap V2 (incl. Sushiswap and Pancakeswap), Uniswap V3, Curve and Balancer. ``Lost'' refers to lost tokens.}
  \label{tab:ammprofile}
  \centering{
  \begin{tabularx}{0.4\textwidth}{ |X|c|c|c|c| }
  \hline
Design & US2 & US3 & Ce & Br \\ \hline
Deposit by \texttt{transfer} 
& \cmark & \xmark & \xmark & \xmark \\ \hline
Return lost tokens
& \cmark & \xmark & \xmark & \xmark \\ \hline
Security risks
& Theft & Lost & Lost & Lost \\ \hline
  \end{tabularx}
}
\end{table}

We characterize top AMMs in terms of whether they support deposit by external \texttt{transfer}, with the result in Table~\ref{tab:ammprofile}. All AMM protocols except for Uniswap V2 do not support deposit by \texttt{transfer} and require the \texttt{approve}-\texttt{transferFrom} workflow to deposit tokens.

%specifies how the AMM pool smart contract should interact with trader, provider and token smart contracts. 
%An AMM protocol materializes the above model, particularly token deposits and withdrawals in supported workflows. Specifically, to deposit tokens $T_{\text{X}}$, a trader EOA can externally call the token's \texttt{transfer} function or call the token's \texttt{approve} function followed by the pool's call of the \texttt{transferFrom} function.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.25\textwidth]{figures/uniswapv2-dilemma.eps}
\end{center}
\caption{Uniswap V2's design and the cause of permissionless withdraw.}
\label{fig:uniswapv2model}
\end{figure}

\noindent
{\bf Insecurity of deposit-by-\texttt{transfer}}: 
When an AMM pool supports deposit-by-\texttt{transfer}, the deposit and withdrawal in a swap could be executed in two separate transactions: As shown in Figure~\ref{fig:uniswapv2model}, the token-depositing transaction $tx_1$ calls the token smart contract, and the token-withdrawing transaction $tx_2$ calls the AMM pool smart contract. Since $T_0$, be it an ERC20 token, does not record the depositor account, it leaves the pool smart contract no way to enforce permission on token withdrawal. A permissionless AMM exposes the trader to the risk of token theft where the deposited value can be extracted by any users or bots including the malicious ones who send withdrawal transactions to frontrun each other.
More formally, we formulate the model of token theft threats in the next paragraph.
In practice, Uniswap V2's pool detects token deposit by tracking the pool's balance update and allows whoever comes the first to withdraw as many tokens as bounded by the balance update.

\noindent
{\bf Design choice D2: Token lost-and-found}: 
While an AMM pool supports token swaps and utility management, it also needs to responsibly handle token lost-and-found. 
When deployed on Ethereum blockchain, there is no way preventing a trader, potentially absentminded, from depositing tokens to the pool. A token is  mistakenly deposited by externally calling \texttt{transfer} function.
Receiving a mistakenly deposited token, a pool can choose to return it to the original owner, or to keep it. In the latter case, the token is forever lost to the trader.
By manually analyzing the relevant smart contracts, we profile the AMMs in support of token lost-and-found in Table~\ref{tab:ammprofile}: Uniswap V2 returns the mistakenly deposited tokens (using a function \texttt{skim}), while all other AMMs do not return.

A non-returning AMM pool exposes the traders to the risk of lost tokens. In practice, AMM instances based on Uniswap V3, Curve, and Balancer are all subject to the lost-token risk. We did a measurement study that detect lost tokens out of the atomicity violations (more specifically, standalone withdrawal of Violation II) on these AMM instances. Due to the space limit, we defer the measurement of lost tokens to Appendix~\ref{sec:losttokens}.

Overall, an AMM pool designer faces a dilemma, whether to handle deposit by \texttt{transfer}. 
To handle such deposit, as in Uniswap V2, the AMM exposes its customer traders to the risk of token theft. Not to handle such deposit, as in all other protocols, the AMM risk their customers to lost tokens. This security-utility tradeoff is depicted in Table~\ref{tab:ammprofile}.

\subsection{Secure AMM Protocols}

We propose a secure protocol design of AMM pools. In our protocol, we follow Uniswap V3's design and require the AMM pool to accept only the deposits made by the \texttt{approve}-\texttt{transferFrom} workflow. By this means, the pool smart contract can keep track of swap-intended token deposits and thus can enforce permission checks on token withdrawal. That is, token withdrawal is granted only when its receiver is the same with the original depositor. By this means, it eradicates the risk of the token thefts.

The risk of lost token is caused by the incapability of tracking token transfer history in the ERC20 standard. While changing ERC20 standard can help fix the issue, it is not practical given the large-scale deployment of ERC20 tokens on Ethereum. We propose a protocol to mitigate lost tokens with off-chain assistance. 

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.3\textwidth]{figures/mitigate_losttokens.eps}
\end{center}
\caption{Trustless design to mitigate lost token risks}
\label{fig:mitiglost}
\end{figure}

In our protocol, we assume a lost-and-found smart contract (called the service) that has the privilege to approve a request to return token deposits. Suppose a user Alice makes a mistake to deposit tokens to our AMM pool by calling the unsupported \texttt{transfer} function. The token deposit transaction is $tx1$. After finding the mistake, Alice may request refund by contacting the lost-and-found service. Alice's request includes $tx1$ and enough blocks after $tx1$ (inclusively) to verifies $tx1$'s finality on Ethereum. Using the information, the service smart contract then verifies the finality of $tx1$ on Ethereum. It also checks various conditions including whether it is the AMM pool that receives token deposit from $tx1$ and the request is signed by Alice's secret key. If the conditions are met, the service calls a privileged function \texttt{returnToken} on the AMM pool. Figure~\ref{fig:mitiglost} presents our trustless lost-and-found protocol.

\subsection{Hardening Deployed AMM Instances}

{\bf Lost-and-found service off-chain}: We propose running a lost-and-found off-chain web service. This off-chain service monitors the on-chain state for profitability and collects extractable value ahead of actual attacks. To do so, the service takes an aggressive strategy by directly monitoring the vulnerable deposits (i.e., $P_1$, $P_3$, $P_4$) and withdrawing immediately upon discovery. For token interest $P_2$, the service monitors mempool for stealing transactions sent to the pools supporting token interests. Upon the discovery, the service sends transactions to frontrun the stealing transactions. 

In essence, this service performs the same functionality with thief attackers in discovering profitability opportunities on-chain, but it is benign in the sense that it stores the extracted value and allows victims to claim their tokens. Technically, given value deposited by Account $V$, the service stores the value and allows $V$ or any other account with $V$'s signature to claim the value.

{\bf Fuzzing router smart contracts}: For the risky swaps caused by buggy router contracts (i.e., $P_4$), one can mitigate the problem by developing more secure router smart contracts. Here, to ensure that the router calls deposit and withdrawal in all possible code path, we fuzz the router smart contract using a fuzzing framework Echidna~\cite{DBLP:conf/issta/GriecoSCFG20}. Specifically, we develop a test oracle that defines swap atomicity and a smart contract rewriter to automatically insert the oracle to the target router smart contract. The test oracle records all the \texttt{transfer}/\texttt{transferFrom}/\texttt{swap} invocations and checks if there is a standalone invocation in the end of execution.   

\section{Related Work}
\label{sec:rw}

We survey the most relevant works and compare them against this one. Due to the space limit, we defer the extended related work to Appendix~\ref{appdx:rw}.

{\bf DeFi attacks and BEV}: In DeFi, a primary class of attacks exploit Blockchain extractable value or BEV. BEV is the amount of value that can be extracted by reordering transactions. 
Torres, et al.~\cite{DBLP:conf/uss/TorresCS21} detect frontrunning attacks from Ethereum transactions by the attack signature being a pair of successful and failed transactions. Qin et al.~\cite{DBLP:journals/corr/abs-2101-05511} measure and characterize four BEV-exploiting attacks, including liquidation, sandwich attacks, arbitrage and transaction relay, on Ethereum. Wang, et al.~\cite{DBLP:journals/corr/abs-2105-02784} detect the instances of arbitrage on Uniswap-V2, by finding profitable cycles on the token-transfer graph. Zhou, et al.~\cite{DBLP:conf/sp/ZhouQCLG21} discover arbitrage opportunities by finding profitable cycles among token-token exchange rates in real time. Xia, et al.~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21} detect scam tokens listed on Uniswap V2 that impersonate other tokens to trick their traders; the attack signature is that the scam token's pool has a shorter-lived life span of transactions than the normal pools.

Arbitrage and sandwich attacks are two known patterns to extract BEV from AMM. In arbitrage, the profitable opportunities come from the difference in token exchange rates between AMM pools. In sandwich attacks, the profitable opportunities come from the imminent price changes caused by pending trades. 1) Both BEV attacks exploit or manipulate token prices. In both attacks, the attacker monitors certain conditions on the token prices to determine the timing of value extraction.
In this work, the ``extractable value'' stolen from the theft comes from the AMM design flaw that allows permissionless withdrawal. To extract the value, the attacker does not monitor token prices; instead, she monitors the presence of exploitable deposit (non-standard token deposit such as rebase) to determine when to extract the value.
2) In addition, in existing arbitrage and sandwich attacks, the attack success does not require breaking atomicity of individual AMM operations. That is, a successful sandwich attack (or arbitrage attack) can be composed of a sequence of token swaps that are atomic. By contrast, the theft attacks studied in this work requires breaking atomicity of AMM operations.
Therefore, the theft attacks studied in this work are fundamentally different from the BEV-based attacks~\cite{DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2101-05511,DBLP:journals/corr/abs-2105-02784,DBLP:conf/sp/ZhouQCLG21}, due to their difference in causes and execution conditions. 

{\bf Smart contract vulnerabilities and attacks}: Existing research has covered the automatic discovery of new smart-contract vulnerability~\cite{DBLP:conf/ccs/LuuCOSH16,DBLP:conf/uss/KruppR18} and detection of attack instances of known vulnerabilities~\cite{DBLP:conf/uss/ZhangZZL20,DBLP:conf/uss/ZhouYXCY020,DBLP:conf/uss/SuSDL0XL21,DBLP:conf/uss/0001L21}. These two lines of researches tackle generic program-level attacks such as reentrancy attacks and transaction ordering dependencies, which are not DeFi specific as in this work.

\section{Responsible Disclosure}
\label{sec:disclosure}

We have reported the discovered atomicity violations and the vulnerabilities to Uniswap's bug bounty program (\url{https://uniswap.org/bug-bounty}). The bugs have been confirmed. Further details on bug reporting are documented on the anonymized Google document~\cite{me:bugreport:defiant}. 

\section{Conclusion}
\label{sec:conclude}

This paper presents the first measurement study of atomicity violations and token theft attacks on popular Uniswap DEXes on Ethereum. The study unearths more than $465$ thousand thefts and stolen tokens worth of a total of $3.5$ million USD. It uncovers a range of previously unknown patterns of vulnerable deposits (e.g., token interest and supply adjustment), exposes real-world attackers' adaptive strategies to send malicious withdrawals, and reveals their systematic behavior in preparing, executing, and finalizing theft attacks. Finally, it presents mitigation schemes to remedy the deployed DEXes running immutable smart contracts.


==> text/old/v8_intro.tex <==
\section{Introduction}

Recent years witnessed the rise of Decentralized Finance (DeFi) on blockchains. A prominent class of DeFi applications is the Decentralized Exchange (DEX) which allows a trader account to swap their assets from one token to another. 
On Ethereum, deployed DEX instances including Uniswap~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer} all run AMM protocols or automated market maker, which account for more than $95\%$ of the DEX activities all time~\cite{me:etherscan:topdex}, attracting hundreds of millions of transactions today (as of July, 2022). Other than token swap, an AMM\footnote{We use the terms AMM and DEX interchangeably in this paper.} supports liquidity addition/removal in which a liquidity-provider account deposits tokens as a reserve for subsequent token swaps.

AMM can be misused. A well studied class of AMM misuses are sandwich attacks and arbitrage~\cite{DBLP:conf/sp/DaianGKLZBBJ20,DBLP:journals/corr/abs-2101-05511,DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2105-02784}. In both attacks, the attacker account extracts illicit value by sending multiple transactions in crafted order. Recent research has shown the large scale of sandwich attacks and arbitrage on Ethereum~\cite{DBLP:journals/corr/abs-2101-05511,DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2105-02784}. 
Another AMM misuse is to list scam tokens~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21} that impersonate other tokens and trick their traders. In these known misuse patterns, each attack is composed of multiple AMM operations, such as a cycle of token swaps in arbitrage~\cite{DBLP:journals/corr/abs-2105-02784} and two transactions that frontrun and backrun a victim transaction in a sandwich attack~\cite{DBLP:journals/corr/abs-2101-05511}.
%scam tokens by short-lived span of AMM operations~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21}, etc.

\begin{figure}[b!ht]
\begin{center}
\includegraphics[width=0.26\textwidth]{figures/workflow7.eps}
\end{center}
\caption{Data-analytical workflow to detect AMM operation atomicity violation, stolen tokens and theft attacks.}
\label{fig:workflow7}
\end{figure}

\vspace{2pt}\noindent\textbf{Discovering atomicity violations}. 
This work aims to discover a different class of AMM misuse: atomicity violations. Specifically, an AMM operation, be it a token swap or liquidity management, should execute a sequence of token deposits and withdrawals in an all-or-nothing manner (i.e., atomic operation execution). Violation of the operation atomicity could imply security risks and attacks. For instance, a token swap executed by a standalone withdrawal (i.e., without the matching deposit) can suggest an incident of token theft in which someone can withdraw value without sending any deposit to the AMM. Atomicity violation is different from the known AMM misuses that manifest in multi-operation sequences and that do not entail the violation of individual operations' atomicity.

By joining and analyzing more than $60$ million transactions on Ethereum and Binance Smart Chain (BSC), to our surprise, we find atomicity violations widely exist among deployed AMM services: 
Commiting these violations are the most popular services in practice, including Uniswap V2~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer}.
In total, they execute more than $74$ thousand AMM operations violating atomicity, exhibiting various patterns including standalone token deposit, standalone withdrawal, account mismatch, and value mismatch.

\vspace{2pt}\noindent\textbf{Understanding atomicity violations}. 
To understand the nature of the atomicity violations, that is, whether they occur by accident or are committed intentionally, we formulate the following hypothesis: 1) The atomicity violations in which the deposited value is below the value withdrawn could indicate token thefts in which a thief account attacks by extracting value from a victim AMM or trader account. 2) The atomicity violations in which the deposited value exceeds the value withdrawn could indicate AMM denial of service in which a victim trader depositing value is declined of withdrawal service. Specifically, we focus on the lost-token risks in which the victim trader deposits tokens by mistakes.

We detect the attack instances of token thefts out of the discovered atomicity violations. Attack detection poses challenges because the ground truth (i.e., accounts' intention and behavior) may be off the blockchain and is not directly observable. For instance, in verifying that a standalone token withdrawal is caused by a theft, one has to know that the depositor and withdrawer accounts are controlled by two distinct physical users, which is known to be an intractable problem with only on-chain data and which is not solved by existing heuristics such as address clustering~\cite{DBLP:conf/fc/Victor20,DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:conf/sp/HuangALIBMLLSM18,DBLP:books/daglib/0040621}  (see \S~\ref{sec:discoveryproblem} for detail).

To workaround the lack of ground truth, we analyze AMM protocols, model rational attackers' strategies, and use them as indicators to match the involved accounts' observable behaviors on-chain. For instance, given that the value in a theft would be publicly extractable, a rational attacker would want to minimize the deposit-to-withdrawal delay to frontrun competing thieves. For another instance, to minimize the attack failure rate, a rational attacker would read AMM states (e.g., token balances), exhibiting certain observable patterns on her trace of function calls (e.g., calling \texttt{balanceOf}). We propose an algorithm to discover thefts by matching them against these indicators.

Overall, we develop an end-to-end transaction-analytical pipeline, depicted in Figure~\ref{fig:workflow7}, to discover atomicity violations, to detect the attacks of theft and lost tokens, and to characterize attackers' systematic behavior in commiting these cyber-crimes.

%We found in practice the exploitable deposits can be created in a variety of unexpected application scenarios, including free token giveaways (i.e., airdropping), tokens redistributing fees to privileged shareholder accounts, tokens bearing interest, tokens that can adjust or rebase total supply, buggy smart contracts, and unsafe user interface that executes a swap in two separate transactions, etc. 

\vspace{2pt}\noindent\textbf{Findings}. 
We found the AMM services based on the Uniswap V2 protocol exhibit atomicity violations that allow for more value withdrawn than deposited. On these AMM instances including Uniswap V2, Sushiswap and Pancakeswap, we aim to validate the threat of token thefts (1). Other AMM instances including Uniswap V3, Balancer and Curve exhibit atomicity violations that allow for more value deposited than that withdrawn. We aim to validate the threat of lost tokens (2).

1) On the Ethereum mainnet and BSC fork, we discover $465$ thousand theft attacks mounted by $258$ distinct attacker accounts, inflicting a loss of more than $3.7$ million USD stolen from $978$ victim traders.
Each attack instance we found matches at least one indicator described above. Interesting attacker behavior was observed in practice. For instance, real-world attackers {\it adapt} to the different patterns of exploitable deposits and exhibit different behavior: When the attacker is to extract value from interest-bearing tokens, she waits long enough, typically hundreds of Ethereum blocks, for the interest to accumulate and to become profitable. To extract deposits of other patterns, the same attacker instead wastes no time extracting the illicit value, typically within one or two blocks.

We further study attackers' and victims' behavior by tracking their money flow and actions to create/destroy smart contracts. Our study uncovers the systematic criminal activities: the crime bosses use mixer services to hide their identities while sending commissions and instructions. After the attack, the money is sent to various DeFi services to maximize illicit profit. Exploit smart contracts are widely used to improve attack success rates.

2) We also detect, from the standalone deposits on Uniswap V3, Curve and Balancer, the $215$\jiaqi{Done} incidents of lost tokens worth a total of $56,700$ USD. Given a standalone deposit, our method to detect whether it results in lost token is whether it relies to deposit similar amount of tokens. 

\vspace{2pt}\noindent\textbf{Mitigation}. 
%why it is hard to design secure AMM in practice?
Empirically, all deployed AMM instances including Uniswap V2/V3, Sushiswap, Pancakeswap, Balancer and Curve are vulnerable to either token  theft or DoS like lost tokens. This is not by accident: It shows a fundamental challenge to secure AMM in practice where the AMM needs to recognize various token deposit mechanisms with limited information. 

%One cause of the atomicity violations is that certain non-standard token operations unspecified in the AMM protocols (e.g., rebasing token supply and interest-bearing tokens) are mistreated as token deposit that allows subsequent token withdrawal to succeed. This manifests in standalone withdrawals. Another cause is that certain token deposits are not intended for withdrawal (e.g., airdrop and token lost-and-found), which results in standalone deposits.

To mitigate the risks, we first propose secure AMM protocols that require rewriting and redeployment of smart contracts. To mitigate token thefts, the secure AMM prohibits exploitable token deposits for security at the expense of more restrictive interfaces in AMM operations. To avoid lost token risks, the AMM smart contract is extended with a BtcRelay~\cite{me:btcrelay,DBLP:conf/aft/DaveasKKZ20} like capability to verify the transaction requesting token returns. 

Besides, we propose mitigation schemes retrofittable over a deployed AMM instance without upgrading the smart contracts. These schemes harden the security of an off-chain infrastructure and application-layer smart contracts on top of AMMs.

\vspace{2pt}\noindent\textbf{Contributions}. This paper's contributions are outlined as follows: 

\vspace{2pt}\noindent$\bullet$\textit{ New findings}. We discover a total of $3.5$ million USD worth of stolen value by measuring and analyzing atomicity violations on three popular Uniswap V2 services on Ethereum and BSC. 
The discovered token theft attacks uncover the previously unknown patterns of extractable value  (e.g., token rebase, interest, airdrop, mishandled contract exception) and expose the adaptive attack strategies that occur offline and otherwise would have been hidden. We further study the criminal infrastructures and campaigns mounted to systematically prepare, execute and finalize the theft attacks.

%We also formulate and measure the risk of lost tokens on other DEX services including Uniswap V3, Balancer and Curve. The result reveals lost tokens worth of XXX USD across more than XXX transactions on Ethereum. 

\vspace{2pt}\noindent$\bullet$\textit{ New techniques}. We develop an end-to-end analytical pipeline to detect atomicity violations and relevant attacks from Ethereum transaction traces, including an efficient join algorithm and various heuristics to automatically discover and cross-check token theft and lost tokens. 
%XXX: Also we propose mitigation schemes including a fuzzer and test oracle to automatically detect mishandled exceptions in smart contracts.

%This work leads to the findings that shed light on the current and future underground ecosystem that strategically exploits the atomicity violation to gain illicit profit.

\noindent
{\bf Roadmap}: \S~\ref{sec:background} introduces the background of Ethereum transactions, tokens and DEX. Discovery of atomicity violations is described in \S~\ref{sec:detectriskyswap}. Detection and characterization of theft attacks are presented in \S~\ref{sec:attack}. Detection of lost tokens is in \S~\ref{sec:losttokens}. 
Countermeasures are presented in \S~\ref{sec:mitigate}. Related work is described in \S~\ref{sec:rw}. Responsible disclosure is discussed in \S~\ref{sec:disclosure} with the conclusion in \S~\ref{sec:conclude}. 

\ignore{
\noindent
{\bf System overview}: 
To discover the misuses, our approach is to find the mismatch between an AMM's governing protocol and its use history (collected from Ethereum transactions). Specifically, our approach takes as input the AMM protocol specification and filtered transactions/events collected from blockchain exploration service (XXX). It produces the discovered AMM operations that violate the protocol specification. Internally, it joins the records of different token-transfer operations across transactions. To reduce the search space (e.g., a naive join would entail cross-product on all transactions' powerset), we develop an efficient linear algorithm that takes advantage of the invariant observed from the Uniswap-V2's smart contract program.

1) We found all AMM protocols except for Uniswap V2 choose not to handle token deposit by external \texttt{transfer} (i.e., a trader deposits a token to a pool's account by externally calling the ERC20 \texttt{transfer} function). This is shown in Table~\ref{tab:policy}. Users of these AMMes risk lost tokens, where tokens are deposited by mistake and the users can not retrieve them back. Such cases of standalone token deposits are found to widely exist on these AMMes, out of which we detect the lost-token cases. We verify the lost tokens by making sense of the same-trader behavior in other relevant transactions. For instance, we found on Uniswap V3, a standalone token deposit is commonly followed by the AMM's token swap, which indicates the trader mistakenly deposits tokens by using deprecated swap API. 

2) The Uniswap V2 protocol accepts token deposits by external \texttt{transfer}. This design choice leaves the pool smart contract unable to track the original depositor (see Figure~\ref{XXX}) and forces it to accept a token withdrawal without enforcing permission. This flawed design, which we call permissionless withdrawal, affects various AMM operations (including token swaps, liquidity addition/removal, and returning lost token) and has adverse impacts on all Uniswap V2 based instances (including Uniswap V2, Sushiswap and Pancakeswap). The permissionless withdrawal gives rise to a new class of token theft threats in which Alice's exploitable token deposit can be extracted by malicious trader Bob, if Bob sends the token-withdrawal transaction first. By studying relevant transactions, we reveal various patterns of exploitable deposits in practice that lead to actual token theft. These causes include both standard and non-standard token balance updates, interest-bearing tokens, and buggy AMM-caller smart contracts. 

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.325\textwidth]{figures/automata3.eps}
\end{center}
\caption{Matchmaking in two rounds to detect risky swaps (Type-II and Type-III swaps).}
\label{fig:automata}
\end{figure}
}


\section{Background}
\label{sec:background}

Ethereum blockchain supports two types of addresses: An externally owned account (EOA), which is an Ether owner's public key, and a contract account (CA), which refers to the immutable memory address to which the smart contract is deployed on miners. An Ethereum transaction is a binding between its sender address and receiver address.

Most widely deployed tokens on Ethereum are fungible tokens in which each unit is interchangeable with and indistinguishable from any other unit. ERC20 is the most adopted standard of fungible tokens on Ethereum. ERC20 functions include \texttt{transfer} which allows a token owner to transfer her tokens to another account, \texttt{approve} which allows an owner to delegate the spending of her tokens to another delegatee account, \texttt{transferFrom} that allows a delegatee account to spend tokens on behalf of the original owner under the approved token limit, \texttt{balanceOf} that allows anyone to get an account’s token balance, etc.

An AMM or automated market maker is a dominant form of decentralized exchange (DEX) deployed on Ethereum blockchains. An AMM runs one or multiple ``pools'' in smart contracts. An AMM pool owns two tokens, say $T_0$ and $T_1$. An AMM pool minimally supports two operations: 1) token swap between a trader account and the pool smart contract, and 2) liquidity addition/removal between a provider account and the pool smart contract. The trader and liquidity provider can be either an EOA or a CA.

In a token-swap operation, the trader deposits $dx$ units of token $T_0$ to the pool's account and receives from the pool $dy$ units of token $T_1$. The AMM internally determines the token exchange rate (or value of $dy$) by enforcing the invariant on some function. For instance, Uniswap is a constant-product market maker where the invariant function is the product of the two token balance.

In an add-liquidity operation, the liquidity provider deposits $dx$ units of token $T_0$, deposits $dy$ units of token $T_1$, and withdraws a certain amount of ``base'' tokens $T_{\texttt{LP}}$. A remove-liquidity workflow is the reverse of add-liquidity, in that the liquidity provider deposits tokens $T_{\texttt{LP}}$ and withdraws tokens $T_0$ and $T_1$ at a certain ratio.

\begin{table}[!htbp] %force in current page, disable float.
\centering{\scriptsize
\begin{tabularx}{0.5\textwidth}{ |l|X|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
Layer & $swapT.$ workflow & $addL.$ workflow \\ \hline
Uniswap V2~\cite{me:uniswapv2:pool}
& $T_0$.\texttt{transfer}(trader,amountOut) & $T_0$.\texttt{transfer}(trader,amountOut) \\ 
& pool.\texttt{swap}(amountOut, to\_addr) & $T_1$.\texttt{transfer}(trader,amountOut) \\ 
 & & pool.\texttt{mint}(to\_addr) \\ 
\hline
Uniswap V3
& pool.\texttt{swapXXX}(amountOut, to\_addr) & pool.\texttt{addLXXX}(to\_addr) \\ 
\hline
\end{tabularx}
}
\caption{Uniswap V2/V3's API in $swapToken$ and $addLiquidity$ represents $addLiquidity$ workflow.}
\label{tab:uniswapv2:api}
\end{table}




==> text/old/v9.1_intro_afterXFWang.tex <==
\section{Introduction}

Recent years have witnessed the rise of Decentralized Finance (DeFi) on blockchains. A prominent class of DeFi applications is Decentralized Exchange (DEX) that allows a trader account to swap their assets from one type of tokens to another. 
On Ethereum, deployed DEX instances including Uniswap~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer} all run AMM protocols or automated market maker, which account for more than $95\%$ of the DEX activities all time~\cite{me:etherscan:topdex}, attracting hundreds of millions of transactions today (as of July, 2022). Other than token swap, an AMM\footnote{We use the terms AMM and DEX interchangeably in this paper.} supports liquidity addition/removal in which a liquidity-provider account deposits tokens as a reserve for subsequent token swaps.

AMM can be misused. A well studied class of AMM misuses are sandwich attacks and arbitrage~\cite{DBLP:conf/sp/DaianGKLZBBJ20,DBLP:journals/corr/abs-2101-05511,DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2105-02784,DBLP:conf/sp/ZhouQCLG21}. In both attacks, the attacker account extracts illicit value by sending multiple transactions in a crafted order. Recent research has shown the large scale of sandwich attacks and arbitrage on Ethereum~\cite{DBLP:journals/corr/abs-2101-05511,DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2105-02784,DBLP:conf/sp/ZhouQCLG21}. 
Another AMM misuse is to list scam tokens~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21} that impersonate other tokens to trick their traders. In these known misuse patterns, each attack is composed of multiple AMM operations, such as a cycle of token swaps in arbitrage~\cite{DBLP:journals/corr/abs-2105-02784} and two transactions that frontrun and backrun a victim transaction in a sandwich attack~\cite{DBLP:journals/corr/abs-2101-05511}.
%scam tokens by short-lived span of AMM operations~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21}, etc.

\begin{figure}[b!ht]
\begin{center}
\includegraphics[width=0.375\textwidth]{figures/workflow7.eps}
\end{center}
\caption{Data-analytical workflow to detect AMM operation atomicity violation and token theft attacks.}
\label{fig:workflow7}
\end{figure}

\vspace{2pt}\noindent\textbf{Discovering atomicity violations}. 
This work aims to study a different class of AMM misuses: atomicity violations. Specifically, an AMM operation, be it a token swap or liquidity management, should execute a sequence of token deposits and withdrawals in an all-or-nothing manner (i.e., atomic operation execution). Violation of the operation atomicity could imply the presence of security risks or even attacks. For instance, executing a token swap by a standalone withdrawal (i.e., without the matching deposit) could indicate an incident of theft in which a thief withdraws value without making any deposit to the AMM. For another instance, a token swap by a standalone deposit (without a matching withdrawal) could mean an adversarial AMM denying the withdrawal request from the trader who has made a deposit.
Note that atomicity violation is different from the known AMM misuses that manifest in multi-operation sequences and do not entail the violation of individual operations' atomicity.

By connecting together and analyzing over $60$ million transactions on Ethereum and Binance Smart Chain (BSC), to our surprise, we find that atomicity violations widely exist among deployed AMM services: 
Committing these violations are the most popular services, including Uniswap V2~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer}.
In total, they have performed more than $74$ thousand AMM operations violating atomicity, which exhibit various patterns including standalone token deposit, standalone withdrawal, account mismatch, and value mismatch.

%To understand the nature of the atomicity violations, that is, whether they occur by accident or are committed intentionally, we formulate the following hypothesis: 1) The atomicity violations in which the deposited value is below the value withdrawn could indicate token thefts in which a thief account attacks by extracting value from a victim AMM or trader account. 2) The atomicity violations in which the deposited value exceeds the value withdrawn could indicate AMM denial of service in which a victim trader depositing value is declined of withdrawal service. Specifically, we focus on the lost-token risks in which the victim trader deposits tokens by mistakes.

\vspace{2pt}\noindent\textbf{Understanding atomicity violations}. 
We aim to understand the nature of the atomicity violations, whether they are accidents or intentional crimes. While different atomicity violations can be attributed to different threats (e.g., denial of service mentioned above), we mainly focus on the prominent cases of token theft in our measurement result.

Detecting theft from the atomicity violations is challenging. This is because the ground truth often includes off-chain activities unaccounted for.
%which are unobservable. 
For instance, when attributing a standalone withdrawal to theft, one has to know that the party making the deposit to accounts and the party withdrawing from the accounts are controlled by two distinct physical entities, which is known to be an intractable problem with only on-chain data; known heuristics such as address clustering~\cite{DBLP:conf/fc/Victor20,DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:conf/sp/HuangALIBMLLSM18,DBLP:books/daglib/0040621} do not apply here (see \S~\ref{sec:discoveryproblem} for detail).

To address this challenge, we focus on making sense of the accounts' on-chain behaviors and matching them to the rational attack strategies we identify through analyzing the AMM protocols. For instance, a rational thief in fear of being frontrun by competing thieves would send crafted transactions with the minimal deposit-to-withdrawal delay, which can indicate the occurrence of an attack. For another instance, to avoid the failure of theft, a careful thief would check on-chain states extensively (e.g., token balances) before committing the theft; these pre-attack operations (e.g., calling token function \texttt{balanceOf}) could indicate an intentional theft. We propose an algorithm to capture the account behavior with such indicators and automatically detect thefts.

Overall, our method is an end-to-end transaction-analysis pipeline, depicted in Figure~\ref{fig:workflow7}, which first discovers atomicity violations and then detects and characterizes theft attacks.

%We found in practice the exploitable deposits can be created in a variety of unexpected application scenarios, including free token giveaways (i.e., airdropping), tokens redistributing fees to privileged shareholder accounts, tokens bearing interest, tokens that can adjust or rebase total supply, buggy smart contracts, and unsafe user interface that executes a swap in two separate transactions, etc. 

\vspace{2pt}\noindent\textbf{Findings}. 
On the Ethereum mainnet and BSC fork, we discover $465$ thousand theft attacks mounted by $258$ distinct attacker accounts, inflicting a loss of more than $3.7$ million USD on $978$ victim accounts.
Each attack instance we find matches at least one indicator. Interesting attacker behavior has been observed in practice. For instance, real-world attackers {\it adapt} to the different patterns of exploitable deposits and exhibit different behavior: When the attacker is to extract value from interest-bearing tokens, she waits long enough, typically hundreds of Ethereum blocks, for the interest to accumulate and to become profitable. To steal other kinds of deposits, such as observing token rebase,
%of other patterns, 
the same attacker instead wastes no time extracting the illicit value, typically within one or two blocks.

We further study attackers' and victims' behavior by tracking their money flow and their actions to create/destroy smart contracts. Our study uncovers the systematic criminal activities: the crime bosses use mixer services to hide their identities while sending commissions and instructions. After the attack, the money is sent to various DeFi services to maximize illicit profit. Exploit smart contracts are widely used to improve attack success rates.

From the violations that are not attributed to theft, we further detect the instance of potential denial of service. Particularly, we formulate the problem of detecting lost tokens where the deposits are made by mistake, and the AMM refuses to return the tokens. We propose threat indicators by assuming the victim accounts' rational behavior after lost tokens. Our measurement result on Ethereum confirms the existence of lost tokens on Uniswap V3, CUrve and Balancer (inflicting a total value of 57,000 USD lost unfairly by these AMMes). We note that the atomicity violations could imply other threats than theft and lost tokens, and a comprehensive study is left for future research. 
%is out of the scope of this work.

\vspace{2pt}\noindent\textbf{Mitigation}. 
%why it is hard to design secure AMM in practice?
Our empirical study shows that all six popular AMM services (i.e., Uniswap V2/V3, Pancakeswap, Sushiswap, Balancer, and Curve) are vulnerable to either the threat of theft or DoS like lost tokens. This unsatisfactory state of affairs in practice is not by accident: It reveals a fundamental design challenge in securing AMM where the AMM smart contract with limited information needs to recognize token deposits of various intentions.

%One cause of the atomicity violations is that certain non-standard token operations unspecified in the AMM protocols (e.g., rebasing token supply and interest-bearing tokens) are mistreated as token deposit that allows subsequent token withdrawal to succeed. This manifests in standalone withdrawals. Another cause is that certain token deposits are not intended for withdrawal (e.g., airdrop and token lost-and-found), which results in standalone deposits.

To mitigate the risks, we have made the first attempt to design secure AMM protocols that require rewriting and redeployment of smart contracts. To mitigate token thefts, the secure AMM prohibits exploitable token deposits for security at the expense of more restrictive interfaces in AMM operations. To avoid lost tokens, the AMM smart contract is extended with a BtcRelay~\cite{me:btcrelay,DBLP:conf/aft/DaveasKKZ20} such as the capability to verify the transaction requesting token returns. 
Besides, we propose mitigation schemes retrofittable to a deployed AMM instance without upgrading the smart contracts. These schemes harden the security of an off-chain infrastructure and application-layer smart contracts on top of AMMs.

\vspace{2pt}\noindent\textbf{Contributions}. Our contributions are outlined below: 

\vspace{2pt}\noindent$\bullet$\textit{ New findings}. We discover a total of $3.5$ million USD worth of stolen value by measuring and analyzing atomicity violations on three popular Uniswap V2 services on Ethereum and BSC. 
The discovered token thefts uncover the previously unknown patterns of extractable value  (e.g., token rebase, interest, airdrop, mishandled contract exception) and expose the adaptive attack strategies that occur offline and otherwise would have been hidden. We further study the criminal infrastructures and campaigns mounted to prepare, execute and finalize the theft attacks systematically.

\vspace{2pt}\noindent$\bullet$\textit{ New techniques}. We develop an end-to-end analytical pipeline to detect atomicity violations and relevant attacks from Ethereum transaction traces, including an efficient join algorithm and various heuristics to automatically discover and cross-check token theft and lost tokens. 

\noindent
{\bf Roadmap}: \S~\ref{sec:background} introduces the background of Ethereum transactions, tokens and DEX. The discovery of atomicity violations is described in \S~\ref{sec:detectriskyswap}. Detection and characterization of theft attacks are presented in \S~\ref{sec:attack}. Detection of lost tokens is in \S~\ref{sec:losttokens}. 
Countermeasures are presented in \S~\ref{sec:mitigate}. Related work is described in \S~\ref{sec:rw}. Responsible disclosure is discussed in \S~\ref{sec:disclosure} with the conclusion in \S~\ref{sec:conclude}.

\section{Background}
\label{sec:background}

Ethereum blockchain supports two types of addresses: An externally owned account (EOA), which is an Ether owner's public key, and a contract account (CA), which refers to the immutable memory address to which the smart contract is deployed on miners. An Ethereum transaction is a binding between its sender address and receiver address.

Most widely deployed tokens on Ethereum are fungible tokens in which each unit is interchangeable with and indistinguishable from any other unit. ERC20 is the most adopted standard of fungible tokens on Ethereum. ERC20 functions include \texttt{transfer} which allows a token owner to transfer her tokens to another account, \texttt{approve} which allows an owner to delegate the spending of her tokens to another delegatee account, \texttt{transferFrom} that allows a delegatee account to spend tokens on behalf of the original owner under the approved token limit, \texttt{balanceOf} that allows anyone to get an account’s token balance, etc.

An AMM or automated market maker is a dominant form of decentralized exchange (DEX) deployed on Ethereum blockchains. An AMM runs one or multiple ``pools'' in smart contracts. An AMM pool owns two tokens, say $T_0$ and $T_1$. An AMM pool minimally supports two operations: 1) token swap between a trader account and the pool smart contract, and 2) liquidity addition/removal between a provider account and the pool smart contract. The trader and liquidity provider can be either an EOA or a CA.

In a token-swap operation, the trader deposits $dx$ units of token $T_0$ to the pool's account and receives from the pool $dy$ units of token $T_1$. The AMM internally determines the token exchange rate (or value of $dy$) by enforcing the invariant on some function. For instance, Uniswap is a constant-product market maker where the invariant function is the product of the two token balance.

In an add-liquidity operation, the liquidity provider deposits $dx$ units of token $T_0$, deposits $dy$ units of token $T_1$, and withdraws a certain amount of ``base'' tokens $T_{\texttt{LP}}$. A remove-liquidity workflow is the reverse of add-liquidity, in that the liquidity provider deposits tokens $T_{\texttt{LP}}$ and withdraws tokens $T_0$ and $T_1$ at a certain ratio.


\begin{table}[!htbp] %force in current page, disable float.
\centering{\small
\begin{tabularx}{0.5\textwidth}{ |l|X|l| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
Layer & $swapT.$ workflow & $addL.$ workflow \\ \hline
Uniswap V2
& $T_0$.\texttt{transfer}() & $T_0$.\texttt{transfer}() \\ 
& pool.\texttt{swap}() & $T_1$.\texttt{transfer}() \\ 
 & & pool.\texttt{mint}() \\ 
\hline
Uniswap V3
& pool.\texttt{swap}() & pool.\texttt{mint}() \\ 
\hline
Balancer
& pool.\texttt{swapExactAmountIn}() & pool.\texttt{joinpool}() \\ 
\hline
Curve
& pool.\texttt{exchange}() & pool.\texttt{add\_liquidity}() \\ 
\hline
\end{tabularx}
}
\caption{Uniswap V2/V3's API in $swapToken$ and $addLiquidity$ represents $addLiquidity$ workflow.}
\label{tab:uniswapv2:api}
\end{table}









%------------------old version---------------------------


\ignore{Recent years witnessed the rise of Decentralized Finance (DeFi) on blockchains. A prominent class of DeFi applications is the Decentralized Exchange (DEX) which allows a trader account to swap their assets from one token to another. 
On Ethereum, deployed DEX instances including Uniswap~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer} all run AMM protocols or automated market maker, which account for more than $95\%$ of the DEX activities all time~\cite{me:etherscan:topdex}, attracting hundreds of millions of transactions today (as of July, 2022). Other than token swap, an AMM\footnote{We use the terms AMM and DEX interchangeably in this paper.} supports liquidity addition/removal in which a liquidity-provider account deposits tokens as a reserve for subsequent token swaps.

AMM can be misused. A well studied class of AMM misuses are sandwich attacks and arbitrage~\cite{DBLP:conf/sp/DaianGKLZBBJ20,DBLP:journals/corr/abs-2101-05511,DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2105-02784}. In both attacks, the attacker account extracts illicit value by sending multiple transactions in crafted order. Recent research has shown the large scale of sandwich attacks and arbitrage on Ethereum~\cite{DBLP:journals/corr/abs-2101-05511,DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2105-02784}. 
Another AMM misuse is to list scam tokens~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21} that impersonate other tokens and trick their traders. In these known misuse patterns, each attack is composed of multiple AMM operations, such as a cycle of token swaps in arbitrage~\cite{DBLP:journals/corr/abs-2105-02784} and two transactions that frontrun and backrun a victim transaction in a sandwich attack~\cite{DBLP:journals/corr/abs-2101-05511}.
%scam tokens by short-lived span of AMM operations~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21}, etc.

\begin{figure}[b!ht]
\begin{center}
\includegraphics[width=0.325\textwidth]{figures/workflow7.eps}
\end{center}
\caption{Data-analytical workflow to detect AMM operation atomicity violation, stolen tokens and theft attacks.}
\label{fig:workflow7}
\end{figure}

\vspace{2pt}\noindent\textbf{Discovering atomicity violations}. 
This work aims to discover a different class of AMM misuse: atomicity violations. Specifically, an AMM operation, be it a token swap or liquidity management, should execute a sequence of token deposits and withdrawals in an all-or-nothing manner (i.e., atomic operation execution). Violation of the operation atomicity could imply security risks and attacks. For instance, executing a token swap by a standalone withdrawal (i.e., without the matching deposit) can suggest an incident of theft in which a thief can withdraw value without sending any deposit to the AMM. For another instance, a token swap by a standalone deposit (without a matching withdrawal) could mean an adversarial AMM denying its withdrawal service to the trader having done deposit.
Note that atomicity violation is different from the known AMM misuses that manifest in multi-operation sequences and that do not entail the violation of individual operations' atomicity.

By joining and analyzing more than $60$ million transactions on Ethereum and Binance Smart Chain (BSC), to our surprise, we find atomicity violations widely exist among deployed AMM services: 
Commiting these violations are the most popular services in practice, including Uniswap V2~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer}.
In total, they execute $671,400$ AMM operations violating atomicity, exhibiting various patterns including standalone token deposit, standalone withdrawal, account mismatch, and value mismatch.

%To understand the nature of the atomicity violations, that is, whether they occur by accident or are committed intentionally, we formulate the following hypothesis: 1) The atomicity violations in which the deposited value is below the value withdrawn could indicate token thefts in which a thief account attacks by extracting value from a victim AMM or trader account. 2) The atomicity violations in which the deposited value exceeds the value withdrawn could indicate AMM denial of service in which a victim trader depositing value is declined of withdrawal service. Specifically, we focus on the lost-token risks in which the victim trader deposits tokens by mistakes.

\vspace{2pt}\noindent\textbf{Understanding atomicity violations}. 
We aim to understand the nature of the atomicity violations, whether they are accidents or intentional crimes. While different atomicity violations can be attributed to different threats (e.g., denial of service mentioned above), we mainly focus on the prominent cases of token theft in our measurement result.

Detecting theft attacks out of the atomicity violations poses challenges. This is because the ground truth often includes off-chain activities which are unobservable. For instance, in attributing a standalone withdrawal to theft, one has to know that the depositor and withdrawer accounts are controlled by two distinct physical entities, which is known to be an intractable problem with only on-chain data; the existing heuristics such as address clustering~\cite{DBLP:conf/fc/Victor20,DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:conf/sp/HuangALIBMLLSM18,DBLP:books/daglib/0040621} don't apply here (see \S~\ref{sec:discoveryproblem} for detail).

To workaround the difficulty, we focus on making sense of the accounts' on-chain behaviors and matching them to the rational attack strategies we extract from analyzing the AMM protocols. For instance, a rational thief in fear of being frontrun by competing thieves would send crafted transactions with minimal deposit-to-withdrawal delay, which can indicate an attack. For another instance, to avoid the failure of theft, a careful thief would check on-chain states extensively (e.g., token balances) before committing the theft; these pre-attack actions (e.g., calling token function \texttt{balanceOf}) can indicate an intentional theft. We propose an algorithm to match account behavior with indicators and automatically detect thefts.

Overall, our method is an end-to-end transaction-analysis pipeline, depicted in Figure~\ref{fig:workflow7}, that first discovers atomicity violations and then detects and characterizes theft attacks.

%We found in practice the exploitable deposits can be created in a variety of unexpected application scenarios, including free token giveaways (i.e., airdropping), tokens redistributing fees to privileged shareholder accounts, tokens bearing interest, tokens that can adjust or rebase total supply, buggy smart contracts, and unsafe user interface that executes a swap in two separate transactions, etc. 

\vspace{2pt}\noindent\textbf{Findings}. 
On the Ethereum mainnet and BSC fork, we discover $465$ thousand theft attacks mounted by $258$ distinct attacker accounts, inflicting a loss of more than $3.7$ million USD stolen from $978$ victim accounts.
Each attack instance we found matches at least one indicator. Interesting attacker behavior was observed in practice. For instance, real-world attackers {\it adapt} to the different patterns of exploitable deposits and exhibit different behavior: When the attacker is to extract value from interest-bearing tokens, she waits long enough, typically hundreds of Ethereum blocks, for the interest to accumulate and to become profitable. To extract deposits of other patterns, the same attacker instead wastes no time extracting the illicit value, typically within one or two blocks.

We further study attackers' and victims' behavior by tracking their money flow and actions to create/destroy smart contracts. Our study uncovers the systematic criminal activities: the crime bosses use mixer services to hide their identities while sending commissions and instructions. After the attack, the money is sent to various DeFi services to maximize illicit profit. Exploit smart contracts are widely used to improve attack success rates.

We also detect, from the standalone deposits on Uniswap V3, Curve and Balancer, the $215$\jiaqi{Done} incidents of lost tokens worth a total of $56,700$ USD. Given a standalone deposit, our method to detect whether it results in lost token is whether it relies to deposit similar amount of tokens. 

\vspace{2pt}\noindent\textbf{Mitigation}. 
%why it is hard to design secure AMM in practice?
Empirically, all deployed AMM instances including Uniswap V2/V3, Sushiswap, Pancakeswap, Balancer and Curve are vulnerable to either token  theft or DoS like lost tokens. This is not by accident: It shows a fundamental challenge to secure AMM in practice where the AMM needs to recognize various token deposit mechanisms with limited information. 

%One cause of the atomicity violations is that certain non-standard token operations unspecified in the AMM protocols (e.g., rebasing token supply and interest-bearing tokens) are mistreated as token deposit that allows subsequent token withdrawal to succeed. This manifests in standalone withdrawals. Another cause is that certain token deposits are not intended for withdrawal (e.g., airdrop and token lost-and-found), which results in standalone deposits.

To mitigate the risks, we first propose secure AMM protocols that require rewriting and redeployment of smart contracts. To mitigate token thefts, the secure AMM prohibits exploitable token deposits for security at the expense of more restrictive interfaces in AMM operations. To avoid lost token risks, the AMM smart contract is extended with a BtcRelay~\cite{me:btcrelay,DBLP:conf/aft/DaveasKKZ20} like capability to verify the transaction requesting token returns. 

Besides, we propose mitigation schemes retrofittable over a deployed AMM instance without upgrading the smart contracts. These schemes harden the security of an off-chain infrastructure and application-layer smart contracts on top of AMMs.

\vspace{2pt}\noindent\textbf{Contributions}. This paper's contributions are outlined as follows: 

\vspace{2pt}\noindent$\bullet$\textit{ New findings}. We discover a total of $3.5$ million USD worth of stolen value by measuring and analyzing atomicity violations on three popular Uniswap V2 services on Ethereum and BSC. 
The discovered token theft attacks uncover the previously unknown patterns of extractable value  (e.g., token rebase, interest, airdrop, mishandled contract exception) and expose the adaptive attack strategies that occur offline and otherwise would have been hidden. We further study the criminal infrastructures and campaigns mounted to systematically prepare, execute and finalize the theft attacks.

%We also formulate and measure the risk of lost tokens on other DEX services including Uniswap V3, Balancer and Curve. The result reveals lost tokens worth of XXX USD across more than XXX transactions on Ethereum. 

\vspace{2pt}\noindent$\bullet$\textit{ New techniques}. We develop an end-to-end analytical pipeline to detect atomicity violations and relevant attacks from Ethereum transaction traces, including an efficient join algorithm and various heuristics to automatically discover and cross-check token theft and lost tokens. 
%XXX: Also we propose mitigation schemes including a fuzzer and test oracle to automatically detect mishandled exceptions in smart contracts.

%This work leads to the findings that shed light on the current and future underground ecosystem that strategically exploits the atomicity violation to gain illicit profit.

\noindent
{\bf Roadmap}: \S~\ref{sec:background} introduces the background of Ethereum transactions, tokens and DEX. Discovery of atomicity violations is described in \S~\ref{sec:detectriskyswap}. Detection and characterization of theft attacks are presented in \S~\ref{sec:attack}. Detection of lost tokens is in \S~\ref{sec:losttokens}. 
Countermeasures are presented in \S~\ref{sec:mitigate}. Related work is described in \S~\ref{sec:rw}. Responsible disclosure is discussed in \S~\ref{sec:disclosure} with the conclusion in \S~\ref{sec:conclude}. 
}



==> text/old/v9_intro_beforeXFWang.tex <==
\section{Introduction}

Recent years have witnessed the rise of Decentralized Finance (DeFi) on blockchains. A prominent class of DeFi applications is Decentralized Exchange (DEX) that allows a trader account to swap their assets from one type of tokens to another. 
On Ethereum, deployed DEX instances including Uniswap~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer} all run AMM protocols or automated market maker, which account for more than $95\%$ of the DEX activities all time~\cite{me:etherscan:topdex}, attracting hundreds of millions of transactions today (as of July, 2022). Other than token swap, an AMM\footnote{We use the terms AMM and DEX interchangeably in this paper.} supports liquidity addition/removal in which a liquidity-provider account deposits tokens as a reserve for subsequent token swaps.

AMM can be misused. A well studied class of AMM misuses are sandwich attacks and arbitrage~\cite{DBLP:conf/sp/DaianGKLZBBJ20,DBLP:journals/corr/abs-2101-05511,DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2105-02784}. In both attacks, the attacker account extracts illicit value by sending multiple transactions in a crafted order. Recent research has shown the large scale of sandwich attacks and arbitrage on Ethereum~\cite{DBLP:journals/corr/abs-2101-05511,DBLP:conf/uss/TorresCS21,DBLP:journals/corr/abs-2105-02784}. 
Another AMM misuse is to list scam tokens~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21} that impersonate other tokens to trick their traders. In these known misuse patterns, each attack is composed of multiple AMM operations, such as a cycle of token swaps in arbitrage~\cite{DBLP:journals/corr/abs-2105-02784} and two transactions that frontrun and backrun a victim transaction in a sandwich attack~\cite{DBLP:journals/corr/abs-2101-05511}.
%scam tokens by short-lived span of AMM operations~\cite{DBLP:journals/pomacs/XiaWGSYLZXX21}, etc.

\begin{figure}[b!ht]
\begin{center}
\includegraphics[width=0.375\textwidth]{figures/workflow7.eps}
\end{center}
\caption{Data-analytical workflow to detect AMM operation atomicity violation and token theft attacks.}
\label{fig:workflow7}
\end{figure}


\vspace{2pt}\noindent\textbf{Discovering atomicity violations}. 
This work aims to study a different class of AMM misuses: atomicity violations. Specifically, an AMM operation, be it a token swap or liquidity management, should execute a sequence of token deposits and withdrawals in an all-or-nothing manner (i.e., atomic operation execution). Violation of the operation atomicity could imply the presence of security risks or even attacks. For instance, executing a token swap by a standalone withdrawal (i.e., without the matching deposit) could indicate an incident of theft in which a thief withdraws value without making any deposit to the AMM. For another instance, a token swap by a standalone deposit (without a matching withdrawal) could mean an adversarial AMM denying the withdrawal request from the trader who has made a deposit.
Note that atomicity violation is different from the known AMM misuses that manifest in multi-operation sequences and do not entail the violation of individual operations' atomicity.

By connecting together and analyzing over $60$ million transactions on Ethereum and Binance Smart Chain (BSC), to our surprise, we find that atomicity violations widely exist among deployed AMM services: 
Committing these violations are the most popular services, including Uniswap V2~\cite{me:dex:uniswap,Adams2020UniswapVC}, Sushiswap~\cite{me:sushiswap:1,me:sushiswap:2}, Pancakeswap~\cite{me:pancakeswap:1}, Curve~\cite{me:curve}, and Balancer~\cite{me:balancer}.
In total, they have performed more than $74$ thousand AMM operations violating atomicity, which exhibit various patterns including standalone token deposit, standalone withdrawal, account mismatch, and value mismatch.

%To understand the nature of the atomicity violations, that is, whether they occur by accident or are committed intentionally, we formulate the following hypothesis: 1) The atomicity violations in which the deposited value is below the value withdrawn could indicate token thefts in which a thief account attacks by extracting value from a victim AMM or trader account. 2) The atomicity violations in which the deposited value exceeds the value withdrawn could indicate AMM denial of service in which a victim trader depositing value is declined of withdrawal service. Specifically, we focus on the lost-token risks in which the victim trader deposits tokens by mistakes.

\vspace{2pt}\noindent\textbf{Understanding atomicity violations}. 
We aim to understand the nature of the atomicity violations, whether they are accidents or intentional crimes. While different atomicity violations can be attributed to different threats (e.g., denial of service mentioned above), we mainly focus on the prominent cases of token theft in our measurement result.

Detecting theft from the atomicity violations is challenging. This is because the ground truth often includes off-chain activities unaccounted for.
%which are unobservable. 
For instance, when attributing a standalone withdrawal to theft, one has to know that the party making the deposit to accounts and the party withdrawing from the accounts are controlled by two distinct physical entities, which is known to be an intractable problem with only on-chain data; known heuristics such as address clustering~\cite{DBLP:conf/fc/Victor20,DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13,DBLP:conf/sp/HuangALIBMLLSM18,DBLP:books/daglib/0040621} do not apply here (see \S~\ref{sec:discoveryproblem} for detail).

To address this challenge, we focus on making sense of the accounts' on-chain behaviors and matching them to the rational attack strategies we identify through analyzing the AMM protocols. For instance, a rational thief in fear of being frontrun by competing thieves would send crafted transactions with the minimal deposit-to-withdrawal delay, which can indicate the occurrence of an attack. For another instance, to avoid the failure of theft, a careful thief would check on-chain states extensively (e.g., token balances) before committing the theft; these pre-attack operations (e.g., calling token function \texttt{balanceOf}) could indicate an intentional theft. We propose an algorithm to capture the account behavior with such indicators and automatically detect thefts.

Overall, our method is an end-to-end transaction-analysis pipeline, depicted in Figure~\ref{fig:workflow7}, which first discovers atomicity violations and then detects and characterizes theft attacks.

%We found in practice the exploitable deposits can be created in a variety of unexpected application scenarios, including free token giveaways (i.e., airdropping), tokens redistributing fees to privileged shareholder accounts, tokens bearing interest, tokens that can adjust or rebase total supply, buggy smart contracts, and unsafe user interface that executes a swap in two separate transactions, etc. 

\vspace{2pt}\noindent\textbf{Findings}. 
On the Ethereum mainnet and BSC fork, we discover $465$ thousand theft attacks mounted by $258$ distinct attacker accounts, inflicting a loss of more than $3.7$ million USD on $978$ victim accounts.
Each attack instance we find matches at least one indicator. Interesting attacker behavior has been observed in practice. For instance, real-world attackers {\it adapt} to the different patterns of exploitable deposits and exhibit different behavior: When the attacker is to extract value from interest-bearing tokens, she waits long enough, typically hundreds of Ethereum blocks, for the interest to accumulate and to become profitable. To steal other kinds of deposits, such as XXX,
%of other patterns, 
the same attacker instead wastes no time extracting the illicit value, typically within one or two blocks.

We further study attackers' and victims' behavior by tracking their money flow and their actions to create/destroy smart contracts. Our study uncovers the systematic criminal activities: the crime bosses use mixer services to hide their identities while sending commissions and instructions. After the attack, the money is sent to various DeFi services to maximize illicit profit. Exploit smart contracts are widely used to improve attack success rates.

From the violations that are not attributed to theft, we further detect the instance of potential denial of service. Particularly, we formulate the problem of detecting lost tokens where the deposits are made by mistake, and the AMM refuses to return the tokens. We propose threat indicators by assuming the victim accounts' rational behavior after lost tokens. Our measurement result on Ethereum confirms the existence of lost tokens on Uniswap V3, CUrve and Balancer (inflicting a total value of 57,000 USD lost unfairly by these AMMes). We note that the atomicity violations could imply other threats than theft and lost tokens, and a comprehensive study is left for future research. 
%is out of the scope of this work.

\vspace{2pt}\noindent\textbf{Mitigation}. 
%why it is hard to design secure AMM in practice?
Our empirical study shows that all six popular AMM services (i.e., Uniswap V2/V3, Pancakeswap, Sushiswap, Balancer, and Curve) are vulnerable to either the threat of theft or DoS like lost tokens. This unsatisfactory state of affairs in practice is not by accident: It reveals a fundamental design challenge in securing AMM where the AMM smart contract with limited information needs to recognize token deposits of various intentions.

%One cause of the atomicity violations is that certain non-standard token operations unspecified in the AMM protocols (e.g., rebasing token supply and interest-bearing tokens) are mistreated as token deposit that allows subsequent token withdrawal to succeed. This manifests in standalone withdrawals. Another cause is that certain token deposits are not intended for withdrawal (e.g., airdrop and token lost-and-found), which results in standalone deposits.

To mitigate the risks, we have made the first attempt to design secure AMM protocols that require rewriting and redeployment of smart contracts. To mitigate token thefts, the secure AMM prohibits exploitable token deposits for security at the expense of more restrictive interfaces in AMM operations. To avoid lost tokens, the AMM smart contract is extended with a BtcRelay~\cite{me:btcrelay,DBLP:conf/aft/DaveasKKZ20} like the capability to verify the transaction requesting token returns. 
Besides, we propose mitigation schemes retrofittable to a deployed AMM instance without upgrading the smart contracts. These schemes harden the security of an off-chain infrastructure and application-layer smart contracts on top of AMMs.

\vspace{2pt}\noindent\textbf{Contributions}. This paper's contributions are outlined as follows: 

\vspace{2pt}\noindent$\bullet$\textit{ New findings}. We discover a total of $3.5$ million USD worth of stolen value by measuring and analyzing atomicity violations on three popular Uniswap V2 services on Ethereum and BSC. 
The discovered token theft attacks uncover the previously unknown patterns of extractable value  (e.g., token rebase, interest, airdrop, mishandled contract exception) and expose the adaptive attack strategies that occur offline and otherwise would have been hidden. We further study the criminal infrastructures and campaigns mounted to prepare, execute and finalize the theft attacks systematically.

\vspace{2pt}\noindent$\bullet$\textit{ New techniques}. We develop an end-to-end analytical pipeline to detect atomicity violations and relevant attacks from Ethereum transaction traces, including an efficient join algorithm and various heuristics to automatically discover and cross-check token theft and lost tokens. 

\noindent
{\bf Roadmap}: \S~\ref{sec:background} introduces the background of Ethereum transactions, tokens and DEX. The discovery of atomicity violations is described in \S~\ref{sec:detectriskyswap}. Detection and characterization of theft attacks are presented in \S~\ref{sec:attack}. Detection of lost tokens is in \S~\ref{sec:losttokens}. 
Countermeasures are presented in \S~\ref{sec:mitigate}. Related work is described in \S~\ref{sec:rw}. Responsible disclosure is discussed in \S~\ref{sec:disclosure} with the conclusion in \S~\ref{sec:conclude}. 

\section{Background}
\label{sec:background}

Ethereum blockchain supports two types of addresses: An externally owned account (EOA), which is an Ether owner's public key, and a contract account (CA), which refers to the immutable memory address to which the smart contract is deployed on miners. An Ethereum transaction is a binding between its sender address and receiver address.

Most widely deployed tokens on Ethereum are fungible tokens in which each unit is interchangeable with and indistinguishable from any other unit. ERC20 is the most adopted standard of fungible tokens on Ethereum. ERC20 functions include \texttt{transfer} which allows a token owner to transfer her tokens to another account, \texttt{approve} which allows an owner to delegate the spending of her tokens to another delegatee account, \texttt{transferFrom} that allows a delegatee account to spend tokens on behalf of the original owner under the approved token limit, \texttt{balanceOf} that allows anyone to get an account’s token balance, etc.

An AMM or automated market maker is a dominant form of decentralized exchange (DEX) deployed on Ethereum blockchains. An AMM runs one or multiple ``pools'' in smart contracts. An AMM pool owns two tokens, say $T_0$ and $T_1$. An AMM pool minimally supports two operations: 1) token swap between a trader account and the pool smart contract, and 2) liquidity addition/removal between a provider account and the pool smart contract. The trader and liquidity provider can be either an EOA or a CA.

In a token-swap operation, the trader deposits $dx$ units of token $T_0$ to the pool's account and receives from the pool $dy$ units of token $T_1$. The AMM internally determines the token exchange rate (or value of $dy$) by enforcing the invariant on some function. For instance, Uniswap is a constant-product market maker where the invariant function is the product of the two token balance.

In an add-liquidity operation, the liquidity provider deposits $dx$ units of token $T_0$, deposits $dy$ units of token $T_1$, and withdraws a certain amount of ``base'' tokens $T_{\texttt{LP}}$. A remove-liquidity workflow is the reverse of add-liquidity, in that the liquidity provider deposits tokens $T_{\texttt{LP}}$ and withdraws tokens $T_0$ and $T_1$ at a certain ratio.

\ignore{
\begin{table}[!htbp] %force in current page, disable float.
\centering{\scriptsize
\begin{tabularx}{0.5\textwidth}{ |l|X|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
Layer & $swapT.$ workflow & $addL.$ workflow \\ \hline
Uniswap V2~\cite{me:uniswapv2:pool}
& $T_0$.\texttt{transfer}(trader,amountOut) & $T_0$.\texttt{transfer}(trader,amountOut) \\ 
& pool.\texttt{swap}(amountOut, to\_addr) & $T_1$.\texttt{transfer}(trader,amountOut) \\ 
 & & pool.\texttt{mint}(to\_addr) \\ 
\hline
Uniswap V3
& pool.\texttt{swap}(...) & pool.\texttt{mint}(...) \\ 
\hline
Balancer
& pool.\texttt{swapExactAmountIn}(...) & pool.\texttt{joinpool}(...) \\ 
\hline
Curve
& pool.\texttt{exchange}(...) & pool.\texttt{add_liquidity}(...) \\ 
\hline
\end{tabularx}
}
\caption{Uniswap V2/V3's API in $swapToken$ and $addLiquidity$ represents $addLiquidity$ workflow.}
\label{tab:uniswapv2:api}
\end{table}
}

\begin{table}[!htbp] %force in current page, disable float.
\centering{\footnotesize
\begin{tabularx}{0.5\textwidth}{ |l|X|l| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
Layer & $swapT.$ workflow & $addL.$ workflow \\ \hline
Uniswap V2
& $T_0$.\texttt{transfer}() & $T_0$.\texttt{transfer}() \\ 
& pool.\texttt{swap}() & $T_1$.\texttt{transfer}() \\ 
 & & pool.\texttt{mint}() \\ 
\hline
Uniswap V3
& pool.\texttt{swap}() & pool.\texttt{mint}() \\ 
\hline
Balancer
& pool.\texttt{swapExactAmountIn}() & pool.\texttt{joinpool}() \\ 
\hline
Curve
& pool.\texttt{exchange}() & pool.\texttt{add\_liquidity}() \\ 
\hline
\end{tabularx}
}
\caption{Uniswap V2/V3's API in $swapToken$ and $addLiquidity$ represents $addLiquidity$ workflow.}
\label{tab:uniswapv2:api}
\end{table}




==> text/paper3.tex <==
\section{Discovering Atomicity Violations}
\label{sec:detectviolatingswap}
\label{sec:mmalgo}

\noindent
{\bf Input data}:
Our input data is raw blockchain transactions, including function calls and log events by smart contracts. We obtain the transaction data by crawling Ethereum exploration services including \url{Etherscan.io}~\cite{me:etherscan}, \url{BSCscan.io}~\cite{me:bscscan} and relevant BigQuery datasets~\cite{me:bigquery:ethereumdataset}. 
We only use the event log emitted from the AMM pool smart contract (which we assume is trusted), such as Uniswap V2's pool.
From the raw input data, we attribute the \texttt{transfer}/\texttt{transferFrom} calls to token deposits and withdrawals as described. Besides, we collect the invocations to relevant functions, such as \texttt{swap} in Uniswap V3 in Table~\ref{tab:uniswapv2:api}; from there, we can filter out the deposits and withdrawals that are mapped to atomic operations. 
We also use the pool's events to reconstruct the mapping between deposit value and withdrawal value in the withdrawal record.

\noindent
{\bf Design challenge}:
A naive way of finding atomicity violations is to filter out atomic operations by extensively joining token deposits with withdrawals. Because an atomic AMM operation can contain an arbitrary number of deposits and withdrawals, the naive join needs to be built on the {\it powerset} of token deposits and withdrawals, which is extremely expensive and unscalable (Note that the powerset of $n$ deposits/withdrawals is of $2^n$ elements).
To avoid inefficiency, our observation is that due to Ethereum's single-threaded execution model, a token deposit can be matched only to a subsequent withdrawal before the next deposit occurs. This property allows to join token deposits and withdrawals based on their timings and makes it possible for linear-time search.

\noindent
{\bf The algorithm} takes as input a list of function calls representing token deposits and withdrawals. In the first round, the algorithm equi-joins the function-call records by their transaction IDs. If the deposits and withdrawals in the same transaction also match in value, it emits them as an atomic operation before removing them from the list. If the value does not match, the algorithm merges the intra-transaction deposits and withdrawals into one virtual record (e.g., a deposit of value equal to the originally deposited value deducted by the withdrawn value).

In the second round, the algorithm joins deposits and withdrawals across transactions. It linearly scans the list of deposits and withdrawals sorted by time: For two consecutive deposits, say $d1$ and $d2$, it finds any subset of all withdrawals between $d1$ and $d2$ that matches $d1$ in value. For each match, the algorithm removes the deposit and withdrawals from the list before emitting an atomic operation. The algorithm then reverses the process; that is, for two consecutive withdrawals, it finds a set of deposits between the two withdrawals that match the earlier withdrawal in value.

In the third round, the algorithm linearly scans the remaining list and emits the token deposits and withdrawals as either value mismatch or standalone operations. The pseudocode is in Appendix~\ref{sec:algorithm:detect}.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.29\textwidth]{figures/join_problem2.eps}
\caption{Matchmaking deposits and withdrawals: Matched cases are in green boxes, and mismatches are rendered in red, including standalone withdrawal (I), standalone deposits (II), and deposits of lower value (IV). In the figure, \texttt{tf}/\texttt{tff} refer to functions \texttt{transfer}/\texttt{transferFrom}.}
\vspace{-0.1in}
\label{fig:joinproblem}
\end{figure}

\noindent
{\bf Example}: We show an example of running the atomicity violation discovery algorithm in Uniswap V2. Uniswap V2 supports token deposits by both \texttt{transfer} and \texttt{transferFrom}. It also supports token withdrawals by \texttt{swap} (in $swapToken$) and by \texttt{mint} (in $addLiquidity$). We collect the corresponding function-call records for token deposits and withdrawals. Figure~\ref{fig:joinproblem} shows the collected deposits and withdrawals, ordered by time. 
In the first round, the algorithm identifies and filters out atomic operations by linking deposits and withdrawals through transaction ID, which is \texttt{tff1}-\texttt{swap1}. In the second round, it then matches token deposits and withdrawals by timing. For instance, \texttt{tf2} and \texttt{tf3} are matched to \texttt{mint1} by value, which leads to an atomic $addLiquidity$ operation. In the last round, the algorithm emits the mismatches in the remaining list. Specifically, \texttt{tf4} is mapped to \texttt{swap3}, but their value does not match, thus producing a case of Violation IV. Then there are two standalone operations left in the list, that is, \texttt{tf1} (Violation II) and \texttt{swap2} (I).

%{\it An example}: Figure~\ref{fig:joinproblem} shows how token deposits to a Uniswap pool are matched to token withdrawals from the same pool. The data records storing deposits/withdrawals are aligned and sorted by time. The figure shows two matched cases (i.e., two green boxes). Three mismatch cases are discovered: On the timeline, the first \textsc{transfer} is a standalone deposit (i.e., II). The second \textsc{swap} is a standalone token withdrawal (I). In the red box is a pair of deposits and withdrawals whose value does not match (i.e., IV).

\begin{table}[!htbp] %force in current page, disable float.
\caption{Discovered atomicity violations on top DEXes: value is presented in the unit of million USD, and the number of transactions violating atomicity (i.e., \#tx) is presented in the unit of a thousand.}
\label{tab:swapsviolating}\centering{\scriptsize
\begin{tabularx}{0.5\textwidth}{ lXlllllX } %X is stretching to \textwidth, while c is to match with text width in cell.
\hline
 & Atomic ($10^6$) & I & II & III & IV & V & \#tx ($10^3$) \\ \hline
Uniswap-V2 & $618$ & {\color{red} \bf $1.26$} & $.36$ & {\bf$.49$} & $.09$ & {\color{red} \bf $3.64$} & $212$ \\ \hline
Sushiswap & $.17$ & {$\approx{}0$} & {$.03$} & {\bf$.06$} & $\approx{}0$ & $10^{-3}$ & $.33$ \\ \hline
Pancakeswap & $73$ & {$.53$} & $.12$ & {\bf$.05$} & $.99$ & $0.15$ & $452$ \\ \hline
Uniswap-V3 & $.053$ & $0$ & {$.17$} & $0$ & $0$ & $0.04$ & $.17$\\  \hline
Balancer
& $.013$ & $0$ & {$.74$} & $0$ & $0$ & $0$ & $6.9$ \\ \hline
Curve
& $.13$ & $0$ & $\approx{}0$ & $0$ & $0$ & $0$ & $\approx{}0$\\ \hline 
\end{tabularx}
}
\end{table}

\noindent
{\bf Results}: We conduct the measurement and transaction analysis on all six DEX services.
In particular, we set the minimal $Z\%$ value difference to determine match/mismatch. If a deposit (withdrawal) has $Z\%$ higher value than the paired withdrawal (deposit), it is considered a mismatched case (IV/V). A rule of thumb is to set $Z\%=10\%$ on our dataset, which helps remove the negative cases, such as fees charged by tokens and router smart contracts.
For each DEX, we report the number of swaps and their total value under each category. 
To estimate the value in a violating operation $tx$, we use the exchange rate between the token $T$ and one of the three USD-pegged stablecoins (i.e., $USDT$, $USDC$, and $DAI$). Specifically, we find from the three Uniswap-V2 pools (i.e., $T$-$USDC$, $T$-$USDT$, and $T$-$DAI$) the swap transaction say $tx'$ that occurs at the nearest time to $tx$. We use the exchange rate in $tx'$ to estimate the value of token $T$ in transaction $tx$.
 
The results are in Table~\ref{tab:swapsviolating}, in which the majority of swaps, about $97.9\%$, are atomic. Among the rest that violates atomicity, there are two significant sources (in red): Violation I and V in Uniswap V2. For instance, cases violating I in Uniswap V2 are worth $1.2$ million USD. And cases violating V in Uniswap V2 are worth $3.64$ million USD. 

To explain these violations, we manually inspect the transactions. Cases violating V are caused by the high fees charged by token smart contracts (note that the pool smart contracts are provided by the AMM and their fees are normally standard). Existing research~\cite{DBLP:conf/ccs/0002ZLLWCXZ19} characterizes ERC20 tokens' fees and adversarial behavior in hiding the high fees from customers.

Cases violating I, that is, standalone withdrawals, are caused by non-standard token deposits. Specifically, when we collect transactions, we only consider the ``standard'' token deposits explicitly supported by the Uniswap V2 protocol. However, in practice, various non-standard token operations that update balance (e.g., supply rebase and token interest, as will be discussed in \S~\ref{sec:profitabledeposits}) are mistreated by the Uniswap V2 as a token deposit. Token withdrawals that occur after non-standard deposits can execute successfully. These withdrawals manifest as standalone withdrawals (i.e., Violation I).

{%\color{blue}
%\section{Analysis of Atomicity Violations}
%\label{sec:understanding}
%\label{sec:causeanalysis}

\subsection{Patterns of Violations}
\label{sec:profitabledeposits}

We describe some profitable deposits found in our measurement result. We use Uniswap V2 as an example to show why such deposits are profitable and can be stolen in theft.

\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.475\textwidth]{figures/victimpatterns.eps}
\end{center}
\caption{Patterns of profitable deposits: $R$ is the router smart contract (part of the pool), $T_0$/$T_1$ are the two tokens in the target liquidity pool. Both $P_1$ and $P_2$ are non-standard mechanisms that update token balance. $W$/$D$ refer to withdrawal/deposit (directly via calling \texttt{transfer}).}
\vspace{-0.2in}
\label{fig:patterns}
\end{figure}

\subsubsection{Token Supply Rebase (Pattern $P_1$)}
\label{sec:cases:rebase}

In many real-world tokens, the account balance can be changed by non-standard operations beyond token transfer. We describe an example of {\it token rebase}. Token balance can be elastically adjusted by token issuers for purposes such as stabilizing the token's exchange rates against other tokens. In practice, token rebase is such a non-standard balance-changing function, supported in some widely used tokens, such as AMPL~\cite{me:ampl:token}. When a token, say $T_0$, is rebased, a Uniswap's relevant pool, say for tokens $T_0$ and $T_1$, could have its $T_0$ balance increased. Uniswap falsely assumes that this balance increase is due to some accounts that swap token $T_0$ for token $T_1$. Uniswap's pool would mistakenly admit anyone who requests to withdraw token $T_1$ after the rebase of $T_0$.

\ignore{
{\it Token shareholder}: 
As another example, there are tokens that charge ``tax'' to average owner accounts and redistribute the ``tax'' income among privileged accounts of shareholders. Specifically, these tokens support two kinds of owners, average owner, and token shareholders. When there is a transfer, the token smart contract charges a certain amount of fees. The fees are redistributed to the privileged accounts of token shareholders. Thus, a transfer between average accounts would update the balance of all shareholders' accounts. In a Uniswap's pool of token types $T_0$ and $T_1$, if the pool's account in $T_0$ is a shareholder, any transfers in $T_0$ would increase the pool's balance and create a profitable opportunity.
 
Furthermore, even when the pool receives a token deposit, the deposit may not be intended as a part of the swap. For instance, airdrop is a common practice to promote the use of a new token type, in which token issuers periodically give away newly minted tokens to the current token owners (e.g., in Tokens MILK2~\cite{me:token:milk2} and 3Cs~\cite{me:token:3cs}). When a token, say $T_0$, is airdropped into a Uniswap's pool, the pool holding tokens $T_0$ and $T_1$ would mistakenly treat the transfer as a part of swap from token $T_0$ to $T_1$. Thus, the pool would admit anyone's request to withdraw token $T_1$ after airdrop of token $T_0$ to the pool's account.
}

In general, these non-standard token operations allow for updating the pool's balance but do not intend to withdraw the same value from the pool. We name the pattern $P_1$.

\subsubsection{Interest-bearing Tokens ($P_2$)}
Beyond $P_1$, there are implicit approaches to updating the balance. Many tokens are bearing interest. That is, the balance in the token smart contract increases at a certain rate as time goes by. Suppose a Uniswap pool is of token $T_0$ and $T_1$ where $T_0$ is interest bearing. Similar to $P_1$, the Uniswap pool observing the increase of token $T_0$ would admit the withdrawal of token $T_1$ by anyone who requests it, including a value-extracting attacker. We call this attacker's pattern by $P_2$, which is different from $P_1$. In $P_2$, the attacker simply waits long enough to harvest the extractable value from token interest. 

\subsubsection{External Transfer for Deposit ($P_3$)}

In Uniswap, a trader can externally call token $ T_0$'s transfer function to make a deposit so that she can withdraw token $T_1$ in a separate transaction. We call the pattern of a victim trader sending a transaction to externally transfer token $T_0$ by $P_3$. When $P_3$ occurs, a malicious account can send the withdrawal transaction ahead of the victim's one to claim the value in the pool. This attack is possible because a Uniswap pool receiving a deposit of $T_0$ will approve the next withdrawal of token $T_1$, no matter who sends it. 

\subsubsection{Buggy Router Contracts ($P_4$)}

In the above three patterns, the victim may externally call token $ T_0$'s functions. In the fourth pattern $P_4$, the trader delegates the handling of the swap to a router smart contract that is buggy and violates atomicity. After the trader EOA's transaction, the router smart contract successfully completes the deposit of Token $T_0$ but fails at requesting the withdrawal of Token $T_1$. Thus, anyone who requests the token withdrawal in the next transaction, including an attacker EOA, would succeed in extracting the value illicitly. 
}

\section{Detecting Token Thefts}
\label{sec:attack}

\subsection{The Detection Problem}
\label{sec:discoveryproblem}

\noindent{\bf Theft detection}: 
Our risk analysis (will be presented in \S~\ref{sec:riskanalysis}) shows the pool design flaws (i.e., vulnerability) that enable extractable value, that is, the value {\it can} be extracted by anyone on the Internet. However, whether the value is {\it actually} extracted by real-world attackers, or equivalently, whether the violation operations are actual attack instances, is a different problem. 
The detected atomicity violations, especially I, III, and IV, could present the candidate cases for extracted value, but not (yet) the confirmed cases.

Consider as an example that a token issuer sends a vulnerable rebase transaction to a pool's token, followed by a withdrawal transaction sent by account $A$ (i.e., $P_1$). $A$ may or may not be the token issuer. The former case is not an attack, as the token issuer, aware of the risky rebase, sends the withdrawal to remedy the risk. The latter case may be an attack. In other situations, including $P_3$ and $P_4$, an atomicity violation can also be attributed differently.
\ignore{
For instance, in $P_1$, after a token issuer sends an exploitable rebase transaction, it is equally likely one of the following cases occur: 1) the token issuer, aware of rebase being exploitable, quickly sends a swap request herself to claim the value in the Uniswap pool. 2) An attacker observing the occurrence of rebase operation calls the liquidity pool to withdraw the value there. The former case is not an attack, while the latter one is. In other cases, the same applies: In $P_3$, if the trader sends another transaction to withdraw the value in token $T_1$ right after the transaction of depositing $T_0$, it is a benign case. But if it is an attacker account that withdraws after the external deposit, it constitutes an attack. In $P_4$, if the trader observes the router exception and immediately send a ``make-up'' transaction to claim the value herself, it is a benign case. But if it is a third-party ill-intended account that sends the withdrawal transaction, it constitutes an attack.
}

Distinguishing attacks from benign cases entails checking two essential conditions: {\bf 1) Whether two accounts are controlled by two distinct physical users}: It cannot be an attack if the trader account who makes the profitable deposit in token $T_0$ is controlled by the same physical user with the account who succeed in withdrawing the value in token $T_1$. 
Thus, attack detection becomes the problem of linking two blockchain accounts of the same physical user, which is known to be an intractable problem if the only information known is on-chain data.
{\bf 2) What's a transaction sender's intention}: That is, whether a withdrawal transaction is intended as an attack. Even when the withdrawer and depositor accounts are not the same physical user, they can be friends in  real life, which makes the swap non-attack. Thus, it entails detecting the depositor account's intention in sending the withdrawal request, which, however, can be hidden opaque and pose challenges to detection.

\noindent
{\bf Feasibility of existing approaches}: 
On checking Condition 1), there are existing works that tackle the recovery of account linkage by heuristics specific to Bitcoin's UTXO model~\cite{DBLP:conf/socialcom/ReidH11,DBLP:conf/imc/MeiklejohnPJLMVS13}. The only work for Ethereum~\cite{DBLP:conf/fc/Victor20} presents a linkage heuristic exploiting some DEXes deposit addresses. Specifically, on order book-based DEXes (i.e., IDEX and EtherDelta), trader Alice swapping token $T_0$ for $T_1$ can specify the so-called deposit address who receives $T_1$. Assuming a swap is normal, the sharing of deposit addresses by two traders implies that the two traders are controlled by the same physical user. This work is different from our attack detection problem, where the deposit address heuristic is to detect the case that two accounts are linked, while our problem is to detect if two accounts are unlinked. More importantly, the deposit address heuristic works only under the assumption of normal swaps, while our work deals with atomicity violations. Given an atomicity-violating swap, the deposit address of a swap refers to the attacker. Thus, when an attacker targets two victim traders, it could appear that two traders share the same deposit address. In this attack, the two victim traders do not have to be linked to the same off-chain user.

On checking Condition 2), there are existing works on threat intelligence on blockchains by characterizing attackers' behavior~\cite{DBLP:conf/uss/SuSDL0XL21}. However, their targets are program-level attacks such as reentrancy attacks, and their attack strategies don't apply to the DEX context of this work.

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.4\textwidth]{figures/indicators.eps}
\end{center}
\caption{Rational attack strategies (A1/A2/A3).}
\label{fig:indicators}
\end{figure}

\subsection{The Detection Method}

\noindent{\bf Detection design rationale}: We approach the theft detection problem and tackle the challenges above from three angles: 1) We propose various heuristics to model what a rational attacker account would do (i.e., $I_1,I_2,\dots,I_5$ as will be described). We then match the observable account behavior on-chain to the heuristics. For instance, a heuristic models aggressive accounts who eagerly send withdrawal upon observing an extractable deposit. 

However, given an extractable deposited value, an eager deposit could indicate, besides a malicious thief, a benign user (e.g., a pool safeguard) using an automated process to protect the depositor user's value. To distinguish the two possible cases, 2) we propose to study if there are frontrunning behavior, that is, multiple users sending transactions to withdraw the same value created by an extractable deposit. The idea is that {\it the frontrunning or the competition among multiple users indicates a conflict of interest among the users and that at least one user is ill-intended.} Otherwise, a single safeguard does not have the incentive to send multiple withdrawal transactions to frontrun itself. 

Furthermore, given the identified accounts, 3) we collect their tagged labels by searching forums and social networks on the Internet. The idea is that if an account is reported malicious, the withdrawal transaction from the account is more likely to be an attacker.

Our overall detection method is to cross-check the three independent detection metrics on a candidate instance. We report positive instances if two detection metrics agree with each other.

\noindent{\bf
Method 1: Heuristics-based indicators}: Observing an extractable value created by a deposit, a rational thief would eagerly send the withdrawal transaction that is included in a block as close to the deposit transaction as possible. Based on the heuristic, we propose three indicators $I_1,I_2,I_{12}$ listed below. We defer the description of proposed theft-detection algorithm and additional indicators to Appendix~\ref{appd:extraindicators}.

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator $I_1$: An account whose withdrawal transactions occur consistently within $X_1$ blocks after profitable deposits (i.e., block gap smaller than $X_1$) and whose victim deposits are not caused by token interests (i.e., not $P_2$) is likely to be an attacker. Formally, 
$$
I_1\leq{}X_1
$$
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator $I_2$:
An account whose withdrawal transactions occur consistently more than $X_2$ blocks after profitable deposits (i.e., block gap larger than $X_2$) and whose victim deposits are based on token interests is likely to be an attacker. Formally, 
$$
I_2\geq{}X_2
$$
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator $I_{12}$:
An account whose ratio between indicator $I_2$ and $I_1$ is larger than $X_{12}$ is likely an attacker. 
Intuitively, it shows the attacker's intentional adaptive strategies in exploiting deposits of different patterns.
Formally,
$$
\frac{I_2}{I_1}\geq{}X_{12}
$$
}}\end{center}

{%\color{blue}
An account who always checks the difference between token reserve in the pool smart contract and token balance in the token smart contract before token withdrawal from a pool is likely a general-purpose attacker.  
The idea is that if there is a difference between the return value from a pool's \texttt{getReserves()} function and that from token's \texttt{balanceOf()} function, it indicates the pool has extractable value. And an account's behavior to check the difference shows its intention to extract the value. 
%Note that the indicator is not necessary (i.e., causing false negatives), as a general-purpose attacker can issue RPC queries to read reserves and balances, leaving no trace on-chain.
We thus propose the following attack indicator.

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator $I_4$: The attack signature is a sequence of two function calls 

Suppose $I_4\%$ of all the token withdrawals from an account are preceded by checking the difference between token reserve and balance, that is, calling functions \texttt{pool.getReserves()} and \texttt{erc20token.balanceOf()}. The account is an attacker, if the following condition is met.

$$I_4\geq{}X_4$$
}}\end{center}

Note that this indicator does not require the smart contract to actually withdraw the token $T_1$. 
}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator $I_5$: An account whose withdrawal transactions exclude any token deposit is likely to be an attacker.
%An account whose withdrawal transactions also include token deposits is likely to be a scavenger trader, even though the withdrawal is of higher value than the deposit.
}}\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator $I_6$:
Standalone withdrawal that extract value from deposit patterns $P_1$ and $P_2$ indicate an attacker, because the value in $P_1$ and $P_2$ is intended for AMM pools, not for external accounts. This intuition is materialized into the formula below:
$$
\frac{|P_1|+|P_2|}{\sum_{i}{|P_i|}}\geq{}X_6
$$
}}\end{center}

\noindent{\bf Method 2. Finding frontrunning}: Given each withdrawal involved in a violation, say $w$, we also detect if there are frontrunning withdrawals. We do so by scanning all blocks after the victim deposit and before the $10$th block after the withdrawal. Among these transactions and their internal calls, we find the ones that call the same pool account with $w$. We consider both successful and failed withdrawals. We report if a withdrawal violating atomicity frontruns or is frontrun by at least one other withdrawal as indicator $I_8$.

\begin{center}\fbox{\parbox{0.90\linewidth}{
  Indicator $I_8$:
  An account who has one or more competitors is likely to be an attacker.
  }}\end{center}

\noindent{\bf
Method 3: External incident reports}:
We search the Internet sites, including Google, Twitter, and Reddit. Our searches include the candidate attacker accounts in Table~\ref{tab:attackerview} and keywords such as ``attack, vulnerable, scam, frontrunning, bot, arbitrager, MEV, bots.'' Besides, we check the candidate account's tags on Etherscan and if they are security sensitive.
Out of the $142$ suspected accounts from our results (described next in \S~\ref{sec:theftinstances}), we found $9$ accounts are complained about on the Internet, and $2$ accounts are tagged as MEV bots on Etherscan. 
The ground-truth accounts are presented in Table~\ref{tab:attackerview}, and the full detail of ground truth data collection is in Appendix~\ref{sec:groundtruth}.

{%\color{blue}
\begin{eqnarray}
\nonumber
&& I_1 \leq 2 (= X_1) \\ 
\nonumber
& \lor & I_2 \geq 617 (=X_2) \\
\nonumber
& \lor & {I_2}/{I_1} \geq 19.28 (=X_{12})\\
\nonumber
& \lor & I_4 \geq 97.5\% (= X_4)\\
%\nonumber
& \lor & \frac{\|P_1\|+\|P_2\|}{\sum_i{\|P_i\|}}\geq{}69.2\% (=X_6)
\label{eqn:parameters}
\end{eqnarray}
}

\ignore{
\begin{table}[!htbp] %force in current page, disable float.
\caption{Detection parameters extracted from the ground-truth data}
\label{tab:parameters}\centering{
\begin{tabularx}{0.4\textwidth}{ Xlllll }
  \hline
  Parameters & $X_1$ & $X_2$ & $X_{12}$ & $X_4$ & $X_6$ \\ \hline
  Value & $2$ & $617$ & $19.28$ & $97.5\%$ & $69.2\%$ \\ \hline
\end{tabularx}
}
\end{table}
}

{\color{blue}\tangSide{Resp. Q4}
\noindent{\it Cross-validation}: We cross-validate the results detected under different methods. Specifically, in Method 3, we found $15$ accounts in online user complaints. We use the $15$ accounts as the ground truth to train the parameters in Method 1, namely $X_1,X_2\dots,X_6$. We obtain the trained Method 1 as in Equation~\ref{eqn:parameters}. 

\begin{table}[!htbp] %force in current page, disable float.
\caption{Cross-validate results via different methods}
\label{tab:extractable_value_2}
\centering{
\begin{tabularx}{0.375\textwidth}{ |l|l|l|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
\hline
Method 1 & Method 2 & Method 3 & {\color{purple} \# attacker accounts} \\ \hline
* & * & * & 142 \\ \hline
\cmark & * & * & 139 \\ \hline
* & \cmark & * & 22 \\ \hline
* & * & \cmark & 15 \\ \hline
\cmark & \cmark & * & 22 \\ \hline
%* & \cmark & \cmark & 3 \\ \hline
%\cmark & * & \cmark & 15 \\ \hline
%\cmark & \cmark & \cmark & 3 \\ \hline
\end{tabularx}
}
\end{table}

We then apply the three methods separately on the $142$ candidate accounts we detected earlier. Out of $142$ candidate accounts, $139$ accounts are detected positive under Method 1 with trained parameters. $22$ accounts are detected positive under Method 2. And $15$ accounts are found using Method 3, as shown in Table~\ref{tab:extractable_value_2}. {\color{purple}In summary, suppose we use the dataset of Method 3 as a ground truth and the dataset detected by matching Method 1 {\it or} Method 2. The false negative rate is $0\%$, and the false positive rate is unknown.}


%For instance, account $0x0c08545df4939ef46c1364b5930e840739667467$'s $I_1$ meets the condition ($I_1\leq{}X_1=2$) and account $0xEA674fdDe714fd979de3EdF0F56AA9716B898ec8$ meets the condition that $\frac{I_2}{I_1}=686/0.5=1372>X_{12}=19.28$.


}


\begin{table*}[h]
  \caption{Detected theft instances by accounts: Ground truth and test data. Bold are strong cases suggesting the account is an attacker. Victims include normal accounts and token issuers.}
\label{tab:attackerview}
  \centering{\scriptsize
  \begin{tabular}{p{6.5cm}p{0.6cm}p{1.9cm}p{0.4cm}p{0.4cm}p{0.4cm}p{1.4cm}p{0.2cm}p{0.5cm}p{0.3cm}}
  \hline
  Accounts & Value & {Deposit} & \multicolumn{7}{c}{Attack indicators} \\
  (Potential attacker) & $10^3$ \$ & patterns &$I_1$ & $I_2$ &$I_{12}$ & $I_4$ & $I_5$ &$I_6$&$I_8$\\ \hline
 %\rowcolor{LightCyan!90}
  \rowcolor{aliceblue!15}
  \multicolumn{10}{l}{\it Ground truth data} \\
  \hline
  $0x9799b475dec92bd99bbdd943013325c36157f383$ & 556 & 33$P_1$,4$P_2$,6$P_4$    &422       &371        &0.88  & 0                  &\xmark      &86\% &{\bf \cmark}\\
  \hline
  $0x0c08545df4939ef46c1364b5930e840739667467$ & 101 & 3$P_1$,1$P_4$            &{\bf 1.5} &           &0     & 0                  &\xmark      &75\% &\xmark\\
  \hline
  $0x56178a0d5f301baf6cf3e1cd53d9863437345bf9$ & 101 & 53$P_1$,4$P_2$,2$P_3$,2$P_4$ &13    & 1574      &{\bf121}   & 0                  &\xmark      &93\% &{\bf \cmark}\\
  \hline
  $0x0000000000007f150bd6f54c40a34d7c3d5e9f56$ & 11 & 15$P_2$                   &          &96         &$\infty$& 15 ({\bf 100\%}) &\xmark      &100\% &\xmark\\
  \hline
  $0x7c651d7084b4ba899391d2d4d5d3d47fff823351$ & 1.8 & 2$P_1$                   &68        &           &0     & 0                  &\xmark      &100\% &\xmark\\
  \hline
  $0x00000000e84f2bbdfb129ed6e495c7f879f3e634$ & 0.5 & 9$P_1$,4$P_3$            &{\bf 1.1} &           &0     & 0                  &{\bf \cmark}&69\% &\xmark\\
  \hline
  $0xca850b6833ef86ef0484c6be74b06d61b39df031$ & 0.5 & 40$P_3$                  &{\bf 1.4} &           &0     & 39 ({\bf 98\%})    &\xmark      &0\% &{\bf \cmark}\\
  \hline
  $0x17e8ca1b4798b97602895f63206afcd1fc90ca5f$ & 0 & 1$P_1$                     &3061      &           &0     & 0                  &{\bf \cmark}&100\% &\xmark\\
  \hline
  $0xf90e98f3d8dce44632e5020abf2e122e0f99dfab$ & 0 & 1$P_1$                     &1402      &           &0     & 0                  &\xmark      &100\% &\xmark\\
  \hline
  $0x42d0ba0223700dea8bca7983cc4bf0e000dee772$ & 0.5 & 1$P_3$                   &{\bf 0}   &           &0     & 1  ({\bf 100\%})   &{\bf \cmark}&0\% &\xmark\\
  \hline
  $0xEA674fdDe714fd979de3EdF0F56AA9716B898ec8$ & 0.2 & 2$P_1$,5$P_2$            &{\bf 0.5} &686        &{\bf1372}& 6 ({\bf 86\%})   &{\bf \cmark}&100\% &\xmark\\
  \hline
  $0x000000000025d4386f7fb58984cbe110aee3a4c4$ & 0.2 & 1$P_1$                   &38        &           &0     & 1  ({\bf 100\%})   &\xmark      &100\% &\xmark\\
  \hline
  $0xD224cA0c819e8E97ba0136B3b95ceFf503B79f53$ & 0.1 & 3$P_2$,1$P_3$            &32        &617  &19    & 4  ({\bf 100\%})   &\xmark      &75\% &\xmark\\
  \hline
  $0xb8aaed2e3117fa589eb05b0d7d0c8469d9e41ec5$ & 0.1 & 1097$P_1$                &351       &           &0     & 0                  &\xmark      &100\% &\xmark\\
  \hline
  $0x829BD824B016326A401d083B33D092293333A830$ & 0.1 & 5$P_2$                   &          &696  &$\infty$ & 5  ({\bf 100\%})   &\xmark      &100\% &\xmark\\
  \hline
  %\rowcolor{LightCyan!90}
  \rowcolor{gray!15}
  \multicolumn{10}{l}{\it Test data} \\
  \hline
  $0x2a2e25ad00faac024f6a8d8cdc0fc698fbda71b7$ & 239 & $32P_1$                  &{\bf 0.03}&           &0     & 32 ({\bf 100\%})   &{\bf \cmark}&100\% &\xmark\\
  \hline
  $0xdb40ea5b6d0ef9e45c00c194345b44765a53dd19$ & 113 & $12P_1,2P_2,3P_3$        &{\bf 2.5} &665  &{\bf266}   & 17 ({\bf 100\%})   &{\bf \cmark}&82\%&{\bf \cmark}\\
  \hline
  $0xb6bf45f59b94d31af2b51a5547ef17ff81672743$ & 20 & $1091P_1,131P_2,9P_4$     &224       &600  &2.7   & 1231 ({\bf 100\%}) &{\bf \cmark}&99\%&{\bf \cmark} \\
  \hline
  $0xc762e15cfbf392f4346ee7e8466ca595e571382b$ & 16 & $64P_1,6P_2,13P_4$        &{\bf 3.0} & 5.3       &1.8   & 83 ({\bf 100\%})   &{\bf \cmark}&84\%&{\bf \cmark} \\
  \hline
  $0xa32d3f8a970ab3222ffa1c89cb910abf7b7201d0$ & 6 & $208P_2$                   &          &942 &$\infty$ & 208 ({\bf 100\%})  &{\bf \cmark}&100\%&\xmark \\
  \hline
\ignore{
}
\end{tabular}%
}
\end{table*}
  
\subsection{Results}

\subsubsection{Case Studies}
\label{sec:theftinstances}

We present one case study on two frontrunning withdrawals and two other cases on attacker accounts aggregating multiple withdrawals. The top accounts involved in atomicity violations are characterized in Table~\ref{tab:attackerview}. The metrics include value stolen, causes, attacker indicators, the number of pools attacked, the number of victim accounts, and the label whether the account is an attacker. 

\begin{figure*}[!bhtp]
 \centering
 \includegraphics[width=0.8\textwidth]{figures/casestudy.eps} 
\vspace{-0.1in}
 \caption{Case study: A found case of atomicity violation I shows frontrunning transactions ($tx_2$ and $tx_3$) to withdraw value from a Uniswap V2 pool created by token-rebase transaction $tx_1$. Transaction $tx_2$ with red cross mark is reverted.}
 \label{fig:casestudy}
\end{figure*}

\noindent{\bf Case 0. Frontrunning for claiming rebase}: This case is Violation I involving three transactions depicted in Figure~\ref{fig:casestudy}. First, BASE token issuer Alice (EOA $0x471a$) sends transaction $tx_1$ to rebase the token supply among all BASE token holders, including a Uniswap V2 pool account (CA $0xde5b$). $tx_1$ is included in Ethereum Block $\#11375707$. Then, two accounts, say Bob (EOA $0x24af$) and Charlie (EOA $0x052e$), respectively send transactions $tx_2$ and $tx_3$, to withdraw the extractable value created by the rebase. Both withdrawal transactions externally call some third-party smart contracts before calling the victim pool's ($0xde5b$'s) \texttt{swap()} function. For instance, Bob's withdrawal $tx_2$ externally calls the smart contract of account $0x9799$, which internally calls another smart contract of account $0xa084$, which further internally calls the pool's \texttt{swap} function. Likewise, Charlie's withdrawal $tx_3$ externally calls a smart contract $0xea4d$, which internally calls smart contract $01da$ before internally calling the pool's \texttt{swap} function. While both transactions are included in the same Block $\#11375709$, $tx_2$ is ordered before $tx_3$, and Bob successfully claims the extractable value, leaving Charlie's withdrawal transaction reverted. This whole process is depicted in Figure~\ref{fig:casestudy}.

%with one succeeded in gaining the value (i.e., $tx_2$) while the other (i.e., $tx_3$) gets reverted. The transaction hashes of $tx_1$, $tx_2$ and $tx_3$ are respectively $0xd1c452b3eae46a70ad5b1154d2d802d\\0f3d5a64e22b74d6149e32bd645d174d8$, $0xbe856731f35d8d592601510c511189f\\5e07ee01d7083fcb093d6fd45d92e9112$, and $0xe85a08a9211e05a1eb6a1a7310897185\\c26cf476aef41db5744b3d374bf82505$. 

\noindent
{\bf Case 1: Aggressive attacker}: Account $0x2a2e$ is involved in $32$ atomicity violations and gains more than $2.39*10^5$ USD worth of illicit tokens. All $32$ swaps from this account are sent via a smart contract which checks the pool's profitability before withdrawal ($I_4$). In terms of timing, the malicious withdrawals are always sent in the same block with the risky, profitable deposit. We believe account $0x2a2e$ aggressively monitors the mempool for the target tokens' rebase transactions and if found, sends withdrawals immediately to ``backrun'' the deposits and claim the value.

\ignore{
\noindent
{\bf Case 2: General attacker (A2) w. off-chain monitoring}: Account $0x0c08$ has withdrawn four times and grabbed tokens of $1.01*10^5$ USD. The account directly and externally calls Uniswap pool's swap function to withdraw without checking pool profitability on-chain. The withdrawals are included in exactly one block after the one that includes the risky deposit. We believe Account $ 0x0c08$'s strategy is to monitor the pool profitability from an off-chain vantage point and to immediately send withdrawal by external calls. Because the account monitors the pool profitability instead of the cause (risky deposit), it has to wait until the inclusion of risky deposit that updates the pool state to be profitable. This explains why the inclusion of withdrawal has to be one block after the block including the risky deposit.
}

\noindent
{\bf Case 2: Attacker stealing interest}: Both Accounts $0xdb40$ and $0x5617$ have extracted value from interest-bearing tokens. Their block gaps are large ($665$ and $1574$, respectively). Given that there are enough samples, this consistent behavior shows both accounts' attack strategy to wait long enough for the token interest to accumulate and for the extractable value to be large enough before acting on it.

In general, for all accounts with indicators $I_1$ and $I_2$ in Table~\ref{tab:attackerview}, it is clear that the block gaps for different causes ($I_1$ and $I_2$) differ: The block gaps for non-interest causes are consistently much shorter than those for token interests. It implies that the attackers are aware of the situation (which causes them to exploit) and tailor their strategies to it.

\ignore{
\noindent
{\bf Case 5: Scavenger trader (A3)}: Account $0x9799$ is unlikely an intentional attacker: First, it does not read the token balance or check the pool's profitability before the withdrawal. Second, the block gap between the profitable deposit and malicious withdrawal is large, at hundreds of blocks apart. In addition, the smart contract Account $0x9799$ relays her withdrawal requests also make deposit to the pool. All these indicators show that $0x9799$ is a scavenger trader.
}

\subsubsection{Block Gaps}

\begin{figure}[!ht]
  \begin{center}
    \subfloat[Block gaps and the number of competing attackers]{%
\includegraphics[width=0.235\textwidth]{figures/figure_allrebase_blockdif.eps}
\label{fig:blockdif_1}
    }%
    \subfloat[Block gaps and value stolen]{%
\includegraphics[width=0.235\textwidth]{figures/figure_value_blockdif.eps}
\label{fig:blockdif_2}
    }%
  \end{center}
  \caption{Block gaps and affecting factors}\label{fig:complex}
\end{figure}

Recall that each theft attack runs in two transactions: The first transaction that creates extractable value, and the second transaction that withdraws the value and steals it. Given each detected attack (described in the previous subsection), we measure the gap of the two blocks that include the attack's two transactions, namely block gap. We further report two metrics: the number of competing attackers and the value stolen. For each profitable deposit transaction, say $tx$, we find transactions sent by competing attackers. Here, a competing attacker either directly sends a transaction to withdraw the extractable value created by $tx$ but fails or sends a transaction to read the token balance and pool reserve (which shows the intention to withdraw the value). 

We report the block gaps with the varying number of competitors in Figure~\ref{fig:blockdif_1}. A larger dot in a X/Y coordinate in the figure represents more attacks found with the same X/Y value. The result shows that when there are many competing attackers, the block gap tends to be small. This could be explained: Because the first attacker wins, the more attackers there are, the earlier the withdrawal transaction is sent, namely a smaller block gap.
The result also shows that with few competing attackers comes a large range of block gaps.

We then report the block gaps with varying value stolen in Figure~\ref{fig:blockdif_2}. The result shows that when the stolen value is large, the block gap tends to be small. A possible explanation is that the higher extractable value gives the attacker more incentives to send the withdrawal transaction with higher fees and frontrun other thieves.
 
\subsubsection{Attacker/Victim Behavior over Time}

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_attacker_timeline.eps}
\end{center}
\vspace{-0.1in}
\caption{Attack timeline of top-8 attackers. In the Y axis, attacker accounts are ordered by the total value stolen.
Data from 07/09/2020 (block 10422671) - 06/29/2021 (block 12727620).}
\label{fig:attack}
\end{figure*}

\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{figures/figure_victim_timeline.eps}
\end{center}
\vspace{-0.1in}
\caption{Attack timeline of top-10 victims. In the Y axis, victim accounts are ordered by the total value stolen.
Data from 07/29/2020 (block 10553883) - 01/10/2022 (block 13979019).}
\label{fig:victim}
\end{figure*}

We plot the timeline of the top-8 attackers' activities in Figure~\ref{fig:attack}. The attackers are ranked by the total value stolen, with attacker $0x9799$ being the top-1. Each dot represents a detected attack sent by the attacker's account. The size of the dot represents stolen value. Color represents the exploit pattern. The most successful attacker ($0x9799$) steals value through different causes (including rebase, airdrop, etc.) The attacker's activities last about 
$1.1*10^6$ blocks, which amount to six months. The second attacker ($0x2a2e$) concentrates all her attacks on a one-month span. She exploits exclusively the value created by rebase operations. The third attacker ($0xdb40$) mount attacks sporadically and target value created through two causes: Token interest and rebase operations. The ninth attacker exploits buggy smart contracts to gain illicit profit. The tenth attacker exclusively grabs the value from the token interest in a three-month period. As a result, most top attackers mount multiple attacks consistently, which shows the attacks are intended and not by accident.

We additionally study top victims' behavior. The victims are ranked by the value stolen. In Figure~\ref{fig:victim}, we plot in dots the transactions sent by victims whose deposits are stolen in identified attacks. Different color represents different causes. Additionally, in hollow green circles, we plot the normal transactions sent by the victims and related to Uniswap. The result shows that most victims change behavior after an attack/theft. For instance, victim accounts, including $0x0cd4$ and $0x80cc$, all stop using the vulnerable interface (e.g., partly error) to send a deposit after an attack. However, other victims can repeatedly create extractable value that gets stolen. For instance, account $0x66ac$ repeatedly airdrops tokens to the Uniswap pool, which gets stolen. 

\subsubsection{Value Received by Pools}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Extractable value and its destinations}
\label{tab:extractable_value}
\centering{
\begin{tabularx}{0.425\textwidth}{ |X|l|X| } %X is stretching to \textwidth, while c is to match with text width in cell.
\hline
Value extracted by & Rebase ($P_1$) & External transfer ($P_3$) \\
\hline
External attackers & \$0.81M & \$0.50M \\
\hline
Pools (intended) & \$58.1M & \$1.22M \\
\hline
Pools (accidental) & \$0.65M & \$1.29M \\
\hline
\end{tabularx}
}
\end{table}

\begin{figure}[!htbp]
\begin{center}
  \subfloat[Value created by rebase ($P_1$)]{%
     \includegraphics[width=0.245\textwidth]{figures/figure_rebase_seg.eps}
    \label{fig:moneyflow_1}
  }%
  \subfloat[Value created by external transfers ($P_3$): all pools are between token $XX$ and $WETH$, where $XX$ is the tick on the $x$ axis.]{%
    \includegraphics[width=0.245\textwidth]{figures/figure_underwater_seg.eps}
     \label{fig:moneyflow_2}
     }%
\end{center}
\caption{Extractable value received by the pool versus that by attacker accounts}\label{fig:complex}\vspace{-0.10in}
\end{figure}


Extractable value can be claimed by any account, including an external attacker and the pool itself. Our measurement result so far captures the former case. In this experiment, we measure the extractable value that goes to the pool.

A pool can claim extractable value by calling the \texttt{sync} function, which synchronizes the pool reserve and token balance. In Uniswap, there are three circumstances \texttt{sync} is called: a standalone call to \texttt{sync} in a transaction, \texttt{sync} called after a \texttt{swap} in the same transaction, \texttt{sync} called after an \texttt{addLiquidity} call in the same transaction. In the first case, tokens are sent to the pool intentionally (denoted by ``pool (intended)'' in the table and figures), and in the second and third cases, the pool receives deposit by accident (denoted by ``pool (accidental)''), because it is an irrelevant transaction to \texttt{sync} the reserve and token balance. Informally, we calculate the extractable value that goes to the pool in the following method: We obtain the value of the pool reserve before and after the transaction. We also parse the function call arguments from the transaction data field. We can cross-check the pre-state, post-state, and function arguments to detect the mismatch, which can be attributed to the extractable value. For instance, a normal \texttt{swap} in Uniswap does not change the product in AMM, and a spurious \texttt{swap} that the pool receives extractable value can be detected by the violation of product equality.

Using the above method, we measure the total extractable value claimed by the pool under different patterns, including $P_1$ and $P_3$. The result is presented in Table~\ref{tab:extractable_value}: The total value claimed by the pools is consistently more than $5\times$ of that by external attackers. This suggests ``room'' for the current Uniswap thief to increase their revenue. We further show the total extractable value by different pools/tokens. In Figure~\ref{fig:moneyflow_1}, we plot the extractable value created by different rebase-enabled tokens (Pattern $P_1$). 
Token $AMPL$ has the highest extractable value, most of which goes back to the pool by the token issuer intentionally calling \texttt{sync} function after each \texttt{rebase} call (the ``intended'' case). 
Token $BASE$ is the third highest in total extractable value and has the highest value stolen by external attackers. In Figure~\ref{fig:moneyflow_2}, we plot the extractable value created by external transfers (Pattern $P_3$) against different pools. Here, all the top-value pools we found are between token $WETH$ and another token. The most vulnerable pool is between Token $UNI$ and $WETH$, whose extractable value is $400$ thousand USD in total, among which the $10\%$ value is extracted by external attackers and the rest is mostly sent to the pool intentionally. Token $ YFill$'s value is exclusively extracted by external attackers. Token $ SUSHI$'s deposit is mostly claimed by the pool accidentally. 

\section{Detecting Lost Tokens}
\label{sec:losttokens}

\noindent
{\bf Problem}:
We detect lost tokens out of standalone deposits (i.e., atomicity violation II). On the one hand, the incidents of lost tokens appear as standalone deposits. On the other hand, not every standalone deposit should be attributed to lost tokens. There are other causes, such as token giveaways, and administrative accounts calling privileged AMM operations. 

{%\color{blue}
%\tangSide{In response to Q11}
\noindent
{\bf Methods}: 
We propose two heuristics for detecting lost tokens. 
The first detection heuristic is based on the following intuition: a trader account may use an unsupported mechanism to deposit tokens. She may then realize the mistake and retry the token deposit of the exact same amount using the right mechanism. For instance, Uniswap V3 does not support deposit by \texttt{transfer}. Unaware of the right function, a user may initially call \texttt{transfer} to deposit a token to a Uniswap V3 pool. The user then switches to calling \texttt{approve} of the same amount for the second time. The \texttt{approve} call is accepted by the V3 pool. Based on the heuristic, we propose the following indicator $I_9$:

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator $I_9$: 
Suppose an account Alice sends a standalone deposit (Violation II) of $x$ units of Token $T_0$ to a pool. Alice then sends an atomic swap of the same $x$ units of $T_0$ but using a different mechanism from the standalone deposit. The sequence indicates that the first standalone deposit results in lost $x$ units of Token $T_0$.
}}\end{center}
}

In the second heuristic, the idea is that lost tokens must be deposited by an unprivileged AMM account. And a privileged account, such as an AMM-pool administrator, is entitled to deposit value to an AMM pool, which is unlikely a mistaken deposit. We propose the indicator for lost token below:

\begin{center}\fbox{\parbox{0.90\linewidth}{
Indicator $I_10$: An account that calls privileged AMM functions (e.g., \texttt{setSwapFee()} in Balancer) is an privileged account, and a standalone deposit sent by a privileged account is not attributed to lost tokens.
}}\end{center}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Aggregated results on lost tokens}
\label{tab:lost}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|l|l|l| }
  \hline
   AMM & \# txs & Total value (USD) & Block diff (avg) \\ \hline
   Uniswap-V3 & $20$ & $47928$ & $9013$ \\ \hline
   Balancer & $192$ & $7875$ & $6578$ \\ \hline
   Curve & $3$ & $905$ & $14533$ \\ \hline
\end{tabularx}
}
\end{table}


\noindent
{\bf Results}:
Using the method above, we detect $215$ instances of lost tokens on Uniswap V3, Balancer, and Curve, inflicting a total of lost tokens worth $56708$ USD, as shown in Table~\ref{tab:lost}. Given a standalone deposit, we calculate its value using the token price at the time of the deposit (by using the nearest price with token WETH in Uniswap V2). We record the block difference between the standalone deposit and the follow-up deposit retry sent from the same account. It can be seen block difference on Uniswap V3 is about $9013$ blocks which amounts to about $33$ hours. Detailed case analysis is in Appendix~\ref{sec:losttoken:cases}.

{%\color{blue}
\section{Root Causes \& Countermeasures}
\label{sec:mitigate}

We first present a security analysis of different AMM protocols under the risks of token thefts and lost tokens. We then present our two mitigation designs, a secure redesign of AMM pool and a retrofittable scheme to harden deployed pools' security. 

\subsection{Risk Analysis}
\label{sec:riskanalysis}


\begin{table*}[ht]
%\begin{figure*}[!ht]
\begin{center}
\begin{minipage}{.46\textwidth}
  \includegraphics[width=0.95\textwidth]{figures/mitigate_losttokens.eps}
 \captionof{figure}{AMM pool designs: \texttt{tf}/\texttt{off}/\texttt{appr} refer to ERC20 functions \texttt{transfer}/\texttt{transferFrom}/\texttt{approve}.}
  \label{fig:ammpool:designs}
\end{minipage}
\hspace{0.1in}
\begin{minipage}{.5\textwidth}
  \centering{\footnotesize
  \begin{tabular}[b]{lcc}
  \hline 
  & Direct deposit by & Indirect deposit by  \\ 
  & \texttt{transfer} & \texttt{transferFrom} \\ \hline 
  \multicolumn{3}{l}{{\it Uniswap V2}}\\ \hline
  \ \ \ Swap tokens & \cmark & \xmark  \\ \hline 
  \ \ \ Secure swap against theft & {\color{red} \xmark} & \cmark (N/A) \\ \hline 
  \ \ \ Refund against lost tokens & \cmark & \cmark  \\ \hline 
  \multicolumn{3}{l}{{\it Uniswap V3}} \\ \hline
  \ \ \ Swap tokens & \xmark & \cmark  \\ \hline 
  \ \ \ Secure swap against theft & \cmark (N/A) & \cmark \\ \hline 
  \ \ \ Refund against lost tokens & {\color{red} \xmark}  & {\xmark} \\ \hline 
  \multicolumn{3}{l}{{\it Secure AMM pool redesign (\S~\ref{sec:redesign})}}\\ \hline
  \ \ \ Swap tokens & \cmark & \cmark  \\ \hline 
  \ \ \ Secure swap against theft & \cmark & \cmark \\ \hline     
  \ \ \ Refund against lost tokens & \cmark & \cmark \\ \hline 
  \end{tabular}%
  }
\caption{Risk analysis (red cross marks are risks that pose challenge to fix.)}
\label{tab:ammsecurity}
\end{minipage}
  \end{center}
%\end{figure*}
\end{table*}


\ignore{
\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.3\textwidth]{figures/uniswapv2-dilemma.eps}
\end{center}
\caption{The AMM service supporting token deposit-by-\texttt{transfer}; the functions are specific to the example of Uniswap V2.}
\label{fig:ammpool:designsXX}
\end{figure}
}

% Different designs of AMM pool: Uniswap V2 that only accepts direct deposit by \texttt{transfer}, 
  Uniswap V3 that only accepts indirect deposit by \texttt{approve} and \texttt{transferFrom}, 
  and our secure pool design that supports both direct and indirect deposits with security against theft.

We character AMM protocol by how token deposits are supported. One design adopted in the Uniswap V2 family is to accept direct token deposit by \texttt{transfer}. This is depicted in Figure~\ref{fig:ammpool:designs}, where a trader deposits token $T_0$ by calling $T_0$ smart contract's \texttt{transfer} function. Another design, adopted by Uniswap V3, Balancer and Curve, is to accept {\it indirect token deposit} by \texttt{approve}/\texttt{transferFrom}. In this design, a trader first calls \texttt{approve} to delegate the spending of her token $T_0$ to the pool which then does the swap atomically by calling $T_0$'s \texttt{transferFrom} and $T_1$'s \texttt{transfer} in the same transaction. This is depicted in Figure~\ref{fig:ammpool:designs}.

In the following, we analyze the security of Uniswap V2 as a representative pool supporting direct deposits and the security of Uniswap V3 as a representative pool supporting indirect deposits. 

\noindent
{\bf Risk of Uniswap V2}: Uniswap V2 is insecure against token thefts from direct deposit. Once its pool contract account receives a token deposit via \texttt{transfer}, the deposited value can be withdrawn by any subsequent transaction (i.e., calling \texttt{swap} function). We call this vulnerability by permissionless withdrawal. As analyzed later, this vulnerability applies to any direct-deposit based AMM pool design.

Uniswap V2 supports token refund for standalone (direct) deposit via \texttt{skim} function. For indirect deposit, Uniswap V2 does not allow withdrawal and is thus secured against possible token thefts. Since indirect deposit is through \texttt{approve}, a standalone \texttt{approve} does not decrease the depositor trader's balance. Thus, Uniswap V2 can ``refund'' mis-issued deposit. Note that we scan the Uniswap V2 smart contract code to verify that it does not issue any \texttt{transferFrom} call.

\noindent
{\bf Risk of Uniswap V3}: Uniswap V3 is secure against token thefts. When the deposit is directly made via \texttt{transfer}, V3 does not support it and thus does not allow any withdrawal from it. When the deposit is indirectly made via calling \texttt{approve} function, V3 does allow withdrawal and is secured against theft. This is because with indirect deposit the actual token deposit (done in \texttt{transferFrom}; recall Figure~\ref{fig:ammpool:designs}) is executed in the same transaction with token withdrawal, enforcing both atomicity (against a thief trader's attempt to insert a malicious withdrawal in between) and the match between the deposit sender and withdrawal receiver.

Uniswap V3 does not refund mistaken deposit, regardless whether made directly or indirectly. Because Uniswap V3's pool does not support traders canceling an \texttt{approve} call, as confirmed by the Uniswap team~\cite{me:bugreport:defiant}.

Overall, the risk analysis of Uniswap V2/V3 is presented in {\color{purple} Table~\ref{tab:ammsecurity}}. Cross marks refer to risky operations in the AMM pool. The black ones are easy to fix; for instance, canceling the allowance by a previous \texttt{approve} call is straightforward. More challenging are the two red cross marks associated with direct deposit, that is, to secure a pool supporting direct deposit and token refunding against token theft (as in Uniswap V2).

We additionally characterize other AMM protocols by their support of direct deposits (by \texttt{transfer}) in Table~\ref{tab:ammprofile}. All other AMM instances that don't support direct deposit are subject to the risk of lost tokens.

\begin{table}[!htbp] %force in current page, disable float.
  \caption{High-level characterization of AMM protocols. ``Lost'' refers to lost tokens.}
  \label{tab:ammprofile}
  \centering{\footnotesize
  \begin{tabularx}{0.5\textwidth}{ |X|c|c|c|c| }
  \hline
Design & Uniswap V2 & Uniswap V3 & Balancer & Curve \\ \hline
Direct deposit by \texttt{transfer} 
& \cmark & \xmark & \xmark & \xmark \\ \hline
Risks
& Theft & Lost & Lost & Lost \\ \hline
  \end{tabularx}
}
\end{table}

{\color{blue}\tangSide{Resp. Q1}
\noindent{\bf 
Risk generalizability}: The security risks we discovered in this work stem from the design flaws of ERC20 smart contracts, including both information non-traceability of \text{transfer} in the ERC20 standard (see example below) and exhibiting behavior undefined in the standard.   Thus, the risks are generic and are applicable to any DeFi smart contracts built on ERC20 tokens. 
For instance, implementing the protocol-level fair exchanges~\cite{DBLP:conf/ccs/CampanelliGGN17,DBLP:journals/corr/abs-1911-09148,DBLP:conf/ndss/MalavoltaMSKM19,DBLP:conf/ccs/0001MM19,DBLP:journals/corr/MillerBKM17,DBLP:conf/podc/Herlihy18,DBLP:conf/ccs/CampanelliGGN17}, as surveyed in \S~\ref{sec:rw}, on widely deployed ERC20 tokens on Ethereum could face the same security risks uncovered from this work. 

We manually validate this claim by running an HTLC smart contract\footnote{\url{https://github.com/chatch/hashed-timelock-contract-ethereum}} atop ERC20 tokens with the following tests: An account that deposits value (mis)using ERC20's \texttt{transfer} function (instead of \texttt{approve}-\texttt{transferFrom}) is unable to call either the \texttt{withdraw} function or \texttt{refund} function with success. This implies the mis-deposited tokens are lost.
%We leave it to future work to evaluate more open-source implementations of provable secure protocols.

In general, given a direct deposit made by calling an ERC20 token's \texttt{transfer} function, the DeFi smart contract can decline it (as in Uniswap V3, which leads to lost tokens) or accept it to authorize the withdrawal of the other token. For the latter design, because the call of the token's \texttt{transfer} function does not notify context information (e.g., the \texttt{transfer} sender) to any third-party contract, the DeFi contract cannot determine who the original token depositor is and has to allow permissionless withdrawal, as in Uniswap V2.
}


{\color{blue}\tangSide{Resp. Q3}
\subsection{Countermeasure Design Space}
\label{sec:counter:space}
%\noindent{\bf Can existing BEV mitigation fix the discovered issues of atomicity violation?}

\noindent{\bf 
Existing BEV mitigation}: In the existing literature, protection against BEV is tackled by two design paradigms: 1) designing secure DeFi protocols to eliminate the profitable opportunities and {\it prevent} transaction reordering attacks (by making them unprofitable), and 2) detecting and {\it mitigating} the transaction reordering attacks (by enforcing fair transaction ordering). 

The approaches in the first paradigm are application specific (e.g., protecting AMM pools, such as rerouting against arbitrage~\cite{DBLP:journals/corr/abs-2106-07371}, may not be transferable to protecting lending services). In particular, flashbots and BEV redistribution~\cite{DBLP:conf/ccs/ChitraK22
} are based on the assumption of a trusted off-chain infrastructure that aggressively collects the BEV ahead of adversaries. The second paradigm is generic to DeFi applications, but the current approaches are limited to mitigating frontrunning attacks. Specifically, frontrunning attacks are mitigated by enforcing fair transaction ordering~\cite{DBLP:journals/corr/abs-2203-11520} where the order in which transactions are included into blocks is the same as that transactions are submitted~\cite{me:fairsequencing}. However, backrunning attacks are not mitigated (i.e., not following the second paradigm) but are prevented in an application-specific fashion (i.e., following the first paradigm).

\noindent{\bf 
Applicability of existing mitigations}: To mitigate the security risks associated with atomicity violations, one can start by applying the existing mitigation paradigms. Specifically, one can apply fair transaction ordering techniques to mitigate the theft attacks that exercise frontrunning (e.g., Case 0 studied in \S~\ref{sec:theftinstances}). However, this approach cannot mitigate the aggressive attacker (i.e., Case 1 in \S~\ref{sec:theftinstances}) who exercises backrunning strategies. 

Alternatively, one can customise the BEV-redistribution infrastructure to capture the extractable value caused by permissionless withdrawal. In this defense, one has to assume trust in the off-chain infrastructure. We describe the detail of the custom BEV-redistribution infrastructure in Appendix~\ref{sec:hardening:mevredistribute}. 

In the rest of this section, we focus on redesigning secure AMM pools to eliminate BEV, namely following the second paradigm. Existing approaches in the second paradigm are application specific and inapplicable to the specific case of permissionless withdrawal.
} 

\subsection{Secure AMM Pool Redesign}
\label{sec:redesign}

\noindent{\bf Design goals}: We propose building a secure AMM pool that can swap or refund tokens without losing the security against token theft. This design goal is shown in Table~\ref{tab:ammsecurity}. The difficulty comes from the following: If the ERC20 tokens are directly deposited by calling token function \texttt{transfer(address from, address to, int amount)}, the pool smart contract cannot know the trader who made the deposit (recall Figure~\ref{fig:ammpool:designs} ). Without knowing the depositor account, the pool smart contract is left unable to enforce access control on where the withdrawn/refunded tokens should go. Therefore, the key of the secure pool design is to make the pool smart-contract able to verify the depositor account.

\noindent{\bf Design rationale}:
{\bf Proposed design}: Our AMM pool redesign follows the paradigm in Uniswap V3, that is, supporting swaps by indirect token deposit via \texttt{approve}/\texttt{transferFrom} calls. When an account deposits tokens directly through \texttt{transfer} calls, the AMM pool runs ETHRelay~\cite{DBLP:conf/blockchain2/FrauenthalerSSS20,me:ethrelay,me:btcrelay,me:btcrelay:github} to validate the transaction of direct \texttt{transfer} call. 
If the validation is successful, the pool extracts the original depositor's account. It enforces access controls on the token withdrawal or refund, depending on application needs, so that the original depositor receives the token refund.

Specifically, ETHRelay is a smart-contract procedure that takes as input an Ethereum transaction, say $tx$, and the associated proof (incl. Merkle proof within a block and a sufficient number, say $X$, of block headers). It validates the inclusion of $tx$ in the Ethereum blockchain history. The validation is secure against forged inputs based on the hardness assumption of forging $X$ Ethereum block headers that can pass validation.
The pseudocode of pool redesign and more details are described in Appendix~\ref{appdx:detail:redesign}. 

{%\color{blue}
%\tangSide{In response to Q4.}
The secure AMM redesign can be easily extended to support the case that the original depositor wants to designate a third-party token receiver instead of herself. The secure AMM pool can authorize token withdrawal if a receiver account is explicitly designated and signed by the depositor.}
}

\noindent{\bf Security analysis}: Suppose benign trader Alice sends a transaction $tx_1$ to directly deposit tokens (i.e., calling \texttt{transfer}). Normally, Alice would send the second transaction $tx_2$ to either request refund or finish the swap. 
Now, Adversary Bob sends a transaction $tx_2'$ to frontrun Alice's transaction $tx_2$. If Bob wants to receive the value, he needs to forge another (non-existing) transaction $tx_1'$, where Bob is the depositor account. Bob then prepares a proof of $tx_1'$'s inclusion to pass the ETHRelay validation, which cannot succeed due to the hardness assumption.

{\color{blue}\tangSide{Resp. Q3}
In the case of network congestion, the underlying consensus may cause the delayed inclusion of transactions or even dropping the transactions. Delayed or dropped transactions do not lead to atomicity violation in our countermeasure, assuming that the account having deposited tokens would retry to withdraw the value. Because of the ETHRelay that prevents any other account from withdrawing the value, the retrying of withdrawals by the original depositor account can (eventually) succeed.
}

{\color{blue}\tangSide{Resp. Q7}
\noindent{\bf 
Implementation \& evaluation}: 
We implemented the secure pool redesign by patching Uniswap V3~\cite{me:mitigate:v3} and V2~\cite{me:mitigate:v2}. In the implementation, we remove two functions in Uniswap's original pool contract to make room for our code (Uniswap's original pool contract uses up the maximal $24576$ bytes allowed by an Ethereum transaction). 

We build two testing smart contracts to evaluate the security of our patched contracts. Given a pool contract, our smart contract testing lost-tokens first makes a direct token deposit via ERC20 \texttt{transfer} and then issues a token withdrawal. The success of the token withdrawal means the tested pool does not have the risk of lost tokens. 

Given a pool contact, our smart contract testing permissionless withdrawals first makes a deposit from one account and then issues a withdrawal from another account. The withdrawal failure implies the tested pool's security against permissionless withdrawals. The testing contracts are also included in the open-sourced pool patches.

We have run the two testing smart contracts against our patched pools on Uniswap V2 and V3. The results show both patched contracts are secured against lost tokens and permissionless withdrawal.
}


\section{Responsible Disclosure}
\label{sec:disclosure}

{\color{blue}\tangSide{Resp. Q6}
We disclose the bugs to both affected AMM pools and token developers after the bug discovery. The Uniswap team (\url{https://uniswap.org/bug-bounty}) has confirmed the lost-token bug on V3 but blames users' API misusing for the theft risk on V2. We did not receive feedback from the other teams we sent our report to. Bug reports we sent are documented in the anonymized Google document~\cite{me:bugreport:defiant}. The likely cause of low response rates is that the bugs we found are distinctly caused by the interaction between the pool and token smart contracts, and neither side is willing to take full responsibility for bug fixing.
}

\section{Conclusion}
\label{sec:conclude}

This paper presents the first measurement study of atomicity violations and token theft attacks on popular AMMs on Ethereum. The study unearths more than $55$ thousand thefts and stolen tokens worth a total of $3.88$ million USD. It uncovers a range of previously unknown patterns of vulnerable deposits (e.g., token interest and supply adjustment), exposes real-world attackers' adaptive strategies to send malicious withdrawals, and reveals their systematic behavior in preparing, executing, and finalizing theft attacks. Finally, it presents mitigation schemes to design secure AMM protocols and to harden the deployed AMM services running immutable smart contracts.

\section{Acknowledgment}
\label{sec:acknowledgment}
\textcolor{blue}{The authors thank the reviewers in Euro S\&P'23 and ACM CCS'22. The authors are partially supported by the National Science Foundation under Grants CNS2139801, CNS1815814, and DGE2104532. The authors are also partially supported by Ethereum Foundation. }

\clearpage


==> text/wheels.tex <==
\section{learning}

\subsection{tables}

{\scriptsize \begin{verbatim} in beamer, see beamer_learn_slides. http://en.wikibooks.org/wiki/LaTeX/Tables#The_tabular.2A_environment_-_controlling_table_width
\end{verbatim}}

table with reference~\ref{tab:auth-attack}


\begin{table}[!htbp] %force in current page, disable float.
\caption{Example of authorized searcher attack}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c|c|c|c|c| }
  \hline
   & $p_0$ & $p_1$ & $p_2$ & $p_3$ & $p_4$ \\ \hline
  $r_a$ & $1$ & $0$ & $1$ & $0$ & $?$ \\ \hline
\end{tabularx}
}
\end{table}

tabular (not table)

\begin{tabularx}{0.4\textwidth}{ |X|c|c|c| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
  label1                    & label2 & label3 & label4 \\ \hline
  \multirow{2}{*}{multi-row} 
                             & item2  & item3  & item4  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \hline
  \multicolumn{2}{|l|}{multi-column}   & item3''  & item4''  \\  \hline
  \multirow{5}{*}{\begin{sideways}sideways\end{sideways}}
                             & item2  & item3  & item4  \\ \cline{2-4}
                             & \shortstack[l]{item2'\\item2''}  & item3'  & item4'  \\ \cline{2-4}
                             & \shortstack[r]{item2'\\item2''}  & item3'  & item4'  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \hline
\end{tabularx}

\subsection{figures}


%\begin{wrapfigure}{r}{0.35\textwidth}
\begin{figure}[!ht]
\centering
\includegraphics[width=0.324\textwidth]{figures2/eff_rand_num_sample0.5.eps}
\caption{Wrapped figure}
\label{fig:perf}
\end{figure}
%\end{wrapfigure}

\ifdefined\TTUT
\begin{figure}[!ht]
\begin{center}
    \includegraphics[angle=90, width=0.45\textwidth]{figures2/eff_rand_num_sample0.5.eps}%
\end{center}
%\vspace{-0.15in}
\caption{Easy figure}\label{fig:easy}
\vspace{-0.10in}\end{figure}

\begin{figure*}[!ht]
  \begin{center}
  %\goodgap
    \subfloat[Rotated]{%
      \includegraphics[angle=90, width=0.3\textwidth]{figures2/eff_rand_num_sample0.5.eps}%
      \label{exp:rand_num_1}%
    }%
    %\hspace{-0.2cm}%
    \subfloat[With more shared threads]{%
      \includegraphics[width=0.3\textwidth]{figures2/eff_rand_num_sample2.eps}%
      \label{exp:rand_num_2}%
    }%
    \subfloat[With sample ratio]{%
      \includegraphics[width=0.3\textwidth]{figures2/eff_rand_sample_num10.eps}%
      \label{exp:rand_sample}%
    }%
  \end{center}%\vspace{-0.15in}
  \caption{Performance of optimization algorithm with random graph}\label{fig:complex}\vspace{-0.10in}
\end{figure*}
\fi

\subsection{algorithms}
\begin{algorithm}[h]
\caption{range-query(range $R$)}\small \label{alg:rangequery}
\begin{algorithmic}[1]
  \boldnext\State $\omega_R\leftarrow $ lowest-common-ancestor($R$) \Comment{comments: line number boldened}
  \State $\lambda\leftarrow $ DHT-lookup($f_{md}(\omega_R)$)
  \ForAll{$p \in P$} \Comment{comments: loop over all items}
    \State manipulate each term $p$
  \EndFor
  \If{$\lambda == NULL \And 1 \leq 0$}
      \State \Return lookup($R$.top\_left\_corner)
  \ElsIf{$R\subseteq{\lambda}$}
      \State \Return the keys of $\lambda$ that are in the range $R$
  \Else
      \State \Return recursive-forward($R$, $\omega_R$)
  \EndIf
\end{algorithmic}
\end{algorithm}

\subsection{equations}
\begin{eqnarray}
u &=& \sum_{l=0}^{n-1}{u_l} \mod{q} %\nonumber \\
=(\sum_{l=0}^{n-1}{ \sum_{j=0}^{c-1}{u_{l-j, j}} \mod{q}})\mod{q} \nonumber \\
&=& (\sum_{j=0}^{c-1}{ \sum_{l=0}^{n-1}{ u_{l-j, j} } })\mod{q} %\nonumber \\
=(\sum_{j=0}^{c-1}{ \sum_{i=-j}^{n-1-j}{ u_{i, j} } })\mod{q} \nonumber \\
&=& (\sum_{j=0}^{c-1}{\sum_{i=0}^{n-1}{ u_{i, j} } }) mod q
= (\sum_{i=0}^{n-1}{ \sum_{j=0}^{c-1}{ u_{i, j} }\mod{q} })\mod{q} \nonumber \\
&=& \sum_{i=0}^{n-1}{ v_i }\mod{q} = \sum_{i=0}^{n-1}{ v_i } = v
\end{eqnarray}

With right brace
\begin{eqnarray}
\underline{\sigma}, \epsilon \rightarrow{}\underline{\beta_*}
\begin{cases}
\begin{rcases}
\begin{rcases}
& \sum_{\forall\beta_*>1}{(\beta_* - 1)} \\
& \sum_{\forall\beta_*<1}{(1 - \beta_*)} \\  
\end{rcases} \rightarrow{} \underline{X_1}\% \\
\sum_{\beta_*<1}{1} \rightarrow{} \underline{X_2}\%
\end{rcases}
\end{cases}
 \rightarrow{\beta}
\end{eqnarray}

\subsection{listing}
\lstset{language=SQL, style=Oracle, caption={Rewritten query against a single view table},label=sql:rewritten}
\lstset{frame=lrbt,xleftmargin=\fboxsep,xrightmargin=-\fboxsep} %with bounding box at l(eft)r(right)b(ottom)t(op)
%or you can replace it with "frame=single"
\begin{lstlisting}
  SELECT A, C FROM viewtable
  ORDER BY C LIMIT arg.k
\end{lstlisting}

\definecolor{mygreen}{rgb}{0,0.6,0}
\begin{figure}[h!]
%\begin{scriptsize}
%\begin{tabular}{cc}
%\begin{minipage}{.5\textwidth}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={(*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
public void OnTouchEvent(MotionEvent e) {
Bitmap LoadPicture(String path) {
    ...
    *Bitmap bm = BitmapFactory.decodeFile(file)*;
    return bm;
}

void EditPicture(Bitmap bm) {
    //heavy computational picture editing
    int i = 10 (* $*$ *); //escape to plot * literatelly instead of bolden text
    bm.getPixels(pix, 0, mPhotoWidth, 0, 0, mPhotoWidth, mPhotoHeight);
    for(every pixel) {
      ...
    }  
    
    //embed location information into picture
    (* $*$*)Location loc = getLastKnownLocation(Provider)*;
    (* $*$*)double longitude = loc.getLongitude()*;
    (* $*$*)double latitude = loc.getLatitude()*;
    (* $*$*)EmbedLocation(bm, longitude, latitude);*
}
\end{lstlisting}
%\end{minipage}
%\end{tabular}
%\end{scriptsize}
\caption{Privacy-preserving Offloading Example}
\label{figure:MotivatingExample}
\end{figure}


\subsection{fbox}
\begin{center}
\fbox{This is a sample statement}
\end{center}

\begin{center}\fbox{\parbox{0.90\linewidth}{
This is a long long long statement: 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
}}\end{center}



\subsection{misc}
\begin{itemize}
  \item cmark $\cmark$ and xmark $\xmark$
  \item bold math type $\boldsymbol{<v_0, k>}$
  \item use other than default font size: {``\fontsize{8.5}{9} this's in font size 8.5''}. (second param. should be 1.2$\times$ first param. which is font size
  \item show tilde in url, use \textasciitilde{} rather than \~{}
  \item strike out text, \sout{text/$12$ removed}
  \item color, {\color{red}red}{\color{green}green}
  \item[$\bullet$] big bullet on each item
  \item circled text \circled{2}
  \item A white number inside a black circle: \ballnumber{37}
  \item empty set (beautiful version) $\varnothing$ (needs ``\\usepackage\{amssymb\}''), which renames emptyset, $\emptyset$
  \item stackrel $\stackrel[c]{a}{=}$
\end{itemize}

citation for long breakable url~\cite{me:mssgx}

